Technical Report: Scalable Active Information Acquisition for Multi-Robot Systems

This paper proposes a novel highly scalable non-myopic planning algorithm for multi-robot Active Information Acquisition (AIA) tasks. AIA scenarios include target localization and tracking, active SLAM, surveillance, environmental monitoring and others. The objective is to compute control policies for multiple robots which minimize the accumulated uncertainty of a static hidden state over an a priori unknown horizon. The majority of existing AIA approaches are centralized and, therefore, face scaling challenges. To mitigate this issue, we propose an online algorithm that relies on decomposing the AIA task into local tasks via a dynamic space-partitioning method. The local subtasks are formulated online and require the robots to switch between exploration and active information gathering roles depending on their functionality in the environment. The switching process is tightly integrated with optimizing information gathering giving rise to a hybrid control approach. We show that the proposed decomposition-based algorithm is probabilistically complete for homogeneous sensor teams and under linearity and Gaussian assumptions. We provide extensive simulation results that show that the proposed algorithm can address large-scale estimation tasks that are computationally challenging to solve using existing centralized approaches.

==> Technical Report- Scalable Active Information Acquisition - FinalSubmission/algorithm2e.tex <==
%  algorithm2e.sty --- style file for algorithms
%                      almost everything can be customized by users. See the document for more explanations
%% Copyright 1996-2015 Christophe Fiorio
%
% This work may be distributed and/or modified under the conditions of the LaTeX Project
% Public License, either version 1.3 of this license or (at your option) any later version.
% The latest version of this license is in http://www.latex-project.org/lppl.txt and
% version 1.3 or later is part of all distributions of LaTeX version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
% 
% The Current Maintainer of this work is M. Christophe Fiorio
%
% This work consists of the files algorithm2e.sty and algorithm2e.tex 
% and the associated example files algorithm2e_exAlgoDisjdecomp.tex,
% algorithm2e_exIR.tex, algorithm2e_ex01.tex, algorithm2e_exProg.tex,
% algorithm2e_ex02.tex, algorithm2e_exfor.tex, algorithm2e_ex03.tex,
% algorithm2e_exgeneric.tex, algorithm2e_ex04.tex,  algorithm2e_exgeneric2.tex,
% algorithm2e_ex05.tex, algorithm2e_exnlsty.tex, algorithm2e_ex06.tex,
% algorithm2e_exrepeat.tex, algorithm2e_ex07.tex, algorithm2e_exswitch.tex
%  
%  Report bugs and comments to:
%  - algorithm2e-announce@lirmm.fr  mailing list for announcement about releases^^J%
%  - algorithm2e-discussion@lirmm.fr mailing list for discussion about package^^J%
%  subscribe by emailing sympa@lirmm.fr with 'subscribe <list> <firstname name>'^^J%
%
%  $Id: algorithm2e.sty,v 5.1 2015/10/18 21:37:30 cfiorio Exp $
%
%  PACKAGES REQUIRED:
%
%  - float   (in contrib/supported/float)
%  - ifthen  (in base)
%  - xspace  (in packages/tools)
%  - relsize (in contrib/misc/relsize.sty)
%
%%%%%%%%%%%%%%%  Release 5.1
%
%   Package options: 
%   ---------------
%   - oldcommands                      : to use old command names
%   - french, english, german, ngerman
%      portuguese, czech, italiano,
%      slovak, croatian, spanish       : for the name of the algorithm and some keyword code
%   - onelanguage                      : to simply switch keyword from one language to another without changing
%                                        keyword commands
%   - boxed, boxruled, ruled, tworuled, 
%     algoruled, plain                 : layout of the algorithm
%   - algo2e                           : environment is algorithm2e instead of algorithms and \listofalgorithmes
%                                        instead of \listofalgorithms
%   - slide                            : to use when making slides
%   - noline,lined,vlined              : how block are designed.
%   - shortend, longend, noend         : short or long end keyword as endif for e.g.
%   - linesnumbered                    : auto numbering of the algorithm's lines
%   - linesnumberedhidden              : to hide autonumbered lines (show number on a line with \ShowLn
%   - commentsnumbered, inoutnumbered  : to autonumber comments and inout keywords (by defaut not numbered)
%   - rightnl                          : to have line number on the right instead of on the left as default
%   - algonl                           : line numbers preceded by algo number
%   - scright, scleft                  : right or left justified side comments
%   - fillcomment, nofillcomment       : end mark of comment is flushed to the right so comments fill the line
%   - dotocloa                         : add an entry in the toc for list of algorithms (require tocbibind package)
%   - endfloat                         : add algoendfloat environment pushing algorithm so written to the end of document
%   - resetcount, noresetcount         : start value of line numbers.
%   - algopart,algochapter,algosection : algo numbering within part, chapter or section
%   - titlenumbered,titlenotnumbered   : numbering of title set by \Titleofalgo
%   - figure                           : algorithms are figures, numbered as figures, and put in the list of figures.
%   - procnumbered                     : procedure or function are numbered as algorithm
%   - nokwfunc                         : procedure or function name doens't become a command
%   - norelsize                        : don't use relsize package (useful if it breaks the compatibily)
%   - displayblockmarkers              : display begin, end keywords at start of each block
%  
%   defaults are; english,plain,resetcount,titlenotnumbered
%
%%%%%%%%%%%%%%
%
%   Short summary  
%   -------------
%  
%   algorithm is an environment for writing algorithm in LaTeX2e.
%   Almost all is customizable. You can add keywords, change style, change the layout, ...
%   It provide macros that allow you to create differents sorts of key words, therefore a set of predefined key
%   word is gived.
%
%   IT should be used as follows
%
%   \begin{algorithm}
%       ...
%       ...
%   \end{algorithm}
%
%
%   IMPORTANT : each line MUST end with \;
%
%   Note that if you define macros outside algorithm environment they
%   are avaible in all the document and particulary you can use then
%   inside all algorithms without re-define them.
%  
%   an example:
%
%   \begin{algorithm}
%     \SetAlgoLined
%     \KwIn{this text}
%     \KwOut{how to write algorithm with \LaTeX2e }
%     
%     initialization\;
%     \While{not at end of this document}{
%       read current section\;
%       \eIf{understand}{
%         go to next section\;
%         current section becomes this one\;
%         }{
%         go back to the beginning of current section\;
%         }
%       }
%     \caption{How to write algorithm}
%   \end{algorithm}
%
%
%%%%%%%%%%%%%%         predefined keywords
%
%     \KwIn{input}
%     \KwOut{output}
%     \KwData{input}
%     \KwResult{output}
%     \KwTo                                       % a simple keyword
%     \KwFrom                                     % a simple keyword
%     \KwRet{[value]}
%     \Return{[value]}
%     \Begin{block inside}
%     \eIf{condition}{Then Block}{Else block}     % in blocks
%     \If{condition}{Then block}                  % in a block
%     \uIf{condition}{Then block}                 % in a block unended
%     \lIf{condition}{Else text}                  % on the same line
%     \Else{inside Else}                          % in a block
%     \lElse{Else text}                           % on the same line        
%     \uElse{Else text}                           % in a block unended
%     \ElseIf{inside Elseif}                      % in a block
%     \lElseIf{Elseif text}                       % on the same line        
%     \uElseIf{Elseif text}                       % in a block unended
%     \Switch{Condition}{Switch block}
%     \Case{a case}{case block}                   % in a block
%     \lCase{a case}{case text}                   % on the same line
%     \Other{otherwise block}                     % in a block
%     \lOther{otherwise block}                    % on the same line
%     \For{condition}{text loop}                  % in a block
%     \lFor{condition}{text}                      % on the same line
%     \ForEach{condition}{text loop}              % in a block
%     \lForEach{condition}{text}                  % on the same line
%     \ForPar{condition}{text loop}               % in a block
%     \lForPar{condition}{text}                   % on the same line
%     \While{condition}{text loop}                % in a block
%     \lWhile{condition}{text loop}               % on the same line
%     \Repeat{End condition}{text loop}           % in a block
%     \lRepeat{condition}{text}                   % on the same line
%
%%%%%%%%%%%%%%
%
%   History: 
%
%   -  October 19 2015 - revision 5.1
%                   * CHANGE/ADD: l commands  (the ones as \lIf) can now be used with a
%                              star. If done, no end of line are done, so you can enclose
%                              l command into another one. For example, you can write:
%                              \lForEach{$i$}{\lIf*{foo}{bar}}.
%                               Note that when you use a star, side comments are not allowed.
%                   * CHANGE/ADD: Now you can have a side comment at end of macros which
%                               have a block. For example you can do : 
%                               \Begin(\tcc*[h]{side comment for begin}{text}(\tcc*[h]{side comment after end})
%                               Note: there are some side effects for some commands:
%                              \SetKwProg : macro defined thanks to \SetKwProg are allowed
%                                                   to have no end marker. In this case,
%                                                   beware to end side comment, this can
%                                                   do weird output (but no error)
%                   * CHANGE: \SetKwSwitch defines also an \uOther command which was not
%                               the case until this release.
%                   * CHANGE: \SetStartEndCondition{typo1}{typo2}{typo3} defined two end
%                               conditions (type2 and typo3) : typo3 is no more used for
%                               case condition as typo2 is used which is more consistent
%                               since there is a condition followed by a keyword as for
%                               if-then or other command that are defined using typo2.
%                   * CHANGE: keywords was not language dependant to allow to use multiple
%                               languages in the same document, but some keywords in
%                               different language were having the same keyword that lead
%                               last one declared to replace first one and so you could have some
%                               spanish keywords printed as you were in portuguese. So
%                               this behavior is changed from now:
%                               - localized keywords are defined if according language
%                                  option is defined ; 
%                               - if you want to keep old behaviour and use localized
%                                  keywords without using language option (keep old
%                                  behavior), you can use languagekw option
%                                  (e.g. frenchkw, germankw, ...). Note that you can use
%                                  multiple languagekw options at the same time, in
%                                  contrary of language option. Note also that if you use
%                                  multiple languagekw options, you can get back the same
%                                  problem as previously when keywords was not language
%                                  dependant.
%                   * ADD: new typo styles:
%                               - Arguments of functions have now their own style. By
%                                  default, FuncArgSty is the same as ArgSty. 
%                               - Name of KwProg have now their own sty (they used ArgSty
%                                  previously). By default, ProgSty is still ArgSty.
%                               As usual, \SetFuncArgSty{}, FuncArgSty{} and
%                               \SetProgSty{}, ProgSty{} are macros to set and use these
%                               typo styles.
%                   * ADD: Options to manage algorithm hangindent
%                            Until this revision, long statement acts as classical text and
%                            continue on next line starting from the same point. This makes
%                            difficult to notice that the new lines of text is not a new
%                            statement. Now, hangindent is managed and when a long
%                            statement continue on next lines, lines, except the first,
%                            are indented.
%                            Option: noalgohanging
%                               By default, long statement are indented on subsequent
%                               lines; with this option you get old behavior and lines are
%                               no more indented
%                            Option: hangingcomment 
%                               Comment that are alone on a line (not side comment) are
%                               not driven by algo hanging: subsequent lines of long
%                               comments are indented according to width of start comment
%                               marker. With this option, comment are indented like normal
%                               statement.
%                            Option: hanginginout
%                               As for comment, by default, in/out keywords and input
%                               keywords (defined by \SetKwInOut or \SetKwInput) are not
%                               indented by algorithm hangindent. They are indented
%                               according to width of input keyword. If you want that these
%                               keywords acts like normal statement, use this option.
%                            \SetAlgoHangIndent{length}
%                               This macro allows you to set your own indent length. By
%                               default, \SetAlgoHangIndent{0.5em}
%                   * ADD: Group markers. 
%                            This option is related to block markers of release 5.0. Some
%                            have ask to put also block markers for single line
%                            command. This new feature has been implemented to do this.
%                            So, you can now ask package to put begin and end keywords
%                            automatically at start and end of single line command (see
%                            example in documentation).
%                            These new group markers macros are:
%                            - \AlgoDisplayGroupMarkers and \AlgoDontDisplayGroupMarkers
%                            Note that a new option has also been added: displaygroupmarkers
%                   * ADD: \SetCustomAlgoRuledWidth{length}
%                             set a custom ruled width of ruled and algoruled options ;
%                             note that by the moment you use this macro, rules will have
%                             this fixed length: this can cause strange behavior in
%                             multicolumn mode or other layout that change the line
%                             width. 
%                   * ADD: turkish language option
%                   * FIX: a spurious whitespace which results in a spurious indent in the
%                            user's text right after the end of the algorithm environment
%                            was introduced  in release 5.0. This is fixed now thanks to
%                            Alexander Malkis.
%                   * FIX: there was a problem with margins in caption when option figure
%                            was use with caption package. This is fixed.
%                   * FIX: when changing font size in caption with, interline skip stayed
%                            unchanged and so with a small font was to large. This is fixed.
%                   * FIX: in contrary of that is written in the documentation, ':' what
%                            not in KwSty typo for KwIn and KwOut command. This is fixed. 
%                   * FIX: strange behaviour with label and lines numbered: @currentlabel
%                            was updated according to algo line number not in all
%                            situation. For e.g, with hyperref package, always updated ;
%                            with \nlset also updated, but with \nl or linesnumbered
%                            option, not updated. This "feature" causes different output
%                            with \label command according to options used which is not
%                            that one want. This is solved now, and @currentlabel is
%                            always updated so \label command works always is the same way.
%                   * FIX: some czech keywords
%                   * FIX: some spanish keywords
%                   * FIX: some croatian keywords
%                   * FIX: krantz class changes definition of chapter and get one more
%                            option that classical classes as book.cls or report.cls and
%                            broke fix for hyperref on chapter definition. This is now
%                            fixed and algorithm detects use of krantz class and use then
%                            a definition of chapter working with krantz class.
%                   * FIX: an issue with internal macro which causes ([Q]) use as argument
%                            of some environment to be misprinted (thanks to Martin Schr?der).
%                   * FIX: mispelled name of hyperrefcounter inside internal macro.
%
%   - January 06 2013 - revision 5.0
%                     * CHANGE: SetKwSwitch takes now 9 args: 9th arg is the same as
%                                previous 8th arg ('end of switch' keyword). New 8th arg is
%                                'end of case' keyword. This is due to change of release
%                                3.2 which introduce end after case block... as I never
%                                test with longend option, I never see that the 'end
%                                switch' used for case was not good.
%                     * CHANGE: when no end keyword is defined in a block macro, then
%                                algorithm2e does no more try to print it. So even with lined or noline
%                                option, no empty line is printed (before: a blank end was
%                                printed, so a blank line appeared)
%                     * Internal Change: add some internal function to improve readibility
%                                        (thanks to Philip K. F. H\?lzenspies)
%                     * ADD: Block markers. 
%                            You can now ask package to put begin and end keywords automatically at begin
%                            and end of blocks, it means each group of commands shifted and enclosed in
%                            braces.
%                            This is tricky to use but, combined with \SetStartEndCondition and
%                            redefinition of keywords, you should be abble to simulate any syntax. See
%                            examples in documentation where a generic example is derived in pseudo-code,
%                            python and C by keeping code and changing only style using block markers
%                            macros, \SetStartEndCondition and some redefinition of keywords.
%                            These new block markers macros are:
%                            - \AlgoDisplayBlockMarkers and \AlgoDontDisplayBlockMarkers
%                            - \SetAlgoBlockMarkers{begin marker}{end marker}
%                            - \BlockMarkersSty{text} and \SetBlockMarkersSty
%                            Note that a new option has also been added: displayblockmarkers
%                     * ADD: \leIf macro automatically defined by \SetKwIF: allow to define
%                            an if-then-else on a single line.
%                     * ADD: new macro \SetStartEndCondition{typo1}{typo2}{typo3} which
%                            sets typo around condition in For, If, Switch, Case and
%                            Repeat macros. First two are used around For, If, Swith
%                            conditions, First and third are used for Case and Repeat
%                            condition where condition ends the line. Default definition
%                            is \SetStartEndCondition{ }{ }{}. 
%                            A common alternative is \SetStartEndCondition{ (}{) }{)}
%                            Can also be used to remove space around condition, for
%                            example if you want python style commands:
%                            \SetStartEndCondition{ }{}{} and \SetKwFor{For}{for}{:}{}
%                     * ADD: new environment algomathdisplay which allow display math (like inside \[ \] or $$ $$) 
%                            handling end line and line number
%                     * ADD: new command \SetKwProg{Env}{Title}{is}{end} which defines a macro
%                            \Env{args}{text}. Env is a block with 'Title' (in \CapSty) at the beginning
%                            followed by args followed by 'is' then 'text' is put below inside a block ended
%                            by 'end'. If no 'end' is specified, nothing is written (no
%                            blank line is inserted). Useful to typeset function or prog for example:
%                            \SetKwProg{Fn}{Function}{ is}{end} makes \Fn{afunc(i: int) : int}{return 0\;}                    
%                            writes: 
%                            Function afunc(i: int) : int is
%                            | return 0;
%                            end
%                            or \SetKwProg{Def}{def}{:}{} makes \Def{afunc(i: int)}{return 0\;} writes:
%                            def afunc(i: int):
%                            | return 0
%                            Tip: combine it with \SetKwFunction to write recursive function algorithm. With
%                            example above, you could define \SetKwFunction{\Afunc}{afunc} and then write:
%                            \Def{\Afunc{i:int}{\eIf{i>0}{\KwRet \Afunc{i-1}}{\KwRet 0\;}} that writes:
%                            def afunc(i: int):
%                            | if(i>0):
%                            |     return afunc(i-1)
%                            | else:
%                            |     return 0
%                            with appropriate typo.
%                     * ADD: option croatian: croatian keywords (thanks to Ivan Gavran)
%                     * ADD: option ngerman: same as german option but so can be used with global option ngerman
%                            of babel
%                     * ADD: option spanish: Spanish support (thanks to Mario Abarca)
%                     * ADD: unterminated block: useful to add part separator that doesn't necessary need an end
%                            keyword.  
%                            Designed on the pattern of unterminated if (see \uIf macro) allowing to
%                            add a block that is not terminated by a keyword. Such block are defined in the same
%                            time as a block is defined by adding a macro beginning with u. So, for example,
%                            predefined \SetKwBlock{Begin}{begin}{end} defines now two commands:
%                            - \Begin{} as previously which print a begin - end block
%                            - \uBegin{} that defines a begin only block
%                     * FIX: problem when numbering line inside until condition of
%                            \SetKwRepeat macro: line number was not correctly aligned.
%                     * FIX: dotocloa option which was broken
%                     * FIX: uIf and uCase didn't have same behavior when used with
%                            noline, vlined or lined option. This is fixed. Side effect: no empty
%                            line after an uIf or uCase when used with options lined or vlined
%                     * FIX: a bug with Repeat Until command when use with side comment on Until
%                     * FIX: a bug with side text -- text put into () -- of command macro (SetKwIf and so on)
%                            which was always setting a ';' even after a \DontPrintSemicolon
%                     * FIX: a bug with hyperref and chapter definition (thanks to Hubert Meier)
%                     * FIX: bugs with l macro and side comment
%                     * FIX: revision number
%                     * FIX: fix non ascii character (utf8 not yet recognized by all latex engine)
%                     * FIX: fnum@algocf had an useless parameter which sometimes broke expansion and output an error
%                     * FIX: works now with multicol package
%
%   - december 14 2009 - revision 4.1
%                     * ADD: new command \SetKwHangingKw{Name}{text} (hanging indent with keyword): This creates a
%                            hanging indent much like \texttt{SetKwInput}, except that it removes the trailing `:'
%                            and does not reset numbering (thanks to Nathan Tallent)
%
%   - november 17 2009  - revision 4.00 -
%
%                      * CHANGE: IMPORTANT: some commands have been renamed to have consistent naming (CamlCase
%                                syntax) and old commands are no more available. If you doesn't want to change
%                                your mind or use old latex files, you can use oldcommands option to enable old
%                                commands back.
%                                text. Here are these commands:
%                                - \SetNoLine becomes \SetAlgoNoLine
%                                - \SetVline  becomes \SetAlgoVlined
%                                - \Setvlineskip  becomes \SetVlineSkip
%                                - \SetLine   becomes \SetAlgoLined
%                                - \dontprintsemicolon becomes \DontPrintSemicolon
%                                - \printsemicolon becomes \PrintSemicolon
%                                - \incmargin becomes \IncMargin
%                                - \decmargin becomes \DecMargin
%                                - \setnlskip becomes \SetNlSkip
%                                - \Setnlskip becomes \SetNlSkip
%                                - \setalcapskip becomes \SetAlCapSkip
%                                - \setalcaphskip becomes \SetAlCapHSkip
%                                - \nlSty becomes \NlSty
%                                - \Setnlsty becomes \SetNlSty
%                                - \linesnumbered becomes \LinesNumbered
%                                - \linesnotnumbered becomes \LinesNotNumbered
%                                - \linesnumberedhidden becomes \LinesNumberedHidden
%                                - \showln becomes \ShowLn
%                                - \showlnlabel becomes \ShowLnLabel
%                                - \nocaptionofalgo becomes \NoCaptionOfAlgo
%                                - \restorecaptionofalgo becomes \RestoreCaptionOfAlgo
%                                - \restylealgo becomes \RestyleAlgo
%                                - gIf macros and so on do no more exist
%                      * NEW: - Compatibily with other packages improven by changing name of internal
%                               macros. Algorithm2e can now be used with arabtex for example, if this last is
%                               loaded after algorithm2e package.
%                      * ADD: - OPTION endfloat: endfloat packages doesn't allow float environment inside other
%                               environment. So using it with figure option of algorithm2e makes error. This
%                               option enables a new environment algoendfloat to be used instead of algorithm
%                               environment that put algorithm at the end. algoendfloat environment make
%                               algorithm acting as endfloat figures. This option requires endfloat packages.
%                      * ADD: - OPTION norelsize: starting from this release (v4.00), algorithm2e package uses
%                               relsize package in order to get relative size for lines numbers; but it seems
%                               that some rare classes (such as inform1.cls) are not compatible with relsize; to
%                               have algorithm2e working, this option makes algorithm2e not to load relsize
%                               package and go back to previous definition by using \scriptsize font for lines
%                               numbers.
%                      * ADD: - OPTION onelanguage: allow, if using standard keywords listed below, to switch
%                               from one language to another without changing keywords by using appropriate
%                               language option:
%                               . KwIn, KwOut, KwData, KwResult
%                               . KwTo KwFrom
%                               . KwRet, Return
%                               . Begin
%                               . Repeat
%                               . If, ElseIf, Else
%                               . Switch, Case, Other
%                               . For, ForPar, ForEach, ForAll, While
%                               .
%                      * ADD: - OPTION rightnl: put lines numbers to the right of the algorithm instead of left.
%                      * ADD:   new commands \setRightLinesNumbers and \setLeftLinesNumbers which sets the lines
%                               numbers to the right or to the left of the algorithm.
%                      * ADD: - new kind of keywords: KwArray used to define arrays:
%                               \SetKwArray{Kw}{array} defines an array keywords Kw called array and printed in
%                               DataSty style when call with \Kw. It can be used with one argument which
%                               denotes the element index: \Kw{n} prints array[n] with array in DataSty and n in
%                               ArgSty.
%                      * ADD/FIX: rules of ruled, algoruled, tworuled styles used rules of different sizes! This
%                                 is now fixed. Moreover size of the rules is now controlled by a length and so
%                                 can be customized by the user.
%                                 \algoheightrule is the height of the rules and can be changed via \setlength
%                                 \algoheightruledefault is the default height of he rules (0.8pt)
%                                 \algotitleheightrule is the height of the rule that comes just after the
%                                 caption in ruled and algoruled style; it can be changed via \setlength
%                                 \algotitleheightruledefault is the default height of this rules (0.8pt)
%                                 Thanks to Philippe Dumas who reports the bug and make the suggestion.
%                      * ADD: - \SetAlgoCaptionSeparator which sets the separator between Algorithm 1 and the
%                               title. By default it's ':' and caption looks like "Algorithm 2: title" but now
%                               you can change it by using for example \SetAlgoCaptionSeparator{.} which will
%                               give "Algorithm 3. title"
%                      * ADD: - \SetAlgoLongEnd and \SetAlgoShortEnd and \SetAlgoNoEnd commands which act as
%                               corresponding package options
%                      * ADD: - OPTIONS italiano and slovak as new language (thanks to Roberto Posenato and
%                               Miroslav Binas) 
%                      * CHANGE: - Fnt and Sty macro to have consistent use and naming (see below)
%                      * ADD: - \AlCapSty, \AlCapNameSty, \AlCapFnt, \AlCapNameFnt, \ProcSty, \ProcFnt,
%                               \ProcNameSty, \ProcNameFnt, \ProcArgSty, ProcArgFnt and corresponding "set macro" 
%                               \SetAlCapSty, \SetAlCapNameSty, \SetAlCapFnt, \SetAlCapNameFnt, \SetProcSty,
%                               \SetProcFnt, \SetProcNameSty, \SetProcNameFnt, \SetProcArgSty, \SetProcArgFnt which
%                               control the way caption is printed. Sty macro use command taking one parameter as
%                               argument, Fnt macros use directly command. In Fact caption is printed as follow:
%                               \AlCapSty{\AlCapFnt Algorithm 1:}\AlCapNameSty{\AlCapNameFnt my algorithm}
%                               By default, \AlCapSty is textbf and \AlCapFnt is nothing. \AlCapNameSty keep text 
%                               as it is, and \AlCapNameFnt do nothing also.
%                               You can redefine \AlCapFnt and \AlCapNameFnt by giving macro to \Set commands. For
%                               example, you can do \SetAlCapFnt{\large} to see Algorithm printed in \large font.
%                               You can redefine \AlCapSty, \AlCapFnt, \AlCapNameSty and \AlCapNameFnt with the
%                               corresponding \Set command. For the Sty commands, you have to give in parameter
%                               name of a macro (whithout \)  which takes one argument. For example,
%                               \SetAlCapFnt{textbf} defines the default behaviour. If you want to do more
%                               complicated thing, you should define your own macro and give it to \SetAlCapFnt or
%                               \SetAlCapNameFnt. Here are two examples:
%                               - \newcommand{\mycapsty}[1]{\tiny #1}\SetAlCapNameSty{mycapsty}
%                               - \newcommand{\mycapsty}[1]{\textsl{\small #1}}\SetAlCapNameSty{mycapsty}
%                               Or you can combine the two, for the last example you can also do:
%                               \SetAlCapNameSty{textsl}\SetAlCapNameFnt{\small}
%                               Thanks to Jan Stilhammer who gives me the idea of \AlCapNameFnt.
%                      * CHANGE \AlTitleFnt to match definition of all other Fnt macros and add a \AlTitleSty 
%                               macro (see below) . Now you set \AlTitleFnt by calling \SetAlTitleFnt with 
%                               directly a macro without parameter in argument:
%                               Example: \SetAlTitleFnt{\small} to set title in small font.
%                      * ADD: - \AlTitleSty and \SetAlTitleSty commands to set a style for title. These commands
%                               are defined from a macro taking the text in argument, as \textbf for example. 
%                               To set the TitleSty you have to give name of the macro (without the '\') 
%                               to \SetAlTitleSty. For example \SetAlTitleSty{textbf} to set \textbf style.
%                      * ADD: - new command \SetAlgorithmName{algorithmname}{list of algorithms name} which
%                               redefines name of the algorithms and the sentence list of algorithms. Second
%                               argument is the name that \autoref, from hyperref package, will use. Example:
%                               \SetAlgorithmName{Protocol}{List of protocols} if you prefer protocol than
%                               algorithm.
%                      * ADD: - new \SetAlgoRefName{QXY} which change the default ref (number of the algorithm) by
%                               the name given in parameter (QXY in the example). 
%                      * ADD: - new command \SetAlgoRefRelativeSize{-2} which sets the output size of refs, defined
%                               by \SetAlgoRefName, used in list of algorithms.
%                      * ADD: - two dimensions to control the layout of caption in ruled, algoruled and boxruled
%                               algorithms:
%                               - interspacetitleruled (2pt by defaut) which controls the vertical space between
%                                 rules and title in ruled and algoruled algorithms.
%                               - interspaceboxruled (2\lineskip by default) which controls the vertical space
%                                 between rules and title in boxruled algorithms.
%                               These two dimensions can be changed by using \setlength command.
%                      * ADD: - With the fix (see below) of procedure and function environments, a new feature has
%                               been added: the name of the procedure or function set in caption is automatically
%                               defined as a KwFunction and so can be used as a macro. For example, if inside a
%                               procedure environment you set \caption{myproc()}, you can use \myproc macro in you
%                               main text. Beware that the macro is only defined after the \caption!
%                      * ADD: - OPTION nokwfunc to unable the new feature described above in function and
%                               procedure environment. Useful if you use name of procedure or function that cannot
%                               be a command name as a math display for example.
%                      * ADD: - \SetAlgoNlRelativeSize{number} command which sets the relative size of line
%                               numbers. By default, line numbers are two size smaller than algorithm text. Use
%                               this macro to change this behavior. For example, \SetAlgoNlRelativeSize{0} sets it
%                               to the same size, \SetAlgoNlRelativeSize{-1} to one size smaller and
%                               \SetAlgoNlRelativeSize{1} to one size bigger
%                      * ADD: - \SetAlgoProcName{aname} command which sets the name of Procedure printed by
%                               procedure environment (the environment prints Procedure by default). Second
%                               argument is the name that \autoref, from hyperref package, will use.
%                      * ADD: - \SetAlgoFuncName{aname} command which sets the name of Function printed by
%                               procedure environment (the environment prints Function by default). Second
%                               argument is the name that \autoref, from hyperref package, will use. 
%                      * ADD: - \SetAlgoCaptionLayout{style} command which sets style of the caption; style must
%                               be the name of a macro taking one argument (the text of the caption). Examples
%                               below show how to use it:
%                               . \SetAlgoCaptionLayout{centerline} to have centered caption
%                               . \SetAlgoCaptionLayout{textbf} to have bold caption
%                               If you want to apply two styles in the same time, such as centered bold, you have
%                               to define you own macro and then use \SetAlgoCaptionLayout with its name.
%                      * ADD: - OPTION procnumbered: which makes the procedure and function to be numbered as
%                               algorithm
%                      * ADD: - OPTIONS tworuled and boxruled
%                               these are two new layouts: tworuled acts like ruled but doesn't put a line after
%                               caption ; boxruled surround algorithm by a box, puts caption above and add a line
%                               after caption.
%                      * REMOVE: - SetKwInParam has been deleted since not useful itself because of different
%                                macros which can do the same in a better and a more consistent way as
%                                SetKwFunction or SetKw.
%                      * FIX: - line number is now correctly vertically aligned with math display.
%                      * FIX: - references with hyperref. No more same identifier or missing name error. BUT now
%                               you must NOT use naturalnames option of hyperref packages if you do PdfLaTeX
%                      * FIX: - autoref with hyperref package (thanks to J?rg Sommer who notices the problem).
%                      * FIX: - titlenumbered was not working! fixed.
%                      * FIX: - Else(){} acted like uElse. Corrected.
%                      * FIX: - noend management: when a block was inside another and end of block was following
%                               each other, a blank line was added: it's now corrected.
%                      * FIX: - Function and Procedure environment was no more working as defined originally: the
%                               label was no more name of the procedure, it acts always as if procumbered option
%                               has been used.
%                      * FIX: - line numbers had a fixed size which can be bigger than algorithm text accordingly
%                               to \AlFnt set (see also new command \SetAlgoNlRelativeSize above)
%                      * FIX: - semicolon in comments when dontprintsemicolon is used.
%                      * FIX: - listofalgorithms adds a vertical space before first algo of a chapter as for
%                               listoffigures or listoftables
%                      * FIX: - listofalgorithms with twocolumns mode and some classes which don't allow onecolumn
%                               and so don't define \if@restonecol as prescribed in LaTeX (sig-alternate for
%                               example)
%                      * FIX: - algorithm2e now works with elsart cls and some more classes.
%                      * FIX: - blocks defined by SetKwBlock act now as other blocks (if for instance) and don't
%                               write end in vlined mode, instead they print a small horizontal line as required
%                               by the option.
%                      * FIX: - underfull hbox warning at each end of algorithm environment removed.
%
%                      * INTERNAL CHANGE: - short end keyword are deduce from long end keyword by keeping the
%                                           first one. Allows to avoid double definition.
%                      * INTERNAL CHANGE: - procedure, function and algorithm are now resolved by the same
%                               environment to avoid code duplication. 
%
%   - October  04 2005  - revision 3.9 -
%                      * ADD: - \setalcaphskip command which sets the horizontal skip before Algorithm: in caption
%                               when used in ruled algorithm.
%                      * ADD: - \SetAlgoInsideSkip command which allows to add an extra vertical space before and
%                               after the core of the algorithm (ie: \SetAlgoInsideSkip{bigskip}) 
%                      * CHANGE: - caption, when used with figure option, is no more controlled by algorithm2e
%                                  package and so follows the exact behaviour of figures. The drawback is that you
%                                  cannot change the typo with AlTitleFnt or CapFnt. The avantage is that if you
%                                  use caption package, it works.
%                      * FIX: - problem with numbering line and pdflatex
%                      * FIX: - error when algorithm2e package was used with beamer and listings together
%   - February 12 2005  - revision 3.8 -
%                      * FIX: - extra line with noend option.
%   - February 10 2005  - revision 3.7 -
%                      * ADD: - sidecomment: different macros allowing to put text right after code on the same
%                               line. They are defined in the same time comment macros are defined with a star
%                               after the macro name. By default comments are right justified but this can be
%                               change with appropriate option in the macro. Ex:
%                               . default: \tcc*{side comment}
%                               . same as previous: \tcc*[r]{side comment}
%                               . left justify: \tcc*[l]{side comment}
%                               . here: \tcc*[h]{side comment} don't put the end of line mark before
%                                       comment (; by default) and don't end the line.
%                               . flushed: \tcc*[f]{side comment} same as the precedent but right
%                                 justified
%                      * ADD: - OPTION scright (default): right justified side comments (side comments
%                               are flushed to the righr)
%                      * ADD: - OPTION scleft: left justified side comments (side comments are put right after the
%                               code line)
%                      * ADD: - \SetSideCommentLeft acts as scleft option
%                      * ADD: - \SetSideCommentRight acts as scright option
%                      * ADD: - block like macro side text: all macro defining a block allows now to put text right
%                               after key words by putting text into (). Done to be used with sidecomment macros,
%                               but all text can be used. 
%                               Ex: \eIf(\tcc*[f]{then comment}){test}{then text}(else side text){else text}
%                      * ADD: - OPTION fillcomment (default): end mark of comment is flushed to the right so
%                               comments fill all the width of text.
%                      * ADD: - OPTION nofillcomment: end mark of comment is put right after the comment.
%                      * ADD: - \SetNoFillComment acts as nofillcomment option.
%                      * ADD: - \SetFillComment acts as fillcomment option.
%                      * ADD: - OPTION dotocloa: which adds an entry in the toc for the list of algorithms. This
%                               option load package tocbibind if not already done and so list of figures and list
%                               of tables are also added in the toc. If you want to control which ones of the lists
%                               will be added in the toc, please load package tocbibind before package algorithm
%                               and give it the options you want.
%                      * FIX: - vertical spacing for uif macro with noend option
%                      * FIX: - all the compatibility problems between caption and other packages
%                      * FIX: - typographical differences between list of algorithms and other lists  when in
%                               report or book 
%
%   - January 24 2005  - revision 3.6 -
%                      * FIX: - vertical spacing and space characters at the beginning or end of comments.
%                               line numbers of comments not in the NlSty.
%                               Thanks to Arnaud Giersch for his comments and suggestions.
%                      * FIX: - Set*Sty macro: the styles defined was not protected and was modified by surrounding
%                               context. For example KwTo in a \For{}{} was in bold AND italic instead of just in
%                               bold.
%                      * FIX: - line number misplacement after \Indp
%
%   - January 21 2005  - revision 3.5 -
%                      * ADD: - hidden numbering of the lines. Lines are auto-numbered but numbers are shown only
%                               on lines you specify:
%                               * linesnumberedhidden option or \LinesNumberedHidden macro activate this
%                                 functionnality.
%                               * \ShowLn and \ShowLnLabel{lab} macros make the number visible on the
%                               line. \ShowLnLabel{lab} allows to set a label for this line. 
%                               Thanks to Samson de Jager who makes this suggestion and provides the macros.
%                      * ADD: - \AlCapFnt and \SetAlCapFnt which allow to have a different font for
%                               caption. Works like \AlFnt and \SetAlFnt and by default is the same.
%                      * ADD: - \AlCapSkip skip length. This vertical space is added before caption in plain ou
%                               boxed mode. It allows to change distance between text and caption.
%                      * FIX: - caption compatible with IEEEtran class. 
%                      * FIX: - some vertical spacing error with \uIf macros (Thanks to Arnaud Giersch)
%                      * FIX: - Procedure and Function: lines are also numbered like algorithms
%                      * FIX: - CommentSty was not used for Comments
%
%   - January 10 2005  - revision 3.4 -
%                      * FIX: - caption compatible with new release of Beamer class. 
%
%   - June 16 2004     - revision 3.3 - 
%                      * FIX: - Hyperlink references of Hyperref package works now if compiled with pdflatex 
%                               and [naturalnames] option of hyperref package is used.
%                      * FIX: - algorithm[H] had problem in an list environment - corrected
%                      * FIX: - interline was not so regular in nested blocks - corrected
%                      * ADD  - \SetVlineSkip macro which sets the vertical skip after the little horizontal 
%                               rule which closes a block in Vlined mode. By default 0.8ex
%
%   - June 11 2004     - revision 3.2 - AUTO NUMBERING LINES !!!
%                      * ADD: auto numbering of the lines (the so asked and so long awaiting feature)
%                             this feature is managed by 3 options and 3 commands:
%                             - linesnumbered option: lines of the algo are numbered except for comments and
%                               input/output (KwInput and KwInOut)
%                             - commentsnumbered option: makes comments be numbered
%                             - inoutnumbered option: makes data input/output be numbered
%                             - \nllabel{lab} labels the line so you can cite with \ref{lab}
%                             - \LinesNumbered make the following algorithms having auto-numbered lines
%                             - \linesnotnumbered make the following algorithms having no auto-numbered lines
%                      * Change: algo2e option renames listofalgorithms in listofalgorithmes
%                      * FIX: new solution for compatibility with color package, more robust and not tricky.
%                             Many thanks to David Carlisle for his advices
%
%   - June 09 2004     - revision 3.1 -
%                      * Change: \SetKwSwitch command defines an additionnal macro \uCase and \Case prints end
%                      * Change: now macros SetKw* do a renewcommand if the keyword is already defined. So you can
%                                redefine default definition at your own convenience or change your definition
%                                without introducing a new macro and changing your text.
%                      * ADD: new macro \SetKwIF which do \SetKwIf and
%                             \SetKwIfElseIf.The following default definition has been added:
%                             \SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
%                             and so you get the macros;
%                             \If \eIf \lIf \uIf \ElseIf \uElseIf \lElseIf \Else \uElse \lElse
%                      * ADD: new macro \SetAlgoSkip which allow to fix the vertical skip before and after the
%                             algorithms. Default is smallskip, do \SetAlgoSkip{} if you don't want an extra space
%                             or \SetAlgoSkip{medskip} or \SetAlgoSkip{bigskip} if you want bigger space.
%                      * ADD: macro \SetKwIf defines in addition a new macro \uElse  (depending on wat name you
%                             have given in #2 arg).
%                      * ADD: macro \SetKwIfElseIf defines in addition a new macro \uElse and \ugElseIf (depending
%                             on what name you have given in #2 and #3 arg).
%                      * Change: baseline of algorithm is now top, so two algorithms can be put side by side.
%                      * FIX: Compatibility with color package solved. The problem was due to a redefinition of
%                             standard macros by color package. This solves compatibility problem with other
%                             packages as pstcol or colortbl. (notified by Dirk Fressmann, Antti Tarvainen and Koby
%                             Crammer)
%                      * Fix: extra little shift to the right with boxed style algorithm removed (notified by
%                             P. Tanovski)
%                      * Fix: algoln option was buggy (notified bye Jiaying Shen)
%                      * Fix: german and portuges option didn't work due to bad typo (notified by Martin Sievers,
%                             Thorsten Vitt and Jeronimo Pellegrini)
%                      
%   - February 13 2004 - revision 3.0 -
%                      * Major revision which makes the package independent from float.sty, so now
%                        - algorithm* works better, in particular can be used in multicols environments
%                        - (known bug corrected)
%                          [H] works now for all sort of environment but is handled differently for classic
%                          environment and star environment (algorithm, figure, procedure and function). For star
%                          environment, H acts like for classical figure environment, so it doesn't stay here
%                          absolutely.
%                        - (known bug corrected)
%                          you can use now floatflt package with algorithm package and even with figure
%                          option. Beware that if you want to put an algorithm inside a floatingfigure, it cannot
%                          be floating, so [H] is required and then figure option should not be used, since
%                          standard figure[H] are still floating with LaTeX.
%                      * boxruled: a new style added. Possible now since no style no more defined by the float
%                        package.
%                      * nocaptionofalgo: dosen't print Algorithm #: in the caption for algorithm in ruled or
%                        algoruled style.
%                        note: this is just documentation of a macro which was already in the package.
%   - December 14 2003 - revision 2.52 -
%                      * output message shorter
%                      * French keyword macro \PourTous was missing for longend option, it has been added.
%                      * TitleofAlgo prints Function or Procedure in corresponding environments.
%
%   - October 27 2003  - revision 2.51 - Revision submitted to CTAN archive
%                      * correction of a minor which make caption in procedure
%                        and function to be blanck with pdfscreen package
%                        (thanks to Joel Gossens for the notification)
%                      * add two internal definition to avoid some errors when
%                        used with Hyperref package (Hyperref package need to
%                        define new counter macro from existing ones, and
%                        don't do it for algorithm2e package, so we do it)
%
%   - October 17 2003  - revision 2.50 - first revision for CTAN archive
%                      * add \AlFnt and \SetAlFnt{font} macros: \AlFnt is used at the beginning of the caption and
%                        the body of algorithm in order to define the fonts used for typesetting algorithms. You
%                        can use it elsewhere you want to typeset text as algorithm. For example you can do
%                        \SetAlFnt{\small\sf} to have algorithms typeset in small sf font. Default is nothing so
%                        algorithm is typeset as the text of the document.
%                      * add \AlTitleFnt{text} and \SetAlTitleFnt{font} macros: The {Algorithm: } in the caption is
%                        typeset with \AlTitleFnt{Algorithm:}. You can use it to have text typeset as {Algorithm:}
%                        of captions. Default is textbf.  Default can be redefined by \SetAlTitleFnt{font}, for
%                        example you can do \SetAlTitleFnt{emph}
%                      * add CommentSty typo for text comment.  
%                      * add some compatibility with hyperref package (still an error on multiply defined refs but
%                        pdf correctly generated)
%                      * flush text to left in order to have correct indentation even with class as amsart which
%                        center all figures
%                      * add german, portuguese and czech options for title of algorithms and typo.
%                      * add portuguese translation of predefined keywords * add czech translation of some
%                        predefined keywords
%
%   - December 23 2002 - revision 2.40
%                      * add some French keyword missing
%                      * add function* and procedure* environment like algorithme* environment: print in one column
%                        even if twocolumn option is specified for the document.
%                      * add a new macro \SetKwComment to define macro which writes comments in the text. First
%                        argument is the name of the macro, second is the text put before the comment, third is the
%                        text put at the end of the comment.Default are \tcc and \tcp
%                      * add new options to change the way algo are numbered:
%                        [algopart] algo are numbered within part (counter must exist)
%                        [algochapter] algo are numbered within chapter
%                        [algosection] algo are numbered within section
%
%   - March 27 2002   - revision 2.39
%                      * Gilles Geeraerts: added the \SetKwIfElseIf to manage
%                        if (c)
%                             i;
%                        else if (c)
%                             i;
%                        ...
%                        else
%                             i;
%                        end
%                      * Also added \gIf \gElseIf \gElse.
%
%   - January 02 2001 - revision 2.38
%                      * bugs related to the caption in procedure and function
%                        environment are corrected.
%                      * bug related to option noend (extra vertical space added
%                        after block command as If or For) is corrected.
%                      * czech option language added (thanks to Libor Bus: l.bus@sh.cvut.cz).
%  
%   - October 16 2000 - revision 2.37
%                      * option algo2e added: change the name of environment
%                        algorithm into algorithm2e. So allow to use the package
%                        with some journal style which already define an algorithm
%                        environment.
%  
%   - September 13 2000 - revision 2.36
%                      * option slide added: require package color
%                      * Hack for slide class in order to have correct
%                        margins
%  
%   - November 25 1999 - revision 2.35
%                      * revision number match RCS number
%                      * Thanks to David A. Bader, a new option is added:
%                        noend: no end keywords are printed.
%  
%   - November 19 1999 - revision 2.32
%                      * minor bug on longend option corrected.
%  
%   - August 26 1999 - revision 2.31
%                      * add an option: figure
%                        this option makes algorithms be figure and so are numbered
%                        as figures, have Figure as caption and are put in 
%                        the \listoffigures
%  
%   - January 21 1999 - revision 2.3 beta
%                    add 2 new environments: procedure and function.
%                    These environments works like algorithm environment but:
%                    - the ruled (or algoruled) style is imperative.
%                    - the caption now writes Procedure name....
%                    - the syntax of the \caption command is restricted as
%                      follow: you MUST put a name followed by 2 braces like
%                      this ``()''. You can put arguments inside the braces and
%                      text after. If no argument is given, the braces will be
%                      removed in the title. 
%                    - label now puts the name (the text before the braces in the
%                      caption) of the procedure or function as reference (not
%                      the number like a classic algorithm environment).
%                    There are also two new styles: ProcNameSty and
%                    ProcArgSty. These style are by default the same as FuncSty
%                    and ArgSty but are used in the caption of a procedure or a
%                    function.
%                    
%   - November 28 1996 - revision 2.22
%                    add a new macro \SetKwInParam{arg1}{arg2}{arg3}:
%                    it defines a macro \arg1{name}{arg} which prints name in keyword
%                    style followed byt arg surrounded by arg2 and arg3. The main
%                    application is to a function working as \SetKwInput to be used
%                    in the head of the algorithm. For example
%                    \SetKwInParam{Func}{(}{)} allows
%                    \Func{functionname}{list of arguments} which prints:
%                    \KwSty{functioname(}list of arguments\KwSty{)}
%       
%
%   - November 27 1996 - revision 2.21:
%                    minor bug in length of InOut boxes fixed.
%                    add algorithm* environment.
%
%   - July 12 1996 - revision 2.2: \SetArg and \SetKwArg macros removed.
%                        
%                    \SetArg has been removed since it never has been
%                    documented.
%                    \SetKwArg has been removed since \SetKw can now
%                    take an argument in order to be consistent with
%                    \SetKwData and \SetKwFunction macros.
%
%   - July 04 1996 - revision 2.1: still more LaTeX2e! Minor compatibility break
%
%                    Macros use now \newcommand instead of \def, use of \setlength, 
%                    \newsavebox, ... and other LaTeX2e specific stuff.
%                    The compatibility break:
%                    - \SetData becomes \SetKwData to be more consistent. So the old 
%                      \SetKwData becomes \SetKwInput
%                    - old macros \titleofalgo, \Freetitleofalgo and \freetitleofalgo
%                      from LaTeX209 version which did print a warning message and call 
%                      \Titleofalgo in version 2.0 are now removed!
%
%   - March 13 1996 - revision 2.0: first official major revision.
%   
%
%%%%%%%%%%%%%%
%
%   Known bugs: 
%   -----------
%   - horizontal spacing (indent) doesn't work with revtex4 class.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% for more complete informations you can see algorithm2e.tex
%
%
%%%%%%%%%%%%%%%%%%%%%%%% Identification Part %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\NeedsTeXFormat{LaTeX2e}[1994/12/01]
%
\ProvidesPackage{algorithm2e}[2013/01/06 v5.00 algorithms environments]
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%% Initial Code %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\@makeother\*% some package redefined it as a letter (as color.sty)
\def\@firstword#1 #2\@nil{#1}% an useful fonction
%%%%%%% Utilities:
% \ifArgumentEmpty<c><t><e> ; if c is empty, i.e. {}, then t, else e.
%    Function used internally, but may as well expose it to the user; it's useful
\begingroup
\catcode`\Q=3
\catcode`\T=3
\long\gdef\ALGOCF@argemptyaux#1#2Q#3#4#5T{#4}
\long\gdef\ifArgumentEmpty#1{%
  \begingroup\long\edef\@tempa{\endgroup
    \ALGOCF@argemptyaux#1QQ{\noexpand\@secondoftwo}{\noexpand\@firstoftwo}T%
  }\@tempa
}
\endgroup
% \long\def\ifArgumentEmpty#1{\bgroup
% 	\catcode`\Q=3
% 	\catcode`\T=3
% 	\long\def\@tempa##1##2Q##3##4##5T{##4}%
% 	\xdef\@tempa{\@tempa#1QQ{\noexpand\@secondoftwo}{\noexpand\@firstoftwo}T}%
% \egroup\@tempa}
%%%%%%%%%%%
%
% \algocf@longdef -> shorthand to reduce
%    \expandafter\long\expandafter\def
% to
%    \expandafter\algocf@longdef
% may look insignificant, but reads that much better ;)
\def\algocf@longdef{\long\def}
%
% \algocf@newcommand (and helper \algocf@new@command) behaves like LaTeX's newcommand,
% with two differences:
%  - the argument is not "\<name>", but rather "<name>"; i.e. one level of indirection
%  - if the command exists already, then \renewcommand, rather than \newcommand
\def\algocf@newcommand#1{\expandafter\algocf@new@command\csname#1\endcsname}
\def\algocf@new@command#1{%
	\begingroup \escapechar\m@ne\xdef\@gtempa{{\string#1}}\endgroup
	\expandafter\@ifundefined\@gtempa\newcommand\renewcommand#1}%
%
% \algocf@newcmdside<name><arity><body>
%   The largest time-saver; many commands we define have the pattern:
%     \<name>(<side_text>)<argX><argY>...
%   where "(<side_text>)" is optional. By defining them with this function,
%   the arguments are parsed and renumbered, i.e. the body works as if the
%   command was:
%     \<name><side_text><argX><argY>...
%   and can use \ifArgumentEmpty to see whether its #1 exists (default case
%   for the side text is (), so there's no difference between calling
%     \foo{bar}
%   or
%     \foo(){bar}
%   Technically this is new behaviour, but it shouldn't really occur...
\algocf@longdef\algocf@newcmdside#1#2#3{%
	\expandafter\def\csname#1\endcsname{%
		\@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
	}%
	\expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1){\csname algocf@#1main\endcsname{##1}}%
	\algocf@newcommand{algocf@#1main}[#2]{#3}%
}
%
% a serie of newcmdside macro for block that allows a comment after the end
%     \<name>(<side_text>)<argX><argY>...(<side_text>)% 
%
% 1. kind of begin-end : for command with only one block as begin-end 
\algocf@longdef\algocf@newcmdside@kobe#1#2{% <name of cmd><body of cmd>
  % command starts by checking for side comment at beginning
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
  }%
  % next we strip comment and include it in cmd that get body and check last side comment
  \expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1)##2{\csname algocf@#1checkcomfol\endcsname{##1}{##2}}%
  % now check for last side comment; args are : <first side com (could be empty)>, <body of cmd>
  \expandafter\algocf@longdef\csname algocf@#1checkcomfol\endcsname##1##2{\@ifnextchar({\csname algocf@#1withendcom\endcsname{##1}{##2}}{\csname algocf@#1noendcom\endcsname{##1}{##2}}}% call macro that manages end of command, with or without last side comment
  % finally manage end of macro... with end side comment...
  \expandafter\algocf@longdef\csname algocf@#1withendcom\endcsname##1##2(##3){%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}}%
  % ... or without end side comment
  \expandafter\algocf@longdef\csname algocf@#1noendcom\endcsname##1##2{%
    \csname algocf@#1main\endcsname{##1}{##2}{}}%
  \algocf@newcommand{algocf@#1main}[3]{#2}%
}%
%
% 2. kind of if-else : for command with two blocks as if-then-else 
\algocf@longdef\algocf@newcmdside@koif#1#2{% <name of cmd><body of cmd>
  % command starts by checking for side comment at beginning
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
  }%
  % next we strip comment and include it in cmd that get body and check last side comment
  \expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1)##2##3{\csname algocf@#1checkcomfol\endcsname{##1}{##2}{##3}}%
  % now check for last side comment; args are : <1st side com>, <1st body of cmd>, <2nd body of cmd>
  \expandafter\algocf@longdef\csname algocf@#1checkcomfol\endcsname##1##2##3{\@ifnextchar({\csname algocf@#1withendcom\endcsname{##1}{##2}{##3}}{\csname algocf@#1noendcom\endcsname{##1}{##2}{##3}}}% call macro that manages end of command, with or without last side comment
  % finally manage end of macro... with end side comment...
  \expandafter\algocf@longdef\csname algocf@#1withendcom\endcsname##1##2##3(##4){%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}{##4}}%
  % ... or without end side comment
  \expandafter\algocf@longdef\csname algocf@#1noendcom\endcsname##1##2##3{%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}{}}%
  \algocf@newcommand{algocf@#1main}[4]{#2}%
}%
%
% \algocf@newcmdsides<name><arity><body><tail><closing>
%   Like the command above, but with an optional side text at the end
%   of the command as well, i.e.:
%     \<name>(<side_text>)<argX><argY>(<end_text>)
%   It may be a bit confusing that <arity> doesn't count <end_text>,
%   but since it is for internal use, the naming can be a little more
%   fuzzy. This function behaves as if:
%     <body'> = <body><if end_text: tail{end_text}><closing>
\algocf@longdef\algocf@newcmdsides#1#2#3#4#5{%
	\expandafter\def\csname#1\endcsname{%
		\@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
	}%
	\expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1){\csname algocf@#1main\endcsname{##1}}%
	\algocf@newcommand{algocf@#1main}[#2]{#3\@ifnextchar({\csname algocf@#1end\endcsname}{#4#5}}%
	\expandafter\algocf@longdef\csname algocf@#1end\endcsname(##1){#4{##1}\strut\par}%
}%
%
% definition of commands which can be redefined in options of the package.
%
\newcounter{AlgoLine}%
\setcounter{AlgoLine}{0}%
%
\newcommand{\algocf@algocfref}{\relax}%
\newcommand{\listalgorithmcfname}{}%
\newcommand{\algorithmcfname}{}%
\@ifundefined{algorithmautorefname}{\newcommand{\algorithmautorefname}{algorithm}}{\renewcommand{\algorithmautorefname}{algorithm}}%
\newcommand{\algorithmcflinename}{}%
\newcommand{\algocf@typo}{}%
\newcommand{\@algocf@procname}{}\newcommand{\procedureautorefname}{}%
\newcommand{\SetAlgoProcName}[2]{\renewcommand{\@algocf@procname}{#1}\renewcommand{\procedureautorefname}{#2}}%
\newcommand{\@algocf@funcname}{}\newcommand{\functionautorefname}{}%
\newcommand{\SetAlgoFuncName}[2]{\renewcommand{\@algocf@funcname}{#1}\renewcommand{\functionautorefname}{#2}}%
\newcommand{\@algocf@titleofalgoname}{\algorithmcfname}%
\newcommand{\@algocf@algotitleofalgo}{%
  \renewcommand{\@algocf@titleofalgoname}{\algorithmcfname}}%
\newcommand{\@algocf@proctitleofalgo}{%
  \renewcommand{\@algocf@titleofalgoname}{\algocf@procname}}%
%
\newcommand{\algocf@style}{plain}%
\newcommand{\@ResetCounterIfNeeded}{}%
\newcommand{\@titleprefix}{}%
%
\newcommand{\algocf@numbering}[1]{\newcommand{\algocf@within}{#1}}%
%
\newcommand{\defaultsmacros@algo}{\algocf@defaults@shortend}%
%
\newcommand{\algocf@list}{loa}%
\newcommand{\algocf@float}{algocf}%
%
\newcommand{\algocf@envname}{algorithm}%
\newcommand{\algocf@listofalgorithms}{listofalgorithms}%
%
%
%% redefine chapter so that it adds a vspace in the loa as the original does for lof and lot
% \let\algocf@original@chapter=\chapter%
% \def\chapter{\expandafter\addtocontents{loa}{\protect\addvspace{10\p@}}\algocf@original@chapter}%
%
% bug correction with hyperref submitted by Hubert Meier
\begingroup\expandafter\expandafter\expandafter\endgroup 
\expandafter\ifx\csname @chapter\endcsname\relax\else 
% \let\algocf@original@chapter=\chapter% 
% \def\chapter{\addtocontents{loa}{\protect\addvspace{10\p@}}\algocf@original@chapter}% 
\let\algocf@original@chapter=\@chapter%
\@ifclassloaded{krantz}{%
\def\@chapter[#1][#2]#3{\algocf@original@chapter[#1][#2]{#3}\addtocontents{loa}{\protect\addvspace{10\p@}}}% 
}{%
\def\@chapter[#1]#2{\algocf@original@chapter[#1]{#2}\addtocontents{loa}{\protect\addvspace{10\p@}}}% 
}%
\fi
%
%% if@restonecol is defined in article and book but some other classes don't define it and we need it, so we do
\ifx\if@restonecol\relax\else\newif\if@restonecol\fi%
%
%
%%%%%%%%%%%%%%%%%%%%%% Declaration of Options %%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\RequirePackage{ifthen}%
%
\newboolean{algocf@displayblockmarkers}\setboolean{algocf@displayblockmarkers}{false}%
\DeclareOption{displayblockmarkers}{%
  \setboolean{algocf@displayblockmarkers}{true}%
}
\newboolean{algocf@displaygroupmarkers}{\setboolean{algocf@displaygroupmarkers}{false}
\DeclareOption{displaygroupmarkers}{%
  \setboolean{algocf@displaygroupmarkers}{true}%
}
%
\newboolean{algocf@nokwfunc}\setboolean{algocf@nokwfunc}{false}%
\DeclareOption{nokwfunc}{%
  \setboolean{algocf@nokwfunc}{true}%
}%
%
\newboolean{algocf@oldcommands}\setboolean{algocf@oldcommands}{false}%
\DeclareOption{oldcommands}{%
  \setboolean{algocf@oldcommands}{true}%
}%
%
\newboolean{algocf@leftlinenumber}\setboolean{algocf@leftlinenumber}{true}%
\newcommand{\setLeftLinesNumbers}{\setboolean{algocf@leftlinenumber}{true}}%
\newcommand{\setRightLinesNumbers}{\setboolean{algocf@leftlinenumber}{false}}%
\DeclareOption{rightnl}{%
  \setRightLinesNumbers%
}%
%
\newboolean{algocf@endfloat}\setboolean{algocf@endfloat}{false}%
\DeclareOption{endfloat}{%
  \setboolean{algocf@endfloat}{true}%
  \newcounter{postalgo}\setcounter{postalgo}{0}%
}%
%
\newboolean{algocf@procnumbered}\setboolean{algocf@procnumbered}{false}%
\DeclareOption{procnumbered}{%
  \setboolean{algocf@procnumbered}{true}%
}%
%
\DeclareOption{algo2e}{%
  \renewcommand{\algocf@envname}{algorithm2e}%
  \renewcommand{\algocf@listofalgorithms}{listofalgorithmes}%
}%
%
\newboolean{algocf@slide}\setboolean{algocf@slide}{false}%
\DeclareOption{slide}{%
  \setboolean{algocf@slide}{true}%
}%
%
\newboolean{algocf@figurecaption}\setboolean{algocf@figurecaption}{false}%
\DeclareOption{figure}{%
\renewcommand{\algocf@list}{lof}%
\renewcommand{\algocf@float}{figure}%
\AtBeginDocument{\@ifpackageloaded{caption}{\setboolean{algocf@figurecaption}{true}}{}}%
}%
%
\newboolean{algocf@optonelanguage}\setboolean{algocf@optonelanguage}{false}%
\DeclareOption{onelanguage}{\setboolean{algocf@optonelanguage}{true}}%
%
\newcommand{\algocf@languagechoosen}{english}%
\newboolean{algocf@localkw@english}\setboolean{algocf@localkw@english}{true}%
\DeclareOption{englishkw}{%
\setboolean{algocf@localkw@english}{true}%
}%
%
\DeclareOption{english}{%
\renewcommand{\listalgorithmcfname}{List of Algorithms}%
\renewcommand{\algorithmcfname}{Algorithm}%
\renewcommand{\algorithmautorefname}{algorithm}%
\renewcommand{\algorithmcflinename}{line}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedure}%
\renewcommand{\@algocf@funcname}{Function}%
\renewcommand{\procedureautorefname}{procedure}%
\renewcommand{\functionautorefname}{function}%
\renewcommand{\algocf@languagechoosen}{english}%
}%
%
%----
\newboolean{algocf@localkw@french}\setboolean{algocf@localkw@french}{false}%
\DeclareOption{frenchkw}{%
\setboolean{algocf@localkw@french}{true}%
}%
%
\DeclareOption{french}{%
\renewcommand{\listalgorithmcfname}{Liste des Algorithmes}%
\renewcommand{\algorithmcfname}{Algorithme}%
\renewcommand{\algorithmautorefname}{algorithme}%
\renewcommand{\algorithmcflinename}{ligne}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Proc\'edure}%
\renewcommand{\@algocf@funcname}{Fonction}%
\renewcommand{\procedureautorefname}{proc\'edure}%
\renewcommand{\functionautorefname}{fonction}%
\renewcommand{\algocf@languagechoosen}{french}%
}%
%
%----
\newboolean{algocf@localkw@czech}\setboolean{algocf@localkw@czech}{false}%
\DeclareOption{czechkw}{%
\setboolean{algocf@localkw@czech}{true}%
}%
%
\DeclareOption{czech}{%
\renewcommand{\listalgorithmcfname}{Seznam algoritm\r{u}}%
\renewcommand{\algorithmcfname}{Algoritmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Radek}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funkce}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{czech}%
}%
%
%----
\newboolean{algocf@localkw@german}\setboolean{algocf@localkw@german}{false}%
\DeclareOption{germankw}{%
\setboolean{algocf@localkw@german}{true}%
}%
%
\DeclareOption{german}{%
\renewcommand{\listalgorithmcfname}{Liste der Algorithmen}%
\renewcommand{\algorithmcfname}{Algorithmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Zeile}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Prozedur}%
\renewcommand{\@algocf@funcname}{Funktion}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{german}%
}%
%
%----
\DeclareOption{ngermankw}{%
\setboolean{algocf@localkw@german}{true}%
}%
%
\DeclareOption{ngerman}{%
\renewcommand{\listalgorithmcfname}{Liste der Algorithmen}%
\renewcommand{\algorithmcfname}{Algorithmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Zeile}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Prozedur}%
\renewcommand{\@algocf@funcname}{Funktion}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{german}%
}%
%
%----
\newboolean{algocf@localkw@portuguese}\setboolean{algocf@localkw@portuguese}{false}%
\DeclareOption{portuguesekw}{%
\setboolean{algocf@localkw@portuguese}{true}%
}%
%
\DeclareOption{portuguese}{%
\renewcommand{\listalgorithmcfname}{Lista de Algoritmos}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{linha}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedimento}%
\renewcommand{\@algocf@funcname}{Fun\c{c}\~{a}o}%
\renewcommand{\procedureautorefname}{procedimento}%
\renewcommand{\functionautorefname}{fun\c{c}\~{a}o}%
\renewcommand{\algocf@languagechoosen}{portuguese}%
}%
%
%----
\newboolean{algocf@localkw@italiano}\setboolean{algocf@localkw@italiano}{false}%
\DeclareOption{italianokw}{%
\setboolean{algocf@localkw@italiano}{true}%
}%
%
\DeclareOption{italiano}{%
\renewcommand{\listalgorithmcfname}{Elenco degli algoritmi}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{riga}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funzione}%
\renewcommand{\procedureautorefname}{procedura}%
\renewcommand{\functionautorefname}{funzione}%
\renewcommand{\algocf@languagechoosen}{italiano}%
}%
%----
\newboolean{algocf@localkw@spanish}\setboolean{algocf@localkw@spanish}{false}%
\DeclareOption{spanishkw}{%
\setboolean{algocf@localkw@spanish}{true}%
}%
%
\DeclareOption{spanish}{%
\renewcommand{\listalgorithmcfname}{\'Indice de algoritmos}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{l\'inea}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedimiento}%
\renewcommand{\@algocf@funcname}{Funci\'on}%
\renewcommand{\procedureautorefname}{procedimiento}%
\renewcommand{\functionautorefname}{funci\'on}%
\renewcommand{\algocf@languagechoosen}{spanish}%
}%
%----
\newboolean{algocf@localkw@slovak}\setboolean{algocf@localkw@slovak}{false}%
\DeclareOption{slovakkw}{%
\setboolean{algocf@localkw@slovak}{true}%
}%
%
\DeclareOption{slovak}{%
\renewcommand{\listalgorithmcfname}{Zoznam algoritmov}%
\renewcommand{\algorithmcfname}{Algoritmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Radek}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Proced\'{u}ra}%
\renewcommand{\@algocf@funcname}{Funkcia}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{slovak}%
}%
%
%----
\newboolean{algocf@localkw@croatian}\setboolean{algocf@localkw@croatian}{false}%
\DeclareOption{croatiankw}{%
\setboolean{algocf@localkw@croatian}{true}%
}%
%
\DeclareOption{croatian}{%
\renewcommand{\listalgorithmcfname}{Popis algoritama}%
\renewcommand{\algorithmcfname}{Algoritam}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{redak}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funkcija}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{croatian}%
}%
%%% adding 'turkish' option customization
%
%----
\newboolean{algocf@localkw@turkish}\setboolean{algocf@localkw@turkish}{false}%
\DeclareOption{turkishkw}{%
\setboolean{algocf@localkw@turkish}{true}%
}%
\DeclareOption{turkish}{%
\renewcommand{\listalgorithmcfname}{Algoritma Listesi}%
\renewcommand{\algorithmcfname}{Algoritma}%
\renewcommand{\algorithmautorefname}{algoritma}%
\renewcommand{\algorithmcflinename}{?izgi}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Prosed?r}%
\renewcommand{\@algocf@funcname}{Fonksiyon}%
\renewcommand{\procedureautorefname}{prosed?r}%
\renewcommand{\functionautorefname}{fonksiyon}%
\renewcommand{\algocf@languagechoosen}{turkish}%
}%
%
% OPTIONs plain, boxed, ruled, algoruled & boxruled
%
\newcommand{\algocf@style@plain}{\renewcommand{\algocf@style}{plain}}%
\newcommand{\algocf@style@boxed}{\renewcommand{\algocf@style}{boxed}}%
\newcommand{\algocf@style@ruled}{\renewcommand{\algocf@style}{ruled}}%
\newcommand{\algocf@style@algoruled}{\renewcommand{\algocf@style}{algoruled}}%
\newcommand{\algocf@style@boxruled}{\renewcommand{\algocf@style}{boxruled}}%
\newcommand{\algocf@style@tworuled}{\renewcommand{\algocf@style}{tworuled}}%
\newcommand{\algocf@style@plainruled}{\renewcommand{\algocf@style}{plainruled}}%
\newcommand{\RestyleAlgo}[1]{\csname algocf@style@#1\endcsname}%
\DeclareOption{plain}{\algocf@style@plain}%
\DeclareOption{plainruled}{\algocf@style@plainruled}%
\DeclareOption{boxed}{\algocf@style@boxed}%
\DeclareOption{ruled}{\algocf@style@ruled}%
\DeclareOption{algoruled}{\algocf@style@algoruled}%
\DeclareOption{boxruled}{\algocf@style@boxruled}%
\DeclareOption{tworuled}{\algocf@style@tworuled}%
%
% OPTIONs algopart,algochapter & algosection
%
\DeclareOption{algopart}{\algocf@numbering{part}}%       %algo part numbered
\DeclareOption{algochapter}{\algocf@numbering{chapter}}% %algo chapter numbered
\DeclareOption{algosection}{\algocf@numbering{section}}% %algo section numbered
%
% OPTIONs resetcount & noresetcount
%
\DeclareOption{resetcount}{\renewcommand{\@ResetCounterIfNeeded}{\setcounter{AlgoLine}{0}}}%
\DeclareOption{noresetcount}{\renewcommand{\@ResetCounterIfNeeded}{}}%
%
% OPTIONs algorithm hanging for long lines
%
\newlength{\algocf@hangindent}\setlength{\algocf@hangindent}{.5em}
\newcommand{\SetAlgoHangIndent}[1]{\setlength{\algocf@hangindent}{#1}}
%
\newboolean{algocf@hanging}\setboolean{algocf@hanging}{true}% hanging is handle by default
\newboolean{algocf@hanginginout}\setboolean{algocf@hanginginout}{false}% inout are managed as previously: hanging set by inout keywords
\newboolean{algocf@hangingcomment}\setboolean{algocf@hangingcomment}{false}% comment that are not side comment are indented accordingly to comment mark, not as normal text
\newcommand{\algocf@everyparnl}{\relax}%
\newcommand{\algocf@everyparhanging}{\hangafter=1\hangindent=\algocf@hangindent\relax}%
\newcommand{\algocf@everypar}{\algocf@everyparnl\algocf@everyparhanging}%
\newcommand{\algocf@seteverypar}{%
  \ifthenelse{\boolean{algocf@hanging}}{\everypar{\algocf@everypar}}{\relax}%
}%
%
\newcommand{\algocf@seteveryparnl}[1]{\renewcommand{\algocf@everyparnl}{#1}\everypar{\algocf@everypar}}%
\newcommand{\algocf@seteveryparhanging}[1]{%
\let\algocf@oldeveryparhanging=\algocf@everyparhanging%
\renewcommand{\algocf@everyparhanging}{#1}\everypar{\algocf@everypar}%
}%
\newcommand{\algocf@reseteveryparhanging}{%
\let\algocf@everyparhanging=\algocf@oldeveryparhanging%
\everypar{\algocf@everypar}%
}%
\DeclareOption{hanginginout}{\setboolean{algocf@hanginginout}{true}}%
\DeclareOption{hangingcomment}{\setboolean{algocf@hangingcomment}{true}}%
\DeclareOption{noalgohanging}{%
  \setboolean{algocf@hanginginout}{false}%
  \setboolean{algocf@hangingcomment}{false}%
  \setboolean{algocf@hanging}{false}%
}%
%\newcommand{
%
%
% OPTION linesnumbered
%
\newboolean{algocf@linesnumbered}\setboolean{algocf@linesnumbered}{false}%
\newcommand{\algocf@linesnumbered}{\relax}%
\DeclareOption{linesnumbered}{%
  \setboolean{algocf@linesnumbered}{true}%
  \renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\nl}}%
}%
%
% OPTION linesnumberedhidden
%
\DeclareOption{linesnumberedhidden}{%
  \setboolean{algocf@linesnumbered}{true}%
  \renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\stepcounter{AlgoLine}}}%
}%
%
% OPTION commentsnumbered inoutnumbered
%
\newboolean{algocf@commentsnumbered}\setboolean{algocf@commentsnumbered}{false}%
\DeclareOption{commentsnumbered}{\setboolean{algocf@commentsnumbered}{true}}%
\newboolean{algocf@inoutnumbered}\setboolean{algocf@inoutnumbered}{false}%
\DeclareOption{inoutnumbered}{\setboolean{algocf@inoutnumbered}{true}}%
%
% OPTIONs titlenumbered & titlenotnumbered
%
\DeclareOption{titlenumbered}{%
  \renewcommand{\@titleprefix}{%
    \refstepcounter{\algocf@float}%
    \AlTitleSty{\AlTitleFnt\@algocf@titleofalgoname\ \expandafter\csname the\algocf@float\endcsname\algocf@typo: }%
  }%
}%
%
\DeclareOption{titlenotnumbered}{\renewcommand{\@titleprefix}{%
    \AlTitleSty{\AlTitleFnt\@algocf@titleofalgoname\algocf@typo: }}%
}%
%
% OPTIONs algonl
% line numbered with the counter of the algorithm
%
\DeclareOption{algonl}{\renewcommand{\theAlgoLine}{\expandafter\csname the\algocf@float\endcsname.\arabic{AlgoLine}}}%
%
% OPTIONs lined, vlined & noline
%
\DeclareOption{lined}{\AtBeginDocument{\SetAlgoLined}}%   \SetAlgoLined (default)
\DeclareOption{vlined}{\AtBeginDocument{\SetAlgoVlined}}% \SetAlgoVlined
\DeclareOption{noline}{\AtBeginDocument{\SetAlgoNoLine}}%\SetAlgoNoLine
%
% OPTIONs longend, shotend & noend
%
\DeclareOption{longend}{\AtBeginDocument{\SetAlgoLongEnd}}%  \SetAlgoLongEnd
\DeclareOption{shortend}{\AtBeginDocument{\SetAlgoShortEnd}}%\SetAlgoShortEnd
\DeclareOption{noend}{\AtBeginDocument{\SetAlgoNoEnd}}%      \SetAlgoNoEnd
%
\DeclareOption{nosemicolon}{\AtBeginDocument{\DontPrintSemicolon}}%      \SetAlgoNoEnd
%
% OPTION dotoc
%
\newboolean{algocf@dotocloa}\setboolean{algocf@dotocloa}{false}%
\DeclareOption{dotocloa}{%
  \setboolean{algocf@dotocloa}{true}%
}
%
% OPTION comments
%
\newboolean{algocf@optfillcomment}\setboolean{algocf@optfillcomment}{true}%
\DeclareOption{nofillcomment}{%
  \setboolean{algocf@optfillcomment}{false}%
}%
\DeclareOption{fillcomment}{%
  \setboolean{algocf@optfillcomment}{true}%
}%
%
% OPTION sidecommments
%
\newboolean{algocf@scleft}\setboolean{algocf@scleft}{false}%
\DeclareOption{scleft}{%
  \setboolean{algocf@scleft}{true}%
}%
\DeclareOption{sright}{% default
  \setboolean{algocf@scleft}{false}%
}%
%
% OPTION norelsize
%
\newboolean{algocf@norelsize}\setboolean{algocf@norelsize}{false}%
\DeclareOption{norelsize}{%
  \setboolean{algocf@norelsize}{true}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%% Execution of Options %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\ExecuteOptions{english,plain,resetcount,titlenotnumbered,lined,shortend}%
%
\ProcessOptions%
%
\@algocf@algotitleofalgo% fix name for \TitleOfAlgo to \algorithmcfname by default
%
%%%%%%%%%%%%%%%%%%%%%%%%%% Package Loading %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
\RequirePackage{xspace}%
%
\ifthenelse{\boolean{algocf@endfloat}}{%
  \RequirePackage{endfloat}%
}{\relax}%
%
\ifthenelse{\boolean{algocf@norelsize}}{%
  \newcommand{\relsize}[1]{\scriptsize}%
}{%
  \RequirePackage{relsize}%
}%
%
\ifthenelse{\boolean{algocf@slide}}{\RequirePackage{color}}{}%
%
%
\AtEndOfPackage{%
  \ifthenelse{\boolean{algocf@dotocloa}}{%
    \renewcommand{\listofalgorithms}{\tocfile{\listalgorithmcfname}{loa}}%
  }{\relax}%
}%
%
% if loa in toc required, load tocbibind package if not already done.
\ifthenelse{\boolean{algocf@dotocloa}}{%
  \ifx\@tocextra\undefined%
  \RequirePackage{tocbibind}%
  \fi%
}{\relax}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Main Part %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\newcommand{\algocf@name}{algorithm2e}%
\newcommand{\algocf@date}{october 19 2015}%
\newcommand{\algocf@version}{Release 5.1}%
\newcommand{\algocf@id}{\algocf@version\space -- \algocf@date\space --}%
\typeout{********************************************************^^JPackage `\algocf@name'\space\algocf@id^^J%
         - algorithm2e-announce@lirmm.fr  mailing list for announcement about releases^^J%
         - algorithm2e-discussion@lirmm.fr mailing list for discussion about package^^J%
         subscribe by emailing sympa@lirmm.fr with 'subscribe <list> <firstname name>'^^J%
         - Author: Christophe Fiorio (christophe.fiorio@umontpellier.fr)^^J********************************************************}%
%%
%%
%%
%%
%%
%%
%%%% hyperref compatibility tricks: Hyperref package defines H counters from
   % standard counters (i.e \theHpage from \thepage) and check some particular
   % counters of some packages, unfortunately it doesn't do the same for
   % algorithm2e package but act as Hcounter was defined. To avoid errors we
   % defined \theHalgocf ourself
%%%%
%
\@ifundefined{theHalgocf}{\def\theHalgocf{\thealgocf}}{}%
\@ifundefined{theHAlgoLine}{\def\theHAlgoLine{\theAlgoLine}}{}%
\@ifundefined{theHalgocfproc}{\def\theHalgocfproc{0}}{}%
\@ifundefined{theHalgocffunc}{\def\theHalgocffunc{0}}{}%
\@ifundefined{toclevel@algocf}{\def\toclevel@algocf{0}}{}%
%
% autoref from hyperref needs an autorefname, so we give it.
\def\AlgoLineautorefname{\algorithmcflinename}%
\def\algocfautorefname{\algorithmautorefname}%
\def\algocfprocautorefname{\procedureautorefname}%
\def\algocffuncautorefname{\functionautorefname}%
%%
%%
%%
\newcommand{\@defaultskiptotal}{0.5em}%
\newskip\skiptotal\skiptotal=0.5em%
\newskip\skiplinenumber\skiplinenumber=\hsize\advance\skiplinenumber by-\skiptotal%
\newskip\skiprule%
\newskip\skiphlne%
\newskip\skiptext%
\newskip\skiplength%
\newskip\algomargin%
\newskip\skipalgocfslide\skipalgocfslide=1em%
\newdimen\algowidth%
\newdimen\inoutsize%
\newdimen\inoutindent%
\newdimen\interspacetitleruled\setlength{\interspacetitleruled}{2pt}%
\newdimen\interspacealgoruled\setlength{\interspacealgoruled}{2pt}%
\newdimen\interspacetitleboxruled\setlength{\interspacetitleboxruled}{2\lineskip}%
%
\newcommand{\@algoskip}{\smallskip}%
\newcommand{\SetAlgoSkip}[1]{\renewcommand{\@algoskip}{\csname#1\endcsname}}%
\newcommand{\@algoinsideskip}{\relax}%
\newcommand{\SetAlgoInsideSkip}[1]{\renewcommand{\@algoinsideskip}{\csname#1\endcsname}}%
%
% ruledwidth
%
\newlength{\algocf@ruledwidth}\setlength{\algocf@ruledwidth}{\linewidth}%
\newboolean{algocf@customruledwidth}\setboolean{algocf@customruledwidth}{false}%
\newcommand{\SetCustomAlgoRuledWidth}[1]{%
  \setboolean{algocf@customruledwidth}{true}%
  \ifthenelse{\boolean{algocf@customruledwidth}}{\setlength{\algocf@ruledwidth}{#1}}{\relax}%
}%
%
\newsavebox{\algocf@inoutbox}%
\newsavebox{\algocf@inputbox}%
%%
%%
\newcommand{\arg@e}{}%
\newcommand{\arg@space}{\ }%
\newcommand{\BlankLine}{\vskip 1ex}%
%%
\newcommand{\vespace}{1ex}%
\newcommand{\SetInd}[2]{%
\skiprule=#1%
\skiptext=#2%
\skiplength=\skiptext\advance\skiplength by \skiprule\advance\skiplength by 0.4pt}%
\SetInd{0.5em}{1em}
\algomargin=\leftskip\advance\algomargin by \parindent%
\newcommand{\IncMargin}[1]{\advance\algomargin by #1}%
\newcommand{\DecMargin}[1]{\advance\algomargin by -#1}%
\newcommand{\SetNlSkip}[1]{%
  \renewcommand{\@defaultskiptotal}{#1}%
  \setlength{\skiptotal}{#1}}%
%%
\newskip\AlCapSkip\AlCapSkip=0ex%
\newskip\AlCapHSkip\AlCapSkip=0ex%
\newcommand{\SetAlCapSkip}[1]{\setlength{\AlCapSkip}{#1}}%
\newcommand{\SetAlCapHSkip}[1]{\setlength{\AlCapHSkip}{#1}}%
\SetAlCapHSkip{.5\algomargin}%
%%
%%
\newskip\algoskipindent
\newcommand{\algocf@adjustskipindent}{%
  \algoskipindent=\skiprule%
  \advance\algoskipindent by \skiptext\advance\algoskipindent by 0.4pt}
\algocf@adjustskipindent%
%
\newcommand{\Indentp}[1]{\advance\leftskip by #1}%
\newcommand{\Indp}{\algocf@adjustskipindent\advance\leftskip by \algoskipindent}
\newcommand{\Indpp}{\advance\leftskip by 0.5em}%
\newcommand{\Indm}{\algocf@adjustskipindent\advance\leftskip by -\algoskipindent}
\newcommand{\Indmm}{\advance\leftskip by -0.5em}%
%
%%
%%
%% Line Numbering
%%
%%
% number line style
\newcommand{\algocf@nlrelsize}{-2}\newcommand{\SetAlgoNlRelativeSize}[1]{\renewcommand{\algocf@nlrelsize}{#1}}%
\newcommand{\NlSty}[1]{\textnormal{\textbf{\relsize{\algocf@nlrelsize}#1}}}% default definition
\newcommand{\SetNlSty}[3]{\renewcommand{\NlSty}[1]{\textnormal{\csname#1\endcsname{\relsize{\algocf@nlrelsize}#2##1#3}}}}%
%
% nl definitions
%
\newsavebox{\algocf@nlbox}%
\newcommand{\algocf@printnl}[1]{%
  \ifthenelse{\boolean{algocf@leftlinenumber}}{%
    \skiplinenumber=\skiptotal\advance\skiplinenumber by\leftskip%
    \strut\raisebox{0pt}{\llap{\NlSty{#1}\kern\skiplinenumber}}\ignorespaces%
  }{%
    \sbox\algocf@nlbox{\NlSty{#1}}%
    \skiplinenumber=\hsize\advance\skiplinenumber by-\leftskip\advance\skiplinenumber by-\skiptext%
    \advance\skiplinenumber by\algomargin\advance\skiplinenumber by.3em\advance\skiplinenumber by-\wd\algocf@nlbox%
    % to handle particular case of until: printnl is after 'until' keyword has been writen, so we need to substract length of this keyword
    \advance\skiplinenumber by-\algocf@skipuntil%
    \strut\raisebox{0pt}{\rlap{\kern\skiplinenumber\NlSty{#1\ignorespaces}}}\ignorespaces%
  }%
}%
\newcommand{\algocf@nl@sethref}[1]{%
  \renewcommand{\theHAlgoLine}{\thealgocfproc.#1}%
  \hyper@refstepcounter{AlgoLine}\gdef\@currentlabel{#1}%
}%
\newcommand{\nl}{%
  \@ifundefined{hyper@refstepcounter}{% if not hyperref then do a simple refstepcounter
    \refstepcounter{AlgoLine}\gdef\@currentlabel{\theAlgoLine}%
  }{% else if hyperref, do the anchor so 2 lines in two differents algorithms cannot have the same href
    \stepcounter{AlgoLine}\algocf@nl@sethref{\theAlgoLine}%
  }% now we can do the line numbering
  \algocf@printnl{\theAlgoLine}%
}%
%
\newcommand{\nllabel}[1]{\label{#1}}%
%
\newcommand{\enl}{%
  \@ifundefined{hyper@refstepcounter}{% if not hyperref then do a simple refstepcounter
    \refstepcounter{AlgoLine}\gdef\@currentlabel{\theAlgoLine}%
  }{% else if hyperref, do the anchor so 2 lines in two differents algorithms cannot have the same href
    \stepcounter{AlgoLine}\algocf@nl@sethref{\theAlgoLine}%
  }% now we can do the line numbering
  \skiplinenumber=\hsize\advance\skiplinenumber by-\leftskip%
  \strut\raisebox{0pt}{\rlap{\kern\skiplinenumber\strut\NlSty{\theAlgoLine}}}\ignorespaces%
}%
%% nlset
\newcommand{\nlset}[1]{%
  \@ifundefined{hyper@refstepcounter}{\protected@edef\@currentlabel{#1}}{\algocf@nl@sethref{#1}}\algocf@printnl{#1}%
}%
%
%% lnl definitions
\newcommand{\lnl}[1]{\nl\label{#1}\ignorespaces}%
%
%% lnlset
\newcommand{\lnlset}[2]{\nlset{#2}\label{#1}}%
%
% set char put at end of each line
%
\newcommand{\algocf@endline}{\string;}
\newcommand{\SetEndCharOfAlgoLine}[1]{\renewcommand{\algocf@endline}{#1}}
%
% end of line definition
%
\newcommand{\@endalgocfline}{\algocf@endline}% default definition: printsemicolon
\newcommand{\DontPrintSemicolon}{\renewcommand{\@endalgocfline}{\relax}}%
\newcommand{\PrintSemicolon}{\renewcommand{\@endalgocfline}{\algocf@endline}}%
\newcommand{\@endalgoln}{\@endalgocfline\hfill\strut\par}%
%
% line numbering
%
\newcommand{\LinesNumbered}{\setboolean{algocf@linesnumbered}{true}\renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\nl}}}%
\newcommand{\LinesNotNumbered}{%
  \setboolean{algocf@linesnumbered}{false}%
  \renewcommand{\algocf@linesnumbered}{\relax}%
}%
%
\newcommand{\LinesNumberedHidden}{%
  \setboolean{algocf@linesnumbered}{true}\renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\stepcounter{AlgoLine}}}}%
\newcommand{\ShowLn}{\nlset{\theAlgoLine}\ignorespaces}% display the line number on this line (without labelling)
\newcommand{\ShowLnLabel}[1]{\lnlset{#1}{\theAlgoLine}\ignorespaces}% display the line number and label this line
%
%%
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Styling text commands
%
\newcommand{\AlFnt}{\relax}% default definition
\newcommand{\SetAlFnt}[1]{\renewcommand{\AlFnt}{#1}}%
\newcommand{\AlTitleFnt}{\relax}% default definition
\newcommand{\SetAlTitleFnt}[1]{\renewcommand{\AlTitleFnt}{#1}}%
%
\newcommand{\AlCapFnt}{\relax}% default definition
\newcommand{\SetAlCapFnt}[1]{\renewcommand{\AlCapFnt}{#1}}%
\newcommand{\AlCapNameFnt}{\relax}% default definition
\newcommand{\SetAlCapNameFnt}[1]{\renewcommand{\AlCapNameFnt}{#1}}%
%
\newcommand{\ProcFnt}{\relax}% default definition
\newcommand{\SetProcFnt}[1]{\renewcommand{\ProcFnt}{#1}}%
\newcommand{\ProcNameFnt}{\relax}% default definition
\newcommand{\SetProcNameFnt}[1]{\renewcommand{\ProcNameFnt}{#1}}%
\newcommand{\ProcArgFnt}{\relax}% default definition
\newcommand{\SetProcArgFnt}[1]{\renewcommand{\ProcArgFnt}{#1}}%
%
\newcommand{\AlTitleSty}[1]{\textbf{#1}\unskip}% default definition
\newcommand{\SetAlTitleSty}[1]{\renewcommand{\AlTitleSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\AlCapSty}[1]{\textnormal{\textbf{#1}}\unskip}% default definition
\newcommand{\SetAlCapSty}[1]{\renewcommand{\AlCapSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\AlCapNameSty}[1]{\textnormal{#1}\unskip}% default definition
\newcommand{\SetAlCapNameSty}[1]{\renewcommand{\AlCapNameSty}[1]{\textnormal{\csname #1\endcsname{##1}}\unskip}}%
%
\newcommand{\ProcSty}[1]{\AlCapSty{#1}}%
\newcommand{\SetProcSty}[1]{\renewcommand{\ProcSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProcNameSty}[1]{\AlCapNameSty{#1}}%
\newcommand{\SetProcNameSty}[1]{\renewcommand{\ProcNameSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProcArgSty}[1]{\AlCapNameSty{#1}}%
\newcommand{\SetProcArgSty}[1]{\renewcommand{\ProcArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
%
\newcommand{\KwSty}[1]{\textnormal{\textbf{#1}}\unskip}% default definition
\newcommand{\SetKwSty}[1]{\renewcommand{\KwSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ArgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetArgSty{emph}
\newcommand{\SetArgSty}[1]{\renewcommand{\ArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\FuncArgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetFuncArgSty{emph}
\newcommand{\SetFuncArgSty}[1]{\renewcommand{\FuncArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\FuncSty}[1]{\textnormal{\texttt{#1}}\unskip}%\SetFuncSty{texttt}
\newcommand{\SetFuncSty}[1]{\renewcommand{\FuncSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetProgSty{emphg}
\newcommand{\SetProgSty}[1]{\renewcommand{\ArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\DataSty}[1]{\textnormal{\textsf{#1}}\unskip}%%\SetDataSty{textsf}
\newcommand{\SetDataSty}[1]{\renewcommand{\DataSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\CommentSty}[1]{\textnormal{\texttt{#1}}\unskip}%%\SetDataSty{texttt}
\newcommand{\SetCommentSty}[1]{\renewcommand{\CommentSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\TitleSty}[1]{#1\unskip}%\SetTitleSty{}{}
\newcommand{\SetTitleSty}[2]{\renewcommand{\TitleSty}[1]{%
\csname#1\endcsname{\csname#2\endcsname##1}}\unskip}%
\newcommand{\BlockMarkersSty}[1]{\KwSty{#1}}%
\newcommand{\SetBlockMarkersSty}[1]{\renewcommand{\BlockMarkersSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Block basic commands
%
\newcommand{\algocf@push}[1]{\advance\skiptotal by #1\moveright #1}%
\newcommand{\algocf@pop}[1]{\advance\skiptotal by -#1}%
\newcommand{\algocf@addskiptotal}{\advance\skiptotal by 0.4pt\advance\hsize by -0.4pt\advance\hsize by -\skiplength}% 0.4 pt=width of \vrule
\newcommand{\algocf@subskiptotal}{\advance\skiptotal by -0.4pt\advance\hsize by 0.4pt\advance\hsize by \skiplength}% 0.4 pt=width of \vrule
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% group of instructions definition
%
\skiphlne=.8ex%
\newcommand{\SetVlineSkip}[1]{\skiphlne=#1}%
\newcommand{\algocf@bblock}{\BlockMarkersSty{begin}}%
\newcommand{\algocf@eblock}{\BlockMarkersSty{end}}%
\newcommand{\AlgoDisplayBlockMarkers}{\setboolean{algocf@displayblockmarkers}{true}}%
\newcommand{\AlgoDontDisplayBlockMarkers}{\setboolean{algocf@displayblockmarkers}{false}}%
\newcommand{\AlgoDisplayGroupMarkers}{\setboolean{algocf@displaygroupmarkers}{true}}%
\newcommand{\AlgoDontDisplayGroupMarkers}{\setboolean{algocf@displaygroupmarkers}{false}}%
\newcommand{\algocf@bblockcode}{%
  \ifthenelse{\boolean{algocf@displayblockmarkers}}{\algocf@bblock\par}{\relax}%
}%
\newcommand{\algocf@eblockcode}{%
  \ifthenelse{\boolean{algocf@displayblockmarkers}}{\algocf@eblock\par}{\relax}%
}%
\newcommand{\algocf@bgroupcode}{%
  \ifthenelse{\boolean{algocf@displaygroupmarkers}}{\algocf@bblock}{\relax}%
}%
\newcommand{\algocf@egroupcode}{%
  \ifthenelse{\boolean{algocf@displaygroupmarkers}}{\algocf@eblock}{\relax}%
}%
\newcommand{\SetAlgoBlockMarkers}[2]{%
  \ifArgumentEmpty{#1}{%
    \renewcommand{\algocf@bblock}{\relax}%
  }{%
    \renewcommand{\algocf@bblock}{\BlockMarkersSty{#1}}%
  }% begin marker set
  \ifArgumentEmpty{#2}{%
    \renewcommand{\algocf@eblock}{\relax}%
  }{%
    \renewcommand{\algocf@eblock}{\BlockMarkersSty{#2}}%
  }% end marker set
}
%
%%%%%%%%% block with a vertical line end by a little horizontal line
\newcommand{\algocf@Vline}[1]{%     no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@push{\skiprule}%        move to the right before the vertical rule
  \hbox{\vrule%
    \vtop{\algocf@push{\skiptext}%move the right after the rule
      \vtop{\algocf@addskiptotal #1}\Hlne}}\vskip\skiphlne% inside the block
  \algocf@pop{\skiprule}%\algocf@subskiptotal% restore indentation
  \nointerlineskip}% no vskip after
%
%%%%%%%%% block with a vertical line
\newcommand{\algocf@Vsline}[1]{%    no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@bblockcode%
  \algocf@push{\skiprule}%        move to the right before the vertical rule
  \hbox{\vrule%               the vertical rule
    \vtop{\algocf@push{\skiptext}%move the right after the rule
      \vtop{\algocf@addskiptotal #1}}}% inside the block
  \algocf@pop{\skiprule}% restore indentation
  \algocf@eblockcode%
}
%
\newcommand{\algocf@Hlne}{\hrule height 0.4pt depth 0pt width .5em}%
%
%%%%%%%%%  block without line
\newcommand{\algocf@Noline}[1]{%    no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@bblockcode%
  \algocf@push{\skiprule}%
  \hbox{%
    \vtop{\algocf@push{\skiptext}%
      \vtop{\algocf@addskiptotal #1}}}% inside the block
  \algocf@pop{\skiprule}%
  \algocf@eblockcode%
  % \nointerlineskip% no vskip after
}%
%%%%%%%%%
%
%% default=NoLine
%
\newcommand{\algocf@group}[1]{\algocf@Noline{#1}}% group: set of instruction depending from another (ex: then part of the If)
\newcommand{\algocf@@@eblock}[2]{#1\ifArgumentEmpty{#2}{\relax}{\KwSty{\@algocf@endoption{#2}}\strut\par}}% block: group with a end keyword.
\newcommand{\algocf@@@block}[3]{#1\ifArgumentEmpty{#2}{\ifArgumentEmpty{#3}{\relax}{ #3\relax}}{\KwSty{\@algocf@endoption{#2}}\ifArgumentEmpty{#3}{\relax}{ #3}\strut\par}}% block: group with a end keyword.
\newcommand{\algocf@@block}[3]{\algocf@@@block{#1}{#2}{#3}}% block: group with a end keyword.
\newcommand{\algocf@block}[3]{\algocf@@block{#1}{#2}{#3}}% command that will be used and redefined accordingly to noend option
%\newcommand{\algocf@nblock}[3]{\algocf@@block{#1}{#2}{#3}}% command that will be used and redefined accordingly to noend option
\newcommand{\algocf@setBlock}{%
  \ifthenelse{\boolean{algocf@optnoend}}{%     if no end option
    \renewcommand{\algocf@block}[3]{\algocf@group{##1}}%     block will be a group
  }{%                                          else
    \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}% block stays a block
  }%
}%
%
\newcommand{\Hlne}{}% little hrizontal line ending a block in vline mode
%
\newcommand{\@algocf@endoption}[1]{#1}%
\newboolean{algocf@optnoend}\setboolean{algocf@optnoend}{false}%
%
\newcommand{\SetAlgoLongEnd}{%%%%%%%%%%%%%%%%%%%%%%%%% Long End
  \setboolean{algocf@optnoend}{false}%
  \renewcommand{\@algocf@endoption}[1]{##1}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoShortEnd}{%%%%%%%%%%%%%%%%%%%%%%%% ShortEnd
  \setboolean{algocf@optnoend}{false}%
  \renewcommand{\@algocf@endoption}[1]{\@firstword##1 \@nil}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoNoEnd}{%%%%%%%%%%%%%%%%%%%%%%%%%%% NoEnd
  \setboolean{algocf@optnoend}{true}%
  \renewcommand{\@algocf@endoption}[1]{}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoNoLine}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Noline
\renewcommand{\algocf@@block}[2]{\algocf@@@block{\algocf@Noline{##1}}{##2}}%
\renewcommand{\algocf@group}[1]{\algocf@Noline{##1}}%
\renewcommand{\Hlne}{}}%
%
\newcommand{\SetAlgoVlined}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Vline
\renewcommand{\algocf@@block}[2]{\algocf@Vline{##1}}%
\renewcommand{\algocf@group}[1]{\algocf@Vsline{##1}}%\ifthenelse{\boolean{algocf@optnoend}}{\relax}{\strut\ignorespaces}}%
\renewcommand{\Hlne}{\algocf@Hlne}}%
%
\newcommand{\SetAlgoLined}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Line
\renewcommand{\algocf@@block}[2]{\algocf@@@block{\strut\algocf@Vsline{##1}}{##2}}% no skip after a block so garantie at least one line
\renewcommand{\algocf@group}[1]{\algocf@Vsline{##1}}%\ifthenelse{\boolean{algocf@optnoend}}{\relax}{\strut\ignorespaces}}%
\renewcommand{\Hlne}{}}%
%
\newcommand{\SetNothing}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Noline
\renewcommand{\algocf@@block}[2]{\algocf@Noline{##1}\par}%
%\long
\renewcommand{\algocf@group}[1]{\algocf@Noline{##1}}%
\renewcommand{\Hlne}{}}%
%
%%
%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ``Input:'''s like command 
%
%%%
% text staying at the right of the longer keyword of KwInOut commands 
% (text of KwInOut commands are all vertically aligned)
%
\newcommand{\algocf@newinout}{\par\parindent=\inoutindent}% to put right indentation after a \\ in the KwInOut
\newcommand{\SetKwInOut}[2]{%
  \sbox\algocf@inoutbox{\KwSty{#2\algocf@typo:}}%
  \expandafter\ifx\csname InOutSizeDefined\endcsname\relax% if first time used
    \newcommand\InOutSizeDefined{}\setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
  \else% else keep the larger dimension
    \ifdim\wd\algocf@inoutbox>\inoutsize%
    \setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
    \fi%
  \fi% the dimension of the box is now defined.
  \algocf@newcommand{#1}[1]{%
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@seteveryparhanging{\relax}}%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
%     {\let\\\algocf@newinout\hangindent=\wd\algocf@inoutbox\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo\hfill:}~##1\par}%
    {\let\\\algocf@newinout\hangindent=\inoutindent\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~##1\par}%
    \algocf@linesnumbered% reset the numbering of the lines
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@reseteveryparhanging}%
  }}%
%
%% allow to ajust the skip size of InOut
%%
\newcommand{\ResetInOut}[1]{%
  \sbox\algocf@inoutbox{\hbox{\KwSty{#1\algocf@typo:}\ }}%
  \setlength{\inoutsize}{\wd\algocf@inoutbox}%
  }%
%
% 
%%%
% text staying at the right of the keyword.
%
\newcommand{\algocf@newinput}{\par\parindent=\wd\algocf@inputbox}% to put right indentation after a \\ in the KwInput
\newcommand{\SetKwInput}[2]{%
  \algocf@newcommand{#1}[1]{%
    \sbox\algocf@inputbox{\hbox{\KwSty{#2\algocf@typo:} }}%
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@seteveryparhanging{\relax}}%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
    {\let\\\algocf@newinput\hangindent=\wd\algocf@inputbox\hangafter=1\unhbox\algocf@inputbox##1\par}%
    \algocf@linesnumbered% reset the numbering of the lines
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@reseteveryparhanging}%
  }}%
\newcommand{\SetKwData}[2]{%
  \algocf@newcommand{@#1}[1]{\DataSty{#2(}\ArgSty{##1}\DataSty{)}}%
  \algocf@newcommand{#1}{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\DataSty{#2}\xspace}}%
  }%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% tallent:
%
% Add following macros:
%   \SetKwHangingKw:  [kw] ------------   <= hanging determined by [kw]
%                          ------------
% Should act like a combination of \SetKwInput and \SetKw.
% Based on \SetKwInput:
%   - remove ':' at end of keyword
%   - do not reset numbering
%   - use separate savebox
\newsavebox{\algocf@hangingbox}
\newcommand{\algocf@newhanging}{\par\parindent=\wd\algocf@hangingbox}% to put right indentation after a \\ in the KwInput
\newcommand{\SetKwHangingKw}[2]{%
  \algocf@newcommand{#1}[1]{%
    \sbox\algocf@hangingbox{\hbox{\KwSty{#2}\algocf@typo\ }}%
    {\let\\\algocf@newhanging\hangindent=\wd\algocf@hangingbox\hangafter=1\unhbox\algocf@hangingbox##1\;}%
  }%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Comments macros
%
%%%%
% comment in the text, first argument is the name of the macro, second is
% the text put before the comment, third is the text put at the end of the
% comment.
%
% first side comment justification
\newcommand{\SetSideCommentLeft}{\setboolean{algocf@scleft}{true}}%
\newcommand{\SetSideCommentRight}{\setboolean{algocf@scleft}{false}}%
\newcommand{\SetNoFillComment}{\setboolean{algocf@optfillcomment}{false}}%
\newcommand{\SetFillComment}{\setboolean{algocf@optfillcomment}{true}}%
%
% next comment and side comment
%
\newcommand{\algocf@endmarkcomment}{\relax}%
\newcommand{\algocf@fillcomment}{%
  \ifthenelse{\boolean{algocf@optfillcomment}}{\hfill}{\relax}}%
%
\newcommand{\algocf@startcomment}{%
  \hangindent=\wd\algocf@inputbox\hangafter=1\usebox\algocf@inputbox}%
\newcommand{\algocf@endcomment}{\algocf@fillcomment\algocf@endmarkcomment\ignorespaces\par}%
\newcommand{\algocf@endstartcomment}{\algocf@endcomment\algocf@startcomment\ignorespaces}%
%
\newboolean{algocf@sidecomment}%
\newboolean{algocf@altsidecomment}\setboolean{algocf@altsidecomment}{false}%
\newcommand{\algocf@scpar}{\ifthenelse{\boolean{algocf@altsidecomment}}{\relax}{\par}}%
\newcommand{\algocf@sclfill}{\ifthenelse{\boolean{algocf@scleft}}{\algocf@fillcomment}{\relax}}%
\newcommand{\algocf@scrfill}{\ifthenelse{\boolean{algocf@scleft}}{\relax}{\hfill}}%
\newcommand{\algocf@startsidecomment}{\usebox\algocf@inputbox}%
\newcommand{\algocf@endsidecomment}{\algocf@endmarkcomment\algocf@scpar}%
\newcommand{\algocf@endstartsidecomment}{%
  \algocf@sclfill\algocf@endsidecomment%
  \algocf@scrfill\algocf@startsidecomment\ignorespaces}%
%
\newcommand{\SetKwComment}[3]{%
  \algocf@newcommand{#1}{\@ifstar{\csname algocf@#1@star\endcsname}{\csname algocf@#1\endcsname}}%
	\algocf@newcommand{algocf@#1}[1]{%
      \ifthenelse{\boolean{algocf@hangingcomment}}{\relax}{\algocf@seteveryparhanging{\relax}}%
      \sbox\algocf@inputbox{\CommentSty{\hbox{#2}}}%
      \ifthenelse{\boolean{algocf@commentsnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
      {\renewcommand{\algocf@endmarkcomment}{#3}%
        \let\\\algocf@endstartcomment%
        \algocf@startcomment\CommentSty{%
          \strut\ignorespaces##1\strut\algocf@fillcomment#3}\par}%
      \algocf@linesnumbered% reset the numbering of the lines
      \ifthenelse{\boolean{algocf@hangingcomment}}{\relax}{\algocf@reseteveryparhanging}%
    }%
  %%% side comment definitions
	\algocf@newcommand{algocf@#1@star}[2][]{%
      \ifArgumentEmpty{##1}\relax{% TODO: Is this even necessary, with all those \ifx's?
        \ifthenelse{\boolean{algocf@scleft}}{\setboolean{algocf@sidecomment}{true}}{\setboolean{algocf@sidecomment}{false}}%
        \ifx##1h\setboolean{algocf@altsidecomment}{true}\SetSideCommentLeft\fi%
        \ifx##1f\setboolean{algocf@altsidecomment}{true}\SetSideCommentRight\fi%
        \ifx##1l\setboolean{algocf@altsidecomment}{false}\SetSideCommentLeft\fi%
        \ifx##1r\setboolean{algocf@altsidecomment}{false}\SetSideCommentRight\fi%
      }%
      \sbox\algocf@inputbox{\CommentSty{\hbox{#2}}}%
      \ifthenelse{\boolean{algocf@commentsnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
      {%
        \renewcommand{\algocf@endmarkcomment}{#3}%
        \let\\\algocf@endstartsidecomment%
        % here is the comment
        \ifthenelse{\boolean{algocf@altsidecomment}}{\relax}{\@endalgocfline\ }%
        \algocf@scrfill\algocf@startsidecomment\CommentSty{%
          \strut\ignorespaces##2\strut\algocf@sclfill#3}\algocf@scpar%
      }%
      \algocf@linesnumbered% reset the numbering of the lines
      \ifArgumentEmpty{##1}\relax{%
        \ifthenelse{\boolean{algocf@sidecomment}}{\setboolean{algocf@scleft}{true}}{\setboolean{algocf@scleft}{false}}%
        \setboolean{algocf@altsidecomment}{false}%
      }%
	}%
  }%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwProg
%
\newcommand{\SetKwProg}[4]{%\SetKwProg{Env}{Title}{is}{end} 
	\algocf@newcmdside@koif{#1}{\KwSty{#2}\ifArgumentEmpty{#2}\relax{\ }\ProgSty{##2}\KwSty{#3}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#4}{##4}}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2} \ProgSty{##2}\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode\@endalgocfline\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2} \ProgSty{##2}\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
}%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Kw
%
\newcommand{\SetKw}[2]{%
	\algocf@newcommand{@#1}[1]{\KwSty{#2} \ArgSty{##1}}
	\algocf@newcommand{#1}{\@ifnextchar\bgroup{\csname @#1\endcsname}{\KwSty{#2}\xspace}}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwFunction
%
\newcommand{\SetKwFunction}[2]{%
%%% use of gdef since newcommand doesn't manage to define the macro when SetKwFunction is used in \algocf@caption@proc
  \expandafter\gdef\csname @#1\endcsname##1{\FuncSty{#2(}\FuncArgSty{##1}\FuncSty{)}}%
  \expandafter\gdef\csname#1\endcsname{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\FuncSty{#2}\xspace}}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwTab
%
\newcommand{\SetKwArray}[2]{%
%%% use of gdef since newcommand doesn't manage to define the macro when SetKwFunction is used in \algocf@caption@proc
  \expandafter\gdef\csname @#1\endcsname##1{\DataSty{#2[}\ArgSty{##1}\DataSty{]}}%
  \expandafter\gdef\csname#1\endcsname{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\DataSty{#2}\xspace}}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwBlock
%
\newcommand{\SetKwBlock}[3]{%
	\algocf@newcmdside@kobe{#1}%
    {\KwSty{#2}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##2}{#3}{##3}\par}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% condition typo
%
\newcommand{\algocf@scond}{\ }
\newcommand{\algocf@econd}{\ }
\newcommand{\algocf@ucond}{}
\newcommand{\SetStartEndCondition}[3]{%
  \renewcommand{\algocf@scond}{#1}\renewcommand{\algocf@econd}{#2}\renewcommand{\algocf@ucond}{#3}}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For Switch
%
\newcommand{\SetKwSwitch}[9]{% #1=\Switch #2=\Case #3=\Other #4=switch #5=do #6=case #7=otherwise #8=endcase #9=endsw
%	\algocf@newcmdside{#1}{3}%
	\algocf@newcmdside@koif{#1}%
		{\KwSty{#4}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#9} {##4\relax}}%
%%%% Case
	\algocf@newcmdside@koif{#2}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#8}{##4\relax}}%
    %uCase
	\algocf@newcmdside{u#2}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@group{##3}}%
    %lcase
    \algocf@newcommand{l#2}{\@ifstar{\csname algocf@l#2star\endcsname}{\csname algocf@l#2\endcsname}}%
	\algocf@newcmdside{algocf@l#2}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\ \relax{ ##1}\strut\par}%
	\algocf@newcmdside{algocf@l#2star}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
%%%% Other 
	\algocf@newcmdside@kobe{#3}{\KwSty{#7} \KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##2}{#8}{##3\relax}}%
    %lOther
    \algocf@newcommand{l#3}{\@ifstar{\csname algocf@l#3star\endcsname}{\csname algocf@l#3\endcsname}}%
	\algocf@newcmdside{algocf@l#3}{2}{\KwSty{#7} \KwSty{#5}\algocf@bgroupcode\ ##2\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#3star}{2}{\KwSty{#7} \KwSty{#5}\algocf@bgroupcode\ ##2\algocf@egroupcode}%
    %uOther
	\algocf@newcmdside{u#3}{3}{\KwSty{#7} \KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@group{##2}}%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% If macros
%
\newcommand{\SetKwIF}[8]{% #1=\If #2=\ElseIf #3=\Else #4=if #5=then #6=elseif #7=else #8=endif
% 
% common text
	\algocf@newcommand{#1@ifthen}[1]{\KwSty{#4}\algocf@scond\ArgSty{##1}\algocf@econd\KwSty{#5}}%
	\algocf@newcommand{#1@endif} [2]{\algocf@block{##1}{#8}{##2}}%
	\algocf@newcommand{#1@noend} [1]{\algocf@group{##1}}%
	\algocf@newcommand{#1@else}  [1]{\algocf@group{##1}\KwSty{#7}}%
	\algocf@newcommand{#2@elseif}[1]{\KwSty{#6}\algocf@scond\ArgSty{##1}\algocf@econd\KwSty{#5}}%
	\algocf@newcommand{#3@else}     {\KwSty{#7}}%
%%%% If then { } endif
	\algocf@newcmdside@koif{#1}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##3}{##4\relax}}%
%%%% If then {} else {} endif
    % first command to handle optional side comment of else (so just after first braces)
 	\algocf@newcmdside@kobe{algocf@e#1thenelse}{\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##2}{##3}}%
    % the definition of if-then-else command using command above 
	\algocf@newcmdside{e#1}{3}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@else\endcsname{##3}\csname algocf@e#1thenelse\endcsname}%
    %%% leif
    \algocf@newcommand{le#1}{\@ifstar{\csname algocf@le#1star\endcsname}{\csname algocf@le#1\endcsname}}%
    \algocf@newcmdside{algocf@le#1}{4}{\csname #1@ifthen\endcsname{##2} \algocf@bgroupcode##3 \csname #3@else\endcsname\ ##4\@endalgocfline\ \algocf@egroupcode\ifArgumentEmpty{##1}\relax{##1}\strut\par}%
    \algocf@newcmdside{algocf@le#1star}{4}{\csname #1@ifthen\endcsname{##2} \algocf@bgroupcode##3 \csname #3@else\endcsname\ ##4\algocf@egroupcode}%
%%%% If then 
	% \algocf@newcmdside{l#1}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\
    % ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
	\algocf@newcmdside{u#1}{3}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@noend\endcsname{##3}}%
%%%% ElseIf {} endif
	\algocf@newcmdside@koif{#2}{\csname #2@elseif\endcsname{##2}\relax\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##3}{##4\relax}}%
%%%% ElseIf
    \algocf@newcommand{l#2}{\@ifstar{\csname algocf@l#2star\endcsname}{\csname algocf@l#2\endcsname}}%
	\algocf@newcmdside{algocf@l#2}{3}{\csname #2@elseif\endcsname{##2}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#2star}{3}{\csname #2@elseif\endcsname{##2}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
	\algocf@newcmdside{u#2}{3}{\csname #2@elseif\endcsname{##2}\relax\ifArgumentEmpty{##1}\relax{##1}\csname #1@noend\endcsname{##3}}%
%%%% Else {} endif
	\algocf@newcmdside@kobe{#3}{\csname #3@else\endcsname\ifArgumentEmpty{##1}\relax\ ##1\csname #1@endif\endcsname{##2}{##3\relax}}%
%%%% Else 
    \algocf@newcommand{l#3}{\@ifstar{\csname algocf@l#3star\endcsname}{\csname algocf@l#3\endcsname}}%
	\algocf@newcmdside{algocf@l#3}{2}{\csname #3@else\endcsname\algocf@bgroupcode\ ##2\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#3star}{2}{\csname #3@else\endcsname\algocf@bgroupcode\ ##2\algocf@egroupcode}%
	\algocf@newcmdside{u#3}{2}{\csname #3@else\endcsname\ifArgumentEmpty{##1}\relax\ {##1\relax}\csname #1@noend\endcsname{##2}}%
}% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For macros
%
\newcommand{\SetKwFor}[4]{%
	\algocf@newcmdside@koif{#1}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#4}{##4\relax}}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Repeat macros
%
\newsavebox{\algocf@untilbox}% to handle width of until keyword needed to have good skip
  % for line numbers
\newskip\algocf@skipuntil
\newcommand{\SetKwRepeat}[3]{%
	\algocf@newcmdsides{#1}{3}{%
      \sbox\algocf@untilbox{\KwSty{#3}\algocf@scond}\algocf@skipuntil=\wd\algocf@untilbox%
      \KwSty{#2}\ifArgumentEmpty{##1}\relax{##1}\algocf@group{##3}%
      \KwSty{#3}\algocf@scond% until keyword and start condition typo
      %\advance\skiptotal by\algocf@skipuntil%
      \ArgSty{##2}%
      %\advance\skiptotal by-\algocf@skipuntil%
      \algocf@ucond%
      \algocf@skipuntil=0pt% reset counter
    }{\@endalgocfline}{\strut\par}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2}\algocf@bgroupcode\ ##3\algocf@egroupcode\ \KwSty{#3}\algocf@scond\ArgSty{##2}\algocf@ucond\@endalgocfline\ifArgumentEmpty{##1}\relax{ ##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2}\algocf@bgroupcode\ ##3\algocf@egroupcode\ \KwSty{#3}\algocf@scond\ArgSty{##2}\algocf@ucond}%
}%
%
% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%        Environments definitions     %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%
%% Caption management
%%
% for the following macros:
% #1 is given by caption and is equal to fnum@algocf
% #2 is the text given in argument by the user in the \caption macro
%
%%%%% text of caption
\newcommand{\algocf@captionlayout}[1]{#1}%
\newcommand{\SetAlgoCaptionLayout}[1]{%
  \renewcommand{\algocf@captionlayout}[1]{\csname #1\endcsname{##1}}}%
\newcommand{\algocf@capseparator}{:}%
\newcommand{\SetAlgoCaptionSeparator}[1]{\renewcommand{\algocf@capseparator}{#1}}%
\newcommand{\algocf@captiontext}[2]{%
  \algocf@captionlayout{\AlCapSty{\AlCapFnt #1\algocf@typo\algocf@capseparator}\nobreakspace%
    \AlCapNameSty{\AlCapNameFnt{}#2\endgraf}}}% text of caption
%
%%%%% default caption of algorithm: used if no specific style caption is defined
\newcommand{\algocf@makecaption}[2]{%
  \addtolength{\hsize}{\algomargin}%
  \sbox\@tempboxa{\algocf@captiontext{#1}{#2}}%
  \ifdim\wd\@tempboxa >\hsize%     % if caption is longer than a line
    \hskip .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}% then caption is not centered
  \else%
    \global\@minipagefalse%
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}% else caption is centered
  \fi%
  \addtolength{\hsize}{-\algomargin}%
}%
%
\newsavebox\algocf@capbox%
\newcommand{\algocf@makecaption@plain}[2]{%
  \global\sbox\algocf@capbox{\algocf@makecaption{#1}{#2}}}%
\newcommand{\algocf@makecaption@boxed}[2]{%
  \addtolength{\hsize}{-\algomargin}%
  \global\sbox\algocf@capbox{\algocf@makecaption{#1}{#2}}%
  \addtolength{\hsize}{\algomargin}%
 }%
%
\newcommand{\algocf@makecaption@plainruled}[2]{\algocf@makecaption@plain{#1}{#2}}%
\newcommand{\algocf@makecaption@tworuled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@algoruled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@boxruled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@ruled}[2]{%
  \global\sbox\algocf@capbox{\hskip\AlCapHSkip% .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}}% then caption is not centered
}%
%
\newlength{\algoheightruledefault}\setlength{\algoheightruledefault}{0.8pt}%
\newlength{\algoheightrule}\setlength{\algoheightrule}{\algoheightruledefault}%
\newlength{\algotitleheightruledefault}\setlength{\algotitleheightruledefault}{0.8pt}%
\newlength{\algotitleheightrule}\setlength{\algotitleheightrule}{\algotitleheightruledefault}%
\newcommand{\algocf@caption@plain}{\vskip\AlCapSkip\box\algocf@capbox}%
\newcommand{\algocf@caption@plainruled}{\algocf@caption@plain}%
\newcommand{\algocf@caption@boxed}{\vskip\AlCapSkip\box\algocf@capbox}%
\newcommand{\algocf@caption@ruled}{\box\algocf@capbox\kern\interspacetitleruled\hrule
  width\algocf@ruledwidth height\algotitleheightrule depth0pt\kern\interspacealgoruled}%
\newcommand{\algocf@caption@tworuled}{\box\algocf@capbox\hrule  height0pt depth0pt\kern\interspacealgoruled}%
\newcommand{\algocf@caption@algoruled}{\algocf@caption@ruled}%
\newcommand{\algocf@caption@boxruled}{%
  \addtolength{\hsize}{-0.8pt}%
  \hbox to\hsize{%
    \vrule%\hskip-0.35pt%
    \vbox{%
      \hrule\vskip\interspacetitleboxruled%
      \hbox to\hsize{\unhbox\algocf@capbox\hfill}\vskip\interspacetitleboxruled%
    }% 
    %\hskip-0.35pt%
    \vrule%
  }\nointerlineskip%
  \addtolength{\hsize}{0.8pt}%
}%
%
%
%%%% set caption for the environment
\newcommand{\algocf@captionref}{%
  \renewcommand{\fnum@algocf}[1]{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\algocf@algocfref}}%
  \addtocounter{algocf}{-1}% \caption do a refstepcounter, so we restore the precedent value
  \let\old@thealgocf=\thealgocf\renewcommand{\thealgocf}{{\relsize{\algocf@refrelsize}\algocf@algocfref}}%
  \gdef\@currentlabel{\algocf@algocfref}% let the label use the new ref
}%
%
% Unfortunatly, we also need our own caption to set some specific stuff for special references. But after these
% settings, we call the original caption.
%
\long\def\algocf@caption@algo#1[#2]#3{%
  \ifthenelse{\equal{\algocf@algocfref}{\relax}}{}{\algocf@captionref}%
  \@ifundefined{hyper@refstepcounter}{\relax}{% if hyper@refstepcounter undefind, no hyperref, else...
    \ifthenelse{\equal{\algocf@algocfref}{\relax}}{\renewcommand{\theHalgocf}{\thealgocf}}{% take algocf as Href
      \renewcommand{\theHalgocf}{\algocf@algocfref}}%else if SetAlgoRefName done, take this name as ref.
    \hyper@refstepcounter{algocf}%set algocf as category of ref
  }%
   \algocf@latexcaption{#1}[{#2}]{{#3}}% call original caption
}%
%
% beamer define is own caption overrinding latex caption!
% as we need it, we have put here the original definition
% to handle manual ref, unfortunately we have to add one line to handle algocf@algocfref
\long\def\algocf@latexcaption#1[#2]#3{% original definition of caption
  \par%
  \addcontentsline{\csname ext@#1\endcsname}{#1}%
  {\protect\numberline{\csname the#1\endcsname}{\ignorespaces #2}}%
  \begingroup%
  \@parboxrestore%
  \if@minipage%
    \@setminipage%
  \fi%
  \normalsize%
  \@makecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par%
  \endgroup%
}%
%
% \ifx\beamer@makecaption\undefined%
% \else% beamer detected
\ifx\@makecaption\undefined%
\newcommand{\@makecaption}[2]{\relax}%
\fi%
%%

%
% more and more packages redefine \@caption instead of just \@makecaption which makes algorithm2e
% caption not works since based on standard \@caption. So we force the definition of \@caption to be
% the standard one (the one from LaTeX) inside algorithm environment.
%
% unfortunately, makecaption is called with \ignorespace #3 so 
% we can't do the @currentlabel definition inside \algocf@captionproctext
\long\def\algocf@caption@proc#1[#2]#3{%
  \ifthenelse{\boolean{algocf@nokwfunc}}{\relax}{%
    \SetKwFunction{\algocf@captname#3@}{\algocf@captname#3@}%
  }%
  % we tell hyperref to use algocfproc as category and to take the appropriate ref.
  \ifthenelse{\boolean{algocf@func}}{\def\@proc@func{algocffunc}}{\def\@proc@func{algocfproc}}%
  \@ifundefined{hyper@refstepcounter}{\relax}{% if hyper@refstepcounter undefind, no hyperref, else...
    \ifthenelse{\boolean{algocf@procnumbered}}{% 
      \expandafter\def\csname theH\@proc@func\endcsname{\thealgocf}%if procnumbered, take \thealgocf as ref
    }{%
      \expandafter\def\csname theH\@proc@func\endcsname{\algocf@captname#3@}%else take procedure or function name
    }%
    \hyper@refstepcounter{\@proc@func}%
  }%
  \ifthenelse{\boolean{algocf@procnumbered}}{\relax}{%
    \addtocounter{algocf}{-1}% \caption do a refstepcounter, so we restore the precedent value
    \gdef\@currentlabel{\algocf@captname#3@}% let the label be the name of the function, not the counter
  }%
  \ifthenelse{\equal{\algocf@captparam#2@}{\arg@e}}{% if no paramater, we remove the ()
    \algocf@latexcaption{#1}[\algocf@procname\nobreakspace\algocf@captname#2@]{#3}%
  }{%                                                 else we give the complete name
    \algocf@latexcaption{#1}[\algocf@procname\nobreakspace#2]{#3}%
  }%
}%
%%
%%% setcaption
\newcommand{\algocf@setcaption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if proc environment, caption text must be changed
    \let\algocf@oldcaptiontext=\algocf@captiontext%
    \renewcommand{\algocf@captiontext}[2]{%
      \algocf@captionproctext{##1}{##2}%
    }%
  }{}%
  \let\algocf@savecaption=\@caption%
  \ifthenelse{\boolean{algocf@procenvironment}}{\let\@caption=\algocf@caption@proc}{\let\@caption=\algocf@caption@algo}%
  \let\algocf@oldmakecaption=\@makecaption%
  \renewcommand{\@makecaption}[2]{%
    \expandafter\csname algocf@makecaption@\algocf@style\endcsname{##1}{##2}%
  }%
}%
%
%%%%% reset caption
%
% since we have force the LaTeX caption for algorithm environment, we must go back to the caption
% used in the text.
\newcommand{\algocf@resetcaption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if proc environment
    \let\thealgocf=\old@thealgocf% restore normal counter printing
    \let\algocf@captiontext=\algocf@oldcaptiontext% restore normal caption text
  }{}%
  \let\@caption=\algocf@savecaption% now restore caption outside algo/proc/func environment
  \let\@makecaption=\algocf@oldmakecaption% and restore makecaption outside outside algo/proc/func environment
  \algocf@resetfnum%
}%
%
%%%%% nocaptionofalgo and restorecaptionofalgo --
\newcommand{\NoCaptionOfAlgo}{%
  \let\@old@algocf@captiontext=\algocf@captiontext%
  \renewcommand{\algocf@captiontext}[2]{\AlCapNameSty{\AlCapNameFnt{}##2}}%
}%
\newcommand{\RestoreCaptionOfAlgo}{%
  \let\algocf@captiontext=\@old@algocf@captiontext%
}%
%
% ----------------------  algocf environment
%
\newcounter{algocfline}%                    % new counter to make lines numbers be internally 
\setcounter{algocfline}{0}%                 % different in different algorithms
\newcounter{algocfproc}% counter to count all algo environment (proc, func), just used by hyperref to avoir "same
\setcounter{algocfproc}{0}% identifier" error caused by algocf being set to '-' for procedure or function or not
  % changed if no caption is given.
%
\expandafter\ifx\csname algocf@within\endcsname\relax% if \algocf@within doesn't exist
\newcounter{algocf}%                        % just define a new counter
\renewcommand{\thealgocf}{\@arabic\c@algocf}% and the way it is printed
\else%                                     else
\newcounter{algocf}[\algocf@within]%        % counter is numbered within \algocf@within
\renewcommand\thealgocf{\csname the\algocf@within\endcsname.\@arabic\c@algocf}%
\fi%
%
\def\fps@algocf{htbp}%        % default
\def\ftype@algocf{10}%        % float type
\def\ext@algocf{\algocf@list} % loa by default, lof if figure option used
\newcommand{\fnum@algocf}{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\thealgocf}}%
\newcommand{\algocf@resetfnum}{\renewcommand{\fnum@algocf}{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\thealgocf}}}%
\newenvironment{algocf}%      % float environment for algorithms
               {\@float{algocf}}%
               {\end@float}%
\newenvironment{algocf*}%     % float* environment for algorithms
               {\@dblfloat{algocf}}%
               {\end@dblfloat}%
%
\def\algocf@seclistalgo{}%
\ifx\l@chapter\undefined\let\algocf@seclistalgo=\section\else\let\algocf@seclistalgo=\chapter\fi%
\@ifundefined{if@restonecol}{\newif\if@restonecol}\relax%
\newcommand\listofalgocfs{%
     \ifx\algocf@seclistalgo\chapter%
      \if@twocolumn\@restonecoltrue\onecolumn\else\@restonecolfalse\fi%
    \fi%
     \algocf@seclistalgo*{\listalgorithmcfname}%
       \@mkboth{\MakeUppercase\listalgorithmcfname}%
               {\MakeUppercase\listalgorithmcfname}%
     \@starttoc{loa}%
    \ifx\algocf@seclistalgo\chapter%
      \if@restonecol\twocolumn\fi%
    \fi%
}
%
\newcommand*\l@algocf{\@dottedtocline{1}{1em}{2.3em}}% line of the list
%
% ----------------------  algorithm environment
%
%%%%%%%
%%
%% Algorithm environment definition
%%
%%%%%%%
%%
%
\newsavebox\algocf@algoframe%
\def\@algocf@pre@plain{\relax}%  action to be done before printing the algo.
\def\@algocf@post@plain{\relax}% action to be done after printing the algo.
\def\@algocf@capt@plain{bottom}% where the caption should be localized.
\def\@algocf@pre@boxed{\noindent\begin{lrbox}{\algocf@algoframe}}
\def\@algocf@post@boxed{\end{lrbox}\framebox[\hsize]{\box\algocf@algoframe}\par}%
\def\@algocf@capt@boxed{under}%
\def\@algocf@pre@ruled{\hrule height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@ruled{\kern\interspacealgoruled\hrule height\algoheightrule\relax}%
\def\@algocf@capt@ruled{top}%
\def\@algocf@pre@algoruled{\hrule width\algocf@ruledwidth height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@algoruled{\kern\interspacealgoruled\hrule width\algocf@ruledwidth height\algoheightrule \relax}%
\def\@algocf@capt@algoruled{top}%
\def\@algocf@pre@tworuled{\hrule height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@tworuled{\kern\interspacealgoruled\hrule height\algoheightrule\relax}%
\def\@algocf@capt@tworuled{top}%
\def\@algocf@pre@boxruled{\noindent\begin{lrbox}{\algocf@algoframe}}%
\def\@algocf@post@boxruled{\end{lrbox}\framebox[\hsize]{\box\algocf@algoframe}\par}%
\def\@algocf@capt@boxruled{above}%
\def\@algocf@pre@plainruled{\@algocf@pre@ruled}%  action to be done before printing the algo.
\def\@algocf@post@plainruled{\@algocf@post@ruled\kern\interspacealgoruled}%  action to be done before printing the algo.
\def\@algocf@capt@plainruled{under}%
%
\newcommand{\noalgocaption}{\def\@algocf@capt@ruled{none}}
%
%% before algocf environment (not figure environment)
\newcommand{\@algocf@init@caption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if we are inside a procedure/function environment
    \@algocf@proctitleofalgo% set Titleofalgo to Procedure: or Function:
                            % accordingly to the environment
    \let\old@thealgocf=\thealgocf\ifthenelse{\boolean{algocf@procnumbered}}{\relax}{%
      \renewcommand{\thealgocf}{-}}%
  }{% else inside environment algorithm
    \@algocf@algotitleofalgo% fix name for \Titleofalgo to \algorithmcfname
  }%
  \algocf@setcaption%       set caption to our caption style
}%
%
\newcommand{\@algofloatboxreset}{\@setminipage}
\newcommand{\@algocf@init}{%
  \refstepcounter{algocfline}%
  \stepcounter{algocfproc}%to have a different counter for each environment and being abble to make the difference
    %between href of algoline in different algorithms.
  \ifthenelse{\boolean{algocf@optnoend}}{%
      \renewcommand{\algocf@block}[3]{\algocf@group{##1}}%
    }{%
      \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}%
    }%
}%
%% after the end of algocf or figure environment
\newcommand{\@algocf@term@caption}{%
  \algocf@resetcaption% restore original caption
}%
%
\newcommand{\@algocf@term}{%
  \setboolean{algocf@algoH}{false}% no H by default
  \ifthenelse{\boolean{algocf@optnoend}}{%
    \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}%
  }{%
    \renewcommand{\algocf@block}[2]{\algocf@group{##1}}%
  }%
  \SetAlgoRefName{\relax}%
}%
%
%%%%%%%%%%%%%%%%%
%% makethealgo: macro which print effectively the algo in its box
%% 
\newsavebox\algocf@algobox%
\newcommand{\algocf@makethealgo}{%
  \vtop{%
    % place caption above if needed  bye the style
    \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{above}}%
    {\csname algocf@caption@\algocf@style\endcsname}{}%
    %
    % precommand according to the style
    \csname @algocf@pre@\algocf@style\endcsname%
    % place caption at top if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{top}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
    %
    \box\algocf@algobox% the algo
    % place caption at bottom if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{bottom}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
    % postcommand according to the style
    \csname @algocf@post@\algocf@style\endcsname%
    % place caption under if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{under}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
  }%
}%
%%%%%%%%%%%%%%%%%%%
%
%% at the beginning of algocf or figure environment
\newenvironment{algomathdisplay}{\[}{\@endalgocfline\]\ifthenelse{\boolean{algocf@linesnumbered}}{\nl}{\relax}}%
\newcommand{\@algocf@start}{%
  \@algoskip%
  \begin{lrbox}{\algocf@algobox}%
  \setlength{\algowidth}{\hsize}%
  \vbox\bgroup% save all the algo in a box
  \hbox to\algowidth\bgroup\hbox to \algomargin{\hfill}\vtop\bgroup%
  \ifthenelse{\boolean{algocf@slide}}{\parskip 0.5ex\color{black}}{}%
  % initialization
  \addtolength{\hsize}{-1.5\algomargin}%
  \let\@mathsemicolon=\;\def\;{\ifmmode\@mathsemicolon\else\@endalgoln\fi}%
  \raggedright\AlFnt{}%
  \ifthenelse{\boolean{algocf@slide}}{\IncMargin{\skipalgocfslide}}{}%
  \@algoinsideskip%
%   \let\@emathdisplay=\]\def\]{\algocf@endline\@emathdisplay\nl}%
}%
%
%% at the end of algocf or figure environment
\newcommand{\@algocf@finish}{%
  \@algoinsideskip%
  \egroup%end of vtop which contain all the text
  \hfill\egroup%end of hbox wich contains [margin][vtop]
  \ifthenelse{\boolean{algocf@slide}}{\DecMargin{\skipalgocfslide}}{}%
  %
  \egroup%end of main vbox
  \end{lrbox}%
  \algocf@makethealgo% print the algo
  \@algoskip%
  % restore dimension and macros
  \setlength{\hsize}{\algowidth}%
  \lineskip\normallineskip\setlength{\skiptotal}{\@defaultskiptotal}%
  \let\;=\@mathsemicolon%  
  \let\]=\@emathdisplay%
}%
%
%%%%%%%%%%%%%%%%%%%%
%% basic definition of the environment algorithm
%%
%
\newboolean{algocf@procenvironment}\setboolean{algocf@procenvironment}{false}%
\newboolean{algocf@func}\setboolean{algocf@func}{false}%
\newboolean{algocf@algoH}\setboolean{algocf@algoH}{false}%
\newboolean{algocf@algostar}\setboolean{algocf@algostar}{false}%
%
%%% environment for {algorithm}[H]
\newenvironment{algocf@Here}{\noindent%
  \def\@captype{algocf}% if not defined, caption exit with an error
  \begin{minipage}{\hsize}%
}{%
  \end{minipage}%\par%
}%
%%% real algorithm environment which manages H and * option
%    \let\algocf@originalfloatboxreset=\@floatboxreset%
%    \let\@floatboxreset=\@algofloatboxreset%
\newenvironment{algocf@algorithm}[1][htbp]{%
   \ifthenelse{\equal{\algocf@float}{figure}}{%
     \ifthenelse{\boolean{algocf@figurecaption}}{\captionsetup{margin={-\algomargin,\algomargin}}}{}%
   }{}%
   \@algocf@init%
   \ifthenelse{\equal{\algocf@float}{figure}}{% if option figure set
     \ifthenelse{\boolean{algocf@algostar}}{% if algorithm* with figure option
       \begin{figure*}[#1]% call figure*
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
         \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }{% else algorithm environment with figure option
       \begin{figure}[#1]%  call figure
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
          \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }%
   }{% else normal algorithm environment
     \@algocf@init@caption%
     \ifthenelse{\equal{#1}{H}}{% if [H] algorithm
       \if@twocolumn\@latex@error{[H] in two columns mode is not allowed for algorithms}\fi% TODO: SCREAM if H in two colums!
       \setboolean{algocf@algoH}{true}\begin{algocf@Here}% call corresponding environment
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
         \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }{% else floating algorithm environment
       \ifthenelse{\boolean{algocf@algostar}}{% if algorithm*
         \begin{algocf*}[#1]% call algocf*
           \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
           \let\algocf@oldeverypar=\everypar%
           \algocf@seteverypar%
       }{% else algorithm environment
         \begin{algocf}[#1]%  call algcf
           \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
           \let\algocf@oldeverypar=\everypar%
           \algocf@seteverypar%
       }%
     }%
   }% fin test option figure ou pas
   \@algocf@start% 
   \@ResetCounterIfNeeded%
   \algocf@linesnumbered\ignorespaces%
}{%
  \@algocf@finish%
  \ifthenelse{\equal{\algocf@float}{figure}}{%
     \ifthenelse{\boolean{algocf@algostar}}{% if algorithm* with figure option
       \let\everypar=\algocf@oldeverypar%
       \end{figure*}% call figure*
     }{% else algorithm environment with figure option
       \let\everypar=\algocf@oldeverypar%
       \end{figure}%  call figure
     }%
  }{%
    \@algocf@term@caption%
    \ifthenelse{\boolean{algocf@algoH}}{% if [H] algorithm
      \let\everypar=\algocf@oldeverypar%
      \end{algocf@Here}\par% call corresponding environment
     }{% else floating algorithm environment
       \ifthenelse{\boolean{algocf@algostar}}{% if algorithm*
         \let\everypar=\algocf@oldeverypar%
         \end{algocf*}% call algocf*
       }{% else algorithm environment
         \let\everypar=\algocf@oldeverypar%
         \end{algocf}%  call algocf
       }%
     }%
  }%
  \@algocf@term\ignorespacesafterend%
}%
%
%%% user algorithm environment
\newenvironment{\algocf@envname}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{false}\gdef\algocfautorefname{\algorithmautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%%% user algorithm* environment
\newenvironment{\algocf@envname*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{false}\gdef\algocfautorefname{\algorithmautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%
%%%
%
\expandafter\newcommand\csname\algocf@listofalgorithms\endcsname{%
  \ifthenelse{\equal{\algocf@float}{figure}}{\listoffigures}{\listofalgocfs}%
}%
%%%
%%%
%
% ----------------------  procedure and function environments
%
%
% -- new style (used in particular in the caption of function and procedure environments)
%
% three macros to extract parts of the caption
\gdef\algocf@captname#1(#2)#3@{#1}  % keep characters before the first brace
\gdef\algocf@captparam#1(#2)#3@{#2} % keep character in between the braces
\gdef\algocf@captother#1(#2)#3@{#3} % keep character after the braces
%
%%% Text of caption for Procedure or Function
\newcommand{\algocf@captionproctext}[2]{%
  {%
    \ProcSty{\ProcFnt\algocf@procname\ifthenelse{\boolean{algocf@procnumbered}}{\nobreakspace\thealgocf\algocf@typo\algocf@capseparator}{\relax}}%
    \nobreakspace\ProcNameSty{\ProcNameFnt\algocf@captname #2@}% Name of the procedure in ProcName Style. 
    \ifthenelse{\equal{\algocf@captparam #2@}{\arg@e}}{}{% if no argument, write nothing
      \ProcNameSty{\ProcNameFnt(}\ProcArgSty{\ProcArgFnt\algocf@captparam #2@}\ProcNameSty{\ProcNameFnt)}%else put arguments in ProcArgSty:
    }% endif
    \algocf@captother #2@%
  }%
}%
%
%
% -- procedure and function environments are defined from algocf@algorithm environment
%
\newenvironment{procedure}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{false}%
  \newcommand{\algocf@procname}{\@algocf@procname}\gdef\algocfprocautorefname{\procedureautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
\newenvironment{function}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{true}%
  \newcommand{\algocf@procname}{\@algocf@funcname}\gdef\algocffuncautorefname{\functionautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
\newenvironment{procedure*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{false}%
  \newcommand{\algocf@procname}{\@algocf@procname}\gdef\algocfprocautorefname{\procedureautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
\newenvironment{function*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{true}%
  \newcommand{\algocf@procname}{\@algocf@funcname}\gdef\algocffuncautorefname{\functionautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
%
%%%%%%%%%%%%%%%%%%%%
%% definition of algondfloat environment
%%
\ifthenelse{\boolean{algocf@endfloat}}{% if endfloat option then
\newcommand{\algoplace}{% macro which is used to writhe algorithm about there
   \begin{center}%
     [\algorithmcfname~\thepostfig\ about here.]%
   \end{center}%
}%
\newcommand{\algoendfloat}{% use as a \begin{algoendfloat} environment to start scanning of line
%  \immediate\openout\@mainfff\jobname.fff%
  \efloat@condopen{fff}
  \efloat@iwrite{fff}{\string\begin{\algocf@envname}}%
    \if@domarkers%
       \ifthenelse{\equal{\algocf@list}{lof}}{%
         \addtocounter{postfig}{1}%
       }{%
         \addtocounter{postalgo}{1}%
       }%
       \algoplace%
    \fi%
    \bgroup%
    \let\do\ef@makeinnocent\dospecials%
    \ef@makeinnocent\^^L% and whatever other special cases
    \endlinechar`\^^M \catcode`\^^M=12 \ef@xalgocfendfloat}%
}{\relax}%%%% end of endfloat option ifthenelse
%% some macros useful for endfloat option that cannot be defined inside the ifthenelse
%scan algoendfloat algorithm and write the text into .fff file
{\catcode`\^^M=12 \endlinechar=-1 %
 \gdef\ef@xalgocfendfloat#1^^M{% scan the lines inside algoendfloat environment being read by latex
   \def\test{#1}% test is the line being currently scan by latex
   \ifx\test\ef@endalgocftest% if it is \end{algoendfloat}
     \def\next{% define next as to not continue the scan and write \end{algorithm} into .fff file
       \egroup\end{algoendfloat}%
       \efloat@iwrite{fff}{\string\end{\algocf@envname}}%
       \efloat@iwrite{fff}{\string\efloatseparator}%
       \efloat@iwrite{fff}{ }%
     }%
     \else% else write the current line being scanned by latex and set next to continue the scan
       \efloat@iwrite{fff}{#1}%
       \let\next\ef@xalgocfendfloat%
     \fi% endif
     \next}% next is continue if it was else condition, else it does not continue the scan and write end to file
}%
% test if the scan is finish by looking at the string \end{algoendfloat}
{\escapechar=-1%
 \xdef\ef@endalgocftest{\string\\end\string\{algoendfloat\string\}}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
\newcommand{\TitleOfAlgo}[1]{\@titleprefix\ 
  \TitleSty{#1}\par\smallskip}%
%
\newcommand{\SetAlgorithmName}[3]{%
  \renewcommand{\listalgorithmcfname}{#3}%
  \renewcommand{\algorithmcfname}{#1}%
  \renewcommand{\algorithmautorefname}{#2}%
}%
%
\newcommand{\algocf@refrelsize}{-2}\newcommand{\SetAlgoRefRelativeSize}[1]{\renewcommand{\algocf@refrelsize}{#1}}%
\newcommand{\SetAlgoRefName}[1]{%
  \renewcommand{\algocf@algocfref}{#1}%
}%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
% -------------------------   Default Definitions
%
%%
%%
%
\SetKwComment{tcc}{/* }{ */}%
\SetKwComment{tcp}{// }{}%
%
%\newcommand{\algocf@defaults@common}{
%
%
% english keywords (default)
%
\SetKwHangingKw{KwHData}{Data$\rightarrow$}
\SetKwInput{KwIn}{Input}%
\SetKwInput{KwOut}{Output}%
\SetKwInput{KwData}{Data}%
\SetKwInput{KwResult}{Result}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
%
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
%
% French keywords
%
\ifthenelse{\boolean{algocf@localkw@french}\OR\equal{\algocf@languagechoosen}{french}}{%
%\SetKwInOut{AlgDonnees}{Donn\'ees}\SetKwInOut{AlgRes}{R\'esultat}
\SetKwHangingKw{HDonnees}{Donnees$\rightarrow$}
\SetKwInput{Donnees}{Donn\'ees}%
\SetKwInput{Res}{R\'esultat}%
\SetKwInput{Entree}{Entr\'ees}%
\SetKwInput{Sortie}{Sorties}%
\SetKw{KwA}{\`a}%
\SetKw{Retour}{retourner}%
\SetKwBlock{Deb}{d\'ebut}{fin}%
\SetKwRepeat{Repeter}{r\'ep\'eter}{jusqu'\`a}%
%
\SetKwIF{Si}{SinonSi}{Sinon}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwSwitch{Suivant}{Cas}{Autre}{suivant}{faire}{cas o\`u}{autres cas}{fin cas}{fin d'alternative}%
\SetKwFor{Pour}{pour}{faire}{fin pour}%
\SetKwFor{PourPar}{pour}{faire en parall\`ele}{fin pour}%
\SetKwFor{PourCh}{pour chaque}{faire}{fin pour chaque}%
\SetKwFor{PourTous}{pour tous les}{faire}{fin pour tous}%
\SetKwFor{Tq}{tant que}{faire}{fin tq}%
}{}%
%
% --- German keywords
%
\ifthenelse{\boolean{algocf@localkw@german}\OR\equal{\algocf@languagechoosen}{german}}{%
\SetKwInput{Ein}{Eingabe}%KwIn
\SetKwInput{Aus}{Ausgabe}%KwOut
\SetKwInput{Daten}{Daten}%KwData
\SetKwInput{Ergebnis}{Ergebnis}%KwResult
\SetKw{Bis}{bis}%KwTo
\SetKw{KwZurueck}{zur\"uck}%KwRet
\SetKw{Zurueck}{zur\"uck}%Return
\SetKwBlock{Beginn}{Beginn}{Ende}%Begin
\SetKwRepeat{Wiederh}{wiederhole}{bis}%Repeat
%
\SetKwIF{Wenn}{SonstWenn}{Sonst}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwSwitch{Unterscheide}{Fall}{Anderes}{unterscheide}{tue}{Fall}{sonst}{Ende Fall}{Ende Unt.}%Switch
\SetKwFor{Fuer}{f\"ur}{tue}{Ende f\"ur}%For
\SetKwFor{FuerPar}{f\"ur}{tue gleichzeitig}{Ende gleichzeitig}%ForPar
\SetKwFor{FuerJedes}{f\"ur jedes}{tue}{Ende f\"ur}%ForEach
\SetKwFor{FuerAlle}{f\"ur alle}{tue}{Ende f\"ur}%ForAll
\SetKwFor{Solange}{solange}{tue}{Ende solange}%While
}{}%
%
% --- Czech keywords
%
\ifthenelse{\boolean{algocf@localkw@czech}\OR\equal{\algocf@languagechoosen}{czech}}{%
\SetKwInput{Vst}{Vstup}%
\SetKwInput{Vyst}{V\'{y}stup}%
\SetKwInput{Vysl}{V\'{y}sledek}%
}{}%
%
% --- Portuguese keywords
%
\ifthenelse{\boolean{algocf@localkw@portuguese}\OR\equal{\algocf@languagechoosen}{portuguese}}{%
\SetKwInput{Entrada}{Entrada}%
\SetKwInput{Saida}{Sa\'{i}da}%
\SetKwInput{Dados}{Dados}%
\SetKwInput{Resultado}{Resultado}%
\SetKw{Ate}{at\'{e}}
\SetKw{KwRetorna}{retorna}%
\SetKw{Retorna}{retorna}%
\SetKwBlock{Inicio}{in\'{i}cio}{fim}%
\SetKwRepeat{Repita}{repita}{at\'{e}}%
%
\SetKwIF{Se}{SenaoSe}{Senao}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwSwitch{Selec}{Caso}{Outro}{selecione}{fa\c{c}a}{caso}{sen\~{a}o}{fim caso}{fim selec}%
\SetKwFor{Para}{para}{fa\c{c}a}{fim para}%
\SetKwFor{ParaPar}{para}{fa\c{c}a em paralelo}{fim para}
\SetKwFor{ParaCada}{para cada}{fa\c{c}a}{fim para cada}%
\SetKwFor{ParaTodo}{para todo}{fa\c{c}a}{fim para todo}%
\SetKwFor{Enqto}{enquanto}{fa\c{c}a}{fim enqto}%
}{}%
%
% --- Italian keywords
%
\ifthenelse{\boolean{algocf@localkw@italiano}\OR\equal{\algocf@languagechoosen}{italiano}}{%
\SetKwInput{KwIng}{Ingresso}%
\SetKwInput{KwUsc}{Uscita}%
\SetKwInput{KwDati}{Dati}%
\SetKwInput{KwRisult}{Risultato}%
\SetKw{KwA}{a}%
\SetKw{KwRitorna}{ritorna}%
\SetKw{Ritorna}{ritorna}%
\SetKwBlock{Inizio}{inizio}{fine}%
\SetKwRepeat{Ripeti}{ripeti}{finch\'e}%
%
\SetKwIF{Sea}{AltSe}{Altrimenti}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{endsw}%
\SetKwFor{Per}{per}{fai}{fine per}%
\SetKwFor{PerPar}{per}{fai in parallelo}{fine per}%
\SetKwFor{PerCiascun}{per ciascun}{fai}{fine per ciascun}%
\SetKwFor{PerTutti}{per tutti i}{fai}{fine per tutti}%
\SetKwFor{Finche}{finch\'e}{fai}{fine finch\'e}%
}{}%
%
% --- Spanish keywords
%
\ifthenelse{\boolean{algocf@localkw@spanish}\OR\equal{\algocf@languagechoosen}{spanish}}{%
\SetKwInput{Datos}{Datos}
\SetKwInput{Resultado}{Resultado}
\SetKwInput{Entrada}{Entrada}
\SetKwInput{Salida}{Salida}
\SetKw{KwA}{a}
\SetKw{KwDevolver}{devolver}
\SetKw{Devolver}{devolver}
\SetKwBlock{Inicio}{inicio}{fin}
\SetKwIF{SSi}{EnOtroCasoSi}{EnOtroCaso}{si}{entonces}{sin\'o, si}{sin\'o}{fin si}
\SetKwSwitch{Seleccionar}{Caso}{Otro}{seleccionar}{hacer}{caso}{sin\'o}{fin caso}{fin seleccionar}
\SetKwFor{Para}{para}{hacer}{fin para}
\SetKwFor{ParaPara}{par}{hacer en paralelo}{fin para}
\SetKwFor{EnParalelo}{para}{hacer en paralelo}{fin para}
\SetKwFor{Mientras}{mientras}{hacer}{fin mientras}
\SetKwFor{ParaCada}{para cada}{hacer}{fin para cada}
\SetKwFor{ParaTodo}{para todo}{hacer}{fin para todo}
\SetKwRepeat{Repetir}{repetir}{hasta que}
}{}%
%
% Croatian keywords
%
\ifthenelse{\boolean{algocf@localkw@croatian}\OR\equal{\algocf@languagechoosen}{croatian}}{%
\SetKwInput{KwUlaz}{Ulaz}%KwIn
\SetKwInput{KwIzlaz}{Izlaz}%KwOut
\SetKwInput{KwPodaci}{Podaci}%KwData
\SetKwInput{KwRezultat}{Rezultat}%KwResult
\SetKw{KwDo}{do}%KwTo
\SetKw{KwVrati}{vrati}%KwRet
\SetKw{Vrati}{vrati}%Return
\SetKwBlock{Pocetak}{po\v{c}etak}{kraj}%Begin
\SetKwRepeat{Ponavljaj}{ponavljaj}{dok ne bude}%Repeat
%
\SetKwIF{Ako}{InaceAko}{Inace}{ako}{onda}{ina\v{c}e ako}{ina\v{c}e}{kraj ako}%gIf
\SetKwSwitch{Granaj}{Slucaj}{OstaliSlucajevi}{granaj}{\v{c}ini}{slu\v{c}aj}{ostali slu\v{c}ajevi}{kraj slu\v{c}aj}{kraj granaj}%Switch
\SetKwFor{Za}{za}{\v{c}ini}{kraj za}%For
\SetKwFor{ZaPar}{za}{\v{c}ini paralelno}{kraj za paralelno}%ForPar
\SetKwFor{ZaSvaki}{za svaki}{\v{c}ini}{kraj za svaki}%mForEach
\SetKwFor{ZaSvaku}{za svaku}{\v{c}ini}{kraj za svaku}%fForEach
\SetKwFor{ZaSvako}{za svako}{\v{c}ini}{kraj za svako}%nForEach
\SetKwFor{ZaSve}{za sve}{\v{c}ini}{kraj za sve}%ForAll
\SetKwFor{Dok}{dok}{\v{c}ini}{kraj dok}%While
}{}%

%
% --- Turkish keywords
%
\ifthenelse{\boolean{algocf@localkw@turkish}\OR\equal{\algocf@languagechoosen}{turkish}}{%
\SetKwInput{KwIn}{Girdi}%
\SetKwInput{KwOut}{\c{C}{\i}kt{\i}}%
\SetKwInput{KwData}{Veri}%
\SetKwInput{KwResult}{Sonu\c{c}}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
% %
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
}{}%
%
% --- End 
%}
%
%\algocf@defaults@common
%
% option onelanguage redefinition
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{french}}{%
\SetKwInput{KwIn}{Entr\'ees}%
\SetKwInput{KwOutSortie}{Sorties}%
\SetKwInput{KwData}{Donn\'ees}%
\SetKwInput{KwResult}{R\'esultat}%
\SetKw{KwTo}{\`a}%
\SetKw{KwRet}{retourner}%
\SetKw{Return}{retourner}%
\SetKwBlock{Begin}{d\'ebut}{fin}%
\SetKwRepeat{Repeat}{r\'ep\'eter}{jusqu'\`a}%
%
\SetKwIF{If}{ElseIf}{Else}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwSwitch{Switch}{Case}{Other}{suivant}{faire}{cas o\`u}{autres cas}{fin cas}{fin d'alternative}%
\SetKwFor{For}{pour}{faire}{fin pour}%
\SetKwFor{ForPar}{pour}{faire en parall\`ele}{fin pour}%
\SetKwFor{ForEach}{pour chaque}{faire}{fin pour chaque}%
\SetKwFor{ForAll}{pour tous}{faire}{fin pour tous}%
\SetKwFor{While}{tant que}{faire}{fin tq}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{german}}{%
\SetKwInput{KwIn}{Eingabe}%KwIn
\SetKwInput{KwOut}{Ausgabe}%KwOut
\SetKwInput{KwData}{Daten}%KwData
\SetKwInput{KwResult}{Ergebnis}%KwResult
\SetKw{KwTo}{bis}%KwTo
\SetKw{KwRet}{zur\"uck}%KwRet
\SetKw{Return}{zur\"uck}%Return
\SetKwBlock{Begin}{Beginn}{Ende}%Begin
\SetKwRepeat{Repeat}{wiederhole}{bis}%Repeat
%
\SetKwIF{If}{ElseIf}{Else}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwSwitch{Switch}{Case}{Other}{unterscheide}{tue}{Fall}{sonst}{Ende Fall}{Ende Unt.}%Switch
\SetKwFor{For}{f\"ur}{tue}{Ende f\"ur}%For
\SetKwFor{ForPar}{f\"ur}{tue gleichzeitig}{Ende gleichzeitig}%ForPar
\SetKwFor{ForEach}{f\"ur jedes}{tue}{Ende f\"ur}%ForEach
\SetKwFor{ForAll}{f\"ur alle}{tue}{Ende f\"ur}%ForAll
\SetKwFor{While}{solange}{tue}{Ende solange}%While
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{portuguese}}{%
\SetKwInput{KwIn}{Entrada}%
\SetKwInput{KwOut}{Sa\'{i}da}%
\SetKwInput{KwData}{Dados}%
\SetKwInput{KwResult}{Resultado}%
\SetKw{KwTo}{at\'{e}}
\SetKw{KwRet}{retorna}%
\SetKw{Return}{retorna}%
\SetKwBlock{Begin}{in\'{i}cio}{fim}%
\SetKwRepeat{Repeat}{repita}{at\'{e}}%
%
\SetKwIF{If}{ElseIf}{Else}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwSwitch{Switch}{Case}{Other}{selecione}{fa\c{c}a}{caso}{sen\~{a}o}{fim caso}{fim selec}%
\SetKwFor{For}{para}{fa\c{c}a}{fim para}%
\SetKwFor{ForPar}{para}{fa\c{c}a em paralelo}{fim para}
\SetKwFor{ForEach}{para cada}{fa\c{c}a}{fim para cada}%
\SetKwFor{ForAll}{para todo}{fa\c{c}a}{fim para todo}%
\SetKwFor{While}{enquanto}{fa\c{c}a}{fim enqto}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{italiano}}{%
\SetKwInput{KwIn}{Ingresso}%
\SetKwInput{KwOut}{Uscita}%
\SetKwInput{KwData}{Dati}%
\SetKwInput{KwResult}{Risultato}%
\SetKw{KwTo}{a}%
\SetKw{KwRet}{ritorna}%
\SetKw{Return}{ritorna}%
\SetKwBlock{Begin}{inizio}{fine}%
\SetKwRepeat{Repeat}{ripeti}{finch\'e}%
%
\SetKwIF{If}{ElseIf}{Else}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{endsw}%
\SetKwFor{For}{per}{fai}{fine per}%
\SetKwFor{ForPar}{per}{fai in parallelo}{fine per}%
\SetKwFor{ForEach}{per ciascun}{fai}{fine per ciascun}%
\SetKwFor{ForAll}{per tutti i}{fai}{fine per tutti}%
\SetKwFor{While}{finch\'e}{fai}{fine finch\'e}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{spanish}}{%
\SetKwInput{KwIn}{Entrada}%
\SetKwInput{KwOut}{Salida}%
\SetKwInput{KwData}{Datos}%
\SetKwInput{KwResult}{Resultado}%
\SetKw{KwTo}{a}%
\SetKw{KwRet}{devolver}%
\SetKw{Return}{devolver}%
\SetKwBlock{Begin}{inicio}{fin}%
\SetKwRepeat{Repeat}{repetir}{hasta que}%
%
\SetKwIF{If}{ElseIf}{Else}{si}{entonces}{si no, si}{en otro caso}{fin si}
\SetKwSwitch{Switch}{Case}{Other}{seleccionar}{hacer}{caso}{si no}{fin caso}{fin seleccionar}
\SetKwFor{For}{para}{hacer}{fin para}%
\SetKwFor{ForPar}{para}{hacer in paralelo}{fin para}%
\SetKwFor{ForEach}{para cada}{hacer}{fin para cada}
\SetKwFor{ForAll}{para todo}{hacer}{fin para todo}
\SetKwFor{While}{mientras}{hacer}{fin mientras}
}{}%
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{croatian}}{%
\SetKwInput{KwIn}{Ulaz}%KwIn
\SetKwInput{KwOut}{Izlaz}%KwOut
\SetKwInput{KwData}{Podaci}%KwData
\SetKwInput{KwResult}{Rezultat}%KwResult
\SetKw{KwTo}{do}%KwTo
\SetKw{KwRet}{vrati}%KwRet
\SetKw{Return}{vrati}%Return
\SetKwBlock{Begin}{po\v{c}etak}{kraj}%Begin
\SetKwRepeat{Repeat}{ponavljaj}{dok ne bude}%Repeat
%
\SetKwIF{If}{ElseIf}{Else}{ako}{onda}{ina\v{c}e ako}{ina\v{c}e}{kraj ako}%gIf
\SetKwSwitch{Switch}{Case}{Other}{granaj}{\v{c}ini}{slu\v{c}aj}{ostali slu\v{c}ajevi}{kraj slu\v{c}aj}{kraj granaj}%Switch
\SetKwFor{For}{za}{\v{c}ini}{kraj za}%For
\SetKwFor{ForPar}{za}{\v{c}ini paralelno}{kraj za paralelno}%ForPar
\SetKwFor{ForEach}{za svaki}{\v{c}ini}{kraj za svaki}%ForEach
\SetKwFor{ForAll}{za sve}{\v{c}ini}{kraj za sve}%ForAll
\SetKwFor{While}{dok}{\v{c}ini}{kraj dok}%While
}{}%
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{turkish}}{%
%
\SetKwInput{KwIn}{Girdi}%
\SetKwInput{KwOut}{\c{C}{\i}kt{\i}}%
\SetKwInput{KwData}{Veri}%
\SetKwInput{KwResult}{Sonu\c{c}}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
%
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
}{}%
%
%
%%%% old commands compatibility
%
\ifthenelse{\boolean{algocf@oldcommands}}{%
\newcommand{\SetNoLine}{\SetAlgoNoLine}%
\newcommand{\SetNoline}{\SetAlgoNoLine}%
\newcommand{\SetVline}{\SetAlgoVlined}%
\newcommand{\SetLine}{\SetAlgoLined}%
%
\newcommand{\dontprintsemicolon}{\DontPrintSemicolon}%
\newcommand{\printsemicolon}{\PrintSemicolon}%
\newcommand{\incmargin}[1]{\IncMargin{#1}}%
\newcommand{\decmargin}[1]{\DecMargin{-#1}}%
\newcommand{\setnlskip}[1]{\SetNlSkip{#1}}%
\newcommand{\Setnlskip}[1]{\SetNlSkip{#1}}%
\newcommand{\setalcapskip}[1]{\SetAlCapSkip{#1}}%
\newcommand{\setalcaphskip}[1]{\SetAlCapHSkip{#1}}%
\newcommand{\nlSty}[1]{\NlSty{#1}}%
\newcommand{\Setnlsty}[3]{\SetNlSty{#1}{#2}{#3}}%
\newcommand{\linesnumbered}{\LinesNumbered}%
\newcommand{\linesnotnumbered}{\LinesNotNumbered}%
\newcommand{\linesnumberedhidden}{\LinesNumberedHidden}%
\newcommand{\showln}{\ShowLn}%
\newcommand{\showlnlabel}[1]{\ShowLnLabel{#1}}%
\newcommand{\nocaptionofalgo}{\NoCaptionOfAlgo}%
\newcommand{\restorecaptionofalgo}{\RestoreCaptionOfAlgo}%
\newcommand{\restylealgo}[1]{\RestyleAlgo{#1}}%
%
\newcommand{\Titleofalgo}[1]{\TitleOfAlgo{#1}}%
% \SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
\newcommand{\SetKwIf}[6]{\SetKwIF{#1}{#2#1}{#2}{#3}{#4}{#5 #1}{#5}{#6}}
%
\SetKwIF{gSi}{gSinonSi}{gSinon}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwIF{gIf}{gElsIf}{gElse}{if}{then}{else if}{else}{end if}%
\SetKwIF{gIf}{gElseIf}{gElse}{if}{then}{else if}{else}{end if}%
\SetKwIF{gWenn}{gSonstWenn}{gSonst}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwIF{gSe}{gSenaoSe}{gSenao}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwIF{gSea}{gAltSe}{gAltrimenti}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKw{Ret}{return}%
\SetKwInput{Data}{Data}%
\SetKwInput{Result}{Result}%
}{%
  \relax%
}%
%
%
%
%%
%%%
%%%% END

==> Technical Report- Scalable Active Information Acquisition - FinalSubmission/files/Intro.tex <==
%env monitoring: tokekar2013tracking
%SLAM: nerurkar2014c
%source seeking: ramirez2018distributed
%sensor placement: vitus2012efficient

The Active Information Acquisition (AIA) problem has recently received considerable attention due to its wide range of applications including target tracking \cite{huang2015bank}, environmental monitoring \cite{lu2018mobile}, active simultaneous localization and mapping (SLAM) \cite{carlone2014active}, active source seeking \cite{atanasov2015distributed}, and search and rescue missions \cite{kumar2004robot}. In each of these scenarios, robots are deployed to collect information about a physical phenomenon of interest; see e.g., Figure \ref{fig:experiment}. %For example, in environmental monitoring, the goal is build spatiotemporal models of pollution propagation, and in target tracking robots are tasked with estimating and tracking the positions of targets of interest. Near-optimal methods for sensor placement and scheduling have been proposed in \cite{krause2008optimizing}. However, approaches for optimizing the trajectories of mobile sensors are either greedy and rarely provide performance guarantees, or non-myopic and optimal but computationally expensive and, therefore, not applicable to large-scale estimation tasks.  

This paper addresses the problem of designing control policies for a team of mobile homogeneous sensors which minimize the accumulated uncertainty of a static landmarks located at uncertain positions over an \textit{a priori} unknown horizon while satisfying user-specified accuracy thresholds. First, we formulate this AIA problem as a centralized stochastic optimal control problem which generates an optimal terminal horizon and a sequence of optimal control policies given measurements to be collected in the future. Under Gaussian and linearity assumptions we can convert the problem into a deterministic optimal control problem, for which optimal control policies can be designed \textit{offline}. To design  sensor policies, we propose a novel algorithm that relies on decomposing the centralized deterministic optimal control problem into local ones via dynamically tessellating the environment into Voronoi cells assuming global information about the hidden state is available. The local subproblems are formulated and solved online and require the robots to switch between exploration and information gathering roles depending on their functionality in the environment. Specifically, a robot switches to an information gathering role if landmarks are estimated to be located inside its Voronoi cell. In this case, sensor-based control actions to localize the landmarks residing within its Voronoi cell are generated by applying our recently proposed sampling-based approach that simultaneously explores both the robot motion space and the information space reachable by the sensors \cite{kantaros2019asymptotically}. On the other hand, a robot adopts an exploration role if no landmarks are estimated to be within its Voronoi region. In this case, control actions are generated using existing area coverage or exploration methods that force the robots to spread in the environment and discover landmarks \cite{Cortes_TRA04, kantaros2015distributed,leung2006active,smith2018distributed,corah2019communication,wang2020autonomous}. As the robots navigate the workspace, they update their Voronoi cells and their roles accordingly. We show that this hybrid control approach results in distributing the burden of information gathering among the robots. Also, we show that the proposed algorithm is probabilistically complete under Gaussian and linearity assumptions. We provide extensive simulation results demonstrating that our algorithm can address large scale estimation tasks that involve hundreds of robots and hidden states with hundreds of dimensions. Finally, we show that the proposed algorithm can also design sensor policies when the linearity assumptions are relaxed.%
%by introducing bias into the sampling process, the proposed algorithm can quickly design paths that achieve desired levels of uncertainty in AIA tasks that involve large teams of robots, workspaces, and dimensions of the hidden state, which is impossible using relevant methods. %\NA{We should emphasize that even though the solution is constructed under linear Gaussian assumptions, it can be used to generate control policies for nonlinear motion and observation models}

 


\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/gazebo.png}
  \caption{Landmark localization scenario: 30 UAVs with limited field-of-view (colored disks) navigating an environment to localize 50 landmarks (red spheres) of interest. Red ellipses denote the uncertainty about the landmark positions; see \cite{sim_AIA}. }
  \label{fig:experiment}
\end{figure}

%\subsection{Related works}
%Our work lies in the larger field of active state estimation. For instance, in \cite{freundlich2018distributed} a distributed optimization algorithm is proposed to control a robotic sensor network to estimate a collection of \textit{static} hidden states so that desired accuracy thresholds and confidence levels are satisfied. A feedforward value iteration algorithm is proposed in \cite{le2009trajectory} that relies on exhaustively searching both the physical workspace and the information space to design optimal open-loop control policies. This work is extended in \cite{atanasov2014information} by pruning the exploration process  while providing suboptimality guarantees. Nevertheless, these approaches are computationally intractable as the planning horizon or the number of robots increases. Decentralized AIA methods, based on coordinate descent, are proposed in \cite{singh2009efficient,atanasov2015decentralized,schlotfeldt2018anytime} with suboptimality guarantees. Nonmyopic control policies for target tracking scenarios are also presented in \cite{charrow2014approximate} that rely on approximate representations of the target's future state. Nevertheless, this approach is specifically designed for tracking a single target using small teams of mobile robots.  Finally, greedy approaches are also proposed in \cite{graham2008cooperative,dames2012decentralized, meyer2015distributed}.
{\bf{Literature Review:}} Relevant approaches to accomplish AIA tasks are typically divided into greedy and nonmyopic. Greedy approaches rely on computing controllers that incur the maximum immediate decrease of an uncertainty measure as, e.g., in \cite{martinez2006optimal,graham2008cooperative,dames2012decentralized,charrow2014approximate,meyer2015distributed}, while they are often accompanied with suboptimality guarantees due to submodular functions that quantify the informativeness of paths \cite{corah2018distributed}. Although myopic approaches are usually preferred in practice due to their computational efficiency, they often get trapped in local optima.
%
To mitigate the latter issue, nonmyopic \textit{search-based} approaches have been proposed that sacrifice computational efficiency in order to design optimal paths. For instance, optimal controllers can be designed by exhaustively searching the physical and the information space \cite{le2009trajectory}. More computationally efficient but suboptimal controllers have also been proposed that rely on pruning the exploration process and on addressing the information gathering problem in a \textit{decentralized} way via coordinate descent \cite{singh2009efficient,atanasov2015decentralized,schlotfeldt2018anytime}. However, these approaches become computationally intractable as the planning horizon or the number of robots increases as decisions are made locally but \textit{sequentially} across the robots. 
%
Nonmyopic \textit{sampling-based} approaches have also been proposed due to their ability to find feasible solutions very fast, see e.g., \cite{levine2010information,hollinger2014sampling,khodayi2019distributed,lan2016rapidly}. Common in these works is that they are \textit{centralized} and, therefore, as the number of robots or the dimensions of the hidden states increase, the state-space that needs to be explored grows exponentially and, as result, sampling-based approaches also fail to compute sensor policies because of either excessive runtime or memory requirements. More scalable but centralized sampling-based approaches that can solve target tracking problems and logic-based AIA tasks involving tens of robots and long planning horizons have also been proposed recently in \cite{kantaros2019asymptotically,kantaros2020semantic}. Scalability comparisons among search-based and sampling-based methods can be found in \cite{kantaros2019asymptotically}. In his paper, we propose a new AIA algorithm that is highly scalable due to the fact that the global AIA task is decomposed into local ones while the robots make local decisions \textit{simultaneously} as they navigate the workspace assuming all-to-all communication for information exchange purposes is available. 

%Specifically, the information-rich RRT algorithm (iRRT), a variant of the RRT algorithm \cite{kuffner2000rrt}, is proposed in \cite{levine2010information} to maximize the accuracy of tracking a mobile target. Nevertheless, this approach is specifically designed for single target tracking problems. % A variant of RRT* \cite{karaman2011sampling} is also proposed in \cite{khodayi2018distributed} for state estimation tasks using teams of robots that communicate intermittently. Similarly, \cite{hollinger2014sampling} build upon the RRT* and RRG algorithms \cite{karaman2011sampling} to design paths that maximize the collected information while respecting budget/resource constraints.  Unlike our work, \cite{hollinger2014sampling} focus on estimating \textit{static} fields of interest. The RRC and $\text{RRC}^*$ algorithms are proposed in \cite{lan2016rapidly} to estimate spatiotemporal fields. Specifically, \cite{lan2016rapidly} approximate the solution of the information gathering problem with periodic trajectories that are constructed offline; however, suboptimality guarantees are not provided.  Common in the above works is that they lack the formal guarantees that our proposed algorithm is accompanied with. Moreover, as the number of robots or the dimension of the hidden states increases, the state-space that needs to be explored grows exponentially and, as result, these sampling-based approaches become computationally intractable. %In fact, \cite{hollinger2014sampling,lan2016rapidly,levine2010information} have only been applied to single-agent systems.
%In contrast to these works, our proposed framework is highly scalable and can efficiently address large-scale estimation tasks. %Moreover, unlike these sampling-based approaches, we provide formal guarantees for the completeness, optimality, and convergence rate of our proposed algorithm.
%



%Our work lies in the larger field of active state estimation. \BS{Cite back to Bajcsy Active Vision perhaps?} For instance, a feedforward value iteration algorithm is proposed in \cite{le2009trajectory} that relies on exhaustively searching both the physical workspace and the information space to design optimal open-loop control policies. This work is extended in \cite{atanasov2014information} by pruning the exploration process  while providing suboptimality guarantees. Nevertheless, these approaches are computationally intractable as the planning horizon or the number of robots increases. Decentralized AIA methods, based on coordinate descent, are proposed in \cite{singh2009efficient,atanasov2015decentralized,schlotfeldt2018anytime} with suboptimality guarantees. Greedy approaches are also proposed in \cite{graham2008cooperative,dames2012decentralized, meyer2015distributed}. Relevant methods are also presented in \cite{freundlich2018distributed,charrow2014approximate}.

%Common in \cite{hollinger2014sampling,lan2016rapidly,levine2010information} is that as the state-space that needs to be explored increases, e.g., as the number of robots or the dimension of the hidden state increases, they cannot design informative paths


%\cite{binney2012branch}
   
%\subsection{Summary of Contributions}
The {\bf{contribution}}  of this paper can be summarized as follows. \textit{First}, we propose a new highly scalable and nonmyopic method that can quickly design control policies achieving desired levels of uncertainty in AIA tasks that involve sensor teams with hundreds of robots and hidden state with hundreds of dimensions. \textit{Second}, we show that the proposed algorithm is probabilistically complete under linearity and Gaussian assumptions. %We emphasize that this is the first AIA sampling-based algorithm supported by these theoretical guarantees. 
\textit{Third}, we provide extensive simulation results that show that the proposed method can efficiently handle large-scale estimation tasks. %which is impossible using existing centralized methods. %Moreover, our comparative simulation results revealed an important drawback of existing sampling-based approaches: exploration of large state-spaces is computationally intractable, unless the sampling operation is biased towards informative sub-spaces.


%To the best of our knowledge, this is the first highly scalable sampling-based approach for information-gathering tasks in complex environments with formal guarantees. Specifically, unlike relevant sampling-based AIA methods, the proposed algorithm is probabilistically complete, asymptotically optimal, and converges exponentially fast to the optimal solution. Moreover, we would like to highlight that this is the first time that such convergence guarantees are provided for sampling-based planning methods; see e.g., \cite{hollinger2014sampling,lan2016rapidly,levine2010information} or even sampling-based approaches for traditional point-to-point navigation \cite{karaman2011sampling}. Finally, we present extensive simulation results that show that by biasing the sampling process, the proposed framework can address large-scale estimation tasks which is not possible using available methods \red{[??]}. 

%The rest of the paper is organized as follows. In Section \ref{sec:PF}, we  formulate the multi-robot active information acquisition problem. The proposed sampling-based algorithm is presented in Section \ref{sec:samplingAlg}. Theoretical guarantees are presented in Section \ref{sec:complOpt} while simulation studies are provided in Section \ref{sec:Sim}.


==> Technical Report- Scalable Active Information Acquisition - FinalSubmission/files/PF.tex <==

% ------------------------------------------------------------------------------- %
\subsection{Robot Motion Model}
Consider $N$ mobile robots that reside in a complex environment $\Omega\subset \reals^d$ with obstacles of arbitrary shape located at $O\subset\Omega$, where $d$ is the dimension of the workspace. The dynamics of the robots are described by $\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t))$,
%
%\begin{equation}\label{eq:rdynamics}
%\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t)),
%\end{equation}
for all $j\in\ccalN:=\{1,\dots,N\}$, where $\bbp_{j}(t) \in \Omega_{\text{free}}:=\Omega \backslash O$ stands for the state of robot $j$ in the obstacle-free space $\Omega_{\text{free}}$, $\bbu_{j}(t) \in\ccalU_j$ stands for a control input in a \textit{finite} space of admissible controls $\ccalU_j$. % is a \textit{finite} space of admissible controllers.
Note that the state $\bbp_{j}$ may belong to a higher dimensional space than $\Omega_{\text{free}}$\BS{Can we make this into a  remark or just remove it? It's extra clutter for something that is fairly straightforward}. For example, this is the case if $\bbp_j(t)$ includes the position and the orientation of robot $j$. Nevertheless, throughout the rest of the paper, for simplicity of notations we denote $\bbp_{j}(t) \in \Omega_{\text{free}}$. Also, note that the considered dynamics can range from simple graph-based dynamics \cite{yaziciouglu2017communication} to arbitrary nonlinear discrete dynamics \cite{fu2016optimal}. Hereafter, for simplicity of notation, we compactly denote the dynamics of all robots as $\bbp(t+1)=\bbf(\bbp(t),\bbu(t))$,
%\begin{equation}\label{eq:rdynamics}
%\bbp(t+1)=\bbf(\bbp(t),\bbu(t)),
%\end{equation}
where $\bbp(t)\in \Omega_{\text{free}}^N$, for all $t\geq 0$, and $\bbu(t)\in\ccalU:=\ccalU_1\times\dots\times\ccalU_N$.
\subsection{Estimation Task}
The task of the robots is to collaboratively estimate a \textit{hidden state} governed by the following dynamics:

\begin{equation} \label{eq:nonlinDynamics}
\bbx(t+1) =\bbg(\bbx(t),\bbw(t)),
\end{equation}
where $\bbx(t)\in\mathbb{R}^{n}$ and $\bbw(t) \in\reals^{d_w}$ denote the hidden state and the process noise at discrete time $t$, respectively. We assume that the process noise $\bbw(t)$ is normally distributed as $\bbw(t) \sim \ccalN(\bb0, \bbQ(t) )$, where $\bbQ(t)$ is the covariance matrix at time $t$. For instance, \eqref{eq:nonlinDynamics} can model static or mobile targets \cite{atanasov2014information}, spatio-temporal fields \cite{lan2016rapidly} or static fields  \cite{bennetts2013towards}.

Moreover, the robots are equipped with sensors to collect measurements associated with $\bbx(t)$ as per the \textit{observation model}: $\bby_j(t)= \bbm_j(\bbp_j(t),\bbx(t),\bbv(t))$, where $\bby_j(t)$ is the measurement signal at discrete time $t$ taken by  robot $j\in\ccalN$. Also, $\bbv_j(t) \sim \ccalN(\bb0, \bbR_j(t) )$ is sensor-state-dependent Gaussian noise with covariance $\bbR_j(t)$. 
 For instance, the observation model $\bbm_j$ can model cameras or RF-based sensors, while $\bby_j(t)$ can consist of range and/or bearing measurements. Hereafter, we compactly denote the observation models of all robots as 
 \begin{equation} \label{eq:NonLinMeasModel}
\bby(t)= \bbm(\bbp(t),\bbx(t),\bbv(t)),~\bbv(t) \sim \ccalN(\bb0, \bbR(t) ).
\end{equation}

The quality of measurements taken by all robots up to a time instant $t$, collected in a vector denoted by $\bby_{0:t}$, can be evaluated using information measures, such as the mutual information between  $\bby_{0:t}$ and $\bbx(t)$ or the conditional entropy of $\bbx(t)$ given $\bby_{0:t}$. Assuming a Gaussian distribution for $\bbx(t)$, i.e., $\bbx(t)\sim\ccalN(\boldsymbol\mu(t),\Sigma(t|\bby_{0:t}))$, alternative uncertainty measures can also be used such as the trace, determinant, or maximum eigenvalue of the covariance matrix $\Sigma(t|\bby_{0:t})$. 

\subsection{Active Information Acquisition}
Given the initial robot configuration $\bbp(0)$ and the hidden state $\bbx(t)$ that evolves as per \eqref{eq:nonlinDynamics}, our goal is to select a \textit{finite} horizon $F\geq 0$ and compute control inputs $\bbu(t)$, for all time instants $t\in\{0,\dots,F\}$, that solve the following stochastic optimal control problem
%
%$$ \abs{\bbx_t - \bar{\bbx}_{ij,t}} \to 0 \text{ as } t \to \infty , \ \forall \bbq \in \Omega, \forall r_{ij}. $$
%
\begin{subequations}
\label{eq:Prob}
\begin{align}
& \min_{\substack{ F, \bbu_{0:F}}} \left[J(F,\bbu_{0:F},\bby_{0:F}) = \sum_{t=0}^{F}   \det\Sigma(t|\bby_{0:t}) \right]  \label{obj1}\\
%&\ \ \st \ \ \ \ \ \ \ \ \ \ \ \ \bbp(F) \in \ccalP_{\text{goal}}, \label{constr1}\\
&\ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \textcolor{red}{\det\Sigma(F|\bby_{0:F})\leq \delta}, \label{constr2} \\
%&\ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \  F\leq \bar{F},\nonumber\\
& \ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \bbp(t) \in \Omega_{\text{free}}^N,  \label{constr3} \\
&\ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \bbp(t+1) = \bbf(\bbp(t),\bbu(t)), \label{constr4} \\
&\ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \bby(t) = \bbm(\bbp(t),\bbx(t),\bbv(t)), \label{constr5}
\end{align}
\end{subequations}
where the constraints hold for all time instants $t\in\{0,\dots,F\}$.
In \eqref{obj1}, with slight abuse of notation, $\bbu_{0:F}$ stands for the sequence of control inputs applied from $t=0$ until $t=F$.
%
% \{\{\bbu_j(t)\}_{j=1}^{N}
%%\Sigma_i(t)
Also, assuming a Gaussian distribution for $\bbx(t)$, $\det\Sigma(t|\bby_{0:t})$ denotes the determinant of the covariance matrix of $\bbx(t)$ given the set of measurements $\bby_{0:t}$. In words, the objective function \eqref{obj1} captures the cumulative uncertainty in the estimation of $\bbx(t)$ after fusing information collected by all robots from $t=0$ up to time $F$. 
%Moreover, the first constraint \eqref{constr1} requires that at time $F$ the configuration of the robots is within $\ccalP_{\text{goal}}\subseteq \Omega_{\text{free}}^N$; see also Remark \ref{rem1}. 
The first constraint \eqref{constr2} requires that the terminal uncertainty of $\bbx(F)$ to be below a user-specified threshold $\delta$; see also Remark \ref{rem1}.
%$h(\bbx(F)|\ccalY_{0:F})$ denotes the terminal entropy of the hidden state $\bbx(F)$ given $\ccalY_{0:F}$. In words, this constraint requires that the terminal uncertainty of $\bbx(F)$ to be below a user-specified threshold $\delta$; see also Remark \ref{rem1}. %Essentially, the thresholds $\delta_i$ allow for user-specified priorities assigned to the targets in their importance.
%Also, in \eqref{eq:Prob}, $G(\bbx_i(t)|\ccalY_{0:t})$ denotes a user-specified uncertainty metric of the hidden state $\bbx_i(t)$ given the measurements, collected in the set $\ccalY_{0:t}$, taken by all robots up to time $t$. In words, the objective function $J(F,\bbu_{0:F},\ccalY_{0:F})$ in \eqref{eq:Prob} captures the cumulative uncertainty in the estimation of all states $\bbx_i(t)$ after fusing information collected by all robots from $t=0$ up to time $F$. Moreover, the first constraint requires that all robots $j$ at time $F$ are within a region $\ccalP_j^{\text{goal}}\subseteq \Omega$ while the second constraint requires that the entropy (uncertainty) $h_i(\bbx_i(F)|\ccalY_{0:F})$ of the state $\bbx_i(F)$ at time instant $F$ should be below a user-specified threshold $\delta_i$. Essentially, the thresholds $\delta_i$ allow the user to specify which hidden states are more important than others.
%
%Note that in the second constraint any other uncertainty metric can also be used in place of the entropy, without any restrictions, such as mutual information or other scalar functions of the covariance matrix and Fisher Information Matrix (FIM). 
%In other words, the first two constraints require that the robots should sufficiently explore the workspace before reaching the goal regions $\ccalP_j^{\text{goal}}$. 
%The third constraint requires that the terminal horizon $F$ should be below a user-specified parameter $\bar{F}>0$.\footnote{In general, the purpose of the third constraint is to ensure that the terminal horizon $F$ is always finite. In practice, we select $\bar{F}$ to be arbitrarily large, but finite, so that the robots have sufficiently enough time to estimate the hidden states.}
%
The second constraint \eqref{constr3} requires that the robots should never collide with obstacles. The last two constraints capture the robot dynamics \eqref{eq:nonlinDynamics} and the observation model \eqref{eq:NonLinMeasModel}.
%\red{DELETE the third constraint. Just say that you assume that the problem is well-defined/feasible, i.e., the optimal solution has a finite path. This is also the case in a shortest path problem. Feasible solution: travel forever and reach the goal after asn inf number of steps. Pick deltai so that this is true...If obj negative then optimal solution is travel forever.}
%in rrt F is finite because you are searching an bounded domain. here you are searching an infinite domain (workspace x information)

\begin{rem}[Optimal Control Problem \eqref{eq:Prob}]\label{rem1}
In \eqref{eq:Prob}, any other optimality metric, not necessarily information-based, can be used in place of \eqref{obj1} as long as it is always positive. If non-positive metrics are selected, e.g., the entropy of $\bbx(t)$, then \eqref{eq:Prob} is not well-defined, since the  optimal terminal horizon $F$ is infinite. On the other hand, in the first constraint \eqref{constr2}, any uncertainty metric can be used without any restrictions. Moreover, note that without the terminal constraint \eqref{constr2}, the optimal solution of \eqref{eq:Prob} is  all robots to stay put, i.e., $ F=0$. 
Additional terminal constraints can be added to \eqref{eq:Prob}, such as, $\bbp(F)\in\ccalP_{\text{goal}}\subseteq\Omega_{\text{free}}^N$, to model joint task planning and estimation scenarios, where, e.g., the robots should eventually visit a user to report an estimate of the hidden state with user-specified accuracy determined by $\delta$.
\end{rem}

%Hereafter, we assume a Gaussian prior distribution for the hidden states $\bbx_i(0)$ is given, i.e., $\bbx_i(0)\sim\ccalN(\hat{\bbx}_i(0),\Sigma_i(0))$. Moreover, we require that the uncertainty metric $G(\bbx_i(t)|\ccalY_{0:t})$ is positive, i.e., $G(\bbx_i(t)|\ccalY_{0:t})\geq 0$, for all $t\geq 0$. For instance, valid selections for $G(\bbx_i(t)|\ccalY_{0:t})$ can be  the determinant, or the trace, or the minimum eigenvalue of the covariance matrix or the FIM. As it will be shown in  Section \ref{sec:convergence}, the positiveness of $G(\bbx_i(t)|\ccalY_{0:t})$ ensures that the optimal horizon $F$ in \eqref{eq:Prob} is finite. 
%where $\Sigma_i(t|\ccalY_{1:t}$ is the covariance matrix of the hidden state $\bbx_i$ at the time instant $t$ given the past measurements $\ccalY_{1:t}$. 

 %This also implies that $J(t,\bbu_{0:t})\geq 0$, for all $t\geq 0$ and, therefore, $J(t,\bbu_{0:t})$ is monotone. To see this, observe that $J(t+1,\bbu_{0:t+1},\ccalY_{0:t+1})= J(t,\bbu_{0:t}, \ccalY_{0:t})+\sum_{i=1}^{M} G(\bbx_i(t+1)|\ccalY_{0:t+1})\geq J(t,\bbu_{0:t},\ccalY_{0:t})\geq 0$, since $\sum_{i=1}^{M} G(\bbx_i(t+1)|\ccalY_{0:t+1})\geq 0$, for all $t\geq 0$. The latter result guarantees that the optimal horizon $t_f$ is finite, since increasing the horizon $t_f$ can only increase the cost  $J(t_f,\bbu_{0:t_f},\ccalY_{0:t_f})$. 
%Note that other positive  uncertainty metrics can be employed

\subsection{Problem Reformulation: A Separation Principle}\label{sec:reform}

The Active Information Acquisition problem in \eqref{eq:Prob} is a stochastic optimal control problem for which, in general, closed-loop control policies are preferred. Nevertheless, assuming linear dynamics for the hidden state in \eqref{eq:nonlinDynamics} and linear observation models in \eqref{eq:NonLinMeasModel}, i.e., 

\begin{equation} \label{eq:dynamics}
\bbx(t+1) =\bbA\bbx(t)  + \bbB\bbd(t) + \bbw(t),
\end{equation}
where $\bbd(t)$ is a control input, and 
\begin{equation} \label{eq:measModel}
\bby(t) = \bbH(\bbx(t))\bbx(t) + \bbv(\bbx(t)),%\bbh(\bbx(t), \bbq, \bbv(t)),
\end{equation}
the stochastic optimal control problem \eqref{eq:Prob} reduces to the following deterministic optimal control problem; see also \cite{atanasov2014information}.

%Deterministic optimal control problem:
\begin{subequations}
\label{eq:Prob2}
\begin{align}
& \min_{\substack{ F, \bbu_{0:F}}} \left[J(F,\bbu_{0:F}) = \sum_{t=0}^{F}  \det\Sigma(t) \right] \label{obj2}\\
%&\ \ \st \ \ \ \ \ \ \ \ \ \ \ \ \bbp(F) \in \ccalP_{\text{goal}}, \label{constr21}\\
& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \det\Sigma(F)\leq \delta,  \label{constr22} \\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \bbp(t) \in \Omega_{\text{free}}^N, \label{constr23} \\
& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \bbp(t+1) = \bbf(\bbp(t),\bbu(t)), \label{constr24}\\
& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \Sigma(t+1) =\rho(\Sigma(t)), \label{constr25}
\end{align}
\end{subequations}
where $\rho(\cdot)$ stands for the Kalman Filter Ricatti map. Note also open loop (offline) policies are optimal solutions to \eqref{eq:Prob2}. Then, the problem that we address in this paper can be summarized as follows%; \red{see also Figure ??}.
%
\begin{problem} \label{prob}(Active Information Acquisition)
Given an initial robot configuration $\bbp(0)$ and a hidden state $\bbx(t)$ that evolves as per \eqref{eq:dynamics}, select a horizon $F$ and compute control inputs $\bbu(t)$ for all time instants $t\in\{0,\dots,F\}$ as per the optimal control problem \eqref{eq:Prob2}.
%
\end{problem}

Finally, throughout the paper we make the following assumption.% and the underlying communication network between the robots.
\begin{assumption} \label{as:assumption}%[State Model]
The dynamics of the state \eqref{eq:dynamics}, the observation model \eqref{eq:measModel}, and process and measurement noise covariances $\bbQ(t)$ and $\bbR(t)$ are known. %Furthermore, the state dynamics \eqref{eq:dynamics} and sensing model \eqref{eq:measModel} are differentiable functions. 
%Finally, we assume that all robots can communicate with each other at any time $t$. 
\end{assumption}

\begin{rem}[Nonlinear \& Noisy Models]
%Note that we assume that the dynamics \eqref{eq:dynamics} and the sensing model \eqref{eq:measModel} are modeled as linear systems. Also, in \eqref{eq:rdynamics} we assume noiseless robot dynamics. As discussed before, 
Note that Assumption \ref{as:assumption} allows for offline computation of optimal policies.  Nevertheless, in Section \ref{sec:Sim}, we show that this assumption can be relaxed; in this case suboptimal controllers are synthesized. \red{[refine remark once simulations are added and problem formulation is finished]}
\end{rem}



==> Technical Report- Scalable Active Information Acquisition - FinalSubmission/files/PF_short.tex <==

% ------------------------------------------------------------------------------- %
%\subsection{Robot Motion Model}
Consider $N$ mobile robots that reside in an environment $\Omega\subset \reals^d$ with obstacles of arbitrary shape located at $O\subset\Omega$, where $d$ is the dimension of the workspace. The dynamics of the $N$ robots are described by %$\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t))$, %$\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t))$,
%
\begin{equation}\label{eq:rdynamics}
\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t)),
\end{equation}
for all $j\in\ccalN:=\{1,\dots,N\}$, where $\bbp_{j}(t) \in \Omega_{\text{free}}:=\Omega \backslash O$ stands for the state (e.g., position and orientation) of robot $j$ in the obstacle-free space $\Omega_{\text{free}}$ at discrete time $t$, $\bbu_{j}(t) \in\ccalU_j$ stands for a control input in a \textit{finite} space of admissible controls $\ccalU_j$. %\NA{state that time is discrete}
%Note that the state $\bbp_{j}$ may belong to a higher dimensional space than $\Omega_{\text{free}}$. For example, this is the case if $\bbp_j(t)$ includes the position and the orientation of robot $j$. Nevertheless, throughout the rest of the paper, for simplicity of notations we denote $\bbp_{j}(t) \in \Omega_{\text{free}}$.\BS{Can we make this into a  remark or just remove it? It's extra clutter for something that is fairly straightforward.} 
%Also, note that the considered dynamics can range from simple graph-based dynamics to arbitrary nonlinear discrete dynamics\NA{This sentence could be removed}. 
Hereafter, we compactly denote the dynamics of all robots as %$\bbp(t+1)=\bbf(\bbp(t),\bbu(t)),$
\begin{equation}\label{eq:rdynamicsC}
\bbp(t+1)=\bbf(\bbp(t),\bbu(t)),
\end{equation}
where $\bbp(t)\in \Omega_{\text{free}}^N$, $\forall t\geq 0$, and $\bbu(t)\in\ccalU:=\ccalU_1\times\dots\times\ccalU_N$.

%\subsection{Estimation Task}
%The task of the robots is to collaboratively estimate a static \textit{hidden state} $\bbx$

The environment is occupied by $M>0$ \textit{static} landmarks located at uncertain positions $\bbx_i$, $i\in\ccalM:=\{1,\dots,M\}$. In particular, the robots are not aware of the true landmark positions but they have access to probability distributions over their positions. Such distributions can be user-specified or produced by Simultaneous Localization and Mapping (SLAM) methods \cite{rosinol2019kimera,bowman2017probabilistic}. Specifically, we assume that the position of landmark $i$ follows an initially known Gaussian distribution $\ccalN(\hat{\bbx}_i(0),\Sigma_i(0))$, where $\hat{\bbx}_i(0)$ and $\Sigma_i(0)$ denote the expected position and the covariance matrix at time $t=0$, respectively. Hereafter, we compactly denote the hidden state by $\bbx$, i.e., $\bbx=[\bbx_1^T,\dots,\bbx_M^T]$. Similarly, we denote by %which at any time $t\geq0$ follows a normal distribution $\ccalN(\hat{\bbx}(t),\Sigma(t))$, where 
$\hat{\bbx}(0)$ the vector that stacks the expected positions $\hat{\bbx}_i(0)$ of all landmarks and $\Sigma(0)$ the block diagonal covariance matrix where the diagonal elements are the individual matrices $\Sigma_i(0)$.
%
%governed by the following dynamics:
%\begin{equation} \label{eq:dynamics}
%\bbx(t+1) =\bbA\bbx(t) + \bbw(t),
%\end{equation}
%%\BS{As discussed with Nikolay, perhaps we should consider removing d(t) here? It just raises the question of how we know the control inputs for this system.}
%where $\bbx(t)\in\mathbb{R}^{n}$ and $\bbw(t) \in\reals^{d_w}$ denote the hidden state and the process noise at discrete time $t$, respectively. We assume that the process noise $\bbw(t)$ is normally distributed as $\bbw(t) \sim \ccalN(\bbd(t), \bbQ(t) )$, where $\bbQ(t)$ is the covariance matrix at time $t$. For instance, $\bbx(t)$ can model the position of static or mobile targets \cite{atanasov2014information}, the state of spatio-temporal fields \cite{lan2016rapidly} or gas concentration  \cite{bennetts2013towards}.

%The task of the robots is to collaboratively achieve desired levels of uncertainty about the hidden states. Assuming that the landmark positions follow Gaussian distribution, we measure the uncertainty about landmark $i$, we measure uncertainty about landmark $i$ using the determinant of its corresponding covariance matrix denoted by $\det(\Sigm)$
The robots are equipped with sensors to collect measurements associated with the hidden states as per the following stochastic linear \textit{observation model} %$\bby_j(t) = \bbM(\bbp_j(t))\bbx + \bbv(t),$ 
\begin{equation} \label{eq:measModel}
\bby_j(t) = \bbM(\bbp_j(t))\bbx + \bbv(t),
\end{equation}
where $\bby_j(t)$ is the measurement signal at discrete time $t$ taken by robot $j\in\ccalN$ associated with the landmark positions $\bbx$. Also, $\bbv(t) \sim \ccalN(\bb0, \bbR(t) )$ is sensor-state-dependent Gaussian noise with covariance $\bbR(t)$. Note that we assume that the robots are homogeneous in terms of their sensing capabilities.\footnote{This assumption is used in Section \ref{sec:complOpt} to ensure that the proposed decomposition-based approach is complete.} For simplicity of notation, hereafter, we compactly denote the observation models of all robots as  
\begin{equation}
    \bby(t)= \bar{\bbM}(\bbp(t))\bbx + \bar{\bbv}(t),~\bar{\bbv}(t) \sim \ccalN(\bb0, \bar{\bbR}(t)).
\end{equation}
%Linear observation models have been used, e.g., in \cite{bennetts2013towards} to estimate a gas concentration field.
Hereafter, we assume the robots can exchange their collected measurements via an all-to-all communication network allowing them to always maintain a common/global estimate of the hidden state. 
 %\begin{equation} \label{eq:measModelC}
%\bby(t)= \bbM(\bbp(t))\bbx + \bbv(t),~\bbv(t) \sim \ccalN(\bb0, \bbR(t) ).
%\end{equation}
%\BS{What about the linearity requirements in the measurement model? That doesn't seem to be captured now since m(x(t)) is a function of x?}
The quality of measurements taken by all robots up to a time instant $t$, collected in a vector denoted by $\bby_{0:t}$, can be evaluated using information measures, such as the mutual information between $\bby_{0:t}$ and $\bbx$, the conditional entropy of $\bbx$ given $\bby_{0:t}$, or the determinant of the a-posteriori covariance matrix, denoted by $\Sigma(t|\bby_{0:t})$. Note that the a-posteriori mean, denoted by $\hat{\bbx}(t|\bby_{0:t})$. and a-posteriori covariance matrix $\Sigma(t|\bby_{0:t})$ can be computed using probabilistic inference methods, e.g., Kalman filter. %\NA{This notation for $\Sigma(t|\bby_{0:t}))$ is not standard and should be explained. The mean $\mu$ also depends on the measurements but it is not conditioned  on them. We should also emphasize somewhere that $M$ depends on $p(t)$.} \BS{This paragraph is slightly misleading. We mention that we can evaluate uncertainty with mutual information or conditional entropy, and go on to list others, but the problem formulation is only valid for positive functions for which mutual information and entropy are not. One thing that might help is putting Remark 2.1 as a footnote with a symbol in this sentence to immediately refer the reader to this fact.}

%\subsection{Active Information Acquisition}
Given the initial robot configuration $\bbp(0)$ and the Gaussian distributions $\ccalN(\bbx_i(0),\Sigma_i(0))$ for the hidden states, our goal is to select a \textit{finite} horizon $F\geq 0$ and compute control inputs $\bbu(t)$, for all time instants $t\in\{0,\dots,F\}$, that solve the following stochastic optimal control problem: %\NA{It is not clear how $\Sigma(t|\bby_{0:t})$ is obtained below and why the target motion model does not appear as a constraint}
%
%$$ \abs{\bbx_t - \bar{\bbx}_{ij,t}} \to 0 \text{ as } t \to \infty , \ \forall \bbq \in \Omega, \forall r_{ij}. $$
%
\begin{subequations}
\label{eq:Prob}
\begin{align}
& \min_{\substack{ F, \bbu_{0:F}}} \left[J(F,\bbu_{0:F},\bby_{0:F}) = \sum_{t=0}^{F}   \det\Sigma(t|\bby_{0:t}) \right]  \label{obj1}\\
%&\ \ \st \ \ \ \ \ \ \ \ \ \ \ \ \bbp(F) \in \ccalP_{\text{goal}}, \label{constr1}\\
&\ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \det\Sigma(F|\bby_{0:F})\leq \delta, \label{constr2} \\
%&\ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \  F\leq \bar{F},\nonumber\\
& \ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \bbp(t) \in \Omega_{\text{free}}^N,  \label{constr3} \\
&\ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \bbp(t+1) = \bbf(\bbp(t),\bbu(t)), \label{constr4} \\
%&\ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \bbx(t+1) =\bbA\bbx(t) + \bbw(t), \label{constrTrgt}\\%\bbx(t+1) =g(\bbx(t), \bbw(t)), \label{constrTrgt}\\
&\ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \bby(t) =\bar{\bbM}(\bbp(t))\bbx + \bar{\bbv}(t), \label{constr5}
\end{align}
\end{subequations}
where the constraints hold for all time instants $t\in\{0,\dots,F\}$.
In \eqref{obj1}, $\bbu_{0:F}$ stands for the sequence of control inputs applied from $t=0$ until $t=F$.
%\begin{subequations}
%\label{eq:Prob}
%\begin{align}
%& \min_{\substack{ F, \bbu_{0:F}}} \left[J(F,\bbu_{0:F},\bby_{0:F}) = \sum_{t=0}^{F}   %\det\Sigma(t|\bby_{0:t}) \right]  \label{obj1}\\
%%&\ \ \st \ \ \ \ \ \ \ \ \ \ \ \ \bbp(F) \in \ccalP_{\text{goal}}, \label{constr1}\\
%&\ \ \ \ \ \ \ \ \ \det\Sigma(F|\bby_{0:F})\leq \delta, \label{constr2} \\
%%&\ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \  F\leq \bar{F},\nonumber\\
%& \ \ \ \ \ \ \ \ \ \bbp(t) \in \Omega_{\text{free}}^N,  \label{constr3} \\
%&\ \ \ \ \ \ \ \ \ \ \bbp(t+1) = \bbf(\bbp(t),\bbu(t)), \label{constr4} \\
%&\ \ \ \ \ \ \ \ \ \  \bbx(t+1) =g(\bbx(t), \bbw(t)), \label{constrTrgt}\\
%&\ \ \ \ \ \ \ \ \ \ \bby(t) =\bbM(\bbp(t))\bbx(t) + \bbv(t), \label{constr5}
%\end{align}
%\end{subequations}
%
% \{\{\bbu_j(t)\}_{j=1}^{N}
%%\Sigma_i(t)
In words, the objective function \eqref{obj1} captures the cumulative uncertainty in the estimation of $\bbx$ after fusing information collected by all robots from $t=0$ up to time $F$. 
%Moreover, the first constraint \eqref{constr1} requires that at time $F$ the configuration of the robots is within $\ccalP_{\text{goal}}\subseteq \Omega_{\text{free}}^N$; see also Remark \ref{rem1}. 
The first constraint \eqref{constr2} requires the terminal uncertainty of $\bbx$ to be below a user-specified threshold $\delta$. %\NA{The entropy $H(\bbx(F)|\bby_{0:F})$ is proportional to $\log\det\Sigma(F|\bby_{0:F})$. Why not make this explicit and simplfiy (4b) by just having a constraint on $\det\Sigma(F|\bby_{0:F})$?}.
%$h(\bbx(F)|\ccalY_{0:F})$ denotes the terminal entropy of the hidden state $\bbx(F)$ given $\ccalY_{0:F}$. In words, this constraint requires that the terminal uncertainty of $\bbx(F)$ to be below a user-specified threshold $\delta$; see also Remark \ref{rem1}. %Essentially, the thresholds $\delta_i$ allow for user-specified priorities assigned to the targets in their importance.
%Also, in \eqref{eq:Prob}, $G(\bbx_i(t)|\ccalY_{0:t})$ denotes a user-specified uncertainty metric of the hidden state $\bbx_i(t)$ given the measurements, collected in the set $\ccalY_{0:t}$, taken by all robots up to time $t$. In words, the objective function $J(F,\bbu_{0:F},\ccalY_{0:F})$ in \eqref{eq:Prob} captures the cumulative uncertainty in the estimation of all states $\bbx_i(t)$ after fusing information collected by all robots from $t=0$ up to time $F$. Moreover, the first constraint requires that all robots $j$ at time $F$ are within a region $\ccalP_j^{\text{goal}}\subseteq \Omega$ while the second constraint requires that the entropy (uncertainty) $h_i(\bbx_i(F)|\ccalY_{0:F})$ of the state $\bbx_i(F)$ at time instant $F$ should be below a user-specified threshold $\delta_i$. Essentially, the thresholds $\delta_i$ allow the user to specify which hidden states are more important than others.
%
%Note that in the second constraint any other uncertainty metric can also be used in place of the entropy, without any restrictions, such as mutual information or other scalar functions of the covariance matrix and Fisher Information Matrix (FIM). 
%In other words, the first two constraints require that the robots should sufficiently explore the workspace before reaching the goal regions $\ccalP_j^{\text{goal}}$. 
%The third constraint requires that the terminal horizon $F$ should be below a user-specified parameter $\bar{F}>0$.\footnote{In general, the purpose of the third constraint is to ensure that the terminal horizon $F$ is always finite. In practice, we select $\bar{F}$ to be arbitrarily large, but finite, so that the robots have sufficiently enough time to estimate the hidden states.}
%
The second constraint \eqref{constr3} requires that the robots should never collide with obstacles. The last two constraints capture the robot dynamics and the sensor model.
%\red{DELETE the third constraint. Just say that you assume that the problem is well-defined/feasible, i.e., the optimal solution has a finite path. This is also the case in a shortest path problem. Feasible solution: travel forever and reach the goal after asn inf number of steps. Pick deltai so that this is true...If obj negative then optimal solution is travel forever.}
%in rrt F is finite because you are searching an bounded domain. here you are searching an infinite domain (workspace x information)

%Hereafter, we assume a Gaussian prior distribution for the hidden states $\bbx_i(0)$ is given, i.e., $\bbx_i(0)\sim\ccalN(\hat{\bbx}_i(0),\Sigma_i(0))$. Moreover, we require that the uncertainty metric $G(\bbx_i(t)|\ccalY_{0:t})$ is positive, i.e., $G(\bbx_i(t)|\ccalY_{0:t})\geq 0$, for all $t\geq 0$. For instance, valid selections for $G(\bbx_i(t)|\ccalY_{0:t})$ can be  the determinant, or the trace, or the minimum eigenvalue of the covariance matrix or the FIM. As it will be shown in  Section \ref{sec:convergence}, the positiveness of $G(\bbx_i(t)|\ccalY_{0:t})$ ensures that the optimal horizon $F$ in \eqref{eq:Prob} is finite. 
%where $\Sigma_i(t|\ccalY_{1:t}$ is the covariance matrix of the hidden state $\bbx_i$ at the time instant $t$ given the past measurements $\ccalY_{1:t}$. 

 %This also implies that $J(t,\bbu_{0:t})\geq 0$, for all $t\geq 0$ and, therefore, $J(t,\bbu_{0:t})$ is monotone. To see this, observe that $J(t+1,\bbu_{0:t+1},\ccalY_{0:t+1})= J(t,\bbu_{0:t}, \ccalY_{0:t})+\sum_{i=1}^{M} G(\bbx_i(t+1)|\ccalY_{0:t+1})\geq J(t,\bbu_{0:t},\ccalY_{0:t})\geq 0$, since $\sum_{i=1}^{M} G(\bbx_i(t+1)|\ccalY_{0:t+1})\geq 0$, for all $t\geq 0$. The latter result guarantees that the optimal horizon $t_f$ is finite, since increasing the horizon $t_f$ can only increase the cost  $J(t_f,\bbu_{0:t_f},\ccalY_{0:t_f})$. 
%Note that other positive  uncertainty metrics can be employed

%\subsection{Problem Reformulation: A Separation Principle}\label{sec:reform}
The Active Information Acquisition (AIA) problem in \eqref{eq:Prob} is a stochastic optimal control problem for which, in general, closed-loop control policies are optimal. Nevertheless, given  the linear observation models, we can apply the separation principle presented in \cite{atanasov2014information} to convert 
\eqref{eq:Prob} to the following deterministic optimal control problem. %\NA{Why is the conditioning on $y_{0:t}$ removed below?}
%Deterministic optimal control problem:
\begin{subequations}
\label{eq:Prob2}
\begin{align}
& \min_{\substack{ F, \bbu_{0:F}}} \left[J(F,\bbu_{0:F}) = \sum_{t=0}^{F}  \det\Sigma(t) \right] \label{obj2}\\
%&\ \ \st \ \ \ \ \ \ \ \ \ \ \ \ \bbp(F) \in \ccalP_{\text{goal}}, \label{constr21}\\
& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \det\Sigma(F)\leq \delta,  \label{constr22} \\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \bbp(t) \in \Omega_{\text{free}}^N, \label{constr23} \\
& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \bbp(t+1) = \bbf(\bbp(t),\bbu(t)), \label{constr24}\\
& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \Sigma(t+1) =\rho(\bbp(t+1),\Sigma(t)), \label{constr25}
\end{align}
\end{subequations}%\BS{Can we use the Problem script here? And not put equation numbers on each line? Rather the whole thing should read Problem 2:}
where $\rho(\cdot)$ stands for the Kalman Filter Ricatti map. Note that open loop (offline) policies are optimal solutions to \eqref{eq:Prob2}. The problem addressed in this paper can be summarized as follows.%\NA{Since entropy is proportional to $\log\det\Sigma(F|\bby_{0:F})$ and since the cost function is positive-additive, the optimal planning horizon is the first hitting time of the condition $H(\bbx(F))\leq \delta$, which as mentioned earlier can just be written in terms of $\det\Sigma(F|\bby_{0:F}) \leq \delta'$. This is a planning problem with goal specified by $\det\Sigma(F|\bby_{0:F}) \leq \delta'$ and stage cost given by $\det\Sigma(t)$. I would relate the proposed biased sampling procedure to a heuristic function for this problem. For example, can you relate the "minimize the distance to the target" intuition to a lower bound on the objective $\sum_{t=0}^{F}  \det\Sigma(t)$?} %; \red{see also Figure ??}.
%
\begin{problem} \label{prob}(Active Information Acquisition)
Given an initial robot configuration $\bbp(0)$ and a Gaussian prior distribution $\ccalN(\hat{\bbx}(0),\Sigma(0))$ for the hidden state $\bbx$, select a horizon $F$ and compute control inputs $\bbu(t)$ for all time instants $t\in\{0,\dots,F\}$ as per \eqref{eq:Prob2}.
%
\end{problem}

Throughout the paper we make the following assumption allows for application of a Kalman filter; see \cite{atanasov2014information}.% and the underlying communication network between the robots.
\begin{assumption} \label{as:assumption}%[State Model]
The measurement noise covariance matrices $\bbR(t)$ are known for all time $t\geq 0$. %Furthermore, the state dynamics \eqref{eq:dynamics} and sensing model \eqref{eq:measModel} are differentiable functions. 
%Finally, we assume that all robots can communicate with each other at any time $t$. 
\end{assumption}

%\begin{rem}[Nonlinear Models]
%Note that we assume that the dynamics \eqref{eq:dynamics} and the sensing model \eqref{eq:measModel} are modeled as linear systems. Also, in \eqref{eq:rdynamics} we assume noiseless robot dynamics. As discussed before, 
%Note that Assumption \ref{as:assumption} allows for offline computation of optimal policies, since the solution to \eqref{eq:Prob2} does not depend on the robot measurements. %In Section \ref{sec:Sim}, we present numerical experiments where this assumption is relaxed.
%\end{rem}
\begin{rem}[Optimal Control Problem \eqref{eq:Prob}]\label{rem1}
In \eqref{eq:Prob}, any other optimality metric, not necessarily information-based, can be used in place of \eqref{obj1} as long as it is always positive. If non-positive metrics are selected, e.g., the entropy of $\bbx$, then \eqref{eq:Prob} is not well-defined, since the  optimal terminal horizon $F$ is infinite. On the other hand, in the first constraint \eqref{constr2}, any uncertainty measure can be used without any restrictions, e.g., scalar functions of the covariance matrix, or mutual information. Moreover, note that without the terminal constraint \eqref{constr2}, the optimal solution of \eqref{eq:Prob} is  all robots to stay put, i.e., $F=0$. 
%Additional terminal constraints can be added to \eqref{eq:Prob}, such as, $\bbp(F)\in\ccalP_{\text{goal}}\subseteq\Omega_{\text{free}}^N$, to model joint task planning and estimation scenarios, where, e.g., the robots should eventually visit a base station to upload an estimate of the hidden state with user-specified accuracy determined by $\delta$.
\end{rem}


==> Technical Report- Scalable Active Information Acquisition - FinalSubmission/files/alg.tex <==

A centralized and offline solution to \eqref{eq:Prob2} is proposed in \cite{kantaros2019asymptotically} that is shown to be optimal under linearity and Gaussian assumptions; nevertheless, a centralized solution can incur a high computational cost as it requires exploring a high dimensional joint space composed of the space of multi-robot states and covariance matrices. As a result, its computational cost increases as the number of robots and landmarks increases. To mitigate these challenges, we propose a distributed and online - but sub-optimal - approach that allows the robots to make local decisions, assuming all-to-all communication, to solve \eqref{eq:Prob2} as they navigate the environment. 

%In Section \ref{sec:decomp}, we show how \eqref{eq:Prob2} can be decomposed into local problems while a computationally efficient method to solve them is presented in Section \ref{sec:sol}

\subsection{Decomposition of AIA Task \& Robot Roles}\label{sec:decomp}

The proposed algorithm is summarized in Algorithm \ref{alg:AIA}. The key idea relies on decomposing \eqref{eq:Prob2} into local optimal control problems, that are formulated and solved online to generate individual robot actions. Decomposition of \eqref{eq:Prob2} into local problems is attained by assigning landmarks to each robot online via a \textit{dynamic} space-partitioning method. 

Specifically, at any time $t\geq0$, the environment is decomposed into Voronoi cells generated by the robot positions $\bbp_j(t)$. The Voronoi cell assigned to robot $j$ at time $t$, denoted by $V_j(t)$, is defined as $ V_j(t)=\set{\bbq\in\Omega~|~\lVert\bbp_j(t)-\bbq\rVert\leq \lVert\bbp_e(t)-\bbq\rVert,~\forall e\neq j}$,
%\begin{equation}
%    V_j(t)=\set{\bbq\in\Omega~|~\lVert\bbp_j(t)-\bbq\rVert\leq \lVert\bbp_e(t)-\bbq\rVert,~\forall e\neq j},
%\end{equation}
i.e., $V_j(t)$ collects all locations $\bbq$ in the workspace that are closer to robot $j$ than to any other robot $e\neq j$ at time $t\geq 0$. Observe that it holds that $\bigcup_{j\in\ccalN}V_j(t)=\Omega$. %Also, note that the each robot can construct its individual Voronoi cell in a distributed fashion by communicating only with its Delaunay neighbors  \cite{Cortes_SIAMJCO05}; see Remark \ref{rem:com}. 

Given $V_j(t)$, robot $j$ is responsible for \textit{actively decreasing the uncertainty of the landmarks that are expected/estimated to lie within its Voronoi cell}. Formally, the landmarks that robot $j$ is responsible for at time $t$ are collected in the following set:
\begin{equation}\label{eq:Aj}
\ccalA_j(t)=\{i\in\ccalM ~|~(\hat{\bbx}_i(t)\in\ccalV_j(t))\wedge (\det\Sigma_j(t)>\delta) \}.
\end{equation}
In words, $\ccalA_j(t)$ collects the landmarks that have not been localized with accuracy determined by $\delta$ and are estimated to be closer to robot $j$ than to any other robot. By definition of the set of $\ccalA_j(t)$ and the fact that $\bigcup_{j\in\ccalN}V_j(t)=\Omega$, we have that every landmark is assigned to exactly one robot and that there are no unassigned landmarks, i.e., $\bigcup_{j\in\ccalN}\ccalA_j(t)=\ccalM$. Notice that the set $\ccalA_j(t)$ may be empty in case the estimated positions of all landmarks are outside the $j$-th Voronoi cell. Depending on the emptiness of the sets $\ccalA_j(t)$, the robots switch between \textit{exploration} and \textit{AIA} roles in the workspace, as follows. 

\subsubsection{Local AIA Strategy} If at time $t=\bar{t}$ there are landmarks assigned to robot $j$, i.e., $\ccalA_j(\bar{t})\neq\emptyset$, then robot $j$ solves the following local AIA problem:
\begin{subequations}
\label{eq:LocalProbb2}
\begin{align}
& \min_{\substack{ F_j, \bbu_{j,\bar{t}:F_j}}} \left[J(F_j,\bbu_{\bar{t}:F_j}) = \sum_{t=\bar{t}}^{F_j}  \sum_{i\in\ccalA_j(\bar{t})}\det\Sigma_i(t) \right] \label{obj3}\\
%&\ \ \st \ \ \ \ \ \ \ \ \ \ \ \ \bbp(F) \in \ccalP_{\text{goal}}, \label{constr21}\\
& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \det\Sigma_i(F_j)\leq \delta, \forall i\in\ccalA_j(\bar{t}) \label{constr32} \\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \bbp_j(t) \in \Omega_{\text{free}}, \label{constr33} \\ % V_j(\bar{t})
& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \bbp_j(t+1) = \bbf_j(\bbp_j(t),\bbu_j(t)), \label{constr34}\\
& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \Sigma(t+1) =\rho(\bbp_j(t+1),\Sigma(t)), \label{constr35}
\end{align}
\end{subequations}
where the constraints \eqref{constr33}-\eqref{constr35} hold for all time instants $t\in[\bar{t},F_j]$. Note that \eqref{eq:LocalProbb2} can viewed as local version of \eqref{eq:Prob2}. In words, \eqref{eq:LocalProbb2} requires robot $j$ to compute a terminal horizon $F_j$ and a sequence of control inputs over this horizon, denoted by  $\bbu_{j,\bar{t}:F_j}$, so that (i) the accumulated uncertainty over the assigned targets is minimized (see \eqref{obj3}), (ii) the terminal uncertainty of the assigned targets is below a user-specified threshold (see \eqref{constr32}) while  (iii) avoiding obstacles and respecting the robot dynamics and the Kalman filter Ricatti equation (see \eqref{constr33}-\eqref{constr35}). Note that in \eqref{constr35}, the  Kalman filter Ricatti equation is applied using only the position of robot $j$ and not the multi-robot state as opposed to \eqref{constr25}. In other words, in \eqref{constr35}, the covariance matrix $\Sigma(t)$ is computed using only local information. For simplicity, we do not add any dependence to robot $j$ to $\Sigma(t)$.
%
Equivalence between the centralized AIA problem \eqref{eq:Prob2} and the local AIA problems in \eqref{eq:LocalProbb2} is discussed in Section \ref{sec:complOpt}. A computationally efficient method to quickly solve the nonlinear optimal control problem \eqref{eq:LocalProbb2} is discussed in Section \ref{sec:aia}.

%[EXPLAIN here that you further decompose it into sequential problems across the assigned targets or in the simulations]


\subsubsection{Exploration Strategy} If at time $t=\bar{t}$, there are no landmarks assigned to robot $j$, i.e., $\ccalA_j(\bar{t})=\emptyset$, then robot $j$ is responsible for \textit{exploring} the environment so that eventually it holds that $\ccalA_j(t)\neq\emptyset$. %, i.e., robot $j$ becomes responsible for localizing a landmark.
%
In this way, the burden of localizing the landmarks is shared among the robots. The latter can be accomplished if these robots adopt an exploration/mapping or an area coverage strategy. For instance, in \cite{yamauchi1997frontier,leung2006active} a frontiers-based exploration strategy is proposed. Specifically, dummy
“exploration” landmarks with locations at the current map frontiers are considered with a known Gaussian prior on their locations. This fake uncertainty in the exploration-landmark locations promises information gain to the robots. In \cite{kantaros2015distributed,Cortes_ESAIMCOCV05}, area coverage methods are proposed assuming robots with range-limited sensors. Specifically, the robots follow a gradient-based policy to maximize an area coverage objective that captures the part of the workspace that lies within the sensing range of all robots. Alternatively, robots with $\ccalA_j(\bar{t})=\emptyset$ can be recruited from robots $e$ with $\ccalA_e(\bar{t})\neq\emptyset$ to help them localize the corresponding landmarks.

%its Voronoi cell to check if there are any landmarks inside it. By definition of $\ccalA_j(t)$, it holds that a landmark may be inside $\ccalV_j(t)$ even though $\ccalA_j(t)=\emptyset$. As an exploration strategy, we employ a frontiers-based approach [???]; however, any exploration algorithm can be employed [???]. Specifically, for all robots $j$, with $\ccalV_j(t)\neq\emptyset$, we introduce dummy “exploration” landmarks with locations $[\bbq_1,\dots,\bbq_{N_d}]$ at the current map frontiers that lie within $\ccalV_j(t)$ and specify a Gaussian prior on their locations with mean $\hat{\bbq}=\bbq$ and block diagonal covariance $\Sigma$ with $N_q$ blocks. This fake uncertainty in the exploration-landmark locations promises information gain to the robots. Specifically, navigating the environment to decrease the uncertainty of the frontier-landmarks, by solving the corresponding local optimal control problem \eqref{eq:LocalProbb2}, allows the robots to explore their Voronoi cells and discover landmarks with inaccurate position estimates.

\subsection{Local Planning for Non-myopic AIA}\label{sec:aia}
In this section, we present a computationally efficient method to solve the local optimal control problem \eqref{eq:LocalProbb2}. %Note that \eqref{eq:LocalProbb2} is a nonlinear optimal control problem that requires to exhaustively search over the joint space of the robot states and covariance matrices, a task that is particularly challenging to accomplish online. To mitigate this, 
Specifically, to solve \eqref{eq:LocalProbb2}, we employ our recently proposed sampling-based algorithm for AIA tasks \cite{kantaros2019asymptotically}. In particular, the employed algorithm relies on incrementally constructing a directed tree that explores both the information space and the physical space. 
%\subsection{Decomposition of \eqref{eq:LocalProbb2} across the landmarks}

%\subsection{Sampling-based Planning for AIA}
In what follows, we denote by $\mathcal{G}_j=\{\mathcal{V}_j,\mathcal{E}_j,J_{\ccalG,j}\}$ the tree constructed by robot $j$ to solve \eqref{eq:LocalProbb2}, where $\ccalV_j$ is the set of nodes and $\ccalE_j\subseteq \ccalV_j\times\ccalV_j$ denotes the set of edges. The set of nodes $\mathcal{V}_j$ contains states of the form $\bbq_j(t)=[\bbp_j(t), \Sigma(t)]$. %\footnote{Throughout the paper, when it is clear from the context, we drop the dependence of $\bbq(t)$ on $t$.} 
The function $J_{\ccalG}:\ccalV_j\rightarrow\mathbb{R}_{+}$ assigns the cost of reaching node $\bbq_j\in\mathcal{V}_j$ from the root of the tree. The root of the tree, denoted by $\bbq_j(0)$, is constructed so that it matches the initial state  $\bbp_j(0)$ of robot $j$ and the prior covariance $\Sigma(0)$, i.e., $\bbq_j(0)=[\bbp_j(0), \Sigma(0)]$. For simplicity of notation, hereafter we drop the dependence of the tree on robot $j$. 
%
The cost of the root $\bbq(0)$ is $J_{\ccalG}(\bbq(0)) = \det\Sigma(0)$,
while the cost of a node $\bbq(t+1)=[\bbp_j(t+1), \Sigma(t+1)]\in\ccalV$, given its parent node $\bbq(t)=[\bbp_j(t), \Sigma(t)]\in\ccalV$, is computed as $J_{\ccalG}(\bbq(t+1))= J_{\ccalG}(\bbq_j(t)) +  \det\Sigma(t+1).$
%\begin{equation}\label{eq:costUpd}
%J_{\ccalG}(\bbq(t+1))= J_{\ccalG}(\bbq_j(t)) +  \det\Sigma(t+1).
%\end{equation}
Observe that by applying this cost function recursively, we get that $J_{\ccalG}(\bbq(t+1)) = J(t,\bbu_{0:t+1})$ which is the objective function in \eqref{eq:LocalProbb2}.


\begin{algorithm}[t]
\footnotesize
\caption{Local Planning for Global AIA Task}
\LinesNumbered
\label{alg:AIA}
\KwIn{ (i) robot dynamics; observation model; (iii) prior Gaussian $\ccalN(\hat{\bbx}(0),\Sigma(0))$; (iv) initial robot configuration $\bbp_j(0)$}
\KwOut{Terminal horizon $F$, and control inputs $\bbu_{0:F}$};\label{rrt:init}
$t=0$\label{alg:init1}\;
Compute Voronoi cell $V_j(0)$ and set of assigned targets $\ccalA_j(0)$\;\label{alg:init1}
\While{$\exists j~\text{s.t.}~\det\Sigma_j(t)>\delta$}{
\If{$\ccalA_j(t)\neq\emptyset$}{
\If{$(t=0)\vee(\ccalA_j(t)\neq \ccalA_j(t-1))$}{
Compute sequence of controllers $\bbu_{j,t:F_j}$ for AIA \cite{kantaros2019asymptotically}\;\label{aia:cntrl1} Apply control input $\bbu_j(t)$\;}
\Else{
Apply the next control input from the most recently computed sequence of control inputs\;} 
}
\Else{
Compute next control input $\bbu_j(t)$ to explore $V_j(t)$\;\label{aia:cntrl2}
}
Collect sensor measurements\;
Update $\hat{\bbx}(t+1)$ and $\Sigma(t+1)$\; 
Update Voronoi cell $V_j(t+1)$ and set $\ccalA_j(t+1)$\;
$t=t+1$\;\label{aia:vor}
}
\end{algorithm}


\normalsize
The tree $\ccalG$ is initialized so that $\ccalV=\{\bbq(0)\}$, $\ccalE=\emptyset$, and $J_{\ccalG}(\bbq(0)) = \det\Sigma(0)$. Also, the tree is built incrementally by adding new states $\bbq_\text{new}$ to $\ccalV$ and corresponding edges to $\ccalE$, at every iteration $n$ of the sampling-based algorithm, based on a \textit{sampling} and \textit{extending-the-tree} operation. 
%
After taking $n_{\text{max}}\geq 0$ samples, where $n_{\text{max}}$ is user-specified, the sampling-based algorithm terminates and returns a solution to Problem \ref{prob}, i.e., a terminal horizon $F$ and a sequence of control inputs $\bbu_{0:F}$. 
%
To extract such a solution, we need first to define the set $\ccalX_g\subseteq\ccalV$ that collects all states $\bbq(t)=[\bbp_j(t), \Sigma(t)]\in\ccalV$ of the tree that satisfy %$\bbp(t)\in\ccalP_{\text{goal}}$ and %%\eqref{constr21}-
$\det\Sigma(F_j)\leq \delta$, for all landmarks that belong to $\ccalA_j(t)$, which is the constraint \eqref{constr32}. Then, among all nodes $\ccalX_g$, we select the node $\bbq(t)\in\ccalX_g$, with the smallest cost $J_{\ccalG}(\bbq(t))$, denoted by $\bbq(t_{\text{end}})$. %\NA{Note that if you relate the biasing to consistent heuristic the search can stop as soon as you find the first terminal state and you will not need to compare all such states. A consistent heuristic allows biasing the search even more by inflating the heurstic (multiplying by a constant $\epsilon$) and still guaranteeing $\epsilon$-suboptimality}. 
Then, the terminal horizon is $F=t_{\text{end}}$, and the control inputs $\bbu_{0:F}$ are recovered by computing the path $\bbq_{0:t_{\text{end}}}$ in $\ccalG$ that connects $\bbq(t_{\text{end}})$ to the root $\bbq(0)$, i.e., $\bbq_{0:t_{\text{end}}}= \bbq(0), \dots, \bbq(t_{\text{end}})$. 
%
Note that satisfaction of the constraints \eqref{constr33}-\eqref{constr35} is guaranteed by construction of $\ccalG$; see \cite{kantaros2019asymptotically}. The core operations of this algorithm, `\textit{sample}' and `\textit{extend}' that are used to incrementally construct the tree $\ccalG$ can be found in \cite{kantaros2019asymptotically}. %are described in Appendix \ref{appB}.

\subsection{Overview of Distributed Hybrid AIA Algorithm}\label{sec:overview}
At any time $t\geq0$ every robot $j$ adopts a role in the environment based on the set $\ccalA_j(t)$. %, i.e., the set of landmarks that are assigned to them. 
If $\ccalA_j(t)=\emptyset$, then robot $j$ adopts an exploration mode aiming to eventually become responsible for localizing landmarks. If $\ccalA_j(t)\neq\emptyset$, then robot $j$ solves \eqref{eq:LocalProbb2} to actively decrease the uncertainty of the assigned landmarks. In both cases, robot $j$ generates a sequence of controls denoted by $\bbu_{j,t:F_j}$. %As the robots apply their control inputs 
%
Once the robots apply their respective control input $\bbu_j(t)$, they communicate via an all-to-all connected network to share their measurements and positions so that they can (i) maintain a global estimate of the hidden state and (ii) update their Voronoi cells $V_j(t+1)$. Based on the new Voronoi cells, the robots locally compute the new sets of assigned targets $\ccalA_j(t+1)$. The robots for which it holds that $\ccalA_j(t+1)=\ccalA_j(t)$ do not update their corresponding sequence of control actions, i.e., they apply the control input $\bbu_j(t+1)$ computed at time $t$. On the other hand, the robots that satisfy $\ccalA_j(t+1)\neq\ccalA_j(t)$ recompute their control actions to accomplish either their assigned AIA or exploration tasks. %, depending on the emptiness of $\ccalA_j(t+1)$.


%\begin{rem}[Communication Requirements]\label{rem:com}
%Note that in general it holds that $\bbx_j(t)\neq \hat{\bbx}_j(t)$ which means that a robot may be responsible for a target that does not lie within its Voronoi cell. Moreover, depending on the multi-robot configuration it is possible that a robot may not be responsible for any targets, i.e., $\ccalA_j(t)=\emptyset$...
%To implement Algorithm \ref{alg:AIA}, all-to-all communication is required to (i) share the collected measurements so that all robots have access to the same estimate for the hidden states; (ii) compute the Voronoi cells.
%\textcolor{blue}{Algorithm \ref{alg:AIA} is distributed in the sense each robot computes locally and online its own control actions by solving the corresponding local problems \eqref{eq:LocalProbb2}. Also, to implement Algorithm \ref{alg:AIA}, all-to-all communication is required as discussed in Section \ref{sec:overview}.}
%Also, to implement Algorithm \ref{alg:AIA}, all-to-all communication is required so that the robots can (i) share their collected measurements to the have the same global estimate for the hidden states and (ii) exchange their positions to compute their respective Voronoi cells.}
%\end{rem}

\subsection{Extensions}\label{sec:extensions}

%\subsubsection{Unknown Number of Landmarks}
%In Section \ref{sec:PF}, we assume that the number of landmarks is known. This  can be relaxed by enforcing all robots with $\ccalA_j(t)=\emptyset$ to adopt an exploration/mapping strategy \cite{leung2006active,smith2018distributed,corah2019communication,wang2020autonomous}. In this case, Algorithm \ref{alg:AIA} terminates when the whole environment has been explored and all landmarks that have been localized with user-specified accuracy $\delta$.

\subsubsection{Mobile Landmarks}
Mobile landmarks can also be considered that are governed by the following known but noisy dynamics: $\bbx_i(t+1) =\bbg_i(\bbx_i(t),\bba_i(t), \bbw_i(t))$,
%\begin{equation} \label{eq:dynamics}
%\bbx_i(t+1) =\bbg_i(\bbx_i(t),\bba_i(t), \bbw_i(t)), 
%\end{equation}
where $\bba_i(t)$ and $\bbw_i(t) \in\reals^{d_w}$ are the control input and the process noise for landmark $i$ at discrete time $t$. We assume that the process noise $\bbw_i(t)$ is uncertain and follows a known normal distribution, i.e., $\bbw(t) \sim \ccalN(0, \bbQ(t))$, where $\bbQ(t)$ is the covariance matrix at time $t$. Assuming that the control inputs $\bba_i(t)$ and the covariance matrices $\bbQ(t)$ are known to the robots for all $t\geq 0$, \cite{kantaros2019asymptotically} can be used to design AIA paths.\footnote{Note that in this case, Algorithm \ref{alg:AIA} is not complete; see also the proof of Theorem \ref{thm:probCompl2}.} %The only difference is that \eqref{eq:predict} will be used to construct the landmark states $\hat{\bbx}_{\text{new}}(t)$, instead of \eqref{eq:updX}, which are then used to define the map $\ccalM_{\text{new}}(t)$.

\subsubsection{Nonlinear Observation Models}
In Section \ref{sec:PF}, we assumed a sensor model that is linear with respect to the landmark positions allowing us to compute offline the a-posteriori covariance matrix without the need of measurements. This assumption can be relaxed by computing the a-posteriori covariance matrices using the linearized observation model about the estimated landmark positions; see Section \ref{sec:Sim}.

%Nevertheless, this assumption may not hold in practice. In this case, during the execution of the sampling-based AIA algorithm \cite{kantaros2019asymptotically},  we compute the a-posteriori covariance matrices using the linearized observation model about the estimated landmark positions; see Section \ref{sec:Sim}.




==> Technical Report- Scalable Active Information Acquisition - FinalSubmission/files/proofs.tex <==
%\section{Proof of Completeness \& Optimality}\label{sec:prop}

In what follows, we denote by $\mathcal{G}^n=\{\mathcal{V}^{n}, \mathcal{E}^{n}, \texttt{Cost}\}$ the tree that has been built by Algorithm \ref{alg:RRT} at the $n$-th iteration. The same notation also extends to $f_{\ccalV}$, $f_{\ccalU}$, and $\bbu_{\text{new}}$. %We also denote by $f_{\ccalV}^n$ and $f_{\ccalU}^n$ the density functions used at iteration $n$ of Algorithm \ref{alg:RRT}. The same notations extends to subsets $\ccalV_{k}$ $k_{\text{rand}}$, and $\bbu_{\text{new}}$. For simplicity of notations, we denote by $\ccalV_{k_{\text{rand}}}^n\subseteq \ccalV^n$ (instead of  $\ccalV_{k_{\text{rand}}^n}^n$) the subset of nodes selected by $f_{\ccalV}^n$ at iteration $n$.
%
%
%
To prove Theorems \ref{thm:probCompl} and \ref{thm:asOpt}, we need to prove the following results. %that rely on the Borel-Cantelli lemma \cite{grimmett2001probability}.

%\begin{lem}[Borel-Cantelli \cite{grimmett2001probability}]\label{lem:bc}
%Consider a sequence of independent events $A=\{A^n\}_{n=1}^{\infty}$. If $\sum_{n=1}^{\infty}\mathbb{P}(A^n)=\infty$ then $\mathbb{P}(\limsup_{n\to\infty} A^n)=1$, i.e., the probability that infinitely many events $A^n$ occur is 1.  
%i.e., the events $A^n$ occur infinitely often meaning that $A^n$ is true for an infinite number of indices $n\in\mathbb{N}_{+}$.
%\end{lem}


\begin{lem}[Sampling $\ccalV_{k_{\text{rand}}}^n$]
Consider any subset $\ccalV_{k}^n$ and any fixed iteration index $n$ and any fixed $k\in\set{1,\dots,K_n}$. Then, there exists an infinite number of subsequent iterations $n+w$,  where $w\in\mathcal{W}$ and $\mathcal{W}\subseteq\mathbb{N}$ is a subsequence of $\mathbb{N}$, at which the subset $\ccalV_{k}^n$ is selected to be the set $\ccalV_{k_{\text{rand}}}^{n+w}$. %\footnote{The subsequences $\ccalK$ and $\ccalK'$}
\label{lem:qrand}
\end{lem}

\begin{proof}
%The proof of this results relies on Lemma \ref{lem:bc}.
Let $A^{\text{rand},n+w}(k)=\{\ccalV_{k_{\text{rand}}}^{n+w}=\ccalV_{k}^n\}$, with $w\in\mathbb{N}$, denote the event that at iteration $n+w$ of Algorithm \ref{alg:RRT} the subset $\ccalV_{k}^n\subseteq\ccalV^n$ is selected by the sampling operation to be the set $\ccalV_{k_{\text{rand}}}^{n+w}$ [line \ref{rrt:samplekrand}, Alg. \ref{alg:RRT}]. Also, let $\mathbb{P}(A^{\text{rand},n+w}(k))$ denote the probability of this event, i.e., $\mathbb{P}(A^{\text{rand},n+w}(k))=f_{\ccalV}^{n+w}(k)$. 

Next, define the infinite sequence of events $A^{\text{rand}}=\{A^{\text{rand},n+w}(k)\}_{w=0}^{\infty}$, for a given subset $\ccalV_{k}^n\subseteq\ccalV^n$. In what follows, we show that the series $\sum_{w=0}^{\infty}\mathbb{P}(A^{\text{rand},n+w}(k))$ diverges and then we complete the proof by applying the Borel-Cantelli lemma \cite{grimmett2001probability}. %Lemma \ref{lem:bc}. 
%
%Recall first that the size of $K_{n+e}$, i.e., the number of  subsets $\ccalV_{T,k}^{n+e}$ cannot grow arbitrarily large as $e\to\infinity$, since it holds that $|\ccalU|=|\ccalU_1\times\ccalU_2\times\dots\times\ccalU_n|<\infty$, by assumption. Also, 

Recall that by Assumption \ref{frand}(i), we have that  given any subset $\ccalV_{k}^n\subseteq\ccalV^n$, the probability $f_{\ccalV}^n(k|\ccalV^n)$ satisfies $f_{\ccalV}^n(k|\ccalV^n)\geq \epsilon$, for any iteration $n$. Thus we have that $\mathbb{P}(A^{\text{rand},n+w}(k))=f_{\ccalV}^{n+w}(k|\ccalV^{n+w})\geq \epsilon>0, 
$
%\begin{equation}\label{ineq1}
%\mathbb{P}(A^{\text{rand},n+w}(k))=f_{\ccalV}^{n+w}(k|\ccalV^{n+w})\geq \epsilon> 0, 
%\end{equation} 
for all $w\in\mathbb{N}$. Note that this result holds for any $k\in\set{1,\dots,K_{n+w}}$ due to Assumption \ref{frand}(i). 
%
%Since \eqref{ineq1} holds for all $w\in\mathbb{N}$, 
Therefore, we have that $\sum_{w=0}^{\infty}\mathbb{P}(A^{\text{rand},n+w}(k))\geq\sum_{w=0}^{\infty}\epsilon.$
%\begin{equation}\label{ineq2}
%\sum_{w=0}^{\infty}\mathbb{P}(A^{\text{rand},n+w}(k))\geq\sum_{w=0}^{\infty}\epsilon.
%\end{equation}
Since $\epsilon$ is a strictly positive constant, we have that $\sum_{w=0}^{\infty}\epsilon$ diverges. Then, %by the comparison test \cite{marsden1993elementary}, 
we conclude that $\sum_{w=0}^{\infty}\mathbb{P}(A^{\text{rand},n+w}(k))=\infty.$
%\begin{equation}\label{res1}
%\sum_{w=0}^{\infty}\mathbb{P}(A^{\text{rand},n+w}(k))=\infty.
%\end{equation}
%
Combining this result and the fact that the events $A^{\text{rand},n+w}(k)$ are independent by Assumption \ref{frand}(ii), we get that $\mathbb{P}(\limsup_{k\to\infty} A^{\text{rand},n+w}(k)=1,$ by the Borel-Cantelli lemma. In other words, the events $A^{\text{rand},n+w}(k)$ occur infinitely often, for all $k\in\{1,\dots,K_n\}$. This equivalently means that for every subset $\ccalV_{k}^n\subseteq\ccalV^n$, for all $n\in\mathbb{N}_{+}$, there exists an infinite subsequence $\mathcal{W}\subseteq \mathbb{N}$ so that for all $w\in\mathcal{W}$ it holds $\ccalV_{k_{\text{rand}}}^{n+w}=\ccalV^{n}$, completing the proof.
\end{proof}
    
%Using Lemma \ref{lem:qrand} we can show the following result for the control input.
\begin{lem}[Sampling $\bbu_{\text{new}}$]
Consider any  subset $\ccalV_{k_{\text{rand}}}^n$ selected by $f_{\ccalV}$ and any fixed iteration index $n$. Then, for any given control input $\bbu\in\ccalU$, there exists an infinite number of subsequent iterations $n+w$, where $w\in\mathcal{W}'$ and $\mathcal{W}'\subseteq\mathcal{W}$ is a subsequence of the sequence of $\mathcal{W}$ defined in Lemma \ref{lem:qrand}, at which the control input $\bbu\in\ccalU$ is selected to be $\bbu_{\text{new}}^{n+w}$.
\label{lem:qnew}
\end{lem}

\begin{proof}
%This proof resembles the proof of Lemma \ref{lem:qrand} and is omitted.
%
Define the infinite sequence of events $A^{\text{new}}=\{A^{\text{new},n+w}(\bbu)\}_{w=0}^{\infty}$, for $\bbu\in\ccalU$, where $A^{\text{new},n+w}(\bbu)=\{\bbu_{\text{new}}^{n+w}=\bbu\}$, for $w\in\mathbb{N}$, denotes the event that at iteration $n+w$ of Algorithm \ref{alg:RRT} the control input $\bbu\in\ccalU$ is selected by the sampling function to be the input $\bbu_{\text{new}}^{n+w}$, given the subset $\ccalV_{k_{\text{rand}}}^n\in\ccalV_{k_{\text{rand}}}^{n+w}$. Moreover, let $\mathbb{P}(A^{\text{new},n+w}(\bbu))$ denote the probability of this event, i.e., $\mathbb{P}(A^{\text{new},n+e}(\bbu))=f_{\ccalU}^{n+w}(\bbu| \ccalV_{k_{\text{rand}}}^{n+w})$. 
%
Now, consider those iterations $n+w$ with $w\in\mathcal{W}$ such that $k_{\text{rand}}^{n+w}=k_{\text{rand}}^n$ by Lemma \ref{lem:qrand}. We will show that the series $\sum_{w\in\ccalK}\mathbb{P}(A^{\text{new},n+w}(\bbu))$ diverges and then we will use Borel-Cantelli lemma  to show that any given $\bbu\in\ccalU$ will be selected infinitely often to be control input $\bbu_{\text{new}}^{n+w}$.
%
By Assumption \ref{fnew}(i)  we have that $\mathbb{P}(A^{\text{new},n+w}(\bbu))=f_{\ccalU}^{n+w}(\bbu| \ccalV_{k_{\text{rand}}}^{n+w})$ is bounded below by a strictly positive constant $\zeta>0$ for all $w\in\ccalW$. 
Therefore, we have that $\sum_{w\in\ccalW}\mathbb{P}(A^{\text{new},n+w}(\bbu))$ diverges, since it is an infinite sum of a strictly positive constant term. Using this result along with the fact that the events $A^{\text{new},n+w}(\bbu)$ are independent, by Assumption \ref{fnew}(ii), we get that $\mathbb{P}(\limsup_{w\to\infty} A^{\text{new},n+w}(\bbu))=1,$ due to the Borel-Cantelli lemma. In words, this means that the events $A^{\text{new},n+w}(\bbu)$ for $w\in\mathcal{W}$ occur infinitely often. Thus, given any subset $\ccalV_{k_{\text{rand}}}^n$, for every control input $\bbu$ and for all $n\in\mathbb{N}_{+}$, there exists an infinite subsequence $\mathcal{W}' \subseteq \mathcal{W}$ so that for all $w\in\mathcal{W}'$ it holds $\bbu_{\text{new}}^{n+w}=\bbu$, completing the proof.
\end{proof}

Before stating the next result, we first define the \textit{reachable} state-space of a state $\bbq(t)=[\bbp(t),\Sigma(t)]\in\ccalV_{k}^n$, denoted by $\ccalR(\bbq(t))$ that collects all states $\bbq(t+1)=[\bbp(t+1), \Sigma(t+1)]$ that can be reached within one time step from $\bbq(t)$.%, where recall that  $\bbp_j(t+1)=\bbf_j(\bbp_j(t),\bbu_j)\in\Omega_{\text{free}}$, $d_i(t+1)=\det\Sigma_i(t+1)=\det\rho(\Sigma_i(t))$. In math, $\ccalR(\bbq(t))$ is defined as follows. 

%\begin{align}\label{eq:reachableSet}
%\ccalR(\bbq(t))&=\{\bbq(t+1)=[\bbp(t+1), \bbd(t+1)]~|~\nonumber \\ &\bbp_j(t+1)=\bbg(\bbp_j(t),\bbu_j), \forall j,\\& d_i(t+1)=\Sigma_i(t+1)=\det\rho(\Sigma_i(t)), \forall i, \forall \bbu\in\ccalU \}\nonumber.
%\end{align}

%\subsection{Proof of Corollary \ref{cor:reach}}
\begin{cor}[Reachable set $\ccalR(\bbq(t))$]\label{cor:reach}
Given any state $\bbq(t)=[\bbp(t),\Sigma(t)]\in\ccalV_{k}^n$, for any $k\in\{1,\dots,K_n\}$, Algorithm \ref{alg:RRT} will add to $\ccalV^n$ all states that belong to the reachable set $\ccalR(\bbq(t))$ will  be added to $\ccalV^{n+w}$, with probability 1, as $w\to\infty$, i.e., $\lim_{w\rightarrow\infty} \mathbb{P}\left(\{\ccalR(\bbq(t))\subseteq\mathcal{V}^{n+w}\}\right)=1.$
%\begin{equation}\label{eq:reach2}
%\lim_{w\rightarrow\infty} %\mathbb{P}\left(\{\ccalR(\bbq(t))\subseteq\mathcal{V}^{n+w}\}%\right)=1.
%\end{equation}
Also, edges from $\bbq(t)$ to all reachable states $\bbq'(t+1)\in\ccalR(\bbq(t))$ will  be added to $\ccalE^{n+w}$, with probability 1, as $w\to\infty$, i.e., $\lim_{w\rightarrow\infty} \mathbb{P}\left(\{\cup_{\bbq'\in\ccalR(\bbq)}(\bbq,\bbq')\subseteq\mathcal{E}^{n+w}\}\right)=1.$
%\begin{equation}\label{eq:reachedge}
%\lim_{w\rightarrow\infty} %\mathbb{P}\left(\{\cup_{\bbq'\in\ccalR(\bbq)}(\bbq,\bbq')\sub%seteq\mathcal{E}^{n+w}\}\right)=1.
%\end{equation}
\end{cor}
\begin{proof}
The proof straightforwardly follows from Lemmas \ref{lem:qrand}-\ref{lem:qnew} and is omitted. 
%Specifically, recall from Lemma \ref{lem:qrand}, that for any given and fixed iteration index $n$, there exists an infinite sequence of iterations $n+e$, $w\in\ccalW$, where the subset $\ccalV_{k}^{n+w}$, for any given and fixed $k$,  will be selected to be the subset $\ccalV_{{k_{\text{rand}}}}^{n+w}$. Also, given a control input $\bbu_{\text{new}}^{n+e}$ sampled by $f_{\ccalU}^{n+w}$, we have that the state $\bbq'=[\bbp'(t+1),\bbd'(t+1)]$, where $\bbp_j(t+1)=\bbg(\bbp_j,\bbu_{j,\text{new}}^{n+w})$, for all robots $j$, will be added to the tree, if $\bbp'(t+1)\in\Omega_{\text{free}}^N$. By Lemma \ref{lem:qnew}, we get that there exist an infinite sequence number of iterations $n+w$, where $w\in\ccalE'\subseteq \ccalE$, where any given control input $\bbu\in\ccalU$ will be selected to be $\bbu_{\text{new}}^{n+w}$. Since it holds that if $\bbq\in\ccalV_{k}^{n}$, then $\bbq\in\ccalV_{k}^{n+w}$, for all $n+w\geq n$, we conclude that all states that belong to the reachable set $\ccalR(\bbq(t))$ will eventually be added to the tree structure. In mathematical terms this can be written as in \eqref{eq:reach2}, completing the first part of the proof. Moreover, observe when a state $\bbq'\in\ccalR(\bbq)$ (where $\bbq$ is selected to be the node $\bbq_{\text{rand}}^{n+w}$) is added to the set of nodes $\ccalV_T^{n+w}$, then the edge $(\bbq,\bbq')$ is also added to the set of edges $\ccalE^{n+w}$ by construction of Algorithm \ref{alg:RRT}. This means that \eqref{eq:reachedge} holds, as well, completing the proof.
\end{proof}

%Given the above results we are now ready to prove that Algorithm \ref{alg:RRT} is probabilistically complete and asymptotically optimal.
%\subsection{Probabilistic Completeness - Proof of Theorem \ref{thm:probCompl}}\label{app:compl}

%To show this result it suffices to show that $\lim_{n\rightarrow\infty} \mathbb{P}\left(A^n(\bbq_{0:F})\right)=1,$
%\begin{equation}\label{eq:show}
%\lim_{n\rightarrow\infty} %\mathbb{P}\left(A^n(\bbq_{0:F})\right)=1,
%\end{equation}
%where  $A^n(\bbq_{0:F})=\{(\bbq(f)\in\ccalV^n) \wedge ((\bbq(f-1), \bbq(f))\in\mathcal{E}^{n}), \forall f\in\{1,\dots,F\} \}$ denotes the event that at iteration $n$ of Algorithm \ref{alg:RRT} the path $\bbq_{0:F}$ in \eqref{eq:path} has been included in the tree $\ccalG^n$, i.e.,  the states $\bbq(f)$ have been added to the set of nodes $\ccalV^n$ and the edges  $(\bbq(f-1), \bbq(f))$ have been to set of edges $\mathcal{E}^{n}$ for all $f\in\{1,\dots,F\}$. %In words, \eqref{eq:show} says that the path \eqref{eq:path} will be detected with probability $1$ as $n\to\infty$. 
{\bf{Proof of Theorem \ref{thm:probCompl}}:}  
By construction of the path $\bbq_{0:F}$, it holds that $\bbq(f)\in\ccalR(\bbq(f-1))$, for all $f\in\{1,\dots,F\}$. Since $\bbq(0)\in\ccalV^1$, it holds that all states $\bbq\in\ccalR(\bbq(0))$, including the state $\bbq(1)$, will be added to $\ccalV^n$ with probability $1$, as $n\to\infty$, due to Corollary \ref{cor:reach}.%; see \eqref{eq:reach2}. 
Once this happens, the edge $(\bbq(0),\bbq(1))$ will be added to set of edges $\ccalE^n$ due to Corollary \ref{cor:reach}.%; see \eqref{eq:reachedge}.
Applying Corollary \ref{cor:reach} inductively, we get that $\lim_{n\rightarrow\infty} \mathbb{P}\left(\{\bbq_f\in\mathcal{V}^{n}\}\right)=1$ and $\lim_{n\rightarrow\infty} \mathbb{P}\left(\{(\bbq(f-1), \bbq(f))\in\mathcal{E}^{n}\}\right)=1$, for all $f\in\{1,\dots,F\}$ meaning that the path $\bbq_{0:F}$ will be added to the tree $\ccalG^n$ with probability $1$ as $n\to\infty$ completing the proof.%\red{[similar to the argument for prob completeness of rrt]}.% Therefore, \eqref{eq:show} holds completing the proof. 
%\begin{equation}\label{eq:prob3}
%\lim_{n\rightarrow\infty} \mathbb{P}\left(A^n(\texttt{path})\right)=1,
%\end{equation}
%for any finite path $\texttt{path}$ that resides in $\Omega_{\text{free}}^N\times\mathbb{R}_{+}$ generated as per the observation model \eqref{eq:measModel} and the robot dynamics \eqref{eq:rdynamics}. This means that if there exists feasible solution to Problem \ref{prob}, then Algorithm \ref{alg:RRT} will detect it with probability $1$ as $n\to\infty$. Therefore, \eqref{eq:show} holds for any feasible path $\texttt{path}$ completing the proof.

%\subsection{Asymptotic optimality - Proof of Theorem \ref{thm:asOpt}}\label{app:opt}
{\bf{Proof of Theorem \ref{thm:asOpt}}:} The proof of this result straightforwardly follows from Theorem \ref{thm:probCompl}. Specifically, recall from Theorem \ref{thm:probCompl} that Algorithm \ref{alg:RRT} can find any feasible path and, therefore, the optimal path as well, with probability $1$, as $n\to\infty$, completing the proof. %The proof for this result straightforwardly follows from Theorem \ref{thm:probCompl}. Specifically, recall from Theorem \ref{thm:probCompl} that Algorithm \ref{alg:RRT} can  find any feasible 

%\section{Convergence Proof}
%\subsection{Proof of Lemma \ref{lem:optHor}}

%This result holds by construction of the objective function in \eqref{eq:Prob2}. Specifically, recall that the cost function $G(\bbx_i(t)|\bbp(t))$ is selected to be positive, i.e., $G(\bbx_i(t)|\bbp(t))\geq 0$, for all $t\geq 0$. This also implies that $J(t,\bbu_{0:t})\geq 0$, for all $t\geq 0$. Given the positiveness of the cost function  $J(t,\bbu_{0:t})$, we show that $J(t,\bbu_{0:t})$ is monotone which then yields the desired result.
%
%Observe that $J(t+1,\bbu_{0:t+1})= J(t,\bbu_{0:t})+\sum_{i=1}^{M} G(\bbx_i(t+1)|\bbp(t+1))\geq J(t,\bbu_{0:t})\geq 0$, since $\sum_{i=1}^{M} G(\bbx_i(t+1)|\bbp(t+1))\geq 0$, for all $t\geq 0$. Thus, we conclude that $J(t,\bbu_{0:t})$ is \textit{monotone}.
%
%Next, consider the following two complementary cases: (i) there exists a finite time instant $\bar{t}\geq 0$ such that $G(\bbx_i(t)|\bbp(t))=0$, for any configuration $\bbp(t)$ and for all $t\geq \bar{t}$ and; and (ii) there does not exist a finite time instant $\bar{t}\geq 0$ such that $G(\bbx_i(t)|\bbp(t))=0$, for all $t\geq \bar{t}$. In the first case, observe that increasing the horizon $F$ can only increase the cost function $J(F,\bbu_{0:F})$ due to its monotonicity, i.e., $\lim_{F\to\infty} J(F,\bbu_{0:F})=\infty$, for any  $\bbu_{0:F}$. Therefore, if the optimum cost $J^*(F,\bbu_{0:F})$ is finite, %\footnote{Note that this a typical assumption in optimization and optimal control problems.} 
%then the optimal horizon $F$ is finite. In the second case, we conclude that  there exist more than one sequence of optimal control inputs that solve \eqref{eq:Prob2} (with cost equal to the optimum cost). Nevertheless, in this case, the optimal horizon can be selected to be  $\bar{t}\geq 0$, which is finite by assumption, completing the proof.
%This implies that the optimal horizon $F$ is finite, since increasing the horizon $F$ can only increase the cost  $J(F,\bbu_{0:F})$, i.e., $\lim_{F\to\infty} J(F,\bbu_{0:F})=\infty$, for any  $\bbu_{0:F}$. Note that if there exists a finite time instant $\bar{t}\geq 0$ such that $G(\bbx_i(t)|\bbp(t))=0$ for all $t\geq \bar{t}$ then $\lim_{F\to\infty} J(F,\bbu_{0:F})$ is finite. In this case, there exist more than one sequence of optimal control inputs that solve \eqref{eq:Prob2} (with cost equal to the optimum cost). Nevertheless, in this case, the optimal horizon can be selected to be  $\bar{t}\geq 0$, which is finite by assumption, completing the proof. \red{[not well written, explain why monotonicity is important]} 

%Lemma \ref{lem:optHor} also implies that the optimal control problem \eqref{eq:Prob2} is well-defined in the sense that the optimal cost $J(F,\bbu_{0:F})$ is finite.
%\subsection{Convergence Rate Bound - Proof of Theorem \ref{thm:conv}}

%[\red{say that the proof is inspired by [?]. briefly mention how the two proofs are different}]
{\bf{Proof of Theorem \ref{thm:conv}}:}
To prove this result, we model the sampling strategy employed by Algorithm \ref{alg:RRT} as a Poisson binomial process. Specifically, we define Bernoulli random variables $Y_n$ at every iteration $n$ of Algorithm \ref{alg:RRT} so that $Y_n=1$ only if the edge $(\bbq(f-1), \bbq(f))$ is added to the tree at iteration $n$, where $f$ is the smallest element of the set $\set{1,\dots,F}$ that satisfies $\bbq(f-1)\in\ccalV^{n-1}$ and $\bbq(f)\notin\ccalV^{n-1}$. Then, using the random variables $Y_n$, we define the random variable $Y=\sum_{n=1}^{n_{\text{max}}}Y_n$ which captures the total number of successes of the random variables $Y_n$ and we show that it follows a Poisson binomial distribution. Finally, we show that $  \mathbb{P}(A^{n_{\text{max}}}(\bbq_{0:F}^*))=\mathbb{P}(Y\geq F)$ which yields \eqref{eq:bnd1} by applying the Chernoff bounds to $Y$. The detailed proof is omitted.%-\eqref{eq:bnd2}.

Let $X_f^n$, for all $f\in\set{1,\dots,F-1}$ denote a Bernoulli random variable associated with iteration $n$ of Algorithm \ref{alg:RRT}, that is equal to $1$ if the edge $(\bbq_{f-1},\bbq_f)$ in $\bbq_{0:F}^*$ is added to the tree at iteration $n$ or has already been added to the tree at a previous iteration $m<n$, and is $0$ otherwise. Observe that $X_1^n$ is equal to  $1$ for all iterations $n\geq 1$ of Algorithm \ref{alg:RRT}, since the tree is rooted at $\bbq_1$ and, therefore, $q_P^1\in\ccalV^n$, for all $n\geq 1$. By construction of the sampling strategy the probability that $X_f^n=1$ is defined as follows


\begin{equation}\label{eq:padd}
\mathbb{P}(X_f^n)=\left\{
                \begin{array}{ll}
f_{\ccalV}^n(\bbq_{f-1})f_{\ccalU}^n(\bbu_{f-1\to f}), ~\mbox{if}~(\bbq_{f-1},\bbq_f)\notin\ccalE^n,\\
1,~~~\mbox{if}~(\bbq_{f-1},\bbq_f)\in\ccalE^n,
                \end{array}
              \right.
\end{equation}
where with slight abuse of notation $\bbu_{f-1\to f}\in\ccalU$ stands for the control input that steers the robots $\bbq_f$ to $\bbq_{f-1}$. Note that such a controller exists since $\bbq_f\in\ccalR(\bbq_{f-1})$ by construction of the path $\bbq_{0:F}^*$, where $\ccalR(\cdot)$ denotes the reachable set.
%
Observe that if $\bbq_{f-1}\notin\ccalV^n$ then $\mathbb{P}(X_f^n)=0$, since $f_{\ccalV}^n(\bbq_{f-1})=0$. Moreover, note that if an edge  $(\bbq_{f-1},\bbq_f)$ already belongs to $\ccalE^n$ from a previous iteration $m<n$ of Algorithm \ref{alg:RRT}, then it trivially holds that $\mathbb{P}(X_f^n)=1$.

Given the random variables $X_f^n$, we define the discrete random variable $Y_n$ initialized as $Y_1=X_1^1$ and for every subsequent iteration $n>1$ defined as 

\begin{equation} \label{eq:Yn}
Y_n=\left\{
                \begin{array}{ll}
                 X_f^n, ~~\mbox{if}~(Y_{n-1}=X_k^{n-1})\wedge(X_f^{n-1}=0)\\
                 X_{f+1}^n, \mbox{if}~(Y_{n-1}=X_f^{n-1})\wedge(X_f^{n-1}=1)\\
                 ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\wedge (f+1\leq F)\\
                  X_F^n, ~~\mbox{if}~(Y_{n-1}=X_f^{n-1})\wedge(X_f^{n-1}=1)\\
                 ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \wedge (f+1> F) \\
                \end{array}.
              \right.
\end{equation}


In words,  $Y_n$ is defined exactly as $Y_{n-1}$, i.e., $Y_n=Y_{n-1}=X_f^{n-1}=X_f^n$, if $Y_{n-1}=X_{f}^{n-1}=0$, i.e., if the edge $(\bbq_{f-1},\bbq_f)$ associated with the random variable $Y_{n-1}=X_f^{n-1}$ does not exist in the tree at iteration $n-1$; see the first case in \eqref{eq:Yn}. %
%
Also, $Y_n=X_{f+1}^n$, if $Y_{n-1}=X_{f}^{n-1}=1$, i.e., if the edge $(\bbq_{f-1},\bbq_f)$ was added to the tree at the previous iteration  $n-1$; see the second case in \eqref{eq:Yn}. 
%
If $f+1>F$ and $X_f^{n-1}=1$, then we define $Y_n=X_F^n$; see the last case in \eqref{eq:Yn}. Note that in this case, $Y_n$ can be defined arbitrarily, i.e., $Y_n=X_{\bar{f}}^n$, for any $\bar{f}\in\set{1,\dots,F}$, since if $f+1>K$ and $X_f^{n-1}=1$, then this means that all edges that appear in $\bbq_{0:F}^*$ have been added to $\ccalE^n$. By convention, in this case we define  $Y_n=X_F^n$.
%
%
%
Since $Y_n$ is equal to $X_n^f$ for some $f\in\{1,\dots,F\}$, as per \eqref{eq:Yn}, for all $n\geq 1$, we get that $Y_n$ also follows a Bernoulli distribution with parameter (probability of success)  $p^{\text{suc}}_n$ equal to the probability of success of $X_n^k$ defined in \eqref{eq:padd}, i.e., $$p^{\text{suc}}_n=\mathbb{P}(X_f^n),$$ where the index $f$ is determined as per \eqref{eq:Yn}.


Given the random variables $Y_n$, $n\in\{1,\dots,n_{\text{max}}\}$, we define the discrete random variable $Y$ as
\begin{equation}\label{eq:Y}
Y=\sum_{n=1}^{n_{\text{max}}}Y_n.
\end{equation}
Observe that $Y$ captures the total number of successes of the random variables $Y_n$ after $n_{\text{max}}>0$ iterations, i.e., if $Y=y$, $y\in\{1,\dots,n_{\text{max}}\}$, then $Y_n=1$ for exactly $y$ random variables $Y_n$. Therefore, if $Y\geq F$, then all edges that appear in the path $\bbq_{0:F}^*$ have been added to the tree, by definition of the random variables $Y_n$ and $Y$ in \eqref{eq:Yn} and \eqref{eq:Y}, respectively. Therefore, we conclude that 

\begin{equation}\label{eq:Psuc}
\mathbb{P}(A^{n_{\text{max}}}(\bbq_{0:F}^*))=\mathbb{P}(Y\geq K).
\end{equation}


In what follows, our goal is to compute the probability $\mathbb{P}(Y\geq K)$. Observe that $Y$ is defined as a sum of Bernoulli random variables $Y_n$ that are not identically distributed as their probabilities of success $p^{\text{suc}}_n$ are not fixed across the iterations $n$, since the definition of $Y_n$ changes at every iteration $n$ as per \eqref{eq:Yn}.
%
%
Therefore, $Y$ follows a Poisson Binomial distribution which has a rather complicated pmf which is valid for small $n$ and numerically unstable for large $n$; see e.g., \cite{choi2002approximating,hong2011computing}. Therefore, instead of computing $\mathbb{P}(Y\geq K)$, we compute a lower bound for $\mathbb{P}(Y\geq K)$ by applying the Chernoff bound to $Y$. 

Specifically, we have that
\begin{align}\label{eq:prbfailk}
&\mathbb{P}(Y<F)<\mathbb{P}(Y\leq F)=\mathbb{P}(Y\leq F\frac{\mu}{\mu})\\&
=\mathbb{P}\left(Y\leq(1-\underbrace{(1-\frac{F}{\mu})}_{=\delta})\mu\right)=\mathbb{P}(Y\leq(1-\delta)\mu)\leq e^{-\frac{\mu\delta^2}{2}},\nonumber
\end{align}
where $\mu$ is the mean value of $Y$ defined as $\mu=\sum_{n=1}^{n_{\text{max}}} p^{\text{suc}}_n$. Also, the last inequality in \eqref{eq:prbfailk} is due to the Chernoff bound in the lower tail of $Y$ and holds for  any $\delta\in(0,1)$. Observe that the Chernoff bound can be applied to $Y$, as it is defined as the sum of \textit{independent} Bernoulli random variables $Y_n$. Specifically, the random variables $Y_n$ are independent since independent samples $\bbq$ can be generated by the proposed sampling process,  specified by the density functions $f_{\ccalV}$ and $f_{\ccalU}$, due to Assumptions \ref{frand}(ii) and \ref{fnew}(ii). Substituting $\delta=1-\frac{F}{\mu}$ in \eqref{eq:prbfailk}, we get 

\begin{equation}\label{eq:bound}
\mathbb{P}(Y<F)\leq e^{-\frac{\mu}{2}+F-\frac{F^2}{\mu}}\leq e^{-\frac{\mu}{2}+F}=e^{-\frac{\sum_{n=1}^{n_{\text{max}}} p^{\text{suc}}_n}{2}+F},
\end{equation}
where the last inequality is due to $e^{-\frac{F^2}{\mu}}\leq 1$. Recall that \eqref{eq:bound} holds for any $\delta=1-\frac{F}{\mu}\in(0,1)$, i.e, for any $n_{\text{max}}$ that satisfies 
\begin{equation}\label{eq:cond1}
0<\delta<1 \implies 0<F<\mu=\sum_{n=1}^{n_{\text{max}}} p^{\text{suc}}_n\implies 0<F<n_{\text{max}},
\end{equation}
where the last inequality in \eqref{eq:cond1} is due to $ p^{\text{suc}}_n\leq 1$. Therefore, \eqref{eq:bound} holds as long as $n_{\text{max}}>F$. 

Note also that the inequality $0<F<\sum_{n=1}^{n_{\text{max}}} p^{\text{suc}}_n$ in \eqref{eq:cond1} is well defined, since $p^{\text{suc}}_n=\mathbb{P}(X_f^n)$ is strictly positive for all $n\geq 1$ by definition of $Y_n$. To show that, observe that if $Y_n=X_f^n$, for some $f\in\{1,\dots,F-1\}$, then it holds that $(\bbq_{f-2},\bbq_{f-1})\in\ccalE^n$, by definition of $Y_n$ in \eqref{eq:Yn}, i.e., $\bbq_{f-1}\in\ccalV^{n}$. Thus, we have that $f_{\ccalV}(\bbq_{f-1})>0$ by Assumption \ref{frand}(i). Also, $f_{\ccalU}(\bbu_{f-1\to f})>0$ by Assumption \ref{fnew}(i). Therefore, we have that $p^{\text{suc}}_n=\mathbb{P}(X_f^n)>0$; see also \eqref{eq:padd}.
%

Thus, we proved that there exist parameters $\alpha_n(\bbq_{0:F}^*)=p^{\text{suc}}_n\in(0,1]$ associated with every iteration $n$ of Algorithm \ref{alg:RRT} such that the probability $\mathbb{P}(A^{n_{\text{max}}}(\texttt{path}))$ of finding the finite path $\bbq_{0:F}^*$  within $n_{\text{max}}>F$ iterations satisfies
%
\begin{equation}
1\geq\mathbb{P}(A^{n_{\text{max}}}(\bbq_{0:F}^*))=1-\mathbb{P}(Y<F)\geq 1-e^{-\frac{\sum_{n=1}^{n_{\text{max}}} \alpha_n(\bbq_{0:F}^*)}{2}+F},\nonumber 
\end{equation}
completing the proof.

==> Technical Report- Scalable Active Information Acquisition - FinalSubmission/files/sim.tex <==
\begin{table*}[]
\caption{Scalability Analysis: The runtimes $T_{\text{plan}}$, $T_{\text{vor}}$, and $T_{\text{total}}$ are in secs, secs, and mins, respectively. }
\label{tab:scale}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
                                                            & \begin{tabular}[c]{@{}l@{}}N=10\\ M=10\end{tabular} & \begin{tabular}[c]{@{}l@{}}N=20\\ M=10\end{tabular} & \begin{tabular}[c]{@{}l@{}}N=50\\ M=10\end{tabular} & \begin{tabular}[c]{@{}l@{}}N=100\\ M=10\end{tabular} & \begin{tabular}[c]{@{}l@{}}N=10\\ M=100\end{tabular} & \begin{tabular}[c]{@{}l@{}}N=20\\ M=100\end{tabular} & \begin{tabular}[c]{@{}l@{}}N=50\\ M=100\end{tabular} & \begin{tabular}[c]{@{}l@{}}N=100\\ M=100\end{tabular} & \begin{tabular}[c]{@{}l@{}}N=300\\ M=100\end{tabular} & \begin{tabular}[c]{@{}l@{}}N=100\\ M=200\end{tabular} & \begin{tabular}[c]{@{}l@{}}N=300\\ M=200\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}$T_{\text{plan}}$/$T_{\text{vor}}$\end{tabular} & 0.11/0.007                                          & 0.12/0.002                                          & 0.13/0.02                                         & 0.12/0.05                                           & 0.18/0.009                                           & 0.19/0.014                                            & 0.17/0.03                                            & 0.20/0.05                                             & 0.26/0.36                                             & 0.31/0.06                                             & 0.36/0.19                                             \\ \hline
$T_{\text{total}}$                                            & 0.7                                            & 1.7                                             & 5.1                                              & 9.2                                           & 2.9                                         & 3.5                                       & 7.8                                            & 17.8                                           &  78.1                                        & 30.6                                              & 98.4                                           \\ \hline
$F$                                             & 38$\pm$5                                            &34$\pm$2                                            & 32$\pm$2                                               & 30$\pm$4                                        & 82$\pm$5                                          & 70$\pm$4                                             & 63$\pm$2                                              & 60$\pm$2                                              & 58$\pm$3                                            & 68$\pm$3                                               & 58$\pm$7                                           \\ \hline
\end{tabular}
\end{table*}


In this section, we present numerical experiments that illustrate the performance of Algorithm \ref{alg:AIA} and show that it can solve large-scale estimation tasks that are computationally challenging to solve using existing centralized methods; see e.g., \cite{kantaros2019asymptotically}. 
%
Specifically, first, we examine the scalability of Algorithm \ref{alg:AIA} for various numbers of robots and landmarks. 
%
We also illustrate the benefit of online re-planning
%show that dynamically updating the targets assigned to the robots and accordingly re-planning results in significant performance gains in terms of the terminal horizon (i.e., the time required to solve the corresponding AIA task) 
compared to offline planning (see Remark \ref{rem:onlineRe}) and investigate the effect of communication on the terminal horizon. Numerical experiments related to mobile landmarks are also provided.
 % such as greedy, (nonmyopic) optimal, or other sampling-based approaches; see Section \ref{sec:comp}. %Finally, we examine the optimality of Algorithm \ref{alg:RRT}; see Section \ref{sec:opt}.
The sampling-based AIA algorithm \cite{kantaros2019asymptotically} is implemented as discussed in Remark \ref{rem:implem} using the biased density functions $f_{\ccalV}$ and $f_{\ccalU}$ designed in \cite{kantaros2019asymptotically} with parameters $p_{\ccalV}=p_{\ccalU}=0.9$. All case studies have been implemented using MATLAB 2016b on a computer with Intel Core i7 3.1GHz and 16Gb RAM. Simulation videos can be found in \cite{sim_AIA}.

%\subsection{Robot Dynamics \& Sensors}\label{sec:rmodel}
%Throughout this section, we consider robots that reside in a non-convex environment $\Omega\subset\mathbb{R}^2$ with obstacles; see e.g., Figure \ref{fig:traj15s}. Also, 

{\bf{Robot Dynamics \& Sensors:}} Throughout this section, we consider robots with differential drive dynamics, where $\bbp_j(t)$ captures both the position and the orientation of the robots. Specifically, the available motion primitives are $u\in\{0,0.1\}\text{m/s}$ and $\omega\in\set{0,5, 10, \dots, 350, 355}\text{deg/s}$.
%
%The linear dynamics are defined as  
%\begin{equation}\label{eq:linRbt}
%\bbp_j(t+1)=\bbp_j(t)+\bbu_j(t),
%\end{equation}
%where $\bbp_j(t)\in\mathbb{R}^2$ denotes the position of robot $j$, and 
%$\left\lVert\bbu_j(t) \right\rVert\in\{0, 0.2\}$, for all robots $j$.
%The nonlinear dynamics are defined as 
%\footnotesize{
%\begin{equation}\label{eq:nonlinRbt}
%\begin{bmatrix}
%   p_j^1(t+1) \\
%  p_j^2(t+1)\\
%  \theta_j(t+1)
%  \end{bmatrix}=  
%  \begin{bmatrix}
%   p_j^1(t) \\
%  p_j^2(t)\\
%  \theta_j(t)
%  \end{bmatrix}+ 
%   
%   \begin{cases}
%        \begin{bmatrix}
%   \tau u \cos(\theta_j(t)+\tau\omega/2) \\
%   \tau u \sin(\theta_j(t)+\tau\omega/2)\\
%  \tau  \omega
%  \end{bmatrix}, \text{if} ~\tau\omega<0.001\\
%  \\
% \begin{bmatrix}
%   \frac{u}{\omega} (\sin(\theta_j(t)+\tau\omega)-\sin(\theta_j(t))) \\
%   \frac{u}{\omega} (\cos(\theta_j(t)) - \cos(\theta_j(t)+\tau\omega)) \\
%  \tau \omega
%  \end{bmatrix}, \text{else},
%    \end{cases}      
%\end{equation}}
%\normalsize
%where $u\in\{0,0.2\}\text{m/s}$ and $\omega\in\set{0,\pm \pi/4,\pm \pi/2, \pm \pi/1.33, \pm \pi}$. Note in \eqref{eq:nonlinRbt}, that the state $\bbp_j(t)$ includes both the position $[p_j^1(t),p_j^2(t)]^T$ and the orientation  $\theta_j(t)$ of the robots, i.e., $\bbp_j(t)=[p_j^1(t),p_j^2(t),\theta_j(t)]^T$.
%
Moreover, we assume that the robots are equipped with omnidirectional, range-only, sensors with limited range of $0.4$m while they reside in $10\times10$ workspace. Every robot $j$ can generate measurements associated with landmark $i$ as per the model $y_{j,i} = \ell_{j,i}(t) + v(t) \ ~\mbox{if}~ \ (\ell_{j,i}(t) \leq 2)$,
%\begin{equation}\label{eq:meassim}
%y_{j,i} = \ell_{j,i}(t) + v(t) \ ~\mbox{if}~ \ (\ell_{j,i}(t) \leq 2) \wedge (i\in\texttt{FOV}_j).
%\end{equation}
%
where $\ell_{j,i}(t)$ is the distance between landmark $i$ and robot $j$, and $v(t) \sim \ccalN(0,\sigma^2(\bbp_j(t),\bbx_i(t)))$ is the measurement noise. Also, we model the measurement noise so that $\sigma$ increases linearly with $\ell_{j,i}(t)$, with slope $0.25$, as long as $\ell_{j,i}(t)\leq 2$; if $\ell_{j,i}(t)> 2$, then $\sigma$ is infinite. Observe that this observation model is nonlinear and, therefore, the separation principle, discussed in Section \ref{sec:PF}, does not hold. Thus, we execute the sampling-based algorithm to solve the local sub-problems \eqref{eq:LocalProbb2} using the linearized observation model about the estimated landmark positions. Also, the robots with no assigned landmarks, i.e., the robots with $\ccalA_j(t)=\emptyset$, navigate the environment so that they maximize an area coverage metric that captures the  region that lies within the sensing range of all robots \cite{Cortes_ESAIMCOCV05}. The latter forces these robots to spread in the environment so that landmarks eventually reside within their region of responsibility distributing the burden of active information gathering across the robots. %; see also Section \ref{sec:vor}.

%Note that, similar to \cite{atanasov2014information}, Algorithm \ref{alg:RRT} can be coupled with a Model Predictive Control approach where the robots redesign their paths every few measurements, to generate adaptive sensor policies. 
%Nevertheless, in Sections \ref{sec:scale} and \ref{sec:opt} we show that Algorithm \ref{alg:RRT} can still synthesize high-quality or even optimal paths. Moreover, similar to \cite{atanasov2014information}, the robots can redesign their paths every few measurements


%\red{say  here that assumption 2.1 does not hold any more (nonlin obs model). also say that the position terminal constraint is ignored here. also briefly discuss the MPC idea due to nonliearities}
%Also, we show that the state-space, for all considered case studies,  that has to be searched is too large to explore using random-walk or greedy approaches or existing decentralized active information gathering methods \red{[RIV]}. 




%\tiny{
%\begin{table}[t]
%\caption{Scalability Analysis}
%\label{tab:comp}
%\begin{center}
%\renewcommand{\arraystretch}{1.5}
%\begin{tabular}{c|c|c|c|c||c|c|c|}
%	\cline{2-7}
%    	\multirow{2}{*}{}		&  \multicolumn{1}{|c|}{}      & \multicolumn{3}{c||}{Linear Robot Dynamics}						&	\multicolumn{3}{c|}{Nonlinear Robot Dynamics}					\\ \cline{1-7} &  N/M		&	Runtime		&	$n$		& Cost~/~F		&	Runtime		&	$n$		& Cost~/~F	\\  \hline				
%\multicolumn{2}{|c|}{1/5}		& 7.83 secs	& 141	& 22.20/120 	& 12.71 secs	& 146	& 24.16/133 \\ \hline
%\multicolumn{2}{|c|}{10/10 }			& 25.32 secs	& 53	& 11.79 / 47		& 55.97 secs	 & 72 & 14.44 / 52 \\ \hline		
%\multicolumn{2}{|c|}{10/20 }			& 27.33 secs	& 51	&  25.12 / 47		& 56.86 secs	 & 88 & 39.35 \ 77 \\ \hline	
%\multicolumn{2}{|c|}{10/35 }			& 27.87 secs & 68	& 44.79 / 	61 	& 58.52 secs	 & 88 & 55.58 / 77 \\ \hline	
%\multicolumn{2}{|c|}{15/20 }			& 41.18 secs	& 48	& 22.85/ 42	& 1.84 mins	 & 68 & 29.78 / 60 \\ \hline	
%\multicolumn{2}{|c|}{15/35 }			& 55.6 secs	& 54	& 36.94/48		& 2.1 mins	 & 82 &49.16 / 68 \\ \hline	
%\multicolumn{2}{|c|}{20/20 }			& 43.41 secs	& 52 	& 21.96 / 46		& 1.64 mins	 & 74 & 31.21 / 59 \\ \hline	
%\multicolumn{2}{|c|}{20/25 }			& 20.9 secs	& 23	& 13.12 / 21		& 1.43 mins	 & 65 & 38.87 / 59 \\ \hline	
%\multicolumn{2}{|c|}{20/35 }			& 42.93 secs	& 46	& 33.20 / 44		& 1.57 mins	 & 66 & 47.8 / 58 \\ \hline	
%\end{tabular}
%\end{center}
%\end{table}}

\begin{figure}[t]
  \centering
%\subfigure[$N/M=1/5$, Cost = $34.47$, $F=374$,  Runtime = 23.74secs]{
%\label{fig:traj15f}
%\includegraphics[width=0.45\linewidth]{figures/traj_1vs5_fast.pdf}}
%
\subfigure[$t=0$]{
    \label{fig:t0}
  %\includegraphics[width=0.45\linewidth]{traj_10vs35.pdf}
  \includegraphics[width=0.45\linewidth]{figures/time1_50_100.pdf}}
 %
% \subfigure[$N/M=1/5$, Cost = $75.03$, $F=374$,  Runtime = 4.19 mins]{
%    \label{fig:biasedGreedy15}
%  \includegraphics[width=0.45\linewidth]{figures/biasedGreedy.pdf}}
   \subfigure[$t=30$]{
    \label{fig:t30}
  \includegraphics[width=0.45\linewidth]{figures/time30_50_100.pdf}}
%\subfigure[$t=40$]{
 %   \label{fig:t40}
%  \includegraphics[width=0.45\linewidth]{figures/time40_50_100.pdf}}
\subfigure[$t=50$]{
    \label{fig:t50}
  \includegraphics[width=0.45\linewidth]{figures/time50_50_100.pdf}}
 %    \subfigure[$t=65$]{
%   \label{fig:t65}
%  \includegraphics[width=0.45\linewidth]{figures/time65_50_100.pdf}}
     \subfigure[Robot Paths]{
    \label{fig:pathsI}
  \includegraphics[width=0.45\linewidth]{figures/paths50_100.pdf}}
%\subfigure[$N=1, M=5$ (infeasible)]{
%    \label{fig:traj15inf}
%\includegraphics[width=0.45\linewidth]{infeasProb_traj.pdf}}
  \caption{Landmark localization scenario: Figures \ref{fig:t0}-\ref{fig:t50} show the configurations of $N=20$ robots at various time instants towards localizing $M=100$ static landmarks. The red diamonds and cyan squares correspond to accurately localized and non-localized landmarks, respectively. The blue and green stars correspond to robots that navigate for information gathering and area coverage purposes, respectively. The circle centered at each robot position illustrates the sensing range while the gray segments depict the Voronoi cells. Figure \ref{fig:pathsI} shows the robot paths where the green and red squares denote the initial and final robot positions.}
  \label{fig:caseI}
\end{figure}

\begin{figure}[t]
  \centering
%\subfigure[$N/M=1/5$, Cost = $34.47$, $F=374$,  Runtime = 23.74secs]{
%\label{fig:traj15f}
%\includegraphics[width=0.45\linewidth]{figures/traj_1vs5_fast.pdf}}
%
\subfigure[Deployment 1]{
    \label{fig:depl1}
  %\includegraphics[width=0.45\linewidth]{traj_10vs35.pdf}
  \includegraphics[width=0.45\linewidth]{figures/Init1.pdf}}
 %
% \subfigure[$N/M=1/5$, Cost = $75.03$, $F=374$,  Runtime = 4.19 mins]{
%    \label{fig:biasedGreedy15}
%  \includegraphics[width=0.45\linewidth]{figures/biasedGreedy.pdf}}
   \subfigure[Deployment 2]{
    \label{fig:depl2}
  \includegraphics[width=0.45\linewidth]{figures/Init2.pdf}}
 \caption{Graphical depiction of initial multi-robot deployments in Table \ref{ta:vor}. The third initial deployment in Table \ref{ta:vor} differs from the second one only in that the y-coordinate of all robot positions is is $0.1$m.}
  \label{fig:configInit}
\end{figure}

%\subsection{Scalability Analysis}\label{sec:scale}
{\bf{Scalability Analysis:}} First, we examine the scalability performance of  Algorithm \ref{alg:AIA} with respect to the number of robots and the number of landmarks. The results are summarized in Table \ref{tab:scale}. In all case studies of Table \ref{tab:scale}, the parameter $\delta$ is selected to be $\delta=1.8\times10^{-6}$, for all $i\in\ccalM$, while all robots initially reside in the bottom-left corner of the $10\text{m}\times10\text{m}$ environment shown in Figure \ref{fig:caseI}. % and  $\ccalP_j^{\text{goal}}$ is selected to be $\ccalP_j^{\text{goal}}=\Omega_{\text{free}}$, for all $j\in\ccalN$.
%
In Table \ref{tab:scale} the first line corresponds to the number of robots and landmarks. In the second line, $T_{\text{plan}}$ refers to the average runtime in seconds required for a robot to compute a control action regardless of their role in the workspace (see lines \ref{aia:cntrl1} and \ref{aia:cntrl2} in Alg. \ref{alg:AIA}). Similarly, $T_{\text{vor}}$ shows the average runtime in seconds to compute the Voronoi cells per iteration of Algorithm \ref{alg:AIA} (see line \ref{aia:vor} in Alg. \ref{alg:AIA}). Note that in our implementation, the Voronoi tessellation has been computed in a centralized fashion and, therefore, the corresponding runtime increases as the number of robots increases. Nevertheless, this runtime is always quite small and, therefore, the Voronoi partitioning does not compromise scalability. In the third and fourth row, $T_{\text{total}}$ and $F$ refer to the mean total runtime in minutes and total number of discrete time instants of $10$ simulations, along with the respective standard deviation, required to find the first feasible solution. Note that Algorithm \ref{alg:AIA} has not been implemented in parallel across the robots; instead, in our implementation the robots make local  but sequential decisions, which explains the increasing runtime $T_{\text{total}}$ as the number $N$ of robots increases. 
%
Observe in Table \ref{tab:scale} that for a given number of landmarks, increasing the number of robots tends to decrease the terminal horizon. Note that the terminal horizon depends on the initial robot configuration. For instance, assuming $N$ robots that are initially uniformly distributed and $M=100$ landmarks, the terminal horizon when $N=20$ and $N=100$ is $35\pm3$ and $15\pm2$, respectively.
%
Finally, observe that the proposed algorithm can solve estimation tasks that involve hundreds of robots and landmarks, a task that is particularly challenging for existing methods; see e.g., the numerical experiments in \cite{kantaros2019asymptotically}. Figure \ref{fig:caseI} shows the paths that $20$ robots followed to localize $M=100$ landmarks. Observe in this figure that the robots dynamically switch roles in the environment. 

%Observe in Table \ref{tab:scale} that Algorithm \ref{alg:RRT} can design feasible paths very fast even for large number of robots and targets regardless of the robot dynamics; see also Figure \ref{fig:traj1020}. Finally, we also applied Algorithm \ref{alg:RRT} to a scenario where a team of $N=7$ differential drive robots should localize and track $M=20$ targets in a significantly larger workspace, such as a residential area, with dimensions $500\text{m}\times1000\text{m}$. In this scenario, the sensing range of the robots is $20\text{m}$, and the motion primitives are selected as $u\in\{0,2\}\text{m/s}$ and $\omega\in\set{0,\pm \pi/4,\pm \pi/2, \pm \pi/1.33, \pm \pi}\text{rad/s}$. Algorithm \ref{alg:RRT} generated robot paths in $12.23$ \text{mins} with terminal horizon $F=3769$ that are depicted in Figure \ref{fig:largeSpace}.

%\subsection{Online vs Offline Planning}\label{sec:vor}
{\bf{Online vs Offline Planning:}} Second, we examine the effect of dynamically updating the Voronoi partitioning - and, consequently, the landmarks assigned to the robots - and accordingly re-planning. The results are summarized in Table \ref{ta:vor} and pertain to a case study with $N=5$ and $M=100$. In Table \ref{ta:vor}, the first row corresponds to three different initial configurations illustrated in Figure \ref{fig:configInit}.  The second and the third row show the mean terminal planning horizon $F_{\text{offline}}$ and $F_{\text{online}}$ of $10$ simulations required to localize all landmarks without and with re-planning, respectively. %(i.e., all robots follow the paths designed offline at time $t=0$) and with re-planning as per Algorithm 1.
%fixed Voronoi cells (as computed at $t=0$) and dynamic Voronoi cells that are continuously updated, respectively.
Observe that the total time is always larger when offline planning is considered. This becomes more pronounced in configuration 1 (Fig. \ref{fig:depl1}), as there are robots that have to stay within a small region the whole time which is not the case when online re-planning is considered due to its adaptive nature. As a result, in an online setting the burden of localizing all $M$ landmarks is shared among all robots resulting in accomplishing the AIA task sooner.


{\bf{Effect of Communication:}} Third, we evaluate the effect of all-time and all-to-all communication among the robots on the estimation performance during online planning. Specifically, here we consider a scenario with $N=50$ robots and $M=100$ static landmarks and we assume that communication occurs intermittently and periodically, i.e., every $T>0$ time units. We observed that increasing the period $T$ results in longer terminal planning horizons $F$, as expected, since the robots plan paths without always having access to global estimates of the hidden state. In particular, for $T=1$ (all-time communication), $T=2$, $T=10$, and $T=15$, the average planning horizon of $10$ simulation studies was $63$, $70$, $125$, and $150$, respectively.

%In this section, we examine the effect of dynamically updating the Voronoi partitioning - and, consequently, the landmarks assigned to the robots - and accordingly re-planning. The results are summarized in Table \ref{ta:vor} where the first row corresponds to the number of robots and landmarks. The second and third row show the total number of discrete time instants $F_{\text{offline}}$ and $F_{\text{online}}$ required to localize all landmarks with no re-planning (i.e., all robots follow the paths designed offline at time $t=0$) and with re-planning.
%fixed Voronoi cells (as computed at $t=0$) and dynamic Voronoi cells that are continuously updated, respectively.
%Observe that the total time is always smaller when online re-planning is considered. The reason is that in the latter case as the robots - that are not responsible for any landmark - spread in the environment to maximize area coverage, they approach non-localized landmarks that fall within their region of responsibility. As a result, the burden of localizing all $M$ landmarks is shared among all robots resulting in accomplishing the AIA sooner. %Recall that updating the Voronoi cells may sacrifice completeness of Algorithm \ref

\begin{table}[]
\caption{Online vs Offline Planning}
\label{ta:vor}
\centering
\begin{tabular}{|l|l|l|l|}
\hline
N=5, M=100     & Deployment 1 & Deployment 2 & Deployment 3 \\ \hline
$F_{\text{offline}}$ & 782 $\pm$  44    & 190 $\pm$ 30     & 210 $\pm$ 30       \\ \hline
$F_{\text{online}}$  & 141 $\pm$ 16     & 137 $\pm$ 8      & 146 $\pm$ 26     \\ \hline
\end{tabular}
\end{table}

%\subsection{Extensions to Mobile Landmarks}\label{sec:mobile}

{\bf{AIA with Drones:}} Algorithm \ref{alg:AIA} generates paths that respect the robot dynamics as captured in \eqref{constr34}. A common limitation of sampling-based algorithms is that the more complex the robot dynamics is, the longer it takes to generate feasible paths; see e.g., \cite{kantaros2019asymptotically}. To mitigate this issue, an approach that we investigate in this case study is to generate paths for simple robot dynamics that need to be followed by robots with more complex dynamics. Particularly, in this section, we present simulation studies that involve a team of $N=30$ AsTech Firefly Unmanned Aerial Vehicles (UAVs) with range limited field of view equal to $10$m that operate in an environment with dimensions $200\text{m}\times 200 \text{m}$ occupied by $M=50$ static landmarks; see Figure \ref{fig:drones}.

\begin{figure}[t]
  \centering
    \subfigure[$t=0$]{
    \label{fig:t01}
    \includegraphics[width=0.48\linewidth]{figures/1.png}}
     \subfigure[]{
    \label{fig:t21}
  \includegraphics[width=0.48\linewidth]{figures/2.png}}
       \subfigure[]{
    \label{fig:t31}
  \includegraphics[width=0.48\linewidth]{figures/3.png}}
 %      \subfigure[$t=73$]{
 %   \label{fig:t73d}
%  \includegraphics[width=0.45\linewidth]{figures/time73_50_100_dyn.pdf}}
     \subfigure[]{
    \label{fig:t41}
  \includegraphics[width=0.48\linewidth]{figures/4.png}}
%\subfigure[$N=1, M=5$ (infeasible)]{
%    \label{fig:traj15inf}
%\includegraphics[width=0.45\linewidth]{infeasProb_traj.pdf}}
 \caption{Landmark localization scenario: Figures \ref{fig:t01}-\ref{fig:t41} show successive snapshots of a team of $N=30$ UAVs with limited field of view (colored disks) towards localizing $M=50$ landmarks (red spheres). %The red diamonds and cyan squares correspond to accurately localized and non-localized targets, respectively. The blue and green stars correspond to robots that navigate for information gathering and area coverage purposes, respectively. The circle centered at each robot position illustrate the sensing range while the gray segments depict the Voronoi cells. 
 The red ellipses denote the uncertainty about the landmark positions. The full video can be found in \cite{sim_AIA}.}
  \label{fig:drones}
\end{figure}

The initial configuration of the UAVs and the landmarks are shown in Figure \ref{fig:t01}. Given the paths generated by Algorithm \ref{alg:AIA} considering differential drive dynamics, we compute minimum jerk trajectories, defined by fifth-order polynomials, that connect consecutive waypoints in the nominal paths. To determine the coefficients of this polynomial, we impose boundary conditions on the UAV positions that require the travel time between consecutive waypoints in the nominal paths to be $T=2$ seconds for all UAVs \cite{lavalle2006planning}. %; see Figure \ref{fig:sync}. 
%Note that the minimum jerk trajectories are smooth enough for the UAVs to follow.  Observe in Figure \ref{fig:paths} that deviation between the nominal paths generated by Algorithm \ref{alg:RRT} and the minimum jerk paths is quite small. %and, in fact, the latter paths still satisfy the assigned specification.
%
The UAVs are controlled to follow the resulting trajectories using the ROS package developed in \cite{Furrer2016}. Snapshots of the UAVs navigating the environment to localize all landmarks are presented in Figure \ref{fig:drones}.

{\bf{Mobile Landmarks:}} Finally, we illustrate the performance of Algorithm \ref{alg:AIA} in an environment with mobile landmarks. Specifically, we consider $M=100$ landmarks, among which $8$ are governed by noisy linear time invariant dynamics in the form of $\bbx_i(t+1)=\bbA_i\bbx_i(t)+\bbB_i\bba_i(t)+\bbw_i(t)$ and the rest are static. The trajectories of all landmarks and robots are illustrated in Figure \ref{fig:caseId}. Observe in this figure that because of the dynamic nature of the landmarks, there are landmarks that need to be revisited to decrease their uncertainty giving rise to target tracking behaviors; see e.g., landmark $95$ in Figures \ref{fig:t50d} and \ref{fig:t60d}. We note that although Algorithm \ref{alg:AIA} is not complete in the presence of dynamic hidden states, it was able to find feasible controllers for a large team of robots and landmarks. %Also, note that in this case study a Voronoi decomposition of the environment may not result in a `fair' decomposition of the global AIA task across the robots as it does not account the 
\begin{figure}[t]
  \centering
%\subfigure[$N/M=1/5$, Cost = $34.47$, $F=374$,  Runtime = 23.74secs]{
%\label{fig:traj15f}
%\includegraphics[width=0.45\linewidth]{figures/traj_1vs5_fast.pdf}}
%
\subfigure[$t=0$]{
    \label{fig:t0d}
  %\includegraphics[width=0.45\linewidth]{traj_10vs35.pdf}
  \includegraphics[width=0.45\linewidth]{figures/time1_50_100.pdf}}
 %
% \subfigure[$N/M=1/5$, Cost = $75.03$, $F=374$,  Runtime = 4.19 mins]{
%    \label{fig:biasedGreedy15}
%  \includegraphics[width=0.45\linewidth]{figures/biasedGreedy.pdf}}
%   \subfigure[$t=30$]{
%    \label{fig:t30d}
%  \includegraphics[width=0.45\linewidth]{figures/time40_50_100_dyn.pdf}}
     \subfigure[$t=50$]{
    \label{fig:t50d}
  \includegraphics[width=0.45\linewidth]{figures/time50_50_100_dyn.pdf}}
       \subfigure[$t=60$]{
    \label{fig:t60d}
  \includegraphics[width=0.45\linewidth]{figures/time60_50_100_dyn.pdf}}
 %      \subfigure[$t=73$]{
 %   \label{fig:t73d}
%  \includegraphics[width=0.45\linewidth]{figures/time73_50_100_dyn.pdf}}
     \subfigure[Robot \& Landmark Paths]{
    \label{fig:pathsId}
  \includegraphics[width=0.45\linewidth]{figures/paths50_100_dyn_v2.pdf}}
%\subfigure[$N=1, M=5$ (infeasible)]{
%    \label{fig:traj15inf}
%\includegraphics[width=0.45\linewidth]{infeasProb_traj.pdf}}
 \caption{Target tracking and localization scenario: Figures \ref{fig:t0d}-\ref{fig:t60d} show the configurations of $N=20$ robots at various time instants towards localizing $M=100$ landmarks among which $8$ are mobile and the rest are static. %The red diamonds and cyan squares correspond to accurately localized and non-localized targets, respectively. The blue and green stars correspond to robots that navigate for information gathering and area coverage purposes, respectively. The circle centered at each robot position illustrate the sensing range while the gray segments depict the Voronoi cells. 
 Figure \ref{fig:pathsId} shows the robot and target paths. The green circles and red squares denote the initial and final robot positions while the magenta diamonds and blue stars denote the initial and final landmark locations. Static landmarks are shown with blue stars.}
  \label{fig:caseId}
\end{figure}
%\subsection{Unknown Number of Landmarks}
%\textcolor{red}{If time and space permit, we can add this subsection...}

%\subsection{Gazebo Simulations(?)}\label{sec:gaz}
%\textcolor{red}{here we need to add a couple of gazebo simulations }



%\textcolor{red}{here we need to add simulations related to at least one the 'extensions': unknown landmarks or mobile targets, or both?}





==> Technical Report- Scalable Active Information Acquisition - FinalSubmission/files/targetTracking.tex <==
In this section, we consider an application to target localization and tracking for Algorithm \ref{alg:RRT}. In this scenario, the hidden state $\bbx(t)$ is created by stacking the positions of all targets at time $t$, i.e., $\bbx(t)=[\bbx_1^T(t),\bbx_2^T(t),\dots,\bbx^T_M(t)]^T$, where $\bbx_i(t)$ is the position of target $i\in\ccalM:=\{1,\dots,M\}$ at time $t$ and $M>0$ is the number of targets. We require the constraint \eqref{constr22} to hold for all states $\bbx_i(F)$, for some $\delta_i$.
%
As discussed in Section \ref{sec:samplingAlg}, any density functions $f_{\ccalV}$ and $f_{\ccalU}$ that satisfy Assumptions \ref{frand} and \ref{fnew} can be employed to generate states $\bbq_{\text{new}}(t)$ in Algorithm \ref{alg:RRT}. In what follows, we design density functions that allow us to address large-scale estimation tasks that involve large teams of robots and targets. The main idea is to build $f_{\ccalV}$ and $f_{\ccalU}$ so that the tree is biased to explore regions of $\Omega_{\text{free}}$ where targets are predicted to be. 

\subsection{Density Function $f_{\ccalV}$} \label{sec:frand}
Let $L(\bbq)$ denote the length (number of hops) of the path that connects the node $\bbq\in\ccalV$ to the root $\bbq(0)$ of the tree. Let also $L_{\text{max}}$ denote the maximum $L(\bbq)$ among all nodes $\bbq\in\ccalV$, i.e.,
$L_{\text{max}}=\max_{\bbq\in\ccalV} L(\bbq)$. Hereafter, we denote by $\ccalL_{\text{max}}$ the set that collects all nodes $\bbq\in\ccalV$ that satisfy $L(\bbq)=L_{\text{max}}$, i.e., $\ccalL_{\text{max}}=\set{\bbq\in\ccalV~|~L(\bbq)=L_{\text{max}}}$.
%
Given the set $\ccalL_{\text{max}}$, we construct the density function $f_{\ccalV}$ so that it is biased to select subsets $\ccalV_k\subseteq\ccalV$ that contain at least one node $\bbq\in\ccalV$ that  belongs to $\ccalL_{\text{max}}$. Specifically, $f_{\ccalV}(k|\ccalV)$ is defined as follows

\begin{equation}\label{eq:frand}
f_{\ccalV}(k|\ccalV)=\left\{
                \begin{array}{ll}
                  p_{\ccalV}\frac{1}{|\ccalK_{\text{max}}|}, ~~~~~~~~~~~~\mbox{if}~k\in\ccalK_{\text{max}}\\
                  (1-p_{\ccalV})\frac{1}{|\ccalV\setminus\ccalK_{\text{max}}|},~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
where % (i) $\ccalL_{\text{max}}\subseteq\ccalV$ is a set that collects the leaf nodes that have the longest path to the root among all other leaf nodes, 
(i) $\ccalK_{\text{max}}$ is a set that collects the indices $k$ of the subsets $\ccalV_k$ that satisfy $\ccalV_k\cap\ccalL_{\text{max}}\neq\emptyset$, and (ii) $p_{\ccalV}\in(0.5,1)$ stands for the probability of selecting \textit{any} subset $\ccalV_k$ that satisfies $\ccalV_k\cap\ccalL_{\text{max}}\neq\emptyset$. Note that $p_{\ccalV}$ can change with iterations $n$ but it should always satisfy $p_{\ccalV}\in(0.5,1)$ to ensure that subsets $\ccalV_k$ with $\ccalV_k\cap\ccalL_{\text{max}}\neq\emptyset$ are selected more often. 

\subsection{Density Function $f_{\ccalU}$}\label{sec:fnew_target}

The density function $f_{\ccalU}$ is designed so that control inputs $\bbu_j$ that drive robot $j$ towards regions that are predicted to be informative are selected more often. Specifically, given a state $\bbq_{\text{rand}}(t)\in\ccalV_{k_{\text{rand}}}$, where $k_{\text{rand}}$ is sampled from $f_{\ccalV}(k|\ccalV)$, we design $f_{\ccalU}(\bbu|\bbq_{\text{rand}}(t))$ as follows.
The construction of $f_{\ccalU}(\bbu|\bbq_{\text{rand}}(t))$ presumes that targets are assigned to each robot, when the robots are in state $\bbq_{\text{rand}}(t)$; the target assignment process is described in Section \ref{sec:targetAs}. Given the assigned targets, $f_{\ccalU}$ is designed so that control inputs $\bbu_j$ that minimize the \textit{geodesic distance} (see e.g., \cite{kantaros2016global}) between the next robot position $\bbp_{j}(t+1)=\bbf_j(\bbp_{j,\text{rand}}(t),\bbu_j)$ and the predicted position of target $j$, denoted by $\hat{\bbx}_i(t+1)$, are selected more often. Note that the predicted position $\hat{\bbx}_i(t+1)$ can be computed using, e.g., the Kalman filter prediction  step. Specifically, $f_{\ccalU}$ is defined as $f_{\ccalU}(\bbu|\bbq_{\text{rand}}(t))= \prod_{j\in\ccalN} f_{\ccalU}^j(\bbu_j)$, where $f_{\ccalU}^j(\bbu_j)$ is constructed as follows.
\begin{equation}\label{eq:fnew}
f_{\ccalU}^j(\bbu_j)=\left\{
                \begin{array}{ll}
                  p_{\ccalU}, ~~~~~~~~~~~~\mbox{if}~(\bbu_j=\bbu_j^*)\wedge(d_{ij} >R_j)\\
                  (1-p_{\ccalU})\frac{1}{|\ccalU_j|},~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
%\hat{\bbx}_i(t+1) - \bbp_j(t+1) \right\rVert_2
%rrt condiotion for steering function here...
where (i) $d_{ij}=\left\lVert\hat{\bbx}_i(t+1) - \bbp_j(t+1) \right\rVert_2$ and $i$ is the index of the target assigned to robot $j$, (ii) $R_j$ denotes the sensing range of robot $j$, and (iii) $\bbu_j^{*}\in\ccalU_j$ is the control input that minimizes the geodesic distance between $\bbp_j(t+1)$ and $\hat{\bbx}_i(t+1)$, i.e., $\bbu_j^*=\argmin_{\bbu_j\in\ccalU_j} \left\lVert \hat{\bbx}_i(t+1) - \bbp_j(t+1) \right\rVert_g,$
%\begin{equation}\label{eq:ujstar}
%\bbu_j^*=\argmin_{\bbu_j\in\ccalU_j} \left\lVert \hat{\bbx}_i(t+1) - \bbp_j(t+1) \right\rVert_g,
%\end{equation}
 where $\left\lVert \cdot \right\rVert_g$ denotes the geodesic norm/distance. Observe that the density functions \eqref{eq:frand} and \eqref{eq:fnew} satisfy Assumptions \ref{frand} and \ref{fnew}, respectively, by construction. 
 %
In words, \eqref{eq:fnew} selects more often control inputs that drive the robots close to the predicted positions $\hat{\bbx}_i(t+1)$ of their corresponding assigned targets $i$, until these predicted positions are within the robots' sensing range. Once this happens, controllers are selected randomly. %In fact, the control input \eqref{eq:ujstar} "convexifies"\BS{What is meant by this statement? Do you just mean that the field of view constraint is now satisfied? } planning in the vicinity of every robot and decreases the rate at which samples $\bbp_{\text{new}}$ are rejected due to collisions with obstacles.

Finally, observe that \eqref{eq:fnew} is designed independently of the sensor models. Alternative density functions $f_{\ccalU}$ can also be proposed in place of \eqref{eq:fnew} that exploit the sensor model. For instance, in case of a bearing sensor or monocular camera, it may be desirable to select control inputs that drive the robots around their assigned targets, once the latter are inside the field-of-view of the corresponding robots (instead of selecting random control inputs); however, such a design process will be explored in the future.
 
 
%In case of the nonlinear dynamics in \eqref{eq:nonlinDynamics}, there may not exist such a control input $\bbu_j^{*}\in\ccalU_j$. In this case, we pick the control action that adjusts the heading $\theta_j(t+1)$, so that it is aligned along the geodesic path that connects $\bbp_j(t+1)$ to $\hat{\bbx}_i(t+1)$ \cite{kantaros2016global}....

\begin{rem}[On-the-fly update of sampling strategy]
Note that once a feasible solution to \eqref{eq:Prob2} is found, or after a user-specified number of iterations, we can switch to uniform density functions by selecting $p_{\ccalU}=p_{\ccalV}=0$ that promote random exploration, or to any other density function. Recall that the theoretical guarantees provided in Section \ref{sec:complOpt} hold even if the density functions $f_{\ccalV}$ and $f_{\ccalU}$ change with iterations $n$ of Algorithm \ref{alg:RRT}, as long as Assumptions \ref{frand} and \ref{fnew} are always satisfied.
\end{rem} 
 
 
%\begin{rem}[Deterministic strategies]
%Deterministic strategies can also be developed to build trees $\ccalG$ so that the nodes that are closer to their assigned targets are extended more often towards them than other nodes. Such approaches would require to store a set $\ccalU_{\bbq}\subseteq\ccalU$ that collects the control inputs that have not been applied to $q\in\ccalV$ yet, for each node $q\in\ccalV$. This way, a control input $\bbu$ is selected from $\ccalU_{\bbq}$ (instead of $\ccalU$ as in Alg. \ref{alg:RRT}), when $q\in\ccalV$ is selected to be extended. This would guarantee that the optimal solution can be found within a finite number of iterations. However, such an approach would require excessive memory requirements as the number of robots increases and the tree grows. 
%\end{rem}

 
 
\subsection{On-the-fly Target Assignment}\label{sec:targetAs}
In what follows, we describe the target assignment process that is executed every time a state $\bbq_{\text{new}}(t+1)=[\bbp_{\text{new}}(t+1),\Sigma_{\text{new}}(t+1)]$ is added to the tree; see also Algorithm \ref{alg:assignment}. The goal of Algorithm \ref{alg:assignment} is to assign targets to each robot when they are in the state $\bbq_{\text{new}}(t+1)$. Specifically, for each state $\bbq(t)\in\ccalV$, we construct a function $s_{\bbq}:\ccalN\to\ccalM$ that assigns to each robot $j\in\ccalN$ a single target $i\in\ccalM$. Hereafter, we denote by $s_{\bbq}(j)$ the target that is assigned to robot $j$ in state $\bbq(t)$. Recall from Section \ref{sec:fnew_target}, that the assigned targets associated with the state $\bbq_{\text{rand}}(t)$ are used to construct $f_{\ccalU}(\bbu|\bbq_{\text{rand}}(t))$. %Hereafter, we drop the dependence of $t$ for simplicity of notations. %In Algorithm \ref{alg:assignment}, the targets that are assigned to the robots when they are in a state $\bbq(t)$ are captured by the vector $\bbs_{\bbq(t)}\in\mathbb(R)^N$. 

\begin{algorithm}[t]
\footnotesize
\caption{On-the-fly Target Assignment}
\LinesNumbered
\label{alg:assignment}
\KwIn { (i) $s_{\bbq_{\text{rand}}}$, (ii) $\det\Sigma(F)$ \& $\delta_i, \forall i\in\ccalM$}
\KwOut {$s_{\bbq_{\text{new}}}:\ccalN\to\ccalM$}
  $s_{\bbq_{\text{new}}}=s_{\bbq_{\text{rand}}}$\;\label{as:init}
 Compute set $\ccalD$ of robots that are candidate to update their assigned targets\;\label{as:D}
 Initialize set of targets to be assigned to robots as $\ccalT_{\text{to-assign}}=\ccalM\setminus\set{\ccalT_{\text{as}}\cup\ccalT_{\text{sat}}}$\; \label{as:Tassign}
\If {$\ccalT_{\text{to-assign}}=\emptyset$}{\label{as:Tassign2}
 $\ccalT_{\text{to-assign}}=T_{\text{unsat}}$\;\label{as:Tassign3}}
%if empty go to goal regions
\For {$j\in\ccalD$}{\label{as:as1}
 $s_{\bbq_{\text{new}}}(j)=i_{\text{closest}}$, where $i_{\text{closest}}\in\ccalT_{\text{to-assign}}$\;\label{as:as2}
 Update $\ccalT_{\text{to-assign}} = \ccalT_{\text{to-assign}}\setminus\set{i_{\text{closest}}}$\;\label{as:upd1s}
\If {$\ccalT_{\text{to-assign}} =\emptyset$}{\label{as:sempty}
 $\ccalT_{\text{to-assign}}=\ccalT_{\text{unsat}}$\;\label{as:upds2}
}
}\label{as:asend}
\end{algorithm} 


%Given the targets assigned to the robots when they are in state  $\bbq_{\text{rand}}(t)$, the density function $f_{\ccalU}$ selects more often control inputs $\bbu_{\text{new}}$ that drive the robots toward the respective assigned targets.

First, the function $s_{\bbq_{\text{new}}}$ is initially defined as $s_{\bbq_{\text{new}}}=s_{\bbq_{\text{rand}}}$, where recall that $\bbq_{\text{rand}}$ is the parent node of $\bbq_{\text{new}}$ in the tree $\ccalG$ [line \ref{as:init}, Alg. \ref{alg:assignment}]. Then, we compute (i) the set $\ccalD\subseteq\ccalN$ that collects the indices of the robots that need to update their assigned targets [line \ref{as:D}, Alg. \ref{alg:assignment}], and (ii) the set $\ccalT_{\text{to-assign}}\subseteq\ccalM$ that collects the indices of the targets that are available to be assigned to the robots in $\ccalD$ [lines \ref{as:Tassign}-\ref{as:Tassign3}, Alg. \ref{alg:assignment}]. Then, targets from $\ccalT_{\text{to-assign}}$ are assigned to the robots in $\ccalD$ [lines \ref{as:as1}-\ref{as:asend}].

In particular, the set $\ccalD$ collects the indices $j\in\ccalN$ of robots that in state $\bbq_{\text{new}}$ either (i) satisfy $\det\Sigma_i(F)\leq \delta_i$, where $i$ is the target assigned to robot $j$, i.e., $i=s_{\bbq_{\text{new}}}(j)$, and $\Sigma_{i,\text{new}}$ is its respective covariance, or (ii) the set $\ccalN_i=\set{j~|~i=\bbs_{j,\bbq_{\text{new}}} }$ that collects the robots that are responsible for target $i$, contains more than one robot, i.e., $|\ccalN_i|>1$, or both (i) and (ii). 
%\footnote{Note that $\det\Sigma_i(F)\leq \delta_i$ may hold due to measurements taken by any robot $r\neq j$, even though $i$ has been assigned to robot $j$.}
%Third, we construct the set $\ccalT_{\text{to-assign}}$ that collects the indices of the targets that should be assigned to the robots $j\in\ccalD$ [lines \ref{as:Tassign}-\ref{as:Tassign4}, Alg. \ref{alg:assignment}]. %
Next, the set $\ccalT_{\text{to-assign}}$ is constructed. First, it is initialized as  $\ccalT_{\text{to-assign}}=\ccalM\setminus\set{\ccalT_{\text{as}}\cup\ccalT_{\text{sat}}}$, where  $\ccalT_{\text{as}}\subseteq\ccalM$ collects the indices of the targets that have already been assigned to robots (recall that, in general, it may hold $M>N$) and $\ccalT_{\text{sat}}\subseteq\ccalM$ collects the indices $i\in\ccalM$ of the targets that already satisfy $\det\Sigma_i(F)\leq \delta_i$ [line \ref{as:Tassign}, Alg. \ref{alg:assignment}]. If $\ccalT_{\text{to-assign}}=\emptyset$, then it is redefined as $\ccalT_{\text{to-assign}}=\ccalT_{\text{unsat}}$, where $\ccalT_{\text{unsat}}$ collects the indices $i\in\ccalM$ of the targets that do not satisfy $\det\Sigma_i(F)\leq \delta_i$ [lines \ref{as:Tassign2}-\ref{as:Tassign3}, Alg. \ref{alg:assignment}].%\footnote{Observe that $\ccalT_{\text{sat}}\cup \ccalT_{\text{unsat}}=\ccalM$. } %Notice that $i\in \ccalT_{\text{unsat}}$ does not necessarily imply that $i\notin\ccalT_{\text{as}}$. 


Given $\ccalD$ and $\ccalT_{\text{to-assign}}$, our goal is to assign the targets  $i\in\ccalT_{\text{to-assign}}$ to the robots $j\in\ccalD$ [lines \ref{as:as1}-\ref{as:asend}, Alg. \ref{alg:assignment}]. To do this, the robots $j\in\ccalD$ sequentially select the closest target $i\in\ccalT_{\text{to-assign}}$ to them, denoted by $i_{\text{closest}}$. Every time a robot $j$ picks a target from $\ccalT_{\text{to-assign}}$, the mapping $s_{\bbq_{\text{new}}}$ and set $\ccalT_{\text{to-assign}}$ are updated as $s_{\bbq_{\text{new}}}(j)=i_{\text{closest}}$ and $\ccalT_{\text{to-assign}} = \ccalT_{\text{to-assign}}\setminus\set{i_{\text{closest}}}$ [lines \ref{as:as2}-\ref{as:upd1s}, Alg. \ref{alg:assignment}]. If during this assignment process, it holds that $\ccalT_{\text{to-assign}}=\emptyset$, then $\ccalT_{\text{to-assign}}$ is reinitialized as $\ccalT_{\text{to-assign}}=\ccalT_{\text{unsat}}$ [lines \ref{as:sempty}-\ref{as:upds2}, Alg. \ref{alg:assignment}]. The latter happens if there more robots in $\ccalD$ than targets to be assigned. %Finally, note that in case there are terminal constraints, Algorithm \ref{alg:assignment} can straightforwardly be extended so that it assigns as pseudo-targets to robots locations in $\ccalP_j^{\text{goal}}$ when there more robots in $\ccalD$ than targets to be assigned.
Finally, note that any other task assignment algorithm can be employed in place of lines \ref{as:as1}-\ref{as:asend} that may improve the performance of Algorithm \ref{alg:RRT}; see e.g., \cite{turpin2014capt,michael2008distributed}.




==> Technical Report- Scalable Active Information Acquisition - FinalSubmission/files/theory.tex <==
%In this section, we examine the completeness of Algorithm \ref{alg:AIA}. To show this, we first need to state the following result borrowed from \cite{kantaros2019asymptotically}. %Specifically, in Theorem \ref{thm:probCompl} and \ref{thm:asOpt}, we show that Algorithm \ref{alg:RRT} is probabilistically complete and asymptotically optimal. Also, in Theorem \ref{thm:conv}, we show that Algorithm \ref{alg:RRT} converges exponentially fast to the optimal solution of Problem \ref{prob}. 
In this section, we show that Algorithm \ref{alg:AIA} is complete  for homogeneous sensor networks and static hidden states, i.e., if there there exists a solution to \eqref{eq:Prob2}, then Algorithm \ref{alg:AIA} will find it. This result is formally stated in Theorem \ref{thm:probCompl2}; to show this, we need first to state the following theorem.

\begin{theorem}[Completeness of Sampling-based AIA \cite{kantaros2019asymptotically}]\label{thm:probCompl}
The sampling-based AIA algorithm described in Section \ref{sec:aia} is probabilistically complete, i.e., if there exists a solution to \eqref{eq:LocalProbb2}, then it will find with probability $1$ a path $\bbq_{j,0:F_j}$, defined as a sequence of states in $\ccalV_j$, i.e., $\bbq_{j,0:F_j} = \bbq_j(0), \bbq_j(1), \bbq_j(2), \dots, \bbq_j(F_j)$, 
%\begin{equation}\label{eq:path}
%\bbq_{0:F} = \bbq(0), \bbq(1), \bbq(2), \dots, \bbq(F),
%\end{equation}
that solves \eqref{eq:LocalProbb2}. %, where $\bbq_j(t)\in\ccalV_j$, for all $t\in\{0,\dots,F_j\}$.
\end{theorem}

\begin{theorem}[Completeness of Distributed AIA Algorithm]\label{thm:probCompl2}
%If the exploration strategy forces robots to explore the whole workspace (\textcolor{red}{make this more formal})
%Consider any robot state $\bbp_j(t)$ and corresponding Voronoi cell $V_j(t)$ at any time instant $t\geq0$. 
Assume that (i) given the initial multi-robot state $\bbp(0)$ and the prior distributions $\ccalN(\hat{\bbx}_i(0),\Sigma_i(0))$, there exists a solution to the centralized optimal control problem \eqref{eq:Prob2}; (ii) the robot dynamics allow all robots to reach any obstacle-free location in $\Omega$. %; (iii) $\bbx_i\in V_j(t)$ for $j\in\ccalA_j(t)$, for all robots $i\in\ccalN$. 
Under assumptions (i)-(ii), Algorithm \ref{alg:AIA} is probabilistically complete, i.e., at any time instant $t$ it will generate a terminal horizon $F_j$ and a sequence of control actions $\bbu_{j,t:F_j}$ for all robots with $\ccalA_j(t)\neq\emptyset$ that solve the respective local problems \eqref{eq:LocalProbb2}. 
\end{theorem}

\begin{proof}
By assumption (i) we have that there exists a solution to the centralized optimal control problem \eqref{eq:Prob2}, i.e., there exists a finite sequence of multi-robot states defined as $\bbp_{0:F}=\bbp(0),\dots,\bbp(F)$ that solves \eqref{eq:Prob2}, where  $\bbp(t)=[\bbp_1(t),\bbp_2(t),\dots,\bbp_N(t)]\in\mathbb{R}^{N\times d}$. First, we show that if there exists such a feasible solution to \eqref{eq:Prob2}, then there exists a feasible sequence that solves \eqref{eq:LocalProbb2} constructed at $t=0$ for any robot $j$. Next, we generalize this result for any time instant $t>0$. Then, we conclude that Algorithm \ref{alg:AIA} is probabilistically complete due to Theorem \ref{thm:probCompl}.

In particular, first, using $\bbp_{0:F}$, we construct a sequence of waypoints, denoted by $\bbp_{0:H}^j$, for any given robot $j$ that solves the corresponding  sub-problem \eqref{eq:LocalProbb2} defined at time $t=0$. This sequence is constructed so that robot $j$ visits all single-robot waypoints $\bbp_r(t)$ that appear in $\bbp_{0:F}$ including those waypoints that refer to robots $r\neq j$, for all $t\in[0,\dots,H]$.
%Formally, this sequence, denoted by $\bbp_{0:H}^j$, is defined as  
%\begin{align*}\label{eq:local}
%\bbp_{0:H}^j=& \underbrace{\bbp_{1,0}(0),\bbp_{2,0}(1),\dots, \bbp_{N,0}(N-1)}_{=\bbp(0)}, \underbrace{\bbp_{1,1}(N),\bbp_{2,1}(N+1),\dots, \bbp_{2N,1}(2N-1)}_{=\bbp(1)},\dots,\\
%&\underbrace{\bbp_{1,F}(FN),\bbp_{2,F}(FN+1),\dots, \bbp_{N,F}((F+1)N-1)}_{=\bbp(F)}
%\end{align*}
%where (i) $\bbp_{r,t'}(t)\in\Omega_{\text{free}}$ refers to the waypoint that robot $j$ should visit at time $t$ which coincide with the position that robot $r$ had at time instant $t'=???$ in the sequence $\bbp_{0:F}$ and (ii) the terminal horizon $H$ is defined as $H=(F+1)N-1$.  
In other words, $\bbp_{0:H}^j$ is constructed by unfolding $\bbp_{0:F}$ and writing it as a sequence of single-robot positions. For instance, the first $N$ waypoints in $\bbp_{0:H}^j$ constitute the multi-robot state $\bbp(0)$ in $\bbp_{0:F}$. Similarly, the second group of $N$ waypoints in $\bbp_{0:H}^j$ constitutes the multi-robot state $\bbp(1)$ in $\bbp_{0:F}$. The same logic applies to all subsequent groups of $N$ waypoints. Thus, the terminal horizon $H$ is $H=(F+1)N-1$. Next we claim that if a robot $j$ follows the path $\bbp_{0:H}^j$, then at time $H$ the terminal uncertainty of \textit{all} landmarks $i$ will satisfy $\det \Sigma_i(H)\leq \delta$ (regardless of the motion of other robots). To show this, first note that during the execution of the multi-robot sequence $\bbp_{0:F}$, at time $t$ the Kalman filter Riccati map is applied sequentially $N$ times for each observation model/robot. On the other hand, during the execution of the single-robot sequence $\bbp_{0:H}^j$, at time $t$ the Riccati map is executed only once as per the observation model of robot $j$. Since (a) all robots have the same observation model, and (b) the hidden state (i.e., the positions of the landmarks) is static, we conclude, by definition of the Kalman filter Riccati map, that the terminal uncertainty of the hidden state when $\bbp_{0:H}^j$ is executed will be the same as the one when $\bbp_{0:F}$ is executed. Since $\bbp_{0:F}$ is a feasible solution to \eqref{eq:Prob2}, then after robot $j$ following $\bbp_{0:H}^j$, we have that $\det \Sigma_i(H)\leq \delta$, for all landmarks $i$, even for those that are not in $\ccalA_j(0)$. Also, by assumption (ii), the path $\bbp_{0:H}^j$ respects the robot dynamics. As a result, $\bbp_{0:H}^j$ is a feasible solution to \eqref{eq:LocalProbb2} constructed at $t=0$.  

Finally, we inductively show that if there exists a solution to  \eqref{eq:LocalProbb2} constructed at $t=0$, there exists a solution to all local problems constructed at future time instants $t>0$. To show this, let $t_1>0$ be the first time instant (after $t=0$) when a new  sub-problem in the form of \eqref{eq:LocalProbb2} is defined. Observe that if at time $t=0$, robot $j$ decides to follow a feasible path $\bbp_{0:H}^j$, not necessarily the path constructed before, then at any time $t>0$, continuing following the corresponding sub-path $\bbp_{t:H}^j$, trivially results in achieving the desired terminal uncertainty of \textit{all} landmarks - including those that belong $\ccalA_j(t_1)$ - by feasibility of $\bbp_{0:H}^j$. 
%
Thus, a feasible solution to \eqref{eq:LocalProbb2} formulated at $t_1$ is the sub-path $\bbp_{t_1:H}^j$ (i.e., a sub-sequence of $\bbp_{0:H}^j$).\footnote{Note that the Voronoi cells are used only for landmark assignment purposes while robot mobility is not restricted within them. Thus, updating the Voronoi cells does not affect feasibility of the paths $\bbp_{t_n:H}^j$.} Following the same logic inductively for all future time instants $t_n$ when \eqref{eq:LocalProbb2} is reformulated, we conclude that there always exists a solution to the all local sub-problems completing the proof.
%
%%%%%%%%%%%%%%%+++++++++++++++
%By applying this logic to all landmarks, we conclude that at any time $t$, a feasible solution to all sub-problems \eqref{eq:LocalProbb2} exists and will be found due to Theorem \ref{thm:probCompl} completing the proof.
%Also, as discussed in \ref{sec:aia}, since $\bigcup_{j\in \ccalN}V_j(t)=\Omega$, we have that every landmark is assigned to a unique robot. Thus, for every landmark $i$ 
\end{proof}

%In the next result, we show that given the initial multi-robot configuration $\bbp(0)$ if there exists a solution to the centralized optimal control problem \eqref{eq:Prob2}, then there exists a solution to all distributed local problems \eqref{eq:LocalProbb2}, for all $t\geq0$.  

%\textcolor{red}{[need to rephrase this result..currently unclear]}
%\begin{cor}
%Under assumptions (i)-(ii) of Theorem \ref{thm:probCompl2}, if there exists a solution to the centralized optimal control problem \eqref{eq:Prob2} given the initial multi-robot configuration $\bbp(0)$, then all local AIA problems \eqref{eq:LocalProbb2} formulated at any time $t$ have a solution.
%\end{cor}

%Theorem \ref{thm:probCompl2} shows that at any time instant $t$, given the current landmark assignment and distributions, if there exists a solution to the centralized optimal control problem \eqref{eq:Prob2}, then there exists a solution to all local problems \eqref{eq:LocalProbb2}. In other words, convergence to a feasible solution is not guaranteed as the landmark assignment changes over time. Nevertheless, in Section \ref{sec:Sim}, we show through extensive simulations that Algorithm \ref{alg:AIA} is capable of finding feasible solutions even when the landmarks are dynamically assigned to the robots. In fact, we show that this results in significant performance gains in terms of the terminal horizon, i.e.,  total discrete time instants required to achieve desired levels of uncertainty for the hidden state. 

%{\bf{Online vs Offline Planning:}} According to Theorem \ref{thm:probCompl2}, Algorithm \ref{alg:AIA} can find at time $t=0$ feasible (offline) paths that solve the centralized problem \eqref{eq:LocalProbb2}. As it will be shown in Section \ref{sec:Sim}, the benefit of dynamically assigning landmarks to robots and accordingly re-planning online is that the burden of localizing all $M$ landmarks is shared among all robots resulting in shorter terminal horizons.
\begin{rem}[Online vs Offline Planning]\label{rem:onlineRe}
According to Theorem \ref{thm:probCompl2}, Algorithm \ref{alg:AIA} can find at time $t=0$ feasible (offline) paths that solve the centralized problem \eqref{eq:LocalProbb2}. As it will be shown in Section \ref{sec:Sim}, the benefit of dynamically assigning landmarks to robots and accordingly re-planning online is that the burden of localizing all $M$ landmarks is shared among all robots resulting in shorter terminal horizons.
\end{rem}

\begin{rem}[Implementation]\label{rem:implem}
A more computationally efficient approach to apply \cite{kantaros2019asymptotically} is to define the goal region $\ccalX_g$ so that it requires only one landmark - instead of all - in $\ccalA_j(t)$ to be localized with accuracy $\delta$. Such an approach may not yield the optimal solution to \eqref{eq:LocalProbb2} due to its myopic nature but it does not sacrifice completeness. This can be shown by following the same logic as in the proof of Theorem \ref{thm:probCompl2}.
%Specifically, let $i$ be the landmark that robot $j$ aims to localize after applying a sequence of control actions denoted by $\bbu_{j,t:\bar{t}}^{\ell_i}$ generated by \cite{kantaros2019asymptotically}. Also, assume that given $V_j(t)$ there exists a solution to \eqref{eq:LocalProbb2}, i.e., there exist measurement locations that if robot $j$ visits then desired levels of uncertainty will be achieved for all landmarks in $\ccalA_j(t)$. All these locations can still be visited assuming simple robot dynamics (e.g., $\bbp_j(t+1) =\bbp_j(t) +\bbu_j(t)$) after robot $j$ applies the control actions in $\bbu_{j,t:\bar{t}}^{\ell_i}$. In fact, a path towards them will be found due to the completeness nature of the AIA algorithm in \cite{kantaros2019asymptotically}. Recall that the time instants when measurement-locations are visited are irrelevant since the landmarks are assumed to be static. 
%a sequence of control inputs $\bbu_{j,t:F_j}$ that solves
\end{rem}

\begin{rem}[Optimality]
Note that to solve the local problem \eqref{eq:LocalProbb2}, information that may be collected by the rest of the robot team is neglected; see also Section \ref{sec:overview}. As a result, the synthesized paths may not constitute an optimal solution to \eqref{eq:Prob2}. This local design of paths sacrifices optimality but it allows for addressing large-scale estimation tasks. % that are computationally challenging to solve using existing centralized methods due to the large-state space that needs to be  explored.}
%However, this information will be taken into account during the execution of the locally synthesized paths since then the robots share their measurements and collectively update their beliefs about the hidden state. 
%Note that Voronoi diagrams are not equitable and, therefore, a landmark may be sensed by more than one robot. O
\end{rem}



==> Technical Report- Scalable Active Information Acquisition - FinalSubmission/files/tree.tex <==
\subsection{Incremental Construction of Trees}\label{sec:constructTree}
At every iteration $n$ of Algorithm \ref{alg:RRT}, a new state $\bbq_\text{new}(t+1) =[\bbp_{\text{new}}(t+1),\Sigma_{\text{new}}(t+1)]$ is sampled. The construction of the state  $\bbq_\text{new}(t+1)$ relies on two steps. Specifically, first we sample a state $\bbp_{\text{new}}(t+1)$ [lines \ref{rrt:samplekrand}-\ref{rrt:sampleu}, Alg. \ref{alg:RRT}]; see Section \ref{sec:sample}. Second, given $\bbp_{\text{new}}(t+1)$ we compute the covariance matrix $\Sigma_{\text{new}}(t+1)$, giving rise to $\bbq_{\text{new}}(t+1)$ which is added to the tree structure [line \ref{rrt:dnew}, Alg. \ref{alg:RRT}]; see Section \ref{sec:extend}.



%To do this, we first sample a state $\bbp_{\text{new}}$; see Section \ref{sec:sample} [lines \ref{rrt:samplekrand}-\ref{rrt:sampleu}, Alg. \ref{alg:RRT}]. Then, we select a state $\bbq_{\text{rand}}(t)=[\bbp_{\text{rand}}(t),\bbd_{\text{rand}}(t)]\in\ccalV$ that will be the parent node of $\bbq_{\text{new}}(t+1)$[line \eqref{rrt:for2}, Alg. \ref{alg:RRT}]. Note that the time instant $t+1$ which $\bbq_{\text{new}}$ is associated with, is determined by the parent node $\bbq(t)$. Given $\bbp_{\text{new}}$ and the parent node $\bbq_{\text{rand}}(t)$, we compute $\bbd_{\text{new}}(t+1)$ which then gives rise to the new state $\bbq_\text{new}(t+1) =[\bbp_{\text{new}}(t+1),\bbd_{\text{new}}(t+1)]$ that will be added to the tree at iteration $n$ [lines \ref{rrt:dnew}-\ref{rrt:updCost}, Alg. \ref{alg:RRT}]; see Section \ref{sec:extend}.

\subsubsection{Sampling Strategy}\label{sec:sample} 
To construct the state $\bbp_{\text{new}}$, we first divide the set of nodes $\ccalV$ into a \textit{finite} number of sets, denoted by $\ccalV_{k}\subseteq\ccalV$, based on the robot-configuration component of the stats $\bbq\in\ccalV$. Specifically, a $\ccalV_{k}$ collects all states $\bbq\in\ccalV$ that share the same robot configuration $\bbp$; see Figure \ref{fig:tree}.%\footnote{Decomposition of $\ccalV$ into subsets $\ccalV_k$ is required to ensure completeness and optimality of Algorithm \ref{alg:RRT}; see Appendix \ref{sec:prop}.}
%$\bbq(t)=[\bbp(t),\Sigma(t)]\in\ccalV$ that have the same robot configuration $\bbp$ but possibly different covariance matrices $\Sigma(t)$ and different time stamps $t$; see Figure \ref{fig:tree}. %Also, note that the states $\bbq\in\ccalV_k$ do not necessarily have the same time stamp $t$, since, in general, there are multiple paths that connect the root $\bbq(0)$ to $\bbq$.
%
By construction of $\ccalV_{k}$, we get that  $\ccalV = \cup_{k=1}^{K_n}\ccalV_{k}$, where $K_n$ is the number of subsets $\ccalV_{k}$ at iteration $n$.
Also, notice that $K_n$ is finite for all iterations $n$, since the set of admissible control inputs $\ccalU$ is finite, by assumption. %for all robots $j$, i.e., the number of all possible different robot configurations contained in $\ccalV$ is finite for all iterations $n$. 
At iteration $n=1$ of Algorithm \ref{alg:RRT}, it holds that $K_1=1$, $\ccalV_1=\ccalV$ [line \ref{rrt:init}, Alg. \ref{alg:RRT}]. %\red{[maybe a figure would make this definition much cleaner]}%%the (global) set V can be 'infinite'!
% 

Second, given the sets $\ccalV_k$, we first sample from a given discrete distribution $f_{\ccalV}(k|\ccalV):\set{1,\dots,K_n}\rightarrow[0,1]$ an index $k\in\set{1,\dots,K_n}$ that points to the set $\ccalV_{k}$ [line \ref{rrt:samplekrand}, Alg. \ref{alg:RRT}]. The density function $f_{\ccalV}(k|\ccalV)$ defines the probability of selecting the set $\ccalV_{k}$ at iteration $n$ of Algorithm \ref{alg:RRT} given the set $\ccalV$. Any density function $f_{\ccalV}$ can be used to draw samples $k_{\text{rand}}$ as long as it satisfies the following assumption.%\NA{It is not allowed to sample control at the same node twice, correct? To me the discrete distributions are more of a prioritization of the search of the tree -- does it have to be random?} %\BS{How do you choose amongst the different possible nodes in the set $\ccalV_k$, once $k$ is chosen?}

Next, given the set $\ccalV_{k_{\text{rand}}}$ sampled from $f_{\ccalV}$ and the corresponding robot state $\bbp_{\text{rand}}$, we sample a control input $\bbu_{\text{new}}\in\ccalU$ from a discrete distribution $f_{\ccalU}(\bbu):\ccalU\rightarrow [0,1]$ [line \ref{rrt:sampleu}, Alg. \ref{alg:RRT}]. 
%
Given a control input $\bbu_{\text{new}}$ sampled from $f_{\ccalU}$, we construct the state $\bbp_{\text{new}}$ as $\bbp_{\text{new}}=\bbf(\bbp_{\text{rand}},\bbu_{\text{new}})$ [line \ref{rrt:sampleu}, Alg. \ref{alg:RRT}]. Any density function $f_{\ccalU}$ can be used to draw samples $\bbu_{\text{new}}$ as long as it satisfies the following assumption.
%The density function $f_{\ccalU}$ should be designed so that it satisfies the following assumption.

\subsubsection{Extending the tree}\label{sec:extend}

If the configuration $\bbp_\text{new}$, constructed as in Section \ref{sec:sample}, does not belong to the obstacle-free space, then the current sample $\bbp_\text{new}$ is rejected and the sampling process is repeated [line \ref{rrt:obsFree}, Alg. \ref{alg:RRT}]. Otherwise, the tree is extended towards states $ \bbq_\text{new}$ that are constructed as follows; see also Figure \ref{fig:tree2}. %\footnote{The condition $(\bbq_\text{rand}(t),\bbq_\text{new}(t))\notin \ccalE$ in line \ref{rrt:newedge} prevents from adding the same edgeadding }%if $\bbp_\text{new}\in \Omega_{\text{free}}^N$ and $(\bbq_\text{rand}(t),\bbq_\text{new}(t))\notin \ccalE$,
%
Given a state $\bbq_{\text{rand}}(t)=[\bbp_{\text{rand}}(t),\Sigma_{\text{rand}}(t)]\in\ccalV_{k_{\text{rand}}}$, we construct a state $ \bbq_\text{new}$ by appending to $\bbp_{\text{new}}(t+1)$, the covariance matrix $\Sigma_{\text{new}}(t+1)$ computed as $\Sigma_{\text{new}}(t+1)=\rho(\bbp_{\text{rand}}(t),\Sigma_{\text{rand}}(t))$, where recall that $\rho(\cdot)$ is the Kalman filter Ricatti map [lines \ref{rrt:dnew}-\ref{rrt:qnew}, Alg. \ref{alg:RRT}]. %
Next, we update the set of nodes and edges of the tree as $\ccalV = \ccalV\cup\{\bbq_{\text{new}}(t+1)\}$ and $\ccalE = \ccalE\cup\{(\bbq_{\text{rand}}(t),\bbq_{\text{new}}(t+1))\}$, respectively [lines \ref{rrt:updV}-\ref{rrt:updE}, Alg. \ref{alg:RRT}]. The cost of the new node $\bbq_{\text{new}}(t+1)$ is computed as in \eqref{eq:costUpd}, i.e., $J_{\ccalG}(\bbq_{\text{new}}(t+1))=J_{\ccalG}(\bbq_{\text{rand}}(t))+\det \Sigma_{\text{new}}(t+1)$ [line \ref{rrt:updCost}, Alg. \ref{alg:RRT}]. Finally, the sets $\ccalV_{k}$ are updated, so that if there already exists a subset $\ccalV_k$ associated with the configuration  $\bbp_{\text{new}}$, then $\ccalV_{k}=\ccalV_{k}\cup\set{\bbq_{\text{new}}(t+1)}$. Otherwise, a new set $\ccalV_{k}$ is created, i.e., $K_n = K_n +1$ and $\ccalV_{K_n}=\set{\bbq_{\text{new}}}$ [lines \ref{rrt:if2}-\ref{rrt:updKn}, Alg. \ref{alg:RRT}]. This process is repeated for all states  $\bbq_{\text{rand}}(t)\in\ccalV_{k_{\text{rand}}}$ [line \ref{rrt:for2}, Alg. \ref{alg:RRT}]. Recall that the states in $\ccalV_{k_{\text{rand}}}$ share the same robot configuration $\bbp_{\text{rand}}$ but they are possibly paired with different time stamps $t$ and covariance matrices $\Sigma(t)$; see Figure \ref{fig:tree}.

%
%Finally, if the state $\bbq_{\text{new}}$ satisfies the constraints captured by the goal set \eqref{eq:goalRegion}, i.e.,  $\bbq_{\text{new}}\in\ccalQ_{\text{goal}}$, then the set $\ccalX_{{g}}$  is updated as $\ccalX_{g} = \ccalX_{g}\cup\set{\bbq_{\text{new}}}$ [lines \ref{rrt:updGoal1}-\ref{rrt:updGoal2}, Alg. \ref{alg:RRT}]. This process is repeated for all states in the set $\ccalV_{k_{\text{rand}}}$ [line \ref{rrt:for2}, Alg. \ref{alg:RRT}]. Algorithm \ref{alg:RRT} terminates after $n_{\text{max}}$ iterations, where $n_{\text{max}}>0$ is user-specified [line \ref{rrt:forn}, Alg. \ref{alg:RRT}]. 

%\begin{rem}[Alternative Approaches]
%Note that an alternative solution to Problem \ref{prob} is to exhaustively search the infinite state-space$\Omega_{\text{free}}^N\times\mathbb{R}_{+}$ in a similar way as e.g., in [LeNy] that relies on feedforward value iteration or as in [Atanasov] that relies on a Reduced Value Iteration. Nevertheless, such approaches do not scale well as the required horizon $F$ or the number of robots increases, since they require at to compute the reachable set of any node $\bbq(t)$ and extend the search tree towards all reachable states. To the contrary, here we extend the nodes $\bbq(t)\in\ccalV$ to a single reachable state in a probabilistic way as described in Section \ref{sec:sample}. As it will be shown in Section \ref{sec:Sim}, this allows us to address large-scale estimation tasks.
%\end{rem}
%


==> algorithm2e.tex <==
%  algorithm2e.sty --- style file for algorithms
%                      almost everything can be customized by users. See the document for more explanations
%% Copyright 1996-2015 Christophe Fiorio
%
% This work may be distributed and/or modified under the conditions of the LaTeX Project
% Public License, either version 1.3 of this license or (at your option) any later version.
% The latest version of this license is in http://www.latex-project.org/lppl.txt and
% version 1.3 or later is part of all distributions of LaTeX version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
% 
% The Current Maintainer of this work is M. Christophe Fiorio
%
% This work consists of the files algorithm2e.sty and algorithm2e.tex 
% and the associated example files algorithm2e_exAlgoDisjdecomp.tex,
% algorithm2e_exIR.tex, algorithm2e_ex01.tex, algorithm2e_exProg.tex,
% algorithm2e_ex02.tex, algorithm2e_exfor.tex, algorithm2e_ex03.tex,
% algorithm2e_exgeneric.tex, algorithm2e_ex04.tex,  algorithm2e_exgeneric2.tex,
% algorithm2e_ex05.tex, algorithm2e_exnlsty.tex, algorithm2e_ex06.tex,
% algorithm2e_exrepeat.tex, algorithm2e_ex07.tex, algorithm2e_exswitch.tex
%  
%  Report bugs and comments to:
%  - algorithm2e-announce@lirmm.fr  mailing list for announcement about releases^^J%
%  - algorithm2e-discussion@lirmm.fr mailing list for discussion about package^^J%
%  subscribe by emailing sympa@lirmm.fr with 'subscribe <list> <firstname name>'^^J%
%
%  $Id: algorithm2e.sty,v 5.1 2015/10/18 21:37:30 cfiorio Exp $
%
%  PACKAGES REQUIRED:
%
%  - float   (in contrib/supported/float)
%  - ifthen  (in base)
%  - xspace  (in packages/tools)
%  - relsize (in contrib/misc/relsize.sty)
%
%%%%%%%%%%%%%%%  Release 5.1
%
%   Package options: 
%   ---------------
%   - oldcommands                      : to use old command names
%   - french, english, german, ngerman
%      portuguese, czech, italiano,
%      slovak, croatian, spanish       : for the name of the algorithm and some keyword code
%   - onelanguage                      : to simply switch keyword from one language to another without changing
%                                        keyword commands
%   - boxed, boxruled, ruled, tworuled, 
%     algoruled, plain                 : layout of the algorithm
%   - algo2e                           : environment is algorithm2e instead of algorithms and \listofalgorithmes
%                                        instead of \listofalgorithms
%   - slide                            : to use when making slides
%   - noline,lined,vlined              : how block are designed.
%   - shortend, longend, noend         : short or long end keyword as endif for e.g.
%   - linesnumbered                    : auto numbering of the algorithm's lines
%   - linesnumberedhidden              : to hide autonumbered lines (show number on a line with \ShowLn
%   - commentsnumbered, inoutnumbered  : to autonumber comments and inout keywords (by defaut not numbered)
%   - rightnl                          : to have line number on the right instead of on the left as default
%   - algonl                           : line numbers preceded by algo number
%   - scright, scleft                  : right or left justified side comments
%   - fillcomment, nofillcomment       : end mark of comment is flushed to the right so comments fill the line
%   - dotocloa                         : add an entry in the toc for list of algorithms (require tocbibind package)
%   - endfloat                         : add algoendfloat environment pushing algorithm so written to the end of document
%   - resetcount, noresetcount         : start value of line numbers.
%   - algopart,algochapter,algosection : algo numbering within part, chapter or section
%   - titlenumbered,titlenotnumbered   : numbering of title set by \Titleofalgo
%   - figure                           : algorithms are figures, numbered as figures, and put in the list of figures.
%   - procnumbered                     : procedure or function are numbered as algorithm
%   - nokwfunc                         : procedure or function name doens't become a command
%   - norelsize                        : don't use relsize package (useful if it breaks the compatibily)
%   - displayblockmarkers              : display begin, end keywords at start of each block
%  
%   defaults are; english,plain,resetcount,titlenotnumbered
%
%%%%%%%%%%%%%%
%
%   Short summary  
%   -------------
%  
%   algorithm is an environment for writing algorithm in LaTeX2e.
%   Almost all is customizable. You can add keywords, change style, change the layout, ...
%   It provide macros that allow you to create differents sorts of key words, therefore a set of predefined key
%   word is gived.
%
%   IT should be used as follows
%
%   \begin{algorithm}
%       ...
%       ...
%   \end{algorithm}
%
%
%   IMPORTANT : each line MUST end with \;
%
%   Note that if you define macros outside algorithm environment they
%   are avaible in all the document and particulary you can use then
%   inside all algorithms without re-define them.
%  
%   an example:
%
%   \begin{algorithm}
%     \SetAlgoLined
%     \KwIn{this text}
%     \KwOut{how to write algorithm with \LaTeX2e }
%     
%     initialization\;
%     \While{not at end of this document}{
%       read current section\;
%       \eIf{understand}{
%         go to next section\;
%         current section becomes this one\;
%         }{
%         go back to the beginning of current section\;
%         }
%       }
%     \caption{How to write algorithm}
%   \end{algorithm}
%
%
%%%%%%%%%%%%%%         predefined keywords
%
%     \KwIn{input}
%     \KwOut{output}
%     \KwData{input}
%     \KwResult{output}
%     \KwTo                                       % a simple keyword
%     \KwFrom                                     % a simple keyword
%     \KwRet{[value]}
%     \Return{[value]}
%     \Begin{block inside}
%     \eIf{condition}{Then Block}{Else block}     % in blocks
%     \If{condition}{Then block}                  % in a block
%     \uIf{condition}{Then block}                 % in a block unended
%     \lIf{condition}{Else text}                  % on the same line
%     \Else{inside Else}                          % in a block
%     \lElse{Else text}                           % on the same line        
%     \uElse{Else text}                           % in a block unended
%     \ElseIf{inside Elseif}                      % in a block
%     \lElseIf{Elseif text}                       % on the same line        
%     \uElseIf{Elseif text}                       % in a block unended
%     \Switch{Condition}{Switch block}
%     \Case{a case}{case block}                   % in a block
%     \lCase{a case}{case text}                   % on the same line
%     \Other{otherwise block}                     % in a block
%     \lOther{otherwise block}                    % on the same line
%     \For{condition}{text loop}                  % in a block
%     \lFor{condition}{text}                      % on the same line
%     \ForEach{condition}{text loop}              % in a block
%     \lForEach{condition}{text}                  % on the same line
%     \ForPar{condition}{text loop}               % in a block
%     \lForPar{condition}{text}                   % on the same line
%     \While{condition}{text loop}                % in a block
%     \lWhile{condition}{text loop}               % on the same line
%     \Repeat{End condition}{text loop}           % in a block
%     \lRepeat{condition}{text}                   % on the same line
%
%%%%%%%%%%%%%%
%
%   History: 
%
%   -  October 19 2015 - revision 5.1
%                   * CHANGE/ADD: l commands  (the ones as \lIf) can now be used with a
%                              star. If done, no end of line are done, so you can enclose
%                              l command into another one. For example, you can write:
%                              \lForEach{$i$}{\lIf*{foo}{bar}}.
%                               Note that when you use a star, side comments are not allowed.
%                   * CHANGE/ADD: Now you can have a side comment at end of macros which
%                               have a block. For example you can do : 
%                               \Begin(\tcc*[h]{side comment for begin}{text}(\tcc*[h]{side comment after end})
%                               Note: there are some side effects for some commands:
%                              \SetKwProg : macro defined thanks to \SetKwProg are allowed
%                                                   to have no end marker. In this case,
%                                                   beware to end side comment, this can
%                                                   do weird output (but no error)
%                   * CHANGE: \SetKwSwitch defines also an \uOther command which was not
%                               the case until this release.
%                   * CHANGE: \SetStartEndCondition{typo1}{typo2}{typo3} defined two end
%                               conditions (type2 and typo3) : typo3 is no more used for
%                               case condition as typo2 is used which is more consistent
%                               since there is a condition followed by a keyword as for
%                               if-then or other command that are defined using typo2.
%                   * CHANGE: keywords was not language dependant to allow to use multiple
%                               languages in the same document, but some keywords in
%                               different language were having the same keyword that lead
%                               last one declared to replace first one and so you could have some
%                               spanish keywords printed as you were in portuguese. So
%                               this behavior is changed from now:
%                               - localized keywords are defined if according language
%                                  option is defined ; 
%                               - if you want to keep old behaviour and use localized
%                                  keywords without using language option (keep old
%                                  behavior), you can use languagekw option
%                                  (e.g. frenchkw, germankw, ...). Note that you can use
%                                  multiple languagekw options at the same time, in
%                                  contrary of language option. Note also that if you use
%                                  multiple languagekw options, you can get back the same
%                                  problem as previously when keywords was not language
%                                  dependant.
%                   * ADD: new typo styles:
%                               - Arguments of functions have now their own style. By
%                                  default, FuncArgSty is the same as ArgSty. 
%                               - Name of KwProg have now their own sty (they used ArgSty
%                                  previously). By default, ProgSty is still ArgSty.
%                               As usual, \SetFuncArgSty{}, FuncArgSty{} and
%                               \SetProgSty{}, ProgSty{} are macros to set and use these
%                               typo styles.
%                   * ADD: Options to manage algorithm hangindent
%                            Until this revision, long statement acts as classical text and
%                            continue on next line starting from the same point. This makes
%                            difficult to notice that the new lines of text is not a new
%                            statement. Now, hangindent is managed and when a long
%                            statement continue on next lines, lines, except the first,
%                            are indented.
%                            Option: noalgohanging
%                               By default, long statement are indented on subsequent
%                               lines; with this option you get old behavior and lines are
%                               no more indented
%                            Option: hangingcomment 
%                               Comment that are alone on a line (not side comment) are
%                               not driven by algo hanging: subsequent lines of long
%                               comments are indented according to width of start comment
%                               marker. With this option, comment are indented like normal
%                               statement.
%                            Option: hanginginout
%                               As for comment, by default, in/out keywords and input
%                               keywords (defined by \SetKwInOut or \SetKwInput) are not
%                               indented by algorithm hangindent. They are indented
%                               according to width of input keyword. If you want that these
%                               keywords acts like normal statement, use this option.
%                            \SetAlgoHangIndent{length}
%                               This macro allows you to set your own indent length. By
%                               default, \SetAlgoHangIndent{0.5em}
%                   * ADD: Group markers. 
%                            This option is related to block markers of release 5.0. Some
%                            have ask to put also block markers for single line
%                            command. This new feature has been implemented to do this.
%                            So, you can now ask package to put begin and end keywords
%                            automatically at start and end of single line command (see
%                            example in documentation).
%                            These new group markers macros are:
%                            - \AlgoDisplayGroupMarkers and \AlgoDontDisplayGroupMarkers
%                            Note that a new option has also been added: displaygroupmarkers
%                   * ADD: \SetCustomAlgoRuledWidth{length}
%                             set a custom ruled width of ruled and algoruled options ;
%                             note that by the moment you use this macro, rules will have
%                             this fixed length: this can cause strange behavior in
%                             multicolumn mode or other layout that change the line
%                             width. 
%                   * ADD: turkish language option
%                   * FIX: a spurious whitespace which results in a spurious indent in the
%                            user's text right after the end of the algorithm environment
%                            was introduced  in release 5.0. This is fixed now thanks to
%                            Alexander Malkis.
%                   * FIX: there was a problem with margins in caption when option figure
%                            was use with caption package. This is fixed.
%                   * FIX: when changing font size in caption with, interline skip stayed
%                            unchanged and so with a small font was to large. This is fixed.
%                   * FIX: in contrary of that is written in the documentation, ':' what
%                            not in KwSty typo for KwIn and KwOut command. This is fixed. 
%                   * FIX: strange behaviour with label and lines numbered: @currentlabel
%                            was updated according to algo line number not in all
%                            situation. For e.g, with hyperref package, always updated ;
%                            with \nlset also updated, but with \nl or linesnumbered
%                            option, not updated. This "feature" causes different output
%                            with \label command according to options used which is not
%                            that one want. This is solved now, and @currentlabel is
%                            always updated so \label command works always is the same way.
%                   * FIX: some czech keywords
%                   * FIX: some spanish keywords
%                   * FIX: some croatian keywords
%                   * FIX: krantz class changes definition of chapter and get one more
%                            option that classical classes as book.cls or report.cls and
%                            broke fix for hyperref on chapter definition. This is now
%                            fixed and algorithm detects use of krantz class and use then
%                            a definition of chapter working with krantz class.
%                   * FIX: an issue with internal macro which causes ([Q]) use as argument
%                            of some environment to be misprinted (thanks to Martin Schr?der).
%                   * FIX: mispelled name of hyperrefcounter inside internal macro.
%
%   - January 06 2013 - revision 5.0
%                     * CHANGE: SetKwSwitch takes now 9 args: 9th arg is the same as
%                                previous 8th arg ('end of switch' keyword). New 8th arg is
%                                'end of case' keyword. This is due to change of release
%                                3.2 which introduce end after case block... as I never
%                                test with longend option, I never see that the 'end
%                                switch' used for case was not good.
%                     * CHANGE: when no end keyword is defined in a block macro, then
%                                algorithm2e does no more try to print it. So even with lined or noline
%                                option, no empty line is printed (before: a blank end was
%                                printed, so a blank line appeared)
%                     * Internal Change: add some internal function to improve readibility
%                                        (thanks to Philip K. F. H\?lzenspies)
%                     * ADD: Block markers. 
%                            You can now ask package to put begin and end keywords automatically at begin
%                            and end of blocks, it means each group of commands shifted and enclosed in
%                            braces.
%                            This is tricky to use but, combined with \SetStartEndCondition and
%                            redefinition of keywords, you should be abble to simulate any syntax. See
%                            examples in documentation where a generic example is derived in pseudo-code,
%                            python and C by keeping code and changing only style using block markers
%                            macros, \SetStartEndCondition and some redefinition of keywords.
%                            These new block markers macros are:
%                            - \AlgoDisplayBlockMarkers and \AlgoDontDisplayBlockMarkers
%                            - \SetAlgoBlockMarkers{begin marker}{end marker}
%                            - \BlockMarkersSty{text} and \SetBlockMarkersSty
%                            Note that a new option has also been added: displayblockmarkers
%                     * ADD: \leIf macro automatically defined by \SetKwIF: allow to define
%                            an if-then-else on a single line.
%                     * ADD: new macro \SetStartEndCondition{typo1}{typo2}{typo3} which
%                            sets typo around condition in For, If, Switch, Case and
%                            Repeat macros. First two are used around For, If, Swith
%                            conditions, First and third are used for Case and Repeat
%                            condition where condition ends the line. Default definition
%                            is \SetStartEndCondition{ }{ }{}. 
%                            A common alternative is \SetStartEndCondition{ (}{) }{)}
%                            Can also be used to remove space around condition, for
%                            example if you want python style commands:
%                            \SetStartEndCondition{ }{}{} and \SetKwFor{For}{for}{:}{}
%                     * ADD: new environment algomathdisplay which allow display math (like inside \[ \] or $$ $$) 
%                            handling end line and line number
%                     * ADD: new command \SetKwProg{Env}{Title}{is}{end} which defines a macro
%                            \Env{args}{text}. Env is a block with 'Title' (in \CapSty) at the beginning
%                            followed by args followed by 'is' then 'text' is put below inside a block ended
%                            by 'end'. If no 'end' is specified, nothing is written (no
%                            blank line is inserted). Useful to typeset function or prog for example:
%                            \SetKwProg{Fn}{Function}{ is}{end} makes \Fn{afunc(i: int) : int}{return 0\;}                    
%                            writes: 
%                            Function afunc(i: int) : int is
%                            | return 0;
%                            end
%                            or \SetKwProg{Def}{def}{:}{} makes \Def{afunc(i: int)}{return 0\;} writes:
%                            def afunc(i: int):
%                            | return 0
%                            Tip: combine it with \SetKwFunction to write recursive function algorithm. With
%                            example above, you could define \SetKwFunction{\Afunc}{afunc} and then write:
%                            \Def{\Afunc{i:int}{\eIf{i>0}{\KwRet \Afunc{i-1}}{\KwRet 0\;}} that writes:
%                            def afunc(i: int):
%                            | if(i>0):
%                            |     return afunc(i-1)
%                            | else:
%                            |     return 0
%                            with appropriate typo.
%                     * ADD: option croatian: croatian keywords (thanks to Ivan Gavran)
%                     * ADD: option ngerman: same as german option but so can be used with global option ngerman
%                            of babel
%                     * ADD: option spanish: Spanish support (thanks to Mario Abarca)
%                     * ADD: unterminated block: useful to add part separator that doesn't necessary need an end
%                            keyword.  
%                            Designed on the pattern of unterminated if (see \uIf macro) allowing to
%                            add a block that is not terminated by a keyword. Such block are defined in the same
%                            time as a block is defined by adding a macro beginning with u. So, for example,
%                            predefined \SetKwBlock{Begin}{begin}{end} defines now two commands:
%                            - \Begin{} as previously which print a begin - end block
%                            - \uBegin{} that defines a begin only block
%                     * FIX: problem when numbering line inside until condition of
%                            \SetKwRepeat macro: line number was not correctly aligned.
%                     * FIX: dotocloa option which was broken
%                     * FIX: uIf and uCase didn't have same behavior when used with
%                            noline, vlined or lined option. This is fixed. Side effect: no empty
%                            line after an uIf or uCase when used with options lined or vlined
%                     * FIX: a bug with Repeat Until command when use with side comment on Until
%                     * FIX: a bug with side text -- text put into () -- of command macro (SetKwIf and so on)
%                            which was always setting a ';' even after a \DontPrintSemicolon
%                     * FIX: a bug with hyperref and chapter definition (thanks to Hubert Meier)
%                     * FIX: bugs with l macro and side comment
%                     * FIX: revision number
%                     * FIX: fix non ascii character (utf8 not yet recognized by all latex engine)
%                     * FIX: fnum@algocf had an useless parameter which sometimes broke expansion and output an error
%                     * FIX: works now with multicol package
%
%   - december 14 2009 - revision 4.1
%                     * ADD: new command \SetKwHangingKw{Name}{text} (hanging indent with keyword): This creates a
%                            hanging indent much like \texttt{SetKwInput}, except that it removes the trailing `:'
%                            and does not reset numbering (thanks to Nathan Tallent)
%
%   - november 17 2009  - revision 4.00 -
%
%                      * CHANGE: IMPORTANT: some commands have been renamed to have consistent naming (CamlCase
%                                syntax) and old commands are no more available. If you doesn't want to change
%                                your mind or use old latex files, you can use oldcommands option to enable old
%                                commands back.
%                                text. Here are these commands:
%                                - \SetNoLine becomes \SetAlgoNoLine
%                                - \SetVline  becomes \SetAlgoVlined
%                                - \Setvlineskip  becomes \SetVlineSkip
%                                - \SetLine   becomes \SetAlgoLined
%                                - \dontprintsemicolon becomes \DontPrintSemicolon
%                                - \printsemicolon becomes \PrintSemicolon
%                                - \incmargin becomes \IncMargin
%                                - \decmargin becomes \DecMargin
%                                - \setnlskip becomes \SetNlSkip
%                                - \Setnlskip becomes \SetNlSkip
%                                - \setalcapskip becomes \SetAlCapSkip
%                                - \setalcaphskip becomes \SetAlCapHSkip
%                                - \nlSty becomes \NlSty
%                                - \Setnlsty becomes \SetNlSty
%                                - \linesnumbered becomes \LinesNumbered
%                                - \linesnotnumbered becomes \LinesNotNumbered
%                                - \linesnumberedhidden becomes \LinesNumberedHidden
%                                - \showln becomes \ShowLn
%                                - \showlnlabel becomes \ShowLnLabel
%                                - \nocaptionofalgo becomes \NoCaptionOfAlgo
%                                - \restorecaptionofalgo becomes \RestoreCaptionOfAlgo
%                                - \restylealgo becomes \RestyleAlgo
%                                - gIf macros and so on do no more exist
%                      * NEW: - Compatibily with other packages improven by changing name of internal
%                               macros. Algorithm2e can now be used with arabtex for example, if this last is
%                               loaded after algorithm2e package.
%                      * ADD: - OPTION endfloat: endfloat packages doesn't allow float environment inside other
%                               environment. So using it with figure option of algorithm2e makes error. This
%                               option enables a new environment algoendfloat to be used instead of algorithm
%                               environment that put algorithm at the end. algoendfloat environment make
%                               algorithm acting as endfloat figures. This option requires endfloat packages.
%                      * ADD: - OPTION norelsize: starting from this release (v4.00), algorithm2e package uses
%                               relsize package in order to get relative size for lines numbers; but it seems
%                               that some rare classes (such as inform1.cls) are not compatible with relsize; to
%                               have algorithm2e working, this option makes algorithm2e not to load relsize
%                               package and go back to previous definition by using \scriptsize font for lines
%                               numbers.
%                      * ADD: - OPTION onelanguage: allow, if using standard keywords listed below, to switch
%                               from one language to another without changing keywords by using appropriate
%                               language option:
%                               . KwIn, KwOut, KwData, KwResult
%                               . KwTo KwFrom
%                               . KwRet, Return
%                               . Begin
%                               . Repeat
%                               . If, ElseIf, Else
%                               . Switch, Case, Other
%                               . For, ForPar, ForEach, ForAll, While
%                               .
%                      * ADD: - OPTION rightnl: put lines numbers to the right of the algorithm instead of left.
%                      * ADD:   new commands \setRightLinesNumbers and \setLeftLinesNumbers which sets the lines
%                               numbers to the right or to the left of the algorithm.
%                      * ADD: - new kind of keywords: KwArray used to define arrays:
%                               \SetKwArray{Kw}{array} defines an array keywords Kw called array and printed in
%                               DataSty style when call with \Kw. It can be used with one argument which
%                               denotes the element index: \Kw{n} prints array[n] with array in DataSty and n in
%                               ArgSty.
%                      * ADD/FIX: rules of ruled, algoruled, tworuled styles used rules of different sizes! This
%                                 is now fixed. Moreover size of the rules is now controlled by a length and so
%                                 can be customized by the user.
%                                 \algoheightrule is the height of the rules and can be changed via \setlength
%                                 \algoheightruledefault is the default height of he rules (0.8pt)
%                                 \algotitleheightrule is the height of the rule that comes just after the
%                                 caption in ruled and algoruled style; it can be changed via \setlength
%                                 \algotitleheightruledefault is the default height of this rules (0.8pt)
%                                 Thanks to Philippe Dumas who reports the bug and make the suggestion.
%                      * ADD: - \SetAlgoCaptionSeparator which sets the separator between Algorithm 1 and the
%                               title. By default it's ':' and caption looks like "Algorithm 2: title" but now
%                               you can change it by using for example \SetAlgoCaptionSeparator{.} which will
%                               give "Algorithm 3. title"
%                      * ADD: - \SetAlgoLongEnd and \SetAlgoShortEnd and \SetAlgoNoEnd commands which act as
%                               corresponding package options
%                      * ADD: - OPTIONS italiano and slovak as new language (thanks to Roberto Posenato and
%                               Miroslav Binas) 
%                      * CHANGE: - Fnt and Sty macro to have consistent use and naming (see below)
%                      * ADD: - \AlCapSty, \AlCapNameSty, \AlCapFnt, \AlCapNameFnt, \ProcSty, \ProcFnt,
%                               \ProcNameSty, \ProcNameFnt, \ProcArgSty, ProcArgFnt and corresponding "set macro" 
%                               \SetAlCapSty, \SetAlCapNameSty, \SetAlCapFnt, \SetAlCapNameFnt, \SetProcSty,
%                               \SetProcFnt, \SetProcNameSty, \SetProcNameFnt, \SetProcArgSty, \SetProcArgFnt which
%                               control the way caption is printed. Sty macro use command taking one parameter as
%                               argument, Fnt macros use directly command. In Fact caption is printed as follow:
%                               \AlCapSty{\AlCapFnt Algorithm 1:}\AlCapNameSty{\AlCapNameFnt my algorithm}
%                               By default, \AlCapSty is textbf and \AlCapFnt is nothing. \AlCapNameSty keep text 
%                               as it is, and \AlCapNameFnt do nothing also.
%                               You can redefine \AlCapFnt and \AlCapNameFnt by giving macro to \Set commands. For
%                               example, you can do \SetAlCapFnt{\large} to see Algorithm printed in \large font.
%                               You can redefine \AlCapSty, \AlCapFnt, \AlCapNameSty and \AlCapNameFnt with the
%                               corresponding \Set command. For the Sty commands, you have to give in parameter
%                               name of a macro (whithout \)  which takes one argument. For example,
%                               \SetAlCapFnt{textbf} defines the default behaviour. If you want to do more
%                               complicated thing, you should define your own macro and give it to \SetAlCapFnt or
%                               \SetAlCapNameFnt. Here are two examples:
%                               - \newcommand{\mycapsty}[1]{\tiny #1}\SetAlCapNameSty{mycapsty}
%                               - \newcommand{\mycapsty}[1]{\textsl{\small #1}}\SetAlCapNameSty{mycapsty}
%                               Or you can combine the two, for the last example you can also do:
%                               \SetAlCapNameSty{textsl}\SetAlCapNameFnt{\small}
%                               Thanks to Jan Stilhammer who gives me the idea of \AlCapNameFnt.
%                      * CHANGE \AlTitleFnt to match definition of all other Fnt macros and add a \AlTitleSty 
%                               macro (see below) . Now you set \AlTitleFnt by calling \SetAlTitleFnt with 
%                               directly a macro without parameter in argument:
%                               Example: \SetAlTitleFnt{\small} to set title in small font.
%                      * ADD: - \AlTitleSty and \SetAlTitleSty commands to set a style for title. These commands
%                               are defined from a macro taking the text in argument, as \textbf for example. 
%                               To set the TitleSty you have to give name of the macro (without the '\') 
%                               to \SetAlTitleSty. For example \SetAlTitleSty{textbf} to set \textbf style.
%                      * ADD: - new command \SetAlgorithmName{algorithmname}{list of algorithms name} which
%                               redefines name of the algorithms and the sentence list of algorithms. Second
%                               argument is the name that \autoref, from hyperref package, will use. Example:
%                               \SetAlgorithmName{Protocol}{List of protocols} if you prefer protocol than
%                               algorithm.
%                      * ADD: - new \SetAlgoRefName{QXY} which change the default ref (number of the algorithm) by
%                               the name given in parameter (QXY in the example). 
%                      * ADD: - new command \SetAlgoRefRelativeSize{-2} which sets the output size of refs, defined
%                               by \SetAlgoRefName, used in list of algorithms.
%                      * ADD: - two dimensions to control the layout of caption in ruled, algoruled and boxruled
%                               algorithms:
%                               - interspacetitleruled (2pt by defaut) which controls the vertical space between
%                                 rules and title in ruled and algoruled algorithms.
%                               - interspaceboxruled (2\lineskip by default) which controls the vertical space
%                                 between rules and title in boxruled algorithms.
%                               These two dimensions can be changed by using \setlength command.
%                      * ADD: - With the fix (see below) of procedure and function environments, a new feature has
%                               been added: the name of the procedure or function set in caption is automatically
%                               defined as a KwFunction and so can be used as a macro. For example, if inside a
%                               procedure environment you set \caption{myproc()}, you can use \myproc macro in you
%                               main text. Beware that the macro is only defined after the \caption!
%                      * ADD: - OPTION nokwfunc to unable the new feature described above in function and
%                               procedure environment. Useful if you use name of procedure or function that cannot
%                               be a command name as a math display for example.
%                      * ADD: - \SetAlgoNlRelativeSize{number} command which sets the relative size of line
%                               numbers. By default, line numbers are two size smaller than algorithm text. Use
%                               this macro to change this behavior. For example, \SetAlgoNlRelativeSize{0} sets it
%                               to the same size, \SetAlgoNlRelativeSize{-1} to one size smaller and
%                               \SetAlgoNlRelativeSize{1} to one size bigger
%                      * ADD: - \SetAlgoProcName{aname} command which sets the name of Procedure printed by
%                               procedure environment (the environment prints Procedure by default). Second
%                               argument is the name that \autoref, from hyperref package, will use.
%                      * ADD: - \SetAlgoFuncName{aname} command which sets the name of Function printed by
%                               procedure environment (the environment prints Function by default). Second
%                               argument is the name that \autoref, from hyperref package, will use. 
%                      * ADD: - \SetAlgoCaptionLayout{style} command which sets style of the caption; style must
%                               be the name of a macro taking one argument (the text of the caption). Examples
%                               below show how to use it:
%                               . \SetAlgoCaptionLayout{centerline} to have centered caption
%                               . \SetAlgoCaptionLayout{textbf} to have bold caption
%                               If you want to apply two styles in the same time, such as centered bold, you have
%                               to define you own macro and then use \SetAlgoCaptionLayout with its name.
%                      * ADD: - OPTION procnumbered: which makes the procedure and function to be numbered as
%                               algorithm
%                      * ADD: - OPTIONS tworuled and boxruled
%                               these are two new layouts: tworuled acts like ruled but doesn't put a line after
%                               caption ; boxruled surround algorithm by a box, puts caption above and add a line
%                               after caption.
%                      * REMOVE: - SetKwInParam has been deleted since not useful itself because of different
%                                macros which can do the same in a better and a more consistent way as
%                                SetKwFunction or SetKw.
%                      * FIX: - line number is now correctly vertically aligned with math display.
%                      * FIX: - references with hyperref. No more same identifier or missing name error. BUT now
%                               you must NOT use naturalnames option of hyperref packages if you do PdfLaTeX
%                      * FIX: - autoref with hyperref package (thanks to J?rg Sommer who notices the problem).
%                      * FIX: - titlenumbered was not working! fixed.
%                      * FIX: - Else(){} acted like uElse. Corrected.
%                      * FIX: - noend management: when a block was inside another and end of block was following
%                               each other, a blank line was added: it's now corrected.
%                      * FIX: - Function and Procedure environment was no more working as defined originally: the
%                               label was no more name of the procedure, it acts always as if procumbered option
%                               has been used.
%                      * FIX: - line numbers had a fixed size which can be bigger than algorithm text accordingly
%                               to \AlFnt set (see also new command \SetAlgoNlRelativeSize above)
%                      * FIX: - semicolon in comments when dontprintsemicolon is used.
%                      * FIX: - listofalgorithms adds a vertical space before first algo of a chapter as for
%                               listoffigures or listoftables
%                      * FIX: - listofalgorithms with twocolumns mode and some classes which don't allow onecolumn
%                               and so don't define \if@restonecol as prescribed in LaTeX (sig-alternate for
%                               example)
%                      * FIX: - algorithm2e now works with elsart cls and some more classes.
%                      * FIX: - blocks defined by SetKwBlock act now as other blocks (if for instance) and don't
%                               write end in vlined mode, instead they print a small horizontal line as required
%                               by the option.
%                      * FIX: - underfull hbox warning at each end of algorithm environment removed.
%
%                      * INTERNAL CHANGE: - short end keyword are deduce from long end keyword by keeping the
%                                           first one. Allows to avoid double definition.
%                      * INTERNAL CHANGE: - procedure, function and algorithm are now resolved by the same
%                               environment to avoid code duplication. 
%
%   - October  04 2005  - revision 3.9 -
%                      * ADD: - \setalcaphskip command which sets the horizontal skip before Algorithm: in caption
%                               when used in ruled algorithm.
%                      * ADD: - \SetAlgoInsideSkip command which allows to add an extra vertical space before and
%                               after the core of the algorithm (ie: \SetAlgoInsideSkip{bigskip}) 
%                      * CHANGE: - caption, when used with figure option, is no more controlled by algorithm2e
%                                  package and so follows the exact behaviour of figures. The drawback is that you
%                                  cannot change the typo with AlTitleFnt or CapFnt. The avantage is that if you
%                                  use caption package, it works.
%                      * FIX: - problem with numbering line and pdflatex
%                      * FIX: - error when algorithm2e package was used with beamer and listings together
%   - February 12 2005  - revision 3.8 -
%                      * FIX: - extra line with noend option.
%   - February 10 2005  - revision 3.7 -
%                      * ADD: - sidecomment: different macros allowing to put text right after code on the same
%                               line. They are defined in the same time comment macros are defined with a star
%                               after the macro name. By default comments are right justified but this can be
%                               change with appropriate option in the macro. Ex:
%                               . default: \tcc*{side comment}
%                               . same as previous: \tcc*[r]{side comment}
%                               . left justify: \tcc*[l]{side comment}
%                               . here: \tcc*[h]{side comment} don't put the end of line mark before
%                                       comment (; by default) and don't end the line.
%                               . flushed: \tcc*[f]{side comment} same as the precedent but right
%                                 justified
%                      * ADD: - OPTION scright (default): right justified side comments (side comments
%                               are flushed to the righr)
%                      * ADD: - OPTION scleft: left justified side comments (side comments are put right after the
%                               code line)
%                      * ADD: - \SetSideCommentLeft acts as scleft option
%                      * ADD: - \SetSideCommentRight acts as scright option
%                      * ADD: - block like macro side text: all macro defining a block allows now to put text right
%                               after key words by putting text into (). Done to be used with sidecomment macros,
%                               but all text can be used. 
%                               Ex: \eIf(\tcc*[f]{then comment}){test}{then text}(else side text){else text}
%                      * ADD: - OPTION fillcomment (default): end mark of comment is flushed to the right so
%                               comments fill all the width of text.
%                      * ADD: - OPTION nofillcomment: end mark of comment is put right after the comment.
%                      * ADD: - \SetNoFillComment acts as nofillcomment option.
%                      * ADD: - \SetFillComment acts as fillcomment option.
%                      * ADD: - OPTION dotocloa: which adds an entry in the toc for the list of algorithms. This
%                               option load package tocbibind if not already done and so list of figures and list
%                               of tables are also added in the toc. If you want to control which ones of the lists
%                               will be added in the toc, please load package tocbibind before package algorithm
%                               and give it the options you want.
%                      * FIX: - vertical spacing for uif macro with noend option
%                      * FIX: - all the compatibility problems between caption and other packages
%                      * FIX: - typographical differences between list of algorithms and other lists  when in
%                               report or book 
%
%   - January 24 2005  - revision 3.6 -
%                      * FIX: - vertical spacing and space characters at the beginning or end of comments.
%                               line numbers of comments not in the NlSty.
%                               Thanks to Arnaud Giersch for his comments and suggestions.
%                      * FIX: - Set*Sty macro: the styles defined was not protected and was modified by surrounding
%                               context. For example KwTo in a \For{}{} was in bold AND italic instead of just in
%                               bold.
%                      * FIX: - line number misplacement after \Indp
%
%   - January 21 2005  - revision 3.5 -
%                      * ADD: - hidden numbering of the lines. Lines are auto-numbered but numbers are shown only
%                               on lines you specify:
%                               * linesnumberedhidden option or \LinesNumberedHidden macro activate this
%                                 functionnality.
%                               * \ShowLn and \ShowLnLabel{lab} macros make the number visible on the
%                               line. \ShowLnLabel{lab} allows to set a label for this line. 
%                               Thanks to Samson de Jager who makes this suggestion and provides the macros.
%                      * ADD: - \AlCapFnt and \SetAlCapFnt which allow to have a different font for
%                               caption. Works like \AlFnt and \SetAlFnt and by default is the same.
%                      * ADD: - \AlCapSkip skip length. This vertical space is added before caption in plain ou
%                               boxed mode. It allows to change distance between text and caption.
%                      * FIX: - caption compatible with IEEEtran class. 
%                      * FIX: - some vertical spacing error with \uIf macros (Thanks to Arnaud Giersch)
%                      * FIX: - Procedure and Function: lines are also numbered like algorithms
%                      * FIX: - CommentSty was not used for Comments
%
%   - January 10 2005  - revision 3.4 -
%                      * FIX: - caption compatible with new release of Beamer class. 
%
%   - June 16 2004     - revision 3.3 - 
%                      * FIX: - Hyperlink references of Hyperref package works now if compiled with pdflatex 
%                               and [naturalnames] option of hyperref package is used.
%                      * FIX: - algorithm[H] had problem in an list environment - corrected
%                      * FIX: - interline was not so regular in nested blocks - corrected
%                      * ADD  - \SetVlineSkip macro which sets the vertical skip after the little horizontal 
%                               rule which closes a block in Vlined mode. By default 0.8ex
%
%   - June 11 2004     - revision 3.2 - AUTO NUMBERING LINES !!!
%                      * ADD: auto numbering of the lines (the so asked and so long awaiting feature)
%                             this feature is managed by 3 options and 3 commands:
%                             - linesnumbered option: lines of the algo are numbered except for comments and
%                               input/output (KwInput and KwInOut)
%                             - commentsnumbered option: makes comments be numbered
%                             - inoutnumbered option: makes data input/output be numbered
%                             - \nllabel{lab} labels the line so you can cite with \ref{lab}
%                             - \LinesNumbered make the following algorithms having auto-numbered lines
%                             - \linesnotnumbered make the following algorithms having no auto-numbered lines
%                      * Change: algo2e option renames listofalgorithms in listofalgorithmes
%                      * FIX: new solution for compatibility with color package, more robust and not tricky.
%                             Many thanks to David Carlisle for his advices
%
%   - June 09 2004     - revision 3.1 -
%                      * Change: \SetKwSwitch command defines an additionnal macro \uCase and \Case prints end
%                      * Change: now macros SetKw* do a renewcommand if the keyword is already defined. So you can
%                                redefine default definition at your own convenience or change your definition
%                                without introducing a new macro and changing your text.
%                      * ADD: new macro \SetKwIF which do \SetKwIf and
%                             \SetKwIfElseIf.The following default definition has been added:
%                             \SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
%                             and so you get the macros;
%                             \If \eIf \lIf \uIf \ElseIf \uElseIf \lElseIf \Else \uElse \lElse
%                      * ADD: new macro \SetAlgoSkip which allow to fix the vertical skip before and after the
%                             algorithms. Default is smallskip, do \SetAlgoSkip{} if you don't want an extra space
%                             or \SetAlgoSkip{medskip} or \SetAlgoSkip{bigskip} if you want bigger space.
%                      * ADD: macro \SetKwIf defines in addition a new macro \uElse  (depending on wat name you
%                             have given in #2 arg).
%                      * ADD: macro \SetKwIfElseIf defines in addition a new macro \uElse and \ugElseIf (depending
%                             on what name you have given in #2 and #3 arg).
%                      * Change: baseline of algorithm is now top, so two algorithms can be put side by side.
%                      * FIX: Compatibility with color package solved. The problem was due to a redefinition of
%                             standard macros by color package. This solves compatibility problem with other
%                             packages as pstcol or colortbl. (notified by Dirk Fressmann, Antti Tarvainen and Koby
%                             Crammer)
%                      * Fix: extra little shift to the right with boxed style algorithm removed (notified by
%                             P. Tanovski)
%                      * Fix: algoln option was buggy (notified bye Jiaying Shen)
%                      * Fix: german and portuges option didn't work due to bad typo (notified by Martin Sievers,
%                             Thorsten Vitt and Jeronimo Pellegrini)
%                      
%   - February 13 2004 - revision 3.0 -
%                      * Major revision which makes the package independent from float.sty, so now
%                        - algorithm* works better, in particular can be used in multicols environments
%                        - (known bug corrected)
%                          [H] works now for all sort of environment but is handled differently for classic
%                          environment and star environment (algorithm, figure, procedure and function). For star
%                          environment, H acts like for classical figure environment, so it doesn't stay here
%                          absolutely.
%                        - (known bug corrected)
%                          you can use now floatflt package with algorithm package and even with figure
%                          option. Beware that if you want to put an algorithm inside a floatingfigure, it cannot
%                          be floating, so [H] is required and then figure option should not be used, since
%                          standard figure[H] are still floating with LaTeX.
%                      * boxruled: a new style added. Possible now since no style no more defined by the float
%                        package.
%                      * nocaptionofalgo: dosen't print Algorithm #: in the caption for algorithm in ruled or
%                        algoruled style.
%                        note: this is just documentation of a macro which was already in the package.
%   - December 14 2003 - revision 2.52 -
%                      * output message shorter
%                      * French keyword macro \PourTous was missing for longend option, it has been added.
%                      * TitleofAlgo prints Function or Procedure in corresponding environments.
%
%   - October 27 2003  - revision 2.51 - Revision submitted to CTAN archive
%                      * correction of a minor which make caption in procedure
%                        and function to be blanck with pdfscreen package
%                        (thanks to Joel Gossens for the notification)
%                      * add two internal definition to avoid some errors when
%                        used with Hyperref package (Hyperref package need to
%                        define new counter macro from existing ones, and
%                        don't do it for algorithm2e package, so we do it)
%
%   - October 17 2003  - revision 2.50 - first revision for CTAN archive
%                      * add \AlFnt and \SetAlFnt{font} macros: \AlFnt is used at the beginning of the caption and
%                        the body of algorithm in order to define the fonts used for typesetting algorithms. You
%                        can use it elsewhere you want to typeset text as algorithm. For example you can do
%                        \SetAlFnt{\small\sf} to have algorithms typeset in small sf font. Default is nothing so
%                        algorithm is typeset as the text of the document.
%                      * add \AlTitleFnt{text} and \SetAlTitleFnt{font} macros: The {Algorithm: } in the caption is
%                        typeset with \AlTitleFnt{Algorithm:}. You can use it to have text typeset as {Algorithm:}
%                        of captions. Default is textbf.  Default can be redefined by \SetAlTitleFnt{font}, for
%                        example you can do \SetAlTitleFnt{emph}
%                      * add CommentSty typo for text comment.  
%                      * add some compatibility with hyperref package (still an error on multiply defined refs but
%                        pdf correctly generated)
%                      * flush text to left in order to have correct indentation even with class as amsart which
%                        center all figures
%                      * add german, portuguese and czech options for title of algorithms and typo.
%                      * add portuguese translation of predefined keywords * add czech translation of some
%                        predefined keywords
%
%   - December 23 2002 - revision 2.40
%                      * add some French keyword missing
%                      * add function* and procedure* environment like algorithme* environment: print in one column
%                        even if twocolumn option is specified for the document.
%                      * add a new macro \SetKwComment to define macro which writes comments in the text. First
%                        argument is the name of the macro, second is the text put before the comment, third is the
%                        text put at the end of the comment.Default are \tcc and \tcp
%                      * add new options to change the way algo are numbered:
%                        [algopart] algo are numbered within part (counter must exist)
%                        [algochapter] algo are numbered within chapter
%                        [algosection] algo are numbered within section
%
%   - March 27 2002   - revision 2.39
%                      * Gilles Geeraerts: added the \SetKwIfElseIf to manage
%                        if (c)
%                             i;
%                        else if (c)
%                             i;
%                        ...
%                        else
%                             i;
%                        end
%                      * Also added \gIf \gElseIf \gElse.
%
%   - January 02 2001 - revision 2.38
%                      * bugs related to the caption in procedure and function
%                        environment are corrected.
%                      * bug related to option noend (extra vertical space added
%                        after block command as If or For) is corrected.
%                      * czech option language added (thanks to Libor Bus: l.bus@sh.cvut.cz).
%  
%   - October 16 2000 - revision 2.37
%                      * option algo2e added: change the name of environment
%                        algorithm into algorithm2e. So allow to use the package
%                        with some journal style which already define an algorithm
%                        environment.
%  
%   - September 13 2000 - revision 2.36
%                      * option slide added: require package color
%                      * Hack for slide class in order to have correct
%                        margins
%  
%   - November 25 1999 - revision 2.35
%                      * revision number match RCS number
%                      * Thanks to David A. Bader, a new option is added:
%                        noend: no end keywords are printed.
%  
%   - November 19 1999 - revision 2.32
%                      * minor bug on longend option corrected.
%  
%   - August 26 1999 - revision 2.31
%                      * add an option: figure
%                        this option makes algorithms be figure and so are numbered
%                        as figures, have Figure as caption and are put in 
%                        the \listoffigures
%  
%   - January 21 1999 - revision 2.3 beta
%                    add 2 new environments: procedure and function.
%                    These environments works like algorithm environment but:
%                    - the ruled (or algoruled) style is imperative.
%                    - the caption now writes Procedure name....
%                    - the syntax of the \caption command is restricted as
%                      follow: you MUST put a name followed by 2 braces like
%                      this ``()''. You can put arguments inside the braces and
%                      text after. If no argument is given, the braces will be
%                      removed in the title. 
%                    - label now puts the name (the text before the braces in the
%                      caption) of the procedure or function as reference (not
%                      the number like a classic algorithm environment).
%                    There are also two new styles: ProcNameSty and
%                    ProcArgSty. These style are by default the same as FuncSty
%                    and ArgSty but are used in the caption of a procedure or a
%                    function.
%                    
%   - November 28 1996 - revision 2.22
%                    add a new macro \SetKwInParam{arg1}{arg2}{arg3}:
%                    it defines a macro \arg1{name}{arg} which prints name in keyword
%                    style followed byt arg surrounded by arg2 and arg3. The main
%                    application is to a function working as \SetKwInput to be used
%                    in the head of the algorithm. For example
%                    \SetKwInParam{Func}{(}{)} allows
%                    \Func{functionname}{list of arguments} which prints:
%                    \KwSty{functioname(}list of arguments\KwSty{)}
%       
%
%   - November 27 1996 - revision 2.21:
%                    minor bug in length of InOut boxes fixed.
%                    add algorithm* environment.
%
%   - July 12 1996 - revision 2.2: \SetArg and \SetKwArg macros removed.
%                        
%                    \SetArg has been removed since it never has been
%                    documented.
%                    \SetKwArg has been removed since \SetKw can now
%                    take an argument in order to be consistent with
%                    \SetKwData and \SetKwFunction macros.
%
%   - July 04 1996 - revision 2.1: still more LaTeX2e! Minor compatibility break
%
%                    Macros use now \newcommand instead of \def, use of \setlength, 
%                    \newsavebox, ... and other LaTeX2e specific stuff.
%                    The compatibility break:
%                    - \SetData becomes \SetKwData to be more consistent. So the old 
%                      \SetKwData becomes \SetKwInput
%                    - old macros \titleofalgo, \Freetitleofalgo and \freetitleofalgo
%                      from LaTeX209 version which did print a warning message and call 
%                      \Titleofalgo in version 2.0 are now removed!
%
%   - March 13 1996 - revision 2.0: first official major revision.
%   
%
%%%%%%%%%%%%%%
%
%   Known bugs: 
%   -----------
%   - horizontal spacing (indent) doesn't work with revtex4 class.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% for more complete informations you can see algorithm2e.tex
%
%
%%%%%%%%%%%%%%%%%%%%%%%% Identification Part %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\NeedsTeXFormat{LaTeX2e}[1994/12/01]
%
\ProvidesPackage{algorithm2e}[2013/01/06 v5.00 algorithms environments]
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%% Initial Code %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\@makeother\*% some package redefined it as a letter (as color.sty)
\def\@firstword#1 #2\@nil{#1}% an useful fonction
%%%%%%% Utilities:
% \ifArgumentEmpty<c><t><e> ; if c is empty, i.e. {}, then t, else e.
%    Function used internally, but may as well expose it to the user; it's useful
\begingroup
\catcode`\Q=3
\catcode`\T=3
\long\gdef\ALGOCF@argemptyaux#1#2Q#3#4#5T{#4}
\long\gdef\ifArgumentEmpty#1{%
  \begingroup\long\edef\@tempa{\endgroup
    \ALGOCF@argemptyaux#1QQ{\noexpand\@secondoftwo}{\noexpand\@firstoftwo}T%
  }\@tempa
}
\endgroup
% \long\def\ifArgumentEmpty#1{\bgroup
% 	\catcode`\Q=3
% 	\catcode`\T=3
% 	\long\def\@tempa##1##2Q##3##4##5T{##4}%
% 	\xdef\@tempa{\@tempa#1QQ{\noexpand\@secondoftwo}{\noexpand\@firstoftwo}T}%
% \egroup\@tempa}
%%%%%%%%%%%
%
% \algocf@longdef -> shorthand to reduce
%    \expandafter\long\expandafter\def
% to
%    \expandafter\algocf@longdef
% may look insignificant, but reads that much better ;)
\def\algocf@longdef{\long\def}
%
% \algocf@newcommand (and helper \algocf@new@command) behaves like LaTeX's newcommand,
% with two differences:
%  - the argument is not "\<name>", but rather "<name>"; i.e. one level of indirection
%  - if the command exists already, then \renewcommand, rather than \newcommand
\def\algocf@newcommand#1{\expandafter\algocf@new@command\csname#1\endcsname}
\def\algocf@new@command#1{%
	\begingroup \escapechar\m@ne\xdef\@gtempa{{\string#1}}\endgroup
	\expandafter\@ifundefined\@gtempa\newcommand\renewcommand#1}%
%
% \algocf@newcmdside<name><arity><body>
%   The largest time-saver; many commands we define have the pattern:
%     \<name>(<side_text>)<argX><argY>...
%   where "(<side_text>)" is optional. By defining them with this function,
%   the arguments are parsed and renumbered, i.e. the body works as if the
%   command was:
%     \<name><side_text><argX><argY>...
%   and can use \ifArgumentEmpty to see whether its #1 exists (default case
%   for the side text is (), so there's no difference between calling
%     \foo{bar}
%   or
%     \foo(){bar}
%   Technically this is new behaviour, but it shouldn't really occur...
\algocf@longdef\algocf@newcmdside#1#2#3{%
	\expandafter\def\csname#1\endcsname{%
		\@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
	}%
	\expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1){\csname algocf@#1main\endcsname{##1}}%
	\algocf@newcommand{algocf@#1main}[#2]{#3}%
}
%
% a serie of newcmdside macro for block that allows a comment after the end
%     \<name>(<side_text>)<argX><argY>...(<side_text>)% 
%
% 1. kind of begin-end : for command with only one block as begin-end 
\algocf@longdef\algocf@newcmdside@kobe#1#2{% <name of cmd><body of cmd>
  % command starts by checking for side comment at beginning
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
  }%
  % next we strip comment and include it in cmd that get body and check last side comment
  \expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1)##2{\csname algocf@#1checkcomfol\endcsname{##1}{##2}}%
  % now check for last side comment; args are : <first side com (could be empty)>, <body of cmd>
  \expandafter\algocf@longdef\csname algocf@#1checkcomfol\endcsname##1##2{\@ifnextchar({\csname algocf@#1withendcom\endcsname{##1}{##2}}{\csname algocf@#1noendcom\endcsname{##1}{##2}}}% call macro that manages end of command, with or without last side comment
  % finally manage end of macro... with end side comment...
  \expandafter\algocf@longdef\csname algocf@#1withendcom\endcsname##1##2(##3){%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}}%
  % ... or without end side comment
  \expandafter\algocf@longdef\csname algocf@#1noendcom\endcsname##1##2{%
    \csname algocf@#1main\endcsname{##1}{##2}{}}%
  \algocf@newcommand{algocf@#1main}[3]{#2}%
}%
%
% 2. kind of if-else : for command with two blocks as if-then-else 
\algocf@longdef\algocf@newcmdside@koif#1#2{% <name of cmd><body of cmd>
  % command starts by checking for side comment at beginning
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
  }%
  % next we strip comment and include it in cmd that get body and check last side comment
  \expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1)##2##3{\csname algocf@#1checkcomfol\endcsname{##1}{##2}{##3}}%
  % now check for last side comment; args are : <1st side com>, <1st body of cmd>, <2nd body of cmd>
  \expandafter\algocf@longdef\csname algocf@#1checkcomfol\endcsname##1##2##3{\@ifnextchar({\csname algocf@#1withendcom\endcsname{##1}{##2}{##3}}{\csname algocf@#1noendcom\endcsname{##1}{##2}{##3}}}% call macro that manages end of command, with or without last side comment
  % finally manage end of macro... with end side comment...
  \expandafter\algocf@longdef\csname algocf@#1withendcom\endcsname##1##2##3(##4){%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}{##4}}%
  % ... or without end side comment
  \expandafter\algocf@longdef\csname algocf@#1noendcom\endcsname##1##2##3{%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}{}}%
  \algocf@newcommand{algocf@#1main}[4]{#2}%
}%
%
% \algocf@newcmdsides<name><arity><body><tail><closing>
%   Like the command above, but with an optional side text at the end
%   of the command as well, i.e.:
%     \<name>(<side_text>)<argX><argY>(<end_text>)
%   It may be a bit confusing that <arity> doesn't count <end_text>,
%   but since it is for internal use, the naming can be a little more
%   fuzzy. This function behaves as if:
%     <body'> = <body><if end_text: tail{end_text}><closing>
\algocf@longdef\algocf@newcmdsides#1#2#3#4#5{%
	\expandafter\def\csname#1\endcsname{%
		\@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
	}%
	\expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1){\csname algocf@#1main\endcsname{##1}}%
	\algocf@newcommand{algocf@#1main}[#2]{#3\@ifnextchar({\csname algocf@#1end\endcsname}{#4#5}}%
	\expandafter\algocf@longdef\csname algocf@#1end\endcsname(##1){#4{##1}\strut\par}%
}%
%
% definition of commands which can be redefined in options of the package.
%
\newcounter{AlgoLine}%
\setcounter{AlgoLine}{0}%
%
\newcommand{\algocf@algocfref}{\relax}%
\newcommand{\listalgorithmcfname}{}%
\newcommand{\algorithmcfname}{}%
\@ifundefined{algorithmautorefname}{\newcommand{\algorithmautorefname}{algorithm}}{\renewcommand{\algorithmautorefname}{algorithm}}%
\newcommand{\algorithmcflinename}{}%
\newcommand{\algocf@typo}{}%
\newcommand{\@algocf@procname}{}\newcommand{\procedureautorefname}{}%
\newcommand{\SetAlgoProcName}[2]{\renewcommand{\@algocf@procname}{#1}\renewcommand{\procedureautorefname}{#2}}%
\newcommand{\@algocf@funcname}{}\newcommand{\functionautorefname}{}%
\newcommand{\SetAlgoFuncName}[2]{\renewcommand{\@algocf@funcname}{#1}\renewcommand{\functionautorefname}{#2}}%
\newcommand{\@algocf@titleofalgoname}{\algorithmcfname}%
\newcommand{\@algocf@algotitleofalgo}{%
  \renewcommand{\@algocf@titleofalgoname}{\algorithmcfname}}%
\newcommand{\@algocf@proctitleofalgo}{%
  \renewcommand{\@algocf@titleofalgoname}{\algocf@procname}}%
%
\newcommand{\algocf@style}{plain}%
\newcommand{\@ResetCounterIfNeeded}{}%
\newcommand{\@titleprefix}{}%
%
\newcommand{\algocf@numbering}[1]{\newcommand{\algocf@within}{#1}}%
%
\newcommand{\defaultsmacros@algo}{\algocf@defaults@shortend}%
%
\newcommand{\algocf@list}{loa}%
\newcommand{\algocf@float}{algocf}%
%
\newcommand{\algocf@envname}{algorithm}%
\newcommand{\algocf@listofalgorithms}{listofalgorithms}%
%
%
%% redefine chapter so that it adds a vspace in the loa as the original does for lof and lot
% \let\algocf@original@chapter=\chapter%
% \def\chapter{\expandafter\addtocontents{loa}{\protect\addvspace{10\p@}}\algocf@original@chapter}%
%
% bug correction with hyperref submitted by Hubert Meier
\begingroup\expandafter\expandafter\expandafter\endgroup 
\expandafter\ifx\csname @chapter\endcsname\relax\else 
% \let\algocf@original@chapter=\chapter% 
% \def\chapter{\addtocontents{loa}{\protect\addvspace{10\p@}}\algocf@original@chapter}% 
\let\algocf@original@chapter=\@chapter%
\@ifclassloaded{krantz}{%
\def\@chapter[#1][#2]#3{\algocf@original@chapter[#1][#2]{#3}\addtocontents{loa}{\protect\addvspace{10\p@}}}% 
}{%
\def\@chapter[#1]#2{\algocf@original@chapter[#1]{#2}\addtocontents{loa}{\protect\addvspace{10\p@}}}% 
}%
\fi
%
%% if@restonecol is defined in article and book but some other classes don't define it and we need it, so we do
\ifx\if@restonecol\relax\else\newif\if@restonecol\fi%
%
%
%%%%%%%%%%%%%%%%%%%%%% Declaration of Options %%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\RequirePackage{ifthen}%
%
\newboolean{algocf@displayblockmarkers}\setboolean{algocf@displayblockmarkers}{false}%
\DeclareOption{displayblockmarkers}{%
  \setboolean{algocf@displayblockmarkers}{true}%
}
\newboolean{algocf@displaygroupmarkers}{\setboolean{algocf@displaygroupmarkers}{false}
\DeclareOption{displaygroupmarkers}{%
  \setboolean{algocf@displaygroupmarkers}{true}%
}
%
\newboolean{algocf@nokwfunc}\setboolean{algocf@nokwfunc}{false}%
\DeclareOption{nokwfunc}{%
  \setboolean{algocf@nokwfunc}{true}%
}%
%
\newboolean{algocf@oldcommands}\setboolean{algocf@oldcommands}{false}%
\DeclareOption{oldcommands}{%
  \setboolean{algocf@oldcommands}{true}%
}%
%
\newboolean{algocf@leftlinenumber}\setboolean{algocf@leftlinenumber}{true}%
\newcommand{\setLeftLinesNumbers}{\setboolean{algocf@leftlinenumber}{true}}%
\newcommand{\setRightLinesNumbers}{\setboolean{algocf@leftlinenumber}{false}}%
\DeclareOption{rightnl}{%
  \setRightLinesNumbers%
}%
%
\newboolean{algocf@endfloat}\setboolean{algocf@endfloat}{false}%
\DeclareOption{endfloat}{%
  \setboolean{algocf@endfloat}{true}%
  \newcounter{postalgo}\setcounter{postalgo}{0}%
}%
%
\newboolean{algocf@procnumbered}\setboolean{algocf@procnumbered}{false}%
\DeclareOption{procnumbered}{%
  \setboolean{algocf@procnumbered}{true}%
}%
%
\DeclareOption{algo2e}{%
  \renewcommand{\algocf@envname}{algorithm2e}%
  \renewcommand{\algocf@listofalgorithms}{listofalgorithmes}%
}%
%
\newboolean{algocf@slide}\setboolean{algocf@slide}{false}%
\DeclareOption{slide}{%
  \setboolean{algocf@slide}{true}%
}%
%
\newboolean{algocf@figurecaption}\setboolean{algocf@figurecaption}{false}%
\DeclareOption{figure}{%
\renewcommand{\algocf@list}{lof}%
\renewcommand{\algocf@float}{figure}%
\AtBeginDocument{\@ifpackageloaded{caption}{\setboolean{algocf@figurecaption}{true}}{}}%
}%
%
\newboolean{algocf@optonelanguage}\setboolean{algocf@optonelanguage}{false}%
\DeclareOption{onelanguage}{\setboolean{algocf@optonelanguage}{true}}%
%
\newcommand{\algocf@languagechoosen}{english}%
\newboolean{algocf@localkw@english}\setboolean{algocf@localkw@english}{true}%
\DeclareOption{englishkw}{%
\setboolean{algocf@localkw@english}{true}%
}%
%
\DeclareOption{english}{%
\renewcommand{\listalgorithmcfname}{List of Algorithms}%
\renewcommand{\algorithmcfname}{Algorithm}%
\renewcommand{\algorithmautorefname}{algorithm}%
\renewcommand{\algorithmcflinename}{line}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedure}%
\renewcommand{\@algocf@funcname}{Function}%
\renewcommand{\procedureautorefname}{procedure}%
\renewcommand{\functionautorefname}{function}%
\renewcommand{\algocf@languagechoosen}{english}%
}%
%
%----
\newboolean{algocf@localkw@french}\setboolean{algocf@localkw@french}{false}%
\DeclareOption{frenchkw}{%
\setboolean{algocf@localkw@french}{true}%
}%
%
\DeclareOption{french}{%
\renewcommand{\listalgorithmcfname}{Liste des Algorithmes}%
\renewcommand{\algorithmcfname}{Algorithme}%
\renewcommand{\algorithmautorefname}{algorithme}%
\renewcommand{\algorithmcflinename}{ligne}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Proc\'edure}%
\renewcommand{\@algocf@funcname}{Fonction}%
\renewcommand{\procedureautorefname}{proc\'edure}%
\renewcommand{\functionautorefname}{fonction}%
\renewcommand{\algocf@languagechoosen}{french}%
}%
%
%----
\newboolean{algocf@localkw@czech}\setboolean{algocf@localkw@czech}{false}%
\DeclareOption{czechkw}{%
\setboolean{algocf@localkw@czech}{true}%
}%
%
\DeclareOption{czech}{%
\renewcommand{\listalgorithmcfname}{Seznam algoritm\r{u}}%
\renewcommand{\algorithmcfname}{Algoritmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Radek}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funkce}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{czech}%
}%
%
%----
\newboolean{algocf@localkw@german}\setboolean{algocf@localkw@german}{false}%
\DeclareOption{germankw}{%
\setboolean{algocf@localkw@german}{true}%
}%
%
\DeclareOption{german}{%
\renewcommand{\listalgorithmcfname}{Liste der Algorithmen}%
\renewcommand{\algorithmcfname}{Algorithmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Zeile}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Prozedur}%
\renewcommand{\@algocf@funcname}{Funktion}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{german}%
}%
%
%----
\DeclareOption{ngermankw}{%
\setboolean{algocf@localkw@german}{true}%
}%
%
\DeclareOption{ngerman}{%
\renewcommand{\listalgorithmcfname}{Liste der Algorithmen}%
\renewcommand{\algorithmcfname}{Algorithmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Zeile}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Prozedur}%
\renewcommand{\@algocf@funcname}{Funktion}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{german}%
}%
%
%----
\newboolean{algocf@localkw@portuguese}\setboolean{algocf@localkw@portuguese}{false}%
\DeclareOption{portuguesekw}{%
\setboolean{algocf@localkw@portuguese}{true}%
}%
%
\DeclareOption{portuguese}{%
\renewcommand{\listalgorithmcfname}{Lista de Algoritmos}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{linha}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedimento}%
\renewcommand{\@algocf@funcname}{Fun\c{c}\~{a}o}%
\renewcommand{\procedureautorefname}{procedimento}%
\renewcommand{\functionautorefname}{fun\c{c}\~{a}o}%
\renewcommand{\algocf@languagechoosen}{portuguese}%
}%
%
%----
\newboolean{algocf@localkw@italiano}\setboolean{algocf@localkw@italiano}{false}%
\DeclareOption{italianokw}{%
\setboolean{algocf@localkw@italiano}{true}%
}%
%
\DeclareOption{italiano}{%
\renewcommand{\listalgorithmcfname}{Elenco degli algoritmi}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{riga}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funzione}%
\renewcommand{\procedureautorefname}{procedura}%
\renewcommand{\functionautorefname}{funzione}%
\renewcommand{\algocf@languagechoosen}{italiano}%
}%
%----
\newboolean{algocf@localkw@spanish}\setboolean{algocf@localkw@spanish}{false}%
\DeclareOption{spanishkw}{%
\setboolean{algocf@localkw@spanish}{true}%
}%
%
\DeclareOption{spanish}{%
\renewcommand{\listalgorithmcfname}{\'Indice de algoritmos}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{l\'inea}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedimiento}%
\renewcommand{\@algocf@funcname}{Funci\'on}%
\renewcommand{\procedureautorefname}{procedimiento}%
\renewcommand{\functionautorefname}{funci\'on}%
\renewcommand{\algocf@languagechoosen}{spanish}%
}%
%----
\newboolean{algocf@localkw@slovak}\setboolean{algocf@localkw@slovak}{false}%
\DeclareOption{slovakkw}{%
\setboolean{algocf@localkw@slovak}{true}%
}%
%
\DeclareOption{slovak}{%
\renewcommand{\listalgorithmcfname}{Zoznam algoritmov}%
\renewcommand{\algorithmcfname}{Algoritmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Radek}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Proced\'{u}ra}%
\renewcommand{\@algocf@funcname}{Funkcia}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{slovak}%
}%
%
%----
\newboolean{algocf@localkw@croatian}\setboolean{algocf@localkw@croatian}{false}%
\DeclareOption{croatiankw}{%
\setboolean{algocf@localkw@croatian}{true}%
}%
%
\DeclareOption{croatian}{%
\renewcommand{\listalgorithmcfname}{Popis algoritama}%
\renewcommand{\algorithmcfname}{Algoritam}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{redak}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funkcija}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{croatian}%
}%
%%% adding 'turkish' option customization
%
%----
\newboolean{algocf@localkw@turkish}\setboolean{algocf@localkw@turkish}{false}%
\DeclareOption{turkishkw}{%
\setboolean{algocf@localkw@turkish}{true}%
}%
\DeclareOption{turkish}{%
\renewcommand{\listalgorithmcfname}{Algoritma Listesi}%
\renewcommand{\algorithmcfname}{Algoritma}%
\renewcommand{\algorithmautorefname}{algoritma}%
\renewcommand{\algorithmcflinename}{?izgi}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Prosed?r}%
\renewcommand{\@algocf@funcname}{Fonksiyon}%
\renewcommand{\procedureautorefname}{prosed?r}%
\renewcommand{\functionautorefname}{fonksiyon}%
\renewcommand{\algocf@languagechoosen}{turkish}%
}%
%
% OPTIONs plain, boxed, ruled, algoruled & boxruled
%
\newcommand{\algocf@style@plain}{\renewcommand{\algocf@style}{plain}}%
\newcommand{\algocf@style@boxed}{\renewcommand{\algocf@style}{boxed}}%
\newcommand{\algocf@style@ruled}{\renewcommand{\algocf@style}{ruled}}%
\newcommand{\algocf@style@algoruled}{\renewcommand{\algocf@style}{algoruled}}%
\newcommand{\algocf@style@boxruled}{\renewcommand{\algocf@style}{boxruled}}%
\newcommand{\algocf@style@tworuled}{\renewcommand{\algocf@style}{tworuled}}%
\newcommand{\algocf@style@plainruled}{\renewcommand{\algocf@style}{plainruled}}%
\newcommand{\RestyleAlgo}[1]{\csname algocf@style@#1\endcsname}%
\DeclareOption{plain}{\algocf@style@plain}%
\DeclareOption{plainruled}{\algocf@style@plainruled}%
\DeclareOption{boxed}{\algocf@style@boxed}%
\DeclareOption{ruled}{\algocf@style@ruled}%
\DeclareOption{algoruled}{\algocf@style@algoruled}%
\DeclareOption{boxruled}{\algocf@style@boxruled}%
\DeclareOption{tworuled}{\algocf@style@tworuled}%
%
% OPTIONs algopart,algochapter & algosection
%
\DeclareOption{algopart}{\algocf@numbering{part}}%       %algo part numbered
\DeclareOption{algochapter}{\algocf@numbering{chapter}}% %algo chapter numbered
\DeclareOption{algosection}{\algocf@numbering{section}}% %algo section numbered
%
% OPTIONs resetcount & noresetcount
%
\DeclareOption{resetcount}{\renewcommand{\@ResetCounterIfNeeded}{\setcounter{AlgoLine}{0}}}%
\DeclareOption{noresetcount}{\renewcommand{\@ResetCounterIfNeeded}{}}%
%
% OPTIONs algorithm hanging for long lines
%
\newlength{\algocf@hangindent}\setlength{\algocf@hangindent}{.5em}
\newcommand{\SetAlgoHangIndent}[1]{\setlength{\algocf@hangindent}{#1}}
%
\newboolean{algocf@hanging}\setboolean{algocf@hanging}{true}% hanging is handle by default
\newboolean{algocf@hanginginout}\setboolean{algocf@hanginginout}{false}% inout are managed as previously: hanging set by inout keywords
\newboolean{algocf@hangingcomment}\setboolean{algocf@hangingcomment}{false}% comment that are not side comment are indented accordingly to comment mark, not as normal text
\newcommand{\algocf@everyparnl}{\relax}%
\newcommand{\algocf@everyparhanging}{\hangafter=1\hangindent=\algocf@hangindent\relax}%
\newcommand{\algocf@everypar}{\algocf@everyparnl\algocf@everyparhanging}%
\newcommand{\algocf@seteverypar}{%
  \ifthenelse{\boolean{algocf@hanging}}{\everypar{\algocf@everypar}}{\relax}%
}%
%
\newcommand{\algocf@seteveryparnl}[1]{\renewcommand{\algocf@everyparnl}{#1}\everypar{\algocf@everypar}}%
\newcommand{\algocf@seteveryparhanging}[1]{%
\let\algocf@oldeveryparhanging=\algocf@everyparhanging%
\renewcommand{\algocf@everyparhanging}{#1}\everypar{\algocf@everypar}%
}%
\newcommand{\algocf@reseteveryparhanging}{%
\let\algocf@everyparhanging=\algocf@oldeveryparhanging%
\everypar{\algocf@everypar}%
}%
\DeclareOption{hanginginout}{\setboolean{algocf@hanginginout}{true}}%
\DeclareOption{hangingcomment}{\setboolean{algocf@hangingcomment}{true}}%
\DeclareOption{noalgohanging}{%
  \setboolean{algocf@hanginginout}{false}%
  \setboolean{algocf@hangingcomment}{false}%
  \setboolean{algocf@hanging}{false}%
}%
%\newcommand{
%
%
% OPTION linesnumbered
%
\newboolean{algocf@linesnumbered}\setboolean{algocf@linesnumbered}{false}%
\newcommand{\algocf@linesnumbered}{\relax}%
\DeclareOption{linesnumbered}{%
  \setboolean{algocf@linesnumbered}{true}%
  \renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\nl}}%
}%
%
% OPTION linesnumberedhidden
%
\DeclareOption{linesnumberedhidden}{%
  \setboolean{algocf@linesnumbered}{true}%
  \renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\stepcounter{AlgoLine}}}%
}%
%
% OPTION commentsnumbered inoutnumbered
%
\newboolean{algocf@commentsnumbered}\setboolean{algocf@commentsnumbered}{false}%
\DeclareOption{commentsnumbered}{\setboolean{algocf@commentsnumbered}{true}}%
\newboolean{algocf@inoutnumbered}\setboolean{algocf@inoutnumbered}{false}%
\DeclareOption{inoutnumbered}{\setboolean{algocf@inoutnumbered}{true}}%
%
% OPTIONs titlenumbered & titlenotnumbered
%
\DeclareOption{titlenumbered}{%
  \renewcommand{\@titleprefix}{%
    \refstepcounter{\algocf@float}%
    \AlTitleSty{\AlTitleFnt\@algocf@titleofalgoname\ \expandafter\csname the\algocf@float\endcsname\algocf@typo: }%
  }%
}%
%
\DeclareOption{titlenotnumbered}{\renewcommand{\@titleprefix}{%
    \AlTitleSty{\AlTitleFnt\@algocf@titleofalgoname\algocf@typo: }}%
}%
%
% OPTIONs algonl
% line numbered with the counter of the algorithm
%
\DeclareOption{algonl}{\renewcommand{\theAlgoLine}{\expandafter\csname the\algocf@float\endcsname.\arabic{AlgoLine}}}%
%
% OPTIONs lined, vlined & noline
%
\DeclareOption{lined}{\AtBeginDocument{\SetAlgoLined}}%   \SetAlgoLined (default)
\DeclareOption{vlined}{\AtBeginDocument{\SetAlgoVlined}}% \SetAlgoVlined
\DeclareOption{noline}{\AtBeginDocument{\SetAlgoNoLine}}%\SetAlgoNoLine
%
% OPTIONs longend, shotend & noend
%
\DeclareOption{longend}{\AtBeginDocument{\SetAlgoLongEnd}}%  \SetAlgoLongEnd
\DeclareOption{shortend}{\AtBeginDocument{\SetAlgoShortEnd}}%\SetAlgoShortEnd
\DeclareOption{noend}{\AtBeginDocument{\SetAlgoNoEnd}}%      \SetAlgoNoEnd
%
\DeclareOption{nosemicolon}{\AtBeginDocument{\DontPrintSemicolon}}%      \SetAlgoNoEnd
%
% OPTION dotoc
%
\newboolean{algocf@dotocloa}\setboolean{algocf@dotocloa}{false}%
\DeclareOption{dotocloa}{%
  \setboolean{algocf@dotocloa}{true}%
}
%
% OPTION comments
%
\newboolean{algocf@optfillcomment}\setboolean{algocf@optfillcomment}{true}%
\DeclareOption{nofillcomment}{%
  \setboolean{algocf@optfillcomment}{false}%
}%
\DeclareOption{fillcomment}{%
  \setboolean{algocf@optfillcomment}{true}%
}%
%
% OPTION sidecommments
%
\newboolean{algocf@scleft}\setboolean{algocf@scleft}{false}%
\DeclareOption{scleft}{%
  \setboolean{algocf@scleft}{true}%
}%
\DeclareOption{sright}{% default
  \setboolean{algocf@scleft}{false}%
}%
%
% OPTION norelsize
%
\newboolean{algocf@norelsize}\setboolean{algocf@norelsize}{false}%
\DeclareOption{norelsize}{%
  \setboolean{algocf@norelsize}{true}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%% Execution of Options %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\ExecuteOptions{english,plain,resetcount,titlenotnumbered,lined,shortend}%
%
\ProcessOptions%
%
\@algocf@algotitleofalgo% fix name for \TitleOfAlgo to \algorithmcfname by default
%
%%%%%%%%%%%%%%%%%%%%%%%%%% Package Loading %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
\RequirePackage{xspace}%
%
\ifthenelse{\boolean{algocf@endfloat}}{%
  \RequirePackage{endfloat}%
}{\relax}%
%
\ifthenelse{\boolean{algocf@norelsize}}{%
  \newcommand{\relsize}[1]{\scriptsize}%
}{%
  \RequirePackage{relsize}%
}%
%
\ifthenelse{\boolean{algocf@slide}}{\RequirePackage{color}}{}%
%
%
\AtEndOfPackage{%
  \ifthenelse{\boolean{algocf@dotocloa}}{%
    \renewcommand{\listofalgorithms}{\tocfile{\listalgorithmcfname}{loa}}%
  }{\relax}%
}%
%
% if loa in toc required, load tocbibind package if not already done.
\ifthenelse{\boolean{algocf@dotocloa}}{%
  \ifx\@tocextra\undefined%
  \RequirePackage{tocbibind}%
  \fi%
}{\relax}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Main Part %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\newcommand{\algocf@name}{algorithm2e}%
\newcommand{\algocf@date}{october 19 2015}%
\newcommand{\algocf@version}{Release 5.1}%
\newcommand{\algocf@id}{\algocf@version\space -- \algocf@date\space --}%
\typeout{********************************************************^^JPackage `\algocf@name'\space\algocf@id^^J%
         - algorithm2e-announce@lirmm.fr  mailing list for announcement about releases^^J%
         - algorithm2e-discussion@lirmm.fr mailing list for discussion about package^^J%
         subscribe by emailing sympa@lirmm.fr with 'subscribe <list> <firstname name>'^^J%
         - Author: Christophe Fiorio (christophe.fiorio@umontpellier.fr)^^J********************************************************}%
%%
%%
%%
%%
%%
%%
%%%% hyperref compatibility tricks: Hyperref package defines H counters from
   % standard counters (i.e \theHpage from \thepage) and check some particular
   % counters of some packages, unfortunately it doesn't do the same for
   % algorithm2e package but act as Hcounter was defined. To avoid errors we
   % defined \theHalgocf ourself
%%%%
%
\@ifundefined{theHalgocf}{\def\theHalgocf{\thealgocf}}{}%
\@ifundefined{theHAlgoLine}{\def\theHAlgoLine{\theAlgoLine}}{}%
\@ifundefined{theHalgocfproc}{\def\theHalgocfproc{0}}{}%
\@ifundefined{theHalgocffunc}{\def\theHalgocffunc{0}}{}%
\@ifundefined{toclevel@algocf}{\def\toclevel@algocf{0}}{}%
%
% autoref from hyperref needs an autorefname, so we give it.
\def\AlgoLineautorefname{\algorithmcflinename}%
\def\algocfautorefname{\algorithmautorefname}%
\def\algocfprocautorefname{\procedureautorefname}%
\def\algocffuncautorefname{\functionautorefname}%
%%
%%
%%
\newcommand{\@defaultskiptotal}{0.5em}%
\newskip\skiptotal\skiptotal=0.5em%
\newskip\skiplinenumber\skiplinenumber=\hsize\advance\skiplinenumber by-\skiptotal%
\newskip\skiprule%
\newskip\skiphlne%
\newskip\skiptext%
\newskip\skiplength%
\newskip\algomargin%
\newskip\skipalgocfslide\skipalgocfslide=1em%
\newdimen\algowidth%
\newdimen\inoutsize%
\newdimen\inoutindent%
\newdimen\interspacetitleruled\setlength{\interspacetitleruled}{2pt}%
\newdimen\interspacealgoruled\setlength{\interspacealgoruled}{2pt}%
\newdimen\interspacetitleboxruled\setlength{\interspacetitleboxruled}{2\lineskip}%
%
\newcommand{\@algoskip}{\smallskip}%
\newcommand{\SetAlgoSkip}[1]{\renewcommand{\@algoskip}{\csname#1\endcsname}}%
\newcommand{\@algoinsideskip}{\relax}%
\newcommand{\SetAlgoInsideSkip}[1]{\renewcommand{\@algoinsideskip}{\csname#1\endcsname}}%
%
% ruledwidth
%
\newlength{\algocf@ruledwidth}\setlength{\algocf@ruledwidth}{\linewidth}%
\newboolean{algocf@customruledwidth}\setboolean{algocf@customruledwidth}{false}%
\newcommand{\SetCustomAlgoRuledWidth}[1]{%
  \setboolean{algocf@customruledwidth}{true}%
  \ifthenelse{\boolean{algocf@customruledwidth}}{\setlength{\algocf@ruledwidth}{#1}}{\relax}%
}%
%
\newsavebox{\algocf@inoutbox}%
\newsavebox{\algocf@inputbox}%
%%
%%
\newcommand{\arg@e}{}%
\newcommand{\arg@space}{\ }%
\newcommand{\BlankLine}{\vskip 1ex}%
%%
\newcommand{\vespace}{1ex}%
\newcommand{\SetInd}[2]{%
\skiprule=#1%
\skiptext=#2%
\skiplength=\skiptext\advance\skiplength by \skiprule\advance\skiplength by 0.4pt}%
\SetInd{0.5em}{1em}
\algomargin=\leftskip\advance\algomargin by \parindent%
\newcommand{\IncMargin}[1]{\advance\algomargin by #1}%
\newcommand{\DecMargin}[1]{\advance\algomargin by -#1}%
\newcommand{\SetNlSkip}[1]{%
  \renewcommand{\@defaultskiptotal}{#1}%
  \setlength{\skiptotal}{#1}}%
%%
\newskip\AlCapSkip\AlCapSkip=0ex%
\newskip\AlCapHSkip\AlCapSkip=0ex%
\newcommand{\SetAlCapSkip}[1]{\setlength{\AlCapSkip}{#1}}%
\newcommand{\SetAlCapHSkip}[1]{\setlength{\AlCapHSkip}{#1}}%
\SetAlCapHSkip{.5\algomargin}%
%%
%%
\newskip\algoskipindent
\newcommand{\algocf@adjustskipindent}{%
  \algoskipindent=\skiprule%
  \advance\algoskipindent by \skiptext\advance\algoskipindent by 0.4pt}
\algocf@adjustskipindent%
%
\newcommand{\Indentp}[1]{\advance\leftskip by #1}%
\newcommand{\Indp}{\algocf@adjustskipindent\advance\leftskip by \algoskipindent}
\newcommand{\Indpp}{\advance\leftskip by 0.5em}%
\newcommand{\Indm}{\algocf@adjustskipindent\advance\leftskip by -\algoskipindent}
\newcommand{\Indmm}{\advance\leftskip by -0.5em}%
%
%%
%%
%% Line Numbering
%%
%%
% number line style
\newcommand{\algocf@nlrelsize}{-2}\newcommand{\SetAlgoNlRelativeSize}[1]{\renewcommand{\algocf@nlrelsize}{#1}}%
\newcommand{\NlSty}[1]{\textnormal{\textbf{\relsize{\algocf@nlrelsize}#1}}}% default definition
\newcommand{\SetNlSty}[3]{\renewcommand{\NlSty}[1]{\textnormal{\csname#1\endcsname{\relsize{\algocf@nlrelsize}#2##1#3}}}}%
%
% nl definitions
%
\newsavebox{\algocf@nlbox}%
\newcommand{\algocf@printnl}[1]{%
  \ifthenelse{\boolean{algocf@leftlinenumber}}{%
    \skiplinenumber=\skiptotal\advance\skiplinenumber by\leftskip%
    \strut\raisebox{0pt}{\llap{\NlSty{#1}\kern\skiplinenumber}}\ignorespaces%
  }{%
    \sbox\algocf@nlbox{\NlSty{#1}}%
    \skiplinenumber=\hsize\advance\skiplinenumber by-\leftskip\advance\skiplinenumber by-\skiptext%
    \advance\skiplinenumber by\algomargin\advance\skiplinenumber by.3em\advance\skiplinenumber by-\wd\algocf@nlbox%
    % to handle particular case of until: printnl is after 'until' keyword has been writen, so we need to substract length of this keyword
    \advance\skiplinenumber by-\algocf@skipuntil%
    \strut\raisebox{0pt}{\rlap{\kern\skiplinenumber\NlSty{#1\ignorespaces}}}\ignorespaces%
  }%
}%
\newcommand{\algocf@nl@sethref}[1]{%
  \renewcommand{\theHAlgoLine}{\thealgocfproc.#1}%
  \hyper@refstepcounter{AlgoLine}\gdef\@currentlabel{#1}%
}%
\newcommand{\nl}{%
  \@ifundefined{hyper@refstepcounter}{% if not hyperref then do a simple refstepcounter
    \refstepcounter{AlgoLine}\gdef\@currentlabel{\theAlgoLine}%
  }{% else if hyperref, do the anchor so 2 lines in two differents algorithms cannot have the same href
    \stepcounter{AlgoLine}\algocf@nl@sethref{\theAlgoLine}%
  }% now we can do the line numbering
  \algocf@printnl{\theAlgoLine}%
}%
%
\newcommand{\nllabel}[1]{\label{#1}}%
%
\newcommand{\enl}{%
  \@ifundefined{hyper@refstepcounter}{% if not hyperref then do a simple refstepcounter
    \refstepcounter{AlgoLine}\gdef\@currentlabel{\theAlgoLine}%
  }{% else if hyperref, do the anchor so 2 lines in two differents algorithms cannot have the same href
    \stepcounter{AlgoLine}\algocf@nl@sethref{\theAlgoLine}%
  }% now we can do the line numbering
  \skiplinenumber=\hsize\advance\skiplinenumber by-\leftskip%
  \strut\raisebox{0pt}{\rlap{\kern\skiplinenumber\strut\NlSty{\theAlgoLine}}}\ignorespaces%
}%
%% nlset
\newcommand{\nlset}[1]{%
  \@ifundefined{hyper@refstepcounter}{\protected@edef\@currentlabel{#1}}{\algocf@nl@sethref{#1}}\algocf@printnl{#1}%
}%
%
%% lnl definitions
\newcommand{\lnl}[1]{\nl\label{#1}\ignorespaces}%
%
%% lnlset
\newcommand{\lnlset}[2]{\nlset{#2}\label{#1}}%
%
% set char put at end of each line
%
\newcommand{\algocf@endline}{\string;}
\newcommand{\SetEndCharOfAlgoLine}[1]{\renewcommand{\algocf@endline}{#1}}
%
% end of line definition
%
\newcommand{\@endalgocfline}{\algocf@endline}% default definition: printsemicolon
\newcommand{\DontPrintSemicolon}{\renewcommand{\@endalgocfline}{\relax}}%
\newcommand{\PrintSemicolon}{\renewcommand{\@endalgocfline}{\algocf@endline}}%
\newcommand{\@endalgoln}{\@endalgocfline\hfill\strut\par}%
%
% line numbering
%
\newcommand{\LinesNumbered}{\setboolean{algocf@linesnumbered}{true}\renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\nl}}}%
\newcommand{\LinesNotNumbered}{%
  \setboolean{algocf@linesnumbered}{false}%
  \renewcommand{\algocf@linesnumbered}{\relax}%
}%
%
\newcommand{\LinesNumberedHidden}{%
  \setboolean{algocf@linesnumbered}{true}\renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\stepcounter{AlgoLine}}}}%
\newcommand{\ShowLn}{\nlset{\theAlgoLine}\ignorespaces}% display the line number on this line (without labelling)
\newcommand{\ShowLnLabel}[1]{\lnlset{#1}{\theAlgoLine}\ignorespaces}% display the line number and label this line
%
%%
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Styling text commands
%
\newcommand{\AlFnt}{\relax}% default definition
\newcommand{\SetAlFnt}[1]{\renewcommand{\AlFnt}{#1}}%
\newcommand{\AlTitleFnt}{\relax}% default definition
\newcommand{\SetAlTitleFnt}[1]{\renewcommand{\AlTitleFnt}{#1}}%
%
\newcommand{\AlCapFnt}{\relax}% default definition
\newcommand{\SetAlCapFnt}[1]{\renewcommand{\AlCapFnt}{#1}}%
\newcommand{\AlCapNameFnt}{\relax}% default definition
\newcommand{\SetAlCapNameFnt}[1]{\renewcommand{\AlCapNameFnt}{#1}}%
%
\newcommand{\ProcFnt}{\relax}% default definition
\newcommand{\SetProcFnt}[1]{\renewcommand{\ProcFnt}{#1}}%
\newcommand{\ProcNameFnt}{\relax}% default definition
\newcommand{\SetProcNameFnt}[1]{\renewcommand{\ProcNameFnt}{#1}}%
\newcommand{\ProcArgFnt}{\relax}% default definition
\newcommand{\SetProcArgFnt}[1]{\renewcommand{\ProcArgFnt}{#1}}%
%
\newcommand{\AlTitleSty}[1]{\textbf{#1}\unskip}% default definition
\newcommand{\SetAlTitleSty}[1]{\renewcommand{\AlTitleSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\AlCapSty}[1]{\textnormal{\textbf{#1}}\unskip}% default definition
\newcommand{\SetAlCapSty}[1]{\renewcommand{\AlCapSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\AlCapNameSty}[1]{\textnormal{#1}\unskip}% default definition
\newcommand{\SetAlCapNameSty}[1]{\renewcommand{\AlCapNameSty}[1]{\textnormal{\csname #1\endcsname{##1}}\unskip}}%
%
\newcommand{\ProcSty}[1]{\AlCapSty{#1}}%
\newcommand{\SetProcSty}[1]{\renewcommand{\ProcSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProcNameSty}[1]{\AlCapNameSty{#1}}%
\newcommand{\SetProcNameSty}[1]{\renewcommand{\ProcNameSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProcArgSty}[1]{\AlCapNameSty{#1}}%
\newcommand{\SetProcArgSty}[1]{\renewcommand{\ProcArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
%
\newcommand{\KwSty}[1]{\textnormal{\textbf{#1}}\unskip}% default definition
\newcommand{\SetKwSty}[1]{\renewcommand{\KwSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ArgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetArgSty{emph}
\newcommand{\SetArgSty}[1]{\renewcommand{\ArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\FuncArgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetFuncArgSty{emph}
\newcommand{\SetFuncArgSty}[1]{\renewcommand{\FuncArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\FuncSty}[1]{\textnormal{\texttt{#1}}\unskip}%\SetFuncSty{texttt}
\newcommand{\SetFuncSty}[1]{\renewcommand{\FuncSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetProgSty{emphg}
\newcommand{\SetProgSty}[1]{\renewcommand{\ArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\DataSty}[1]{\textnormal{\textsf{#1}}\unskip}%%\SetDataSty{textsf}
\newcommand{\SetDataSty}[1]{\renewcommand{\DataSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\CommentSty}[1]{\textnormal{\texttt{#1}}\unskip}%%\SetDataSty{texttt}
\newcommand{\SetCommentSty}[1]{\renewcommand{\CommentSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\TitleSty}[1]{#1\unskip}%\SetTitleSty{}{}
\newcommand{\SetTitleSty}[2]{\renewcommand{\TitleSty}[1]{%
\csname#1\endcsname{\csname#2\endcsname##1}}\unskip}%
\newcommand{\BlockMarkersSty}[1]{\KwSty{#1}}%
\newcommand{\SetBlockMarkersSty}[1]{\renewcommand{\BlockMarkersSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Block basic commands
%
\newcommand{\algocf@push}[1]{\advance\skiptotal by #1\moveright #1}%
\newcommand{\algocf@pop}[1]{\advance\skiptotal by -#1}%
\newcommand{\algocf@addskiptotal}{\advance\skiptotal by 0.4pt\advance\hsize by -0.4pt\advance\hsize by -\skiplength}% 0.4 pt=width of \vrule
\newcommand{\algocf@subskiptotal}{\advance\skiptotal by -0.4pt\advance\hsize by 0.4pt\advance\hsize by \skiplength}% 0.4 pt=width of \vrule
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% group of instructions definition
%
\skiphlne=.8ex%
\newcommand{\SetVlineSkip}[1]{\skiphlne=#1}%
\newcommand{\algocf@bblock}{\BlockMarkersSty{begin}}%
\newcommand{\algocf@eblock}{\BlockMarkersSty{end}}%
\newcommand{\AlgoDisplayBlockMarkers}{\setboolean{algocf@displayblockmarkers}{true}}%
\newcommand{\AlgoDontDisplayBlockMarkers}{\setboolean{algocf@displayblockmarkers}{false}}%
\newcommand{\AlgoDisplayGroupMarkers}{\setboolean{algocf@displaygroupmarkers}{true}}%
\newcommand{\AlgoDontDisplayGroupMarkers}{\setboolean{algocf@displaygroupmarkers}{false}}%
\newcommand{\algocf@bblockcode}{%
  \ifthenelse{\boolean{algocf@displayblockmarkers}}{\algocf@bblock\par}{\relax}%
}%
\newcommand{\algocf@eblockcode}{%
  \ifthenelse{\boolean{algocf@displayblockmarkers}}{\algocf@eblock\par}{\relax}%
}%
\newcommand{\algocf@bgroupcode}{%
  \ifthenelse{\boolean{algocf@displaygroupmarkers}}{\algocf@bblock}{\relax}%
}%
\newcommand{\algocf@egroupcode}{%
  \ifthenelse{\boolean{algocf@displaygroupmarkers}}{\algocf@eblock}{\relax}%
}%
\newcommand{\SetAlgoBlockMarkers}[2]{%
  \ifArgumentEmpty{#1}{%
    \renewcommand{\algocf@bblock}{\relax}%
  }{%
    \renewcommand{\algocf@bblock}{\BlockMarkersSty{#1}}%
  }% begin marker set
  \ifArgumentEmpty{#2}{%
    \renewcommand{\algocf@eblock}{\relax}%
  }{%
    \renewcommand{\algocf@eblock}{\BlockMarkersSty{#2}}%
  }% end marker set
}
%
%%%%%%%%% block with a vertical line end by a little horizontal line
\newcommand{\algocf@Vline}[1]{%     no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@push{\skiprule}%        move to the right before the vertical rule
  \hbox{\vrule%
    \vtop{\algocf@push{\skiptext}%move the right after the rule
      \vtop{\algocf@addskiptotal #1}\Hlne}}\vskip\skiphlne% inside the block
  \algocf@pop{\skiprule}%\algocf@subskiptotal% restore indentation
  \nointerlineskip}% no vskip after
%
%%%%%%%%% block with a vertical line
\newcommand{\algocf@Vsline}[1]{%    no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@bblockcode%
  \algocf@push{\skiprule}%        move to the right before the vertical rule
  \hbox{\vrule%               the vertical rule
    \vtop{\algocf@push{\skiptext}%move the right after the rule
      \vtop{\algocf@addskiptotal #1}}}% inside the block
  \algocf@pop{\skiprule}% restore indentation
  \algocf@eblockcode%
}
%
\newcommand{\algocf@Hlne}{\hrule height 0.4pt depth 0pt width .5em}%
%
%%%%%%%%%  block without line
\newcommand{\algocf@Noline}[1]{%    no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@bblockcode%
  \algocf@push{\skiprule}%
  \hbox{%
    \vtop{\algocf@push{\skiptext}%
      \vtop{\algocf@addskiptotal #1}}}% inside the block
  \algocf@pop{\skiprule}%
  \algocf@eblockcode%
  % \nointerlineskip% no vskip after
}%
%%%%%%%%%
%
%% default=NoLine
%
\newcommand{\algocf@group}[1]{\algocf@Noline{#1}}% group: set of instruction depending from another (ex: then part of the If)
\newcommand{\algocf@@@eblock}[2]{#1\ifArgumentEmpty{#2}{\relax}{\KwSty{\@algocf@endoption{#2}}\strut\par}}% block: group with a end keyword.
\newcommand{\algocf@@@block}[3]{#1\ifArgumentEmpty{#2}{\ifArgumentEmpty{#3}{\relax}{ #3\relax}}{\KwSty{\@algocf@endoption{#2}}\ifArgumentEmpty{#3}{\relax}{ #3}\strut\par}}% block: group with a end keyword.
\newcommand{\algocf@@block}[3]{\algocf@@@block{#1}{#2}{#3}}% block: group with a end keyword.
\newcommand{\algocf@block}[3]{\algocf@@block{#1}{#2}{#3}}% command that will be used and redefined accordingly to noend option
%\newcommand{\algocf@nblock}[3]{\algocf@@block{#1}{#2}{#3}}% command that will be used and redefined accordingly to noend option
\newcommand{\algocf@setBlock}{%
  \ifthenelse{\boolean{algocf@optnoend}}{%     if no end option
    \renewcommand{\algocf@block}[3]{\algocf@group{##1}}%     block will be a group
  }{%                                          else
    \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}% block stays a block
  }%
}%
%
\newcommand{\Hlne}{}% little hrizontal line ending a block in vline mode
%
\newcommand{\@algocf@endoption}[1]{#1}%
\newboolean{algocf@optnoend}\setboolean{algocf@optnoend}{false}%
%
\newcommand{\SetAlgoLongEnd}{%%%%%%%%%%%%%%%%%%%%%%%%% Long End
  \setboolean{algocf@optnoend}{false}%
  \renewcommand{\@algocf@endoption}[1]{##1}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoShortEnd}{%%%%%%%%%%%%%%%%%%%%%%%% ShortEnd
  \setboolean{algocf@optnoend}{false}%
  \renewcommand{\@algocf@endoption}[1]{\@firstword##1 \@nil}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoNoEnd}{%%%%%%%%%%%%%%%%%%%%%%%%%%% NoEnd
  \setboolean{algocf@optnoend}{true}%
  \renewcommand{\@algocf@endoption}[1]{}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoNoLine}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Noline
\renewcommand{\algocf@@block}[2]{\algocf@@@block{\algocf@Noline{##1}}{##2}}%
\renewcommand{\algocf@group}[1]{\algocf@Noline{##1}}%
\renewcommand{\Hlne}{}}%
%
\newcommand{\SetAlgoVlined}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Vline
\renewcommand{\algocf@@block}[2]{\algocf@Vline{##1}}%
\renewcommand{\algocf@group}[1]{\algocf@Vsline{##1}}%\ifthenelse{\boolean{algocf@optnoend}}{\relax}{\strut\ignorespaces}}%
\renewcommand{\Hlne}{\algocf@Hlne}}%
%
\newcommand{\SetAlgoLined}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Line
\renewcommand{\algocf@@block}[2]{\algocf@@@block{\strut\algocf@Vsline{##1}}{##2}}% no skip after a block so garantie at least one line
\renewcommand{\algocf@group}[1]{\algocf@Vsline{##1}}%\ifthenelse{\boolean{algocf@optnoend}}{\relax}{\strut\ignorespaces}}%
\renewcommand{\Hlne}{}}%
%
\newcommand{\SetNothing}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Noline
\renewcommand{\algocf@@block}[2]{\algocf@Noline{##1}\par}%
%\long
\renewcommand{\algocf@group}[1]{\algocf@Noline{##1}}%
\renewcommand{\Hlne}{}}%
%
%%
%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ``Input:'''s like command 
%
%%%
% text staying at the right of the longer keyword of KwInOut commands 
% (text of KwInOut commands are all vertically aligned)
%
\newcommand{\algocf@newinout}{\par\parindent=\inoutindent}% to put right indentation after a \\ in the KwInOut
\newcommand{\SetKwInOut}[2]{%
  \sbox\algocf@inoutbox{\KwSty{#2\algocf@typo:}}%
  \expandafter\ifx\csname InOutSizeDefined\endcsname\relax% if first time used
    \newcommand\InOutSizeDefined{}\setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
  \else% else keep the larger dimension
    \ifdim\wd\algocf@inoutbox>\inoutsize%
    \setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
    \fi%
  \fi% the dimension of the box is now defined.
  \algocf@newcommand{#1}[1]{%
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@seteveryparhanging{\relax}}%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
%     {\let\\\algocf@newinout\hangindent=\wd\algocf@inoutbox\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo\hfill:}~##1\par}%
    {\let\\\algocf@newinout\hangindent=\inoutindent\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~##1\par}%
    \algocf@linesnumbered% reset the numbering of the lines
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@reseteveryparhanging}%
  }}%
%
%% allow to ajust the skip size of InOut
%%
\newcommand{\ResetInOut}[1]{%
  \sbox\algocf@inoutbox{\hbox{\KwSty{#1\algocf@typo:}\ }}%
  \setlength{\inoutsize}{\wd\algocf@inoutbox}%
  }%
%
% 
%%%
% text staying at the right of the keyword.
%
\newcommand{\algocf@newinput}{\par\parindent=\wd\algocf@inputbox}% to put right indentation after a \\ in the KwInput
\newcommand{\SetKwInput}[2]{%
  \algocf@newcommand{#1}[1]{%
    \sbox\algocf@inputbox{\hbox{\KwSty{#2\algocf@typo:} }}%
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@seteveryparhanging{\relax}}%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
    {\let\\\algocf@newinput\hangindent=\wd\algocf@inputbox\hangafter=1\unhbox\algocf@inputbox##1\par}%
    \algocf@linesnumbered% reset the numbering of the lines
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@reseteveryparhanging}%
  }}%
\newcommand{\SetKwData}[2]{%
  \algocf@newcommand{@#1}[1]{\DataSty{#2(}\ArgSty{##1}\DataSty{)}}%
  \algocf@newcommand{#1}{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\DataSty{#2}\xspace}}%
  }%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% tallent:
%
% Add following macros:
%   \SetKwHangingKw:  [kw] ------------   <= hanging determined by [kw]
%                          ------------
% Should act like a combination of \SetKwInput and \SetKw.
% Based on \SetKwInput:
%   - remove ':' at end of keyword
%   - do not reset numbering
%   - use separate savebox
\newsavebox{\algocf@hangingbox}
\newcommand{\algocf@newhanging}{\par\parindent=\wd\algocf@hangingbox}% to put right indentation after a \\ in the KwInput
\newcommand{\SetKwHangingKw}[2]{%
  \algocf@newcommand{#1}[1]{%
    \sbox\algocf@hangingbox{\hbox{\KwSty{#2}\algocf@typo\ }}%
    {\let\\\algocf@newhanging\hangindent=\wd\algocf@hangingbox\hangafter=1\unhbox\algocf@hangingbox##1\;}%
  }%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Comments macros
%
%%%%
% comment in the text, first argument is the name of the macro, second is
% the text put before the comment, third is the text put at the end of the
% comment.
%
% first side comment justification
\newcommand{\SetSideCommentLeft}{\setboolean{algocf@scleft}{true}}%
\newcommand{\SetSideCommentRight}{\setboolean{algocf@scleft}{false}}%
\newcommand{\SetNoFillComment}{\setboolean{algocf@optfillcomment}{false}}%
\newcommand{\SetFillComment}{\setboolean{algocf@optfillcomment}{true}}%
%
% next comment and side comment
%
\newcommand{\algocf@endmarkcomment}{\relax}%
\newcommand{\algocf@fillcomment}{%
  \ifthenelse{\boolean{algocf@optfillcomment}}{\hfill}{\relax}}%
%
\newcommand{\algocf@startcomment}{%
  \hangindent=\wd\algocf@inputbox\hangafter=1\usebox\algocf@inputbox}%
\newcommand{\algocf@endcomment}{\algocf@fillcomment\algocf@endmarkcomment\ignorespaces\par}%
\newcommand{\algocf@endstartcomment}{\algocf@endcomment\algocf@startcomment\ignorespaces}%
%
\newboolean{algocf@sidecomment}%
\newboolean{algocf@altsidecomment}\setboolean{algocf@altsidecomment}{false}%
\newcommand{\algocf@scpar}{\ifthenelse{\boolean{algocf@altsidecomment}}{\relax}{\par}}%
\newcommand{\algocf@sclfill}{\ifthenelse{\boolean{algocf@scleft}}{\algocf@fillcomment}{\relax}}%
\newcommand{\algocf@scrfill}{\ifthenelse{\boolean{algocf@scleft}}{\relax}{\hfill}}%
\newcommand{\algocf@startsidecomment}{\usebox\algocf@inputbox}%
\newcommand{\algocf@endsidecomment}{\algocf@endmarkcomment\algocf@scpar}%
\newcommand{\algocf@endstartsidecomment}{%
  \algocf@sclfill\algocf@endsidecomment%
  \algocf@scrfill\algocf@startsidecomment\ignorespaces}%
%
\newcommand{\SetKwComment}[3]{%
  \algocf@newcommand{#1}{\@ifstar{\csname algocf@#1@star\endcsname}{\csname algocf@#1\endcsname}}%
	\algocf@newcommand{algocf@#1}[1]{%
      \ifthenelse{\boolean{algocf@hangingcomment}}{\relax}{\algocf@seteveryparhanging{\relax}}%
      \sbox\algocf@inputbox{\CommentSty{\hbox{#2}}}%
      \ifthenelse{\boolean{algocf@commentsnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
      {\renewcommand{\algocf@endmarkcomment}{#3}%
        \let\\\algocf@endstartcomment%
        \algocf@startcomment\CommentSty{%
          \strut\ignorespaces##1\strut\algocf@fillcomment#3}\par}%
      \algocf@linesnumbered% reset the numbering of the lines
      \ifthenelse{\boolean{algocf@hangingcomment}}{\relax}{\algocf@reseteveryparhanging}%
    }%
  %%% side comment definitions
	\algocf@newcommand{algocf@#1@star}[2][]{%
      \ifArgumentEmpty{##1}\relax{% TODO: Is this even necessary, with all those \ifx's?
        \ifthenelse{\boolean{algocf@scleft}}{\setboolean{algocf@sidecomment}{true}}{\setboolean{algocf@sidecomment}{false}}%
        \ifx##1h\setboolean{algocf@altsidecomment}{true}\SetSideCommentLeft\fi%
        \ifx##1f\setboolean{algocf@altsidecomment}{true}\SetSideCommentRight\fi%
        \ifx##1l\setboolean{algocf@altsidecomment}{false}\SetSideCommentLeft\fi%
        \ifx##1r\setboolean{algocf@altsidecomment}{false}\SetSideCommentRight\fi%
      }%
      \sbox\algocf@inputbox{\CommentSty{\hbox{#2}}}%
      \ifthenelse{\boolean{algocf@commentsnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
      {%
        \renewcommand{\algocf@endmarkcomment}{#3}%
        \let\\\algocf@endstartsidecomment%
        % here is the comment
        \ifthenelse{\boolean{algocf@altsidecomment}}{\relax}{\@endalgocfline\ }%
        \algocf@scrfill\algocf@startsidecomment\CommentSty{%
          \strut\ignorespaces##2\strut\algocf@sclfill#3}\algocf@scpar%
      }%
      \algocf@linesnumbered% reset the numbering of the lines
      \ifArgumentEmpty{##1}\relax{%
        \ifthenelse{\boolean{algocf@sidecomment}}{\setboolean{algocf@scleft}{true}}{\setboolean{algocf@scleft}{false}}%
        \setboolean{algocf@altsidecomment}{false}%
      }%
	}%
  }%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwProg
%
\newcommand{\SetKwProg}[4]{%\SetKwProg{Env}{Title}{is}{end} 
	\algocf@newcmdside@koif{#1}{\KwSty{#2}\ifArgumentEmpty{#2}\relax{\ }\ProgSty{##2}\KwSty{#3}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#4}{##4}}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2} \ProgSty{##2}\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode\@endalgocfline\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2} \ProgSty{##2}\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
}%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Kw
%
\newcommand{\SetKw}[2]{%
	\algocf@newcommand{@#1}[1]{\KwSty{#2} \ArgSty{##1}}
	\algocf@newcommand{#1}{\@ifnextchar\bgroup{\csname @#1\endcsname}{\KwSty{#2}\xspace}}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwFunction
%
\newcommand{\SetKwFunction}[2]{%
%%% use of gdef since newcommand doesn't manage to define the macro when SetKwFunction is used in \algocf@caption@proc
  \expandafter\gdef\csname @#1\endcsname##1{\FuncSty{#2(}\FuncArgSty{##1}\FuncSty{)}}%
  \expandafter\gdef\csname#1\endcsname{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\FuncSty{#2}\xspace}}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwTab
%
\newcommand{\SetKwArray}[2]{%
%%% use of gdef since newcommand doesn't manage to define the macro when SetKwFunction is used in \algocf@caption@proc
  \expandafter\gdef\csname @#1\endcsname##1{\DataSty{#2[}\ArgSty{##1}\DataSty{]}}%
  \expandafter\gdef\csname#1\endcsname{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\DataSty{#2}\xspace}}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwBlock
%
\newcommand{\SetKwBlock}[3]{%
	\algocf@newcmdside@kobe{#1}%
    {\KwSty{#2}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##2}{#3}{##3}\par}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% condition typo
%
\newcommand{\algocf@scond}{\ }
\newcommand{\algocf@econd}{\ }
\newcommand{\algocf@ucond}{}
\newcommand{\SetStartEndCondition}[3]{%
  \renewcommand{\algocf@scond}{#1}\renewcommand{\algocf@econd}{#2}\renewcommand{\algocf@ucond}{#3}}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For Switch
%
\newcommand{\SetKwSwitch}[9]{% #1=\Switch #2=\Case #3=\Other #4=switch #5=do #6=case #7=otherwise #8=endcase #9=endsw
%	\algocf@newcmdside{#1}{3}%
	\algocf@newcmdside@koif{#1}%
		{\KwSty{#4}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#9} {##4\relax}}%
%%%% Case
	\algocf@newcmdside@koif{#2}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#8}{##4\relax}}%
    %uCase
	\algocf@newcmdside{u#2}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@group{##3}}%
    %lcase
    \algocf@newcommand{l#2}{\@ifstar{\csname algocf@l#2star\endcsname}{\csname algocf@l#2\endcsname}}%
	\algocf@newcmdside{algocf@l#2}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\ \relax{ ##1}\strut\par}%
	\algocf@newcmdside{algocf@l#2star}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
%%%% Other 
	\algocf@newcmdside@kobe{#3}{\KwSty{#7} \KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##2}{#8}{##3\relax}}%
    %lOther
    \algocf@newcommand{l#3}{\@ifstar{\csname algocf@l#3star\endcsname}{\csname algocf@l#3\endcsname}}%
	\algocf@newcmdside{algocf@l#3}{2}{\KwSty{#7} \KwSty{#5}\algocf@bgroupcode\ ##2\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#3star}{2}{\KwSty{#7} \KwSty{#5}\algocf@bgroupcode\ ##2\algocf@egroupcode}%
    %uOther
	\algocf@newcmdside{u#3}{3}{\KwSty{#7} \KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@group{##2}}%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% If macros
%
\newcommand{\SetKwIF}[8]{% #1=\If #2=\ElseIf #3=\Else #4=if #5=then #6=elseif #7=else #8=endif
% 
% common text
	\algocf@newcommand{#1@ifthen}[1]{\KwSty{#4}\algocf@scond\ArgSty{##1}\algocf@econd\KwSty{#5}}%
	\algocf@newcommand{#1@endif} [2]{\algocf@block{##1}{#8}{##2}}%
	\algocf@newcommand{#1@noend} [1]{\algocf@group{##1}}%
	\algocf@newcommand{#1@else}  [1]{\algocf@group{##1}\KwSty{#7}}%
	\algocf@newcommand{#2@elseif}[1]{\KwSty{#6}\algocf@scond\ArgSty{##1}\algocf@econd\KwSty{#5}}%
	\algocf@newcommand{#3@else}     {\KwSty{#7}}%
%%%% If then { } endif
	\algocf@newcmdside@koif{#1}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##3}{##4\relax}}%
%%%% If then {} else {} endif
    % first command to handle optional side comment of else (so just after first braces)
 	\algocf@newcmdside@kobe{algocf@e#1thenelse}{\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##2}{##3}}%
    % the definition of if-then-else command using command above 
	\algocf@newcmdside{e#1}{3}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@else\endcsname{##3}\csname algocf@e#1thenelse\endcsname}%
    %%% leif
    \algocf@newcommand{le#1}{\@ifstar{\csname algocf@le#1star\endcsname}{\csname algocf@le#1\endcsname}}%
    \algocf@newcmdside{algocf@le#1}{4}{\csname #1@ifthen\endcsname{##2} \algocf@bgroupcode##3 \csname #3@else\endcsname\ ##4\@endalgocfline\ \algocf@egroupcode\ifArgumentEmpty{##1}\relax{##1}\strut\par}%
    \algocf@newcmdside{algocf@le#1star}{4}{\csname #1@ifthen\endcsname{##2} \algocf@bgroupcode##3 \csname #3@else\endcsname\ ##4\algocf@egroupcode}%
%%%% If then 
	% \algocf@newcmdside{l#1}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\
    % ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
	\algocf@newcmdside{u#1}{3}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@noend\endcsname{##3}}%
%%%% ElseIf {} endif
	\algocf@newcmdside@koif{#2}{\csname #2@elseif\endcsname{##2}\relax\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##3}{##4\relax}}%
%%%% ElseIf
    \algocf@newcommand{l#2}{\@ifstar{\csname algocf@l#2star\endcsname}{\csname algocf@l#2\endcsname}}%
	\algocf@newcmdside{algocf@l#2}{3}{\csname #2@elseif\endcsname{##2}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#2star}{3}{\csname #2@elseif\endcsname{##2}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
	\algocf@newcmdside{u#2}{3}{\csname #2@elseif\endcsname{##2}\relax\ifArgumentEmpty{##1}\relax{##1}\csname #1@noend\endcsname{##3}}%
%%%% Else {} endif
	\algocf@newcmdside@kobe{#3}{\csname #3@else\endcsname\ifArgumentEmpty{##1}\relax\ ##1\csname #1@endif\endcsname{##2}{##3\relax}}%
%%%% Else 
    \algocf@newcommand{l#3}{\@ifstar{\csname algocf@l#3star\endcsname}{\csname algocf@l#3\endcsname}}%
	\algocf@newcmdside{algocf@l#3}{2}{\csname #3@else\endcsname\algocf@bgroupcode\ ##2\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#3star}{2}{\csname #3@else\endcsname\algocf@bgroupcode\ ##2\algocf@egroupcode}%
	\algocf@newcmdside{u#3}{2}{\csname #3@else\endcsname\ifArgumentEmpty{##1}\relax\ {##1\relax}\csname #1@noend\endcsname{##2}}%
}% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For macros
%
\newcommand{\SetKwFor}[4]{%
	\algocf@newcmdside@koif{#1}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#4}{##4\relax}}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Repeat macros
%
\newsavebox{\algocf@untilbox}% to handle width of until keyword needed to have good skip
  % for line numbers
\newskip\algocf@skipuntil
\newcommand{\SetKwRepeat}[3]{%
	\algocf@newcmdsides{#1}{3}{%
      \sbox\algocf@untilbox{\KwSty{#3}\algocf@scond}\algocf@skipuntil=\wd\algocf@untilbox%
      \KwSty{#2}\ifArgumentEmpty{##1}\relax{##1}\algocf@group{##3}%
      \KwSty{#3}\algocf@scond% until keyword and start condition typo
      %\advance\skiptotal by\algocf@skipuntil%
      \ArgSty{##2}%
      %\advance\skiptotal by-\algocf@skipuntil%
      \algocf@ucond%
      \algocf@skipuntil=0pt% reset counter
    }{\@endalgocfline}{\strut\par}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2}\algocf@bgroupcode\ ##3\algocf@egroupcode\ \KwSty{#3}\algocf@scond\ArgSty{##2}\algocf@ucond\@endalgocfline\ifArgumentEmpty{##1}\relax{ ##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2}\algocf@bgroupcode\ ##3\algocf@egroupcode\ \KwSty{#3}\algocf@scond\ArgSty{##2}\algocf@ucond}%
}%
%
% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%        Environments definitions     %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%
%% Caption management
%%
% for the following macros:
% #1 is given by caption and is equal to fnum@algocf
% #2 is the text given in argument by the user in the \caption macro
%
%%%%% text of caption
\newcommand{\algocf@captionlayout}[1]{#1}%
\newcommand{\SetAlgoCaptionLayout}[1]{%
  \renewcommand{\algocf@captionlayout}[1]{\csname #1\endcsname{##1}}}%
\newcommand{\algocf@capseparator}{:}%
\newcommand{\SetAlgoCaptionSeparator}[1]{\renewcommand{\algocf@capseparator}{#1}}%
\newcommand{\algocf@captiontext}[2]{%
  \algocf@captionlayout{\AlCapSty{\AlCapFnt #1\algocf@typo\algocf@capseparator}\nobreakspace%
    \AlCapNameSty{\AlCapNameFnt{}#2\endgraf}}}% text of caption
%
%%%%% default caption of algorithm: used if no specific style caption is defined
\newcommand{\algocf@makecaption}[2]{%
  \addtolength{\hsize}{\algomargin}%
  \sbox\@tempboxa{\algocf@captiontext{#1}{#2}}%
  \ifdim\wd\@tempboxa >\hsize%     % if caption is longer than a line
    \hskip .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}% then caption is not centered
  \else%
    \global\@minipagefalse%
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}% else caption is centered
  \fi%
  \addtolength{\hsize}{-\algomargin}%
}%
%
\newsavebox\algocf@capbox%
\newcommand{\algocf@makecaption@plain}[2]{%
  \global\sbox\algocf@capbox{\algocf@makecaption{#1}{#2}}}%
\newcommand{\algocf@makecaption@boxed}[2]{%
  \addtolength{\hsize}{-\algomargin}%
  \global\sbox\algocf@capbox{\algocf@makecaption{#1}{#2}}%
  \addtolength{\hsize}{\algomargin}%
 }%
%
\newcommand{\algocf@makecaption@plainruled}[2]{\algocf@makecaption@plain{#1}{#2}}%
\newcommand{\algocf@makecaption@tworuled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@algoruled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@boxruled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@ruled}[2]{%
  \global\sbox\algocf@capbox{\hskip\AlCapHSkip% .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}}% then caption is not centered
}%
%
\newlength{\algoheightruledefault}\setlength{\algoheightruledefault}{0.8pt}%
\newlength{\algoheightrule}\setlength{\algoheightrule}{\algoheightruledefault}%
\newlength{\algotitleheightruledefault}\setlength{\algotitleheightruledefault}{0.8pt}%
\newlength{\algotitleheightrule}\setlength{\algotitleheightrule}{\algotitleheightruledefault}%
\newcommand{\algocf@caption@plain}{\vskip\AlCapSkip\box\algocf@capbox}%
\newcommand{\algocf@caption@plainruled}{\algocf@caption@plain}%
\newcommand{\algocf@caption@boxed}{\vskip\AlCapSkip\box\algocf@capbox}%
\newcommand{\algocf@caption@ruled}{\box\algocf@capbox\kern\interspacetitleruled\hrule
  width\algocf@ruledwidth height\algotitleheightrule depth0pt\kern\interspacealgoruled}%
\newcommand{\algocf@caption@tworuled}{\box\algocf@capbox\hrule  height0pt depth0pt\kern\interspacealgoruled}%
\newcommand{\algocf@caption@algoruled}{\algocf@caption@ruled}%
\newcommand{\algocf@caption@boxruled}{%
  \addtolength{\hsize}{-0.8pt}%
  \hbox to\hsize{%
    \vrule%\hskip-0.35pt%
    \vbox{%
      \hrule\vskip\interspacetitleboxruled%
      \hbox to\hsize{\unhbox\algocf@capbox\hfill}\vskip\interspacetitleboxruled%
    }% 
    %\hskip-0.35pt%
    \vrule%
  }\nointerlineskip%
  \addtolength{\hsize}{0.8pt}%
}%
%
%
%%%% set caption for the environment
\newcommand{\algocf@captionref}{%
  \renewcommand{\fnum@algocf}[1]{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\algocf@algocfref}}%
  \addtocounter{algocf}{-1}% \caption do a refstepcounter, so we restore the precedent value
  \let\old@thealgocf=\thealgocf\renewcommand{\thealgocf}{{\relsize{\algocf@refrelsize}\algocf@algocfref}}%
  \gdef\@currentlabel{\algocf@algocfref}% let the label use the new ref
}%
%
% Unfortunatly, we also need our own caption to set some specific stuff for special references. But after these
% settings, we call the original caption.
%
\long\def\algocf@caption@algo#1[#2]#3{%
  \ifthenelse{\equal{\algocf@algocfref}{\relax}}{}{\algocf@captionref}%
  \@ifundefined{hyper@refstepcounter}{\relax}{% if hyper@refstepcounter undefind, no hyperref, else...
    \ifthenelse{\equal{\algocf@algocfref}{\relax}}{\renewcommand{\theHalgocf}{\thealgocf}}{% take algocf as Href
      \renewcommand{\theHalgocf}{\algocf@algocfref}}%else if SetAlgoRefName done, take this name as ref.
    \hyper@refstepcounter{algocf}%set algocf as category of ref
  }%
   \algocf@latexcaption{#1}[{#2}]{{#3}}% call original caption
}%
%
% beamer define is own caption overrinding latex caption!
% as we need it, we have put here the original definition
% to handle manual ref, unfortunately we have to add one line to handle algocf@algocfref
\long\def\algocf@latexcaption#1[#2]#3{% original definition of caption
  \par%
  \addcontentsline{\csname ext@#1\endcsname}{#1}%
  {\protect\numberline{\csname the#1\endcsname}{\ignorespaces #2}}%
  \begingroup%
  \@parboxrestore%
  \if@minipage%
    \@setminipage%
  \fi%
  \normalsize%
  \@makecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par%
  \endgroup%
}%
%
% \ifx\beamer@makecaption\undefined%
% \else% beamer detected
\ifx\@makecaption\undefined%
\newcommand{\@makecaption}[2]{\relax}%
\fi%
%%

%
% more and more packages redefine \@caption instead of just \@makecaption which makes algorithm2e
% caption not works since based on standard \@caption. So we force the definition of \@caption to be
% the standard one (the one from LaTeX) inside algorithm environment.
%
% unfortunately, makecaption is called with \ignorespace #3 so 
% we can't do the @currentlabel definition inside \algocf@captionproctext
\long\def\algocf@caption@proc#1[#2]#3{%
  \ifthenelse{\boolean{algocf@nokwfunc}}{\relax}{%
    \SetKwFunction{\algocf@captname#3@}{\algocf@captname#3@}%
  }%
  % we tell hyperref to use algocfproc as category and to take the appropriate ref.
  \ifthenelse{\boolean{algocf@func}}{\def\@proc@func{algocffunc}}{\def\@proc@func{algocfproc}}%
  \@ifundefined{hyper@refstepcounter}{\relax}{% if hyper@refstepcounter undefind, no hyperref, else...
    \ifthenelse{\boolean{algocf@procnumbered}}{% 
      \expandafter\def\csname theH\@proc@func\endcsname{\thealgocf}%if procnumbered, take \thealgocf as ref
    }{%
      \expandafter\def\csname theH\@proc@func\endcsname{\algocf@captname#3@}%else take procedure or function name
    }%
    \hyper@refstepcounter{\@proc@func}%
  }%
  \ifthenelse{\boolean{algocf@procnumbered}}{\relax}{%
    \addtocounter{algocf}{-1}% \caption do a refstepcounter, so we restore the precedent value
    \gdef\@currentlabel{\algocf@captname#3@}% let the label be the name of the function, not the counter
  }%
  \ifthenelse{\equal{\algocf@captparam#2@}{\arg@e}}{% if no paramater, we remove the ()
    \algocf@latexcaption{#1}[\algocf@procname\nobreakspace\algocf@captname#2@]{#3}%
  }{%                                                 else we give the complete name
    \algocf@latexcaption{#1}[\algocf@procname\nobreakspace#2]{#3}%
  }%
}%
%%
%%% setcaption
\newcommand{\algocf@setcaption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if proc environment, caption text must be changed
    \let\algocf@oldcaptiontext=\algocf@captiontext%
    \renewcommand{\algocf@captiontext}[2]{%
      \algocf@captionproctext{##1}{##2}%
    }%
  }{}%
  \let\algocf@savecaption=\@caption%
  \ifthenelse{\boolean{algocf@procenvironment}}{\let\@caption=\algocf@caption@proc}{\let\@caption=\algocf@caption@algo}%
  \let\algocf@oldmakecaption=\@makecaption%
  \renewcommand{\@makecaption}[2]{%
    \expandafter\csname algocf@makecaption@\algocf@style\endcsname{##1}{##2}%
  }%
}%
%
%%%%% reset caption
%
% since we have force the LaTeX caption for algorithm environment, we must go back to the caption
% used in the text.
\newcommand{\algocf@resetcaption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if proc environment
    \let\thealgocf=\old@thealgocf% restore normal counter printing
    \let\algocf@captiontext=\algocf@oldcaptiontext% restore normal caption text
  }{}%
  \let\@caption=\algocf@savecaption% now restore caption outside algo/proc/func environment
  \let\@makecaption=\algocf@oldmakecaption% and restore makecaption outside outside algo/proc/func environment
  \algocf@resetfnum%
}%
%
%%%%% nocaptionofalgo and restorecaptionofalgo --
\newcommand{\NoCaptionOfAlgo}{%
  \let\@old@algocf@captiontext=\algocf@captiontext%
  \renewcommand{\algocf@captiontext}[2]{\AlCapNameSty{\AlCapNameFnt{}##2}}%
}%
\newcommand{\RestoreCaptionOfAlgo}{%
  \let\algocf@captiontext=\@old@algocf@captiontext%
}%
%
% ----------------------  algocf environment
%
\newcounter{algocfline}%                    % new counter to make lines numbers be internally 
\setcounter{algocfline}{0}%                 % different in different algorithms
\newcounter{algocfproc}% counter to count all algo environment (proc, func), just used by hyperref to avoir "same
\setcounter{algocfproc}{0}% identifier" error caused by algocf being set to '-' for procedure or function or not
  % changed if no caption is given.
%
\expandafter\ifx\csname algocf@within\endcsname\relax% if \algocf@within doesn't exist
\newcounter{algocf}%                        % just define a new counter
\renewcommand{\thealgocf}{\@arabic\c@algocf}% and the way it is printed
\else%                                     else
\newcounter{algocf}[\algocf@within]%        % counter is numbered within \algocf@within
\renewcommand\thealgocf{\csname the\algocf@within\endcsname.\@arabic\c@algocf}%
\fi%
%
\def\fps@algocf{htbp}%        % default
\def\ftype@algocf{10}%        % float type
\def\ext@algocf{\algocf@list} % loa by default, lof if figure option used
\newcommand{\fnum@algocf}{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\thealgocf}}%
\newcommand{\algocf@resetfnum}{\renewcommand{\fnum@algocf}{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\thealgocf}}}%
\newenvironment{algocf}%      % float environment for algorithms
               {\@float{algocf}}%
               {\end@float}%
\newenvironment{algocf*}%     % float* environment for algorithms
               {\@dblfloat{algocf}}%
               {\end@dblfloat}%
%
\def\algocf@seclistalgo{}%
\ifx\l@chapter\undefined\let\algocf@seclistalgo=\section\else\let\algocf@seclistalgo=\chapter\fi%
\@ifundefined{if@restonecol}{\newif\if@restonecol}\relax%
\newcommand\listofalgocfs{%
     \ifx\algocf@seclistalgo\chapter%
      \if@twocolumn\@restonecoltrue\onecolumn\else\@restonecolfalse\fi%
    \fi%
     \algocf@seclistalgo*{\listalgorithmcfname}%
       \@mkboth{\MakeUppercase\listalgorithmcfname}%
               {\MakeUppercase\listalgorithmcfname}%
     \@starttoc{loa}%
    \ifx\algocf@seclistalgo\chapter%
      \if@restonecol\twocolumn\fi%
    \fi%
}
%
\newcommand*\l@algocf{\@dottedtocline{1}{1em}{2.3em}}% line of the list
%
% ----------------------  algorithm environment
%
%%%%%%%
%%
%% Algorithm environment definition
%%
%%%%%%%
%%
%
\newsavebox\algocf@algoframe%
\def\@algocf@pre@plain{\relax}%  action to be done before printing the algo.
\def\@algocf@post@plain{\relax}% action to be done after printing the algo.
\def\@algocf@capt@plain{bottom}% where the caption should be localized.
\def\@algocf@pre@boxed{\noindent\begin{lrbox}{\algocf@algoframe}}
\def\@algocf@post@boxed{\end{lrbox}\framebox[\hsize]{\box\algocf@algoframe}\par}%
\def\@algocf@capt@boxed{under}%
\def\@algocf@pre@ruled{\hrule height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@ruled{\kern\interspacealgoruled\hrule height\algoheightrule\relax}%
\def\@algocf@capt@ruled{top}%
\def\@algocf@pre@algoruled{\hrule width\algocf@ruledwidth height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@algoruled{\kern\interspacealgoruled\hrule width\algocf@ruledwidth height\algoheightrule \relax}%
\def\@algocf@capt@algoruled{top}%
\def\@algocf@pre@tworuled{\hrule height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@tworuled{\kern\interspacealgoruled\hrule height\algoheightrule\relax}%
\def\@algocf@capt@tworuled{top}%
\def\@algocf@pre@boxruled{\noindent\begin{lrbox}{\algocf@algoframe}}%
\def\@algocf@post@boxruled{\end{lrbox}\framebox[\hsize]{\box\algocf@algoframe}\par}%
\def\@algocf@capt@boxruled{above}%
\def\@algocf@pre@plainruled{\@algocf@pre@ruled}%  action to be done before printing the algo.
\def\@algocf@post@plainruled{\@algocf@post@ruled\kern\interspacealgoruled}%  action to be done before printing the algo.
\def\@algocf@capt@plainruled{under}%
%
\newcommand{\noalgocaption}{\def\@algocf@capt@ruled{none}}
%
%% before algocf environment (not figure environment)
\newcommand{\@algocf@init@caption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if we are inside a procedure/function environment
    \@algocf@proctitleofalgo% set Titleofalgo to Procedure: or Function:
                            % accordingly to the environment
    \let\old@thealgocf=\thealgocf\ifthenelse{\boolean{algocf@procnumbered}}{\relax}{%
      \renewcommand{\thealgocf}{-}}%
  }{% else inside environment algorithm
    \@algocf@algotitleofalgo% fix name for \Titleofalgo to \algorithmcfname
  }%
  \algocf@setcaption%       set caption to our caption style
}%
%
\newcommand{\@algofloatboxreset}{\@setminipage}
\newcommand{\@algocf@init}{%
  \refstepcounter{algocfline}%
  \stepcounter{algocfproc}%to have a different counter for each environment and being abble to make the difference
    %between href of algoline in different algorithms.
  \ifthenelse{\boolean{algocf@optnoend}}{%
      \renewcommand{\algocf@block}[3]{\algocf@group{##1}}%
    }{%
      \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}%
    }%
}%
%% after the end of algocf or figure environment
\newcommand{\@algocf@term@caption}{%
  \algocf@resetcaption% restore original caption
}%
%
\newcommand{\@algocf@term}{%
  \setboolean{algocf@algoH}{false}% no H by default
  \ifthenelse{\boolean{algocf@optnoend}}{%
    \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}%
  }{%
    \renewcommand{\algocf@block}[2]{\algocf@group{##1}}%
  }%
  \SetAlgoRefName{\relax}%
}%
%
%%%%%%%%%%%%%%%%%
%% makethealgo: macro which print effectively the algo in its box
%% 
\newsavebox\algocf@algobox%
\newcommand{\algocf@makethealgo}{%
  \vtop{%
    % place caption above if needed  bye the style
    \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{above}}%
    {\csname algocf@caption@\algocf@style\endcsname}{}%
    %
    % precommand according to the style
    \csname @algocf@pre@\algocf@style\endcsname%
    % place caption at top if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{top}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
    %
    \box\algocf@algobox% the algo
    % place caption at bottom if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{bottom}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
    % postcommand according to the style
    \csname @algocf@post@\algocf@style\endcsname%
    % place caption under if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{under}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
  }%
}%
%%%%%%%%%%%%%%%%%%%
%
%% at the beginning of algocf or figure environment
\newenvironment{algomathdisplay}{\[}{\@endalgocfline\]\ifthenelse{\boolean{algocf@linesnumbered}}{\nl}{\relax}}%
\newcommand{\@algocf@start}{%
  \@algoskip%
  \begin{lrbox}{\algocf@algobox}%
  \setlength{\algowidth}{\hsize}%
  \vbox\bgroup% save all the algo in a box
  \hbox to\algowidth\bgroup\hbox to \algomargin{\hfill}\vtop\bgroup%
  \ifthenelse{\boolean{algocf@slide}}{\parskip 0.5ex\color{black}}{}%
  % initialization
  \addtolength{\hsize}{-1.5\algomargin}%
  \let\@mathsemicolon=\;\def\;{\ifmmode\@mathsemicolon\else\@endalgoln\fi}%
  \raggedright\AlFnt{}%
  \ifthenelse{\boolean{algocf@slide}}{\IncMargin{\skipalgocfslide}}{}%
  \@algoinsideskip%
%   \let\@emathdisplay=\]\def\]{\algocf@endline\@emathdisplay\nl}%
}%
%
%% at the end of algocf or figure environment
\newcommand{\@algocf@finish}{%
  \@algoinsideskip%
  \egroup%end of vtop which contain all the text
  \hfill\egroup%end of hbox wich contains [margin][vtop]
  \ifthenelse{\boolean{algocf@slide}}{\DecMargin{\skipalgocfslide}}{}%
  %
  \egroup%end of main vbox
  \end{lrbox}%
  \algocf@makethealgo% print the algo
  \@algoskip%
  % restore dimension and macros
  \setlength{\hsize}{\algowidth}%
  \lineskip\normallineskip\setlength{\skiptotal}{\@defaultskiptotal}%
  \let\;=\@mathsemicolon%  
  \let\]=\@emathdisplay%
}%
%
%%%%%%%%%%%%%%%%%%%%
%% basic definition of the environment algorithm
%%
%
\newboolean{algocf@procenvironment}\setboolean{algocf@procenvironment}{false}%
\newboolean{algocf@func}\setboolean{algocf@func}{false}%
\newboolean{algocf@algoH}\setboolean{algocf@algoH}{false}%
\newboolean{algocf@algostar}\setboolean{algocf@algostar}{false}%
%
%%% environment for {algorithm}[H]
\newenvironment{algocf@Here}{\noindent%
  \def\@captype{algocf}% if not defined, caption exit with an error
  \begin{minipage}{\hsize}%
}{%
  \end{minipage}%\par%
}%
%%% real algorithm environment which manages H and * option
%    \let\algocf@originalfloatboxreset=\@floatboxreset%
%    \let\@floatboxreset=\@algofloatboxreset%
\newenvironment{algocf@algorithm}[1][htbp]{%
   \ifthenelse{\equal{\algocf@float}{figure}}{%
     \ifthenelse{\boolean{algocf@figurecaption}}{\captionsetup{margin={-\algomargin,\algomargin}}}{}%
   }{}%
   \@algocf@init%
   \ifthenelse{\equal{\algocf@float}{figure}}{% if option figure set
     \ifthenelse{\boolean{algocf@algostar}}{% if algorithm* with figure option
       \begin{figure*}[#1]% call figure*
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
         \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }{% else algorithm environment with figure option
       \begin{figure}[#1]%  call figure
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
          \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }%
   }{% else normal algorithm environment
     \@algocf@init@caption%
     \ifthenelse{\equal{#1}{H}}{% if [H] algorithm
       \if@twocolumn\@latex@error{[H] in two columns mode is not allowed for algorithms}\fi% TODO: SCREAM if H in two colums!
       \setboolean{algocf@algoH}{true}\begin{algocf@Here}% call corresponding environment
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
         \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }{% else floating algorithm environment
       \ifthenelse{\boolean{algocf@algostar}}{% if algorithm*
         \begin{algocf*}[#1]% call algocf*
           \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
           \let\algocf@oldeverypar=\everypar%
           \algocf@seteverypar%
       }{% else algorithm environment
         \begin{algocf}[#1]%  call algcf
           \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
           \let\algocf@oldeverypar=\everypar%
           \algocf@seteverypar%
       }%
     }%
   }% fin test option figure ou pas
   \@algocf@start% 
   \@ResetCounterIfNeeded%
   \algocf@linesnumbered\ignorespaces%
}{%
  \@algocf@finish%
  \ifthenelse{\equal{\algocf@float}{figure}}{%
     \ifthenelse{\boolean{algocf@algostar}}{% if algorithm* with figure option
       \let\everypar=\algocf@oldeverypar%
       \end{figure*}% call figure*
     }{% else algorithm environment with figure option
       \let\everypar=\algocf@oldeverypar%
       \end{figure}%  call figure
     }%
  }{%
    \@algocf@term@caption%
    \ifthenelse{\boolean{algocf@algoH}}{% if [H] algorithm
      \let\everypar=\algocf@oldeverypar%
      \end{algocf@Here}\par% call corresponding environment
     }{% else floating algorithm environment
       \ifthenelse{\boolean{algocf@algostar}}{% if algorithm*
         \let\everypar=\algocf@oldeverypar%
         \end{algocf*}% call algocf*
       }{% else algorithm environment
         \let\everypar=\algocf@oldeverypar%
         \end{algocf}%  call algocf
       }%
     }%
  }%
  \@algocf@term\ignorespacesafterend%
}%
%
%%% user algorithm environment
\newenvironment{\algocf@envname}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{false}\gdef\algocfautorefname{\algorithmautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%%% user algorithm* environment
\newenvironment{\algocf@envname*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{false}\gdef\algocfautorefname{\algorithmautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%
%%%
%
\expandafter\newcommand\csname\algocf@listofalgorithms\endcsname{%
  \ifthenelse{\equal{\algocf@float}{figure}}{\listoffigures}{\listofalgocfs}%
}%
%%%
%%%
%
% ----------------------  procedure and function environments
%
%
% -- new style (used in particular in the caption of function and procedure environments)
%
% three macros to extract parts of the caption
\gdef\algocf@captname#1(#2)#3@{#1}  % keep characters before the first brace
\gdef\algocf@captparam#1(#2)#3@{#2} % keep character in between the braces
\gdef\algocf@captother#1(#2)#3@{#3} % keep character after the braces
%
%%% Text of caption for Procedure or Function
\newcommand{\algocf@captionproctext}[2]{%
  {%
    \ProcSty{\ProcFnt\algocf@procname\ifthenelse{\boolean{algocf@procnumbered}}{\nobreakspace\thealgocf\algocf@typo\algocf@capseparator}{\relax}}%
    \nobreakspace\ProcNameSty{\ProcNameFnt\algocf@captname #2@}% Name of the procedure in ProcName Style. 
    \ifthenelse{\equal{\algocf@captparam #2@}{\arg@e}}{}{% if no argument, write nothing
      \ProcNameSty{\ProcNameFnt(}\ProcArgSty{\ProcArgFnt\algocf@captparam #2@}\ProcNameSty{\ProcNameFnt)}%else put arguments in ProcArgSty:
    }% endif
    \algocf@captother #2@%
  }%
}%
%
%
% -- procedure and function environments are defined from algocf@algorithm environment
%
\newenvironment{procedure}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{false}%
  \newcommand{\algocf@procname}{\@algocf@procname}\gdef\algocfprocautorefname{\procedureautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
\newenvironment{function}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{true}%
  \newcommand{\algocf@procname}{\@algocf@funcname}\gdef\algocffuncautorefname{\functionautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
\newenvironment{procedure*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{false}%
  \newcommand{\algocf@procname}{\@algocf@procname}\gdef\algocfprocautorefname{\procedureautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
\newenvironment{function*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{true}%
  \newcommand{\algocf@procname}{\@algocf@funcname}\gdef\algocffuncautorefname{\functionautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
%
%%%%%%%%%%%%%%%%%%%%
%% definition of algondfloat environment
%%
\ifthenelse{\boolean{algocf@endfloat}}{% if endfloat option then
\newcommand{\algoplace}{% macro which is used to writhe algorithm about there
   \begin{center}%
     [\algorithmcfname~\thepostfig\ about here.]%
   \end{center}%
}%
\newcommand{\algoendfloat}{% use as a \begin{algoendfloat} environment to start scanning of line
%  \immediate\openout\@mainfff\jobname.fff%
  \efloat@condopen{fff}
  \efloat@iwrite{fff}{\string\begin{\algocf@envname}}%
    \if@domarkers%
       \ifthenelse{\equal{\algocf@list}{lof}}{%
         \addtocounter{postfig}{1}%
       }{%
         \addtocounter{postalgo}{1}%
       }%
       \algoplace%
    \fi%
    \bgroup%
    \let\do\ef@makeinnocent\dospecials%
    \ef@makeinnocent\^^L% and whatever other special cases
    \endlinechar`\^^M \catcode`\^^M=12 \ef@xalgocfendfloat}%
}{\relax}%%%% end of endfloat option ifthenelse
%% some macros useful for endfloat option that cannot be defined inside the ifthenelse
%scan algoendfloat algorithm and write the text into .fff file
{\catcode`\^^M=12 \endlinechar=-1 %
 \gdef\ef@xalgocfendfloat#1^^M{% scan the lines inside algoendfloat environment being read by latex
   \def\test{#1}% test is the line being currently scan by latex
   \ifx\test\ef@endalgocftest% if it is \end{algoendfloat}
     \def\next{% define next as to not continue the scan and write \end{algorithm} into .fff file
       \egroup\end{algoendfloat}%
       \efloat@iwrite{fff}{\string\end{\algocf@envname}}%
       \efloat@iwrite{fff}{\string\efloatseparator}%
       \efloat@iwrite{fff}{ }%
     }%
     \else% else write the current line being scanned by latex and set next to continue the scan
       \efloat@iwrite{fff}{#1}%
       \let\next\ef@xalgocfendfloat%
     \fi% endif
     \next}% next is continue if it was else condition, else it does not continue the scan and write end to file
}%
% test if the scan is finish by looking at the string \end{algoendfloat}
{\escapechar=-1%
 \xdef\ef@endalgocftest{\string\\end\string\{algoendfloat\string\}}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
\newcommand{\TitleOfAlgo}[1]{\@titleprefix\ 
  \TitleSty{#1}\par\smallskip}%
%
\newcommand{\SetAlgorithmName}[3]{%
  \renewcommand{\listalgorithmcfname}{#3}%
  \renewcommand{\algorithmcfname}{#1}%
  \renewcommand{\algorithmautorefname}{#2}%
}%
%
\newcommand{\algocf@refrelsize}{-2}\newcommand{\SetAlgoRefRelativeSize}[1]{\renewcommand{\algocf@refrelsize}{#1}}%
\newcommand{\SetAlgoRefName}[1]{%
  \renewcommand{\algocf@algocfref}{#1}%
}%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
% -------------------------   Default Definitions
%
%%
%%
%
\SetKwComment{tcc}{/* }{ */}%
\SetKwComment{tcp}{// }{}%
%
%\newcommand{\algocf@defaults@common}{
%
%
% english keywords (default)
%
\SetKwHangingKw{KwHData}{Data$\rightarrow$}
\SetKwInput{KwIn}{Input}%
\SetKwInput{KwOut}{Output}%
\SetKwInput{KwData}{Data}%
\SetKwInput{KwResult}{Result}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
%
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
%
% French keywords
%
\ifthenelse{\boolean{algocf@localkw@french}\OR\equal{\algocf@languagechoosen}{french}}{%
%\SetKwInOut{AlgDonnees}{Donn\'ees}\SetKwInOut{AlgRes}{R\'esultat}
\SetKwHangingKw{HDonnees}{Donnees$\rightarrow$}
\SetKwInput{Donnees}{Donn\'ees}%
\SetKwInput{Res}{R\'esultat}%
\SetKwInput{Entree}{Entr\'ees}%
\SetKwInput{Sortie}{Sorties}%
\SetKw{KwA}{\`a}%
\SetKw{Retour}{retourner}%
\SetKwBlock{Deb}{d\'ebut}{fin}%
\SetKwRepeat{Repeter}{r\'ep\'eter}{jusqu'\`a}%
%
\SetKwIF{Si}{SinonSi}{Sinon}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwSwitch{Suivant}{Cas}{Autre}{suivant}{faire}{cas o\`u}{autres cas}{fin cas}{fin d'alternative}%
\SetKwFor{Pour}{pour}{faire}{fin pour}%
\SetKwFor{PourPar}{pour}{faire en parall\`ele}{fin pour}%
\SetKwFor{PourCh}{pour chaque}{faire}{fin pour chaque}%
\SetKwFor{PourTous}{pour tous les}{faire}{fin pour tous}%
\SetKwFor{Tq}{tant que}{faire}{fin tq}%
}{}%
%
% --- German keywords
%
\ifthenelse{\boolean{algocf@localkw@german}\OR\equal{\algocf@languagechoosen}{german}}{%
\SetKwInput{Ein}{Eingabe}%KwIn
\SetKwInput{Aus}{Ausgabe}%KwOut
\SetKwInput{Daten}{Daten}%KwData
\SetKwInput{Ergebnis}{Ergebnis}%KwResult
\SetKw{Bis}{bis}%KwTo
\SetKw{KwZurueck}{zur\"uck}%KwRet
\SetKw{Zurueck}{zur\"uck}%Return
\SetKwBlock{Beginn}{Beginn}{Ende}%Begin
\SetKwRepeat{Wiederh}{wiederhole}{bis}%Repeat
%
\SetKwIF{Wenn}{SonstWenn}{Sonst}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwSwitch{Unterscheide}{Fall}{Anderes}{unterscheide}{tue}{Fall}{sonst}{Ende Fall}{Ende Unt.}%Switch
\SetKwFor{Fuer}{f\"ur}{tue}{Ende f\"ur}%For
\SetKwFor{FuerPar}{f\"ur}{tue gleichzeitig}{Ende gleichzeitig}%ForPar
\SetKwFor{FuerJedes}{f\"ur jedes}{tue}{Ende f\"ur}%ForEach
\SetKwFor{FuerAlle}{f\"ur alle}{tue}{Ende f\"ur}%ForAll
\SetKwFor{Solange}{solange}{tue}{Ende solange}%While
}{}%
%
% --- Czech keywords
%
\ifthenelse{\boolean{algocf@localkw@czech}\OR\equal{\algocf@languagechoosen}{czech}}{%
\SetKwInput{Vst}{Vstup}%
\SetKwInput{Vyst}{V\'{y}stup}%
\SetKwInput{Vysl}{V\'{y}sledek}%
}{}%
%
% --- Portuguese keywords
%
\ifthenelse{\boolean{algocf@localkw@portuguese}\OR\equal{\algocf@languagechoosen}{portuguese}}{%
\SetKwInput{Entrada}{Entrada}%
\SetKwInput{Saida}{Sa\'{i}da}%
\SetKwInput{Dados}{Dados}%
\SetKwInput{Resultado}{Resultado}%
\SetKw{Ate}{at\'{e}}
\SetKw{KwRetorna}{retorna}%
\SetKw{Retorna}{retorna}%
\SetKwBlock{Inicio}{in\'{i}cio}{fim}%
\SetKwRepeat{Repita}{repita}{at\'{e}}%
%
\SetKwIF{Se}{SenaoSe}{Senao}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwSwitch{Selec}{Caso}{Outro}{selecione}{fa\c{c}a}{caso}{sen\~{a}o}{fim caso}{fim selec}%
\SetKwFor{Para}{para}{fa\c{c}a}{fim para}%
\SetKwFor{ParaPar}{para}{fa\c{c}a em paralelo}{fim para}
\SetKwFor{ParaCada}{para cada}{fa\c{c}a}{fim para cada}%
\SetKwFor{ParaTodo}{para todo}{fa\c{c}a}{fim para todo}%
\SetKwFor{Enqto}{enquanto}{fa\c{c}a}{fim enqto}%
}{}%
%
% --- Italian keywords
%
\ifthenelse{\boolean{algocf@localkw@italiano}\OR\equal{\algocf@languagechoosen}{italiano}}{%
\SetKwInput{KwIng}{Ingresso}%
\SetKwInput{KwUsc}{Uscita}%
\SetKwInput{KwDati}{Dati}%
\SetKwInput{KwRisult}{Risultato}%
\SetKw{KwA}{a}%
\SetKw{KwRitorna}{ritorna}%
\SetKw{Ritorna}{ritorna}%
\SetKwBlock{Inizio}{inizio}{fine}%
\SetKwRepeat{Ripeti}{ripeti}{finch\'e}%
%
\SetKwIF{Sea}{AltSe}{Altrimenti}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{endsw}%
\SetKwFor{Per}{per}{fai}{fine per}%
\SetKwFor{PerPar}{per}{fai in parallelo}{fine per}%
\SetKwFor{PerCiascun}{per ciascun}{fai}{fine per ciascun}%
\SetKwFor{PerTutti}{per tutti i}{fai}{fine per tutti}%
\SetKwFor{Finche}{finch\'e}{fai}{fine finch\'e}%
}{}%
%
% --- Spanish keywords
%
\ifthenelse{\boolean{algocf@localkw@spanish}\OR\equal{\algocf@languagechoosen}{spanish}}{%
\SetKwInput{Datos}{Datos}
\SetKwInput{Resultado}{Resultado}
\SetKwInput{Entrada}{Entrada}
\SetKwInput{Salida}{Salida}
\SetKw{KwA}{a}
\SetKw{KwDevolver}{devolver}
\SetKw{Devolver}{devolver}
\SetKwBlock{Inicio}{inicio}{fin}
\SetKwIF{SSi}{EnOtroCasoSi}{EnOtroCaso}{si}{entonces}{sin\'o, si}{sin\'o}{fin si}
\SetKwSwitch{Seleccionar}{Caso}{Otro}{seleccionar}{hacer}{caso}{sin\'o}{fin caso}{fin seleccionar}
\SetKwFor{Para}{para}{hacer}{fin para}
\SetKwFor{ParaPara}{par}{hacer en paralelo}{fin para}
\SetKwFor{EnParalelo}{para}{hacer en paralelo}{fin para}
\SetKwFor{Mientras}{mientras}{hacer}{fin mientras}
\SetKwFor{ParaCada}{para cada}{hacer}{fin para cada}
\SetKwFor{ParaTodo}{para todo}{hacer}{fin para todo}
\SetKwRepeat{Repetir}{repetir}{hasta que}
}{}%
%
% Croatian keywords
%
\ifthenelse{\boolean{algocf@localkw@croatian}\OR\equal{\algocf@languagechoosen}{croatian}}{%
\SetKwInput{KwUlaz}{Ulaz}%KwIn
\SetKwInput{KwIzlaz}{Izlaz}%KwOut
\SetKwInput{KwPodaci}{Podaci}%KwData
\SetKwInput{KwRezultat}{Rezultat}%KwResult
\SetKw{KwDo}{do}%KwTo
\SetKw{KwVrati}{vrati}%KwRet
\SetKw{Vrati}{vrati}%Return
\SetKwBlock{Pocetak}{po\v{c}etak}{kraj}%Begin
\SetKwRepeat{Ponavljaj}{ponavljaj}{dok ne bude}%Repeat
%
\SetKwIF{Ako}{InaceAko}{Inace}{ako}{onda}{ina\v{c}e ako}{ina\v{c}e}{kraj ako}%gIf
\SetKwSwitch{Granaj}{Slucaj}{OstaliSlucajevi}{granaj}{\v{c}ini}{slu\v{c}aj}{ostali slu\v{c}ajevi}{kraj slu\v{c}aj}{kraj granaj}%Switch
\SetKwFor{Za}{za}{\v{c}ini}{kraj za}%For
\SetKwFor{ZaPar}{za}{\v{c}ini paralelno}{kraj za paralelno}%ForPar
\SetKwFor{ZaSvaki}{za svaki}{\v{c}ini}{kraj za svaki}%mForEach
\SetKwFor{ZaSvaku}{za svaku}{\v{c}ini}{kraj za svaku}%fForEach
\SetKwFor{ZaSvako}{za svako}{\v{c}ini}{kraj za svako}%nForEach
\SetKwFor{ZaSve}{za sve}{\v{c}ini}{kraj za sve}%ForAll
\SetKwFor{Dok}{dok}{\v{c}ini}{kraj dok}%While
}{}%

%
% --- Turkish keywords
%
\ifthenelse{\boolean{algocf@localkw@turkish}\OR\equal{\algocf@languagechoosen}{turkish}}{%
\SetKwInput{KwIn}{Girdi}%
\SetKwInput{KwOut}{\c{C}{\i}kt{\i}}%
\SetKwInput{KwData}{Veri}%
\SetKwInput{KwResult}{Sonu\c{c}}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
% %
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
}{}%
%
% --- End 
%}
%
%\algocf@defaults@common
%
% option onelanguage redefinition
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{french}}{%
\SetKwInput{KwIn}{Entr\'ees}%
\SetKwInput{KwOutSortie}{Sorties}%
\SetKwInput{KwData}{Donn\'ees}%
\SetKwInput{KwResult}{R\'esultat}%
\SetKw{KwTo}{\`a}%
\SetKw{KwRet}{retourner}%
\SetKw{Return}{retourner}%
\SetKwBlock{Begin}{d\'ebut}{fin}%
\SetKwRepeat{Repeat}{r\'ep\'eter}{jusqu'\`a}%
%
\SetKwIF{If}{ElseIf}{Else}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwSwitch{Switch}{Case}{Other}{suivant}{faire}{cas o\`u}{autres cas}{fin cas}{fin d'alternative}%
\SetKwFor{For}{pour}{faire}{fin pour}%
\SetKwFor{ForPar}{pour}{faire en parall\`ele}{fin pour}%
\SetKwFor{ForEach}{pour chaque}{faire}{fin pour chaque}%
\SetKwFor{ForAll}{pour tous}{faire}{fin pour tous}%
\SetKwFor{While}{tant que}{faire}{fin tq}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{german}}{%
\SetKwInput{KwIn}{Eingabe}%KwIn
\SetKwInput{KwOut}{Ausgabe}%KwOut
\SetKwInput{KwData}{Daten}%KwData
\SetKwInput{KwResult}{Ergebnis}%KwResult
\SetKw{KwTo}{bis}%KwTo
\SetKw{KwRet}{zur\"uck}%KwRet
\SetKw{Return}{zur\"uck}%Return
\SetKwBlock{Begin}{Beginn}{Ende}%Begin
\SetKwRepeat{Repeat}{wiederhole}{bis}%Repeat
%
\SetKwIF{If}{ElseIf}{Else}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwSwitch{Switch}{Case}{Other}{unterscheide}{tue}{Fall}{sonst}{Ende Fall}{Ende Unt.}%Switch
\SetKwFor{For}{f\"ur}{tue}{Ende f\"ur}%For
\SetKwFor{ForPar}{f\"ur}{tue gleichzeitig}{Ende gleichzeitig}%ForPar
\SetKwFor{ForEach}{f\"ur jedes}{tue}{Ende f\"ur}%ForEach
\SetKwFor{ForAll}{f\"ur alle}{tue}{Ende f\"ur}%ForAll
\SetKwFor{While}{solange}{tue}{Ende solange}%While
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{portuguese}}{%
\SetKwInput{KwIn}{Entrada}%
\SetKwInput{KwOut}{Sa\'{i}da}%
\SetKwInput{KwData}{Dados}%
\SetKwInput{KwResult}{Resultado}%
\SetKw{KwTo}{at\'{e}}
\SetKw{KwRet}{retorna}%
\SetKw{Return}{retorna}%
\SetKwBlock{Begin}{in\'{i}cio}{fim}%
\SetKwRepeat{Repeat}{repita}{at\'{e}}%
%
\SetKwIF{If}{ElseIf}{Else}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwSwitch{Switch}{Case}{Other}{selecione}{fa\c{c}a}{caso}{sen\~{a}o}{fim caso}{fim selec}%
\SetKwFor{For}{para}{fa\c{c}a}{fim para}%
\SetKwFor{ForPar}{para}{fa\c{c}a em paralelo}{fim para}
\SetKwFor{ForEach}{para cada}{fa\c{c}a}{fim para cada}%
\SetKwFor{ForAll}{para todo}{fa\c{c}a}{fim para todo}%
\SetKwFor{While}{enquanto}{fa\c{c}a}{fim enqto}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{italiano}}{%
\SetKwInput{KwIn}{Ingresso}%
\SetKwInput{KwOut}{Uscita}%
\SetKwInput{KwData}{Dati}%
\SetKwInput{KwResult}{Risultato}%
\SetKw{KwTo}{a}%
\SetKw{KwRet}{ritorna}%
\SetKw{Return}{ritorna}%
\SetKwBlock{Begin}{inizio}{fine}%
\SetKwRepeat{Repeat}{ripeti}{finch\'e}%
%
\SetKwIF{If}{ElseIf}{Else}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{endsw}%
\SetKwFor{For}{per}{fai}{fine per}%
\SetKwFor{ForPar}{per}{fai in parallelo}{fine per}%
\SetKwFor{ForEach}{per ciascun}{fai}{fine per ciascun}%
\SetKwFor{ForAll}{per tutti i}{fai}{fine per tutti}%
\SetKwFor{While}{finch\'e}{fai}{fine finch\'e}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{spanish}}{%
\SetKwInput{KwIn}{Entrada}%
\SetKwInput{KwOut}{Salida}%
\SetKwInput{KwData}{Datos}%
\SetKwInput{KwResult}{Resultado}%
\SetKw{KwTo}{a}%
\SetKw{KwRet}{devolver}%
\SetKw{Return}{devolver}%
\SetKwBlock{Begin}{inicio}{fin}%
\SetKwRepeat{Repeat}{repetir}{hasta que}%
%
\SetKwIF{If}{ElseIf}{Else}{si}{entonces}{si no, si}{en otro caso}{fin si}
\SetKwSwitch{Switch}{Case}{Other}{seleccionar}{hacer}{caso}{si no}{fin caso}{fin seleccionar}
\SetKwFor{For}{para}{hacer}{fin para}%
\SetKwFor{ForPar}{para}{hacer in paralelo}{fin para}%
\SetKwFor{ForEach}{para cada}{hacer}{fin para cada}
\SetKwFor{ForAll}{para todo}{hacer}{fin para todo}
\SetKwFor{While}{mientras}{hacer}{fin mientras}
}{}%
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{croatian}}{%
\SetKwInput{KwIn}{Ulaz}%KwIn
\SetKwInput{KwOut}{Izlaz}%KwOut
\SetKwInput{KwData}{Podaci}%KwData
\SetKwInput{KwResult}{Rezultat}%KwResult
\SetKw{KwTo}{do}%KwTo
\SetKw{KwRet}{vrati}%KwRet
\SetKw{Return}{vrati}%Return
\SetKwBlock{Begin}{po\v{c}etak}{kraj}%Begin
\SetKwRepeat{Repeat}{ponavljaj}{dok ne bude}%Repeat
%
\SetKwIF{If}{ElseIf}{Else}{ako}{onda}{ina\v{c}e ako}{ina\v{c}e}{kraj ako}%gIf
\SetKwSwitch{Switch}{Case}{Other}{granaj}{\v{c}ini}{slu\v{c}aj}{ostali slu\v{c}ajevi}{kraj slu\v{c}aj}{kraj granaj}%Switch
\SetKwFor{For}{za}{\v{c}ini}{kraj za}%For
\SetKwFor{ForPar}{za}{\v{c}ini paralelno}{kraj za paralelno}%ForPar
\SetKwFor{ForEach}{za svaki}{\v{c}ini}{kraj za svaki}%ForEach
\SetKwFor{ForAll}{za sve}{\v{c}ini}{kraj za sve}%ForAll
\SetKwFor{While}{dok}{\v{c}ini}{kraj dok}%While
}{}%
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{turkish}}{%
%
\SetKwInput{KwIn}{Girdi}%
\SetKwInput{KwOut}{\c{C}{\i}kt{\i}}%
\SetKwInput{KwData}{Veri}%
\SetKwInput{KwResult}{Sonu\c{c}}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
%
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
}{}%
%
%
%%%% old commands compatibility
%
\ifthenelse{\boolean{algocf@oldcommands}}{%
\newcommand{\SetNoLine}{\SetAlgoNoLine}%
\newcommand{\SetNoline}{\SetAlgoNoLine}%
\newcommand{\SetVline}{\SetAlgoVlined}%
\newcommand{\SetLine}{\SetAlgoLined}%
%
\newcommand{\dontprintsemicolon}{\DontPrintSemicolon}%
\newcommand{\printsemicolon}{\PrintSemicolon}%
\newcommand{\incmargin}[1]{\IncMargin{#1}}%
\newcommand{\decmargin}[1]{\DecMargin{-#1}}%
\newcommand{\setnlskip}[1]{\SetNlSkip{#1}}%
\newcommand{\Setnlskip}[1]{\SetNlSkip{#1}}%
\newcommand{\setalcapskip}[1]{\SetAlCapSkip{#1}}%
\newcommand{\setalcaphskip}[1]{\SetAlCapHSkip{#1}}%
\newcommand{\nlSty}[1]{\NlSty{#1}}%
\newcommand{\Setnlsty}[3]{\SetNlSty{#1}{#2}{#3}}%
\newcommand{\linesnumbered}{\LinesNumbered}%
\newcommand{\linesnotnumbered}{\LinesNotNumbered}%
\newcommand{\linesnumberedhidden}{\LinesNumberedHidden}%
\newcommand{\showln}{\ShowLn}%
\newcommand{\showlnlabel}[1]{\ShowLnLabel{#1}}%
\newcommand{\nocaptionofalgo}{\NoCaptionOfAlgo}%
\newcommand{\restorecaptionofalgo}{\RestoreCaptionOfAlgo}%
\newcommand{\restylealgo}[1]{\RestyleAlgo{#1}}%
%
\newcommand{\Titleofalgo}[1]{\TitleOfAlgo{#1}}%
% \SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
\newcommand{\SetKwIf}[6]{\SetKwIF{#1}{#2#1}{#2}{#3}{#4}{#5 #1}{#5}{#6}}
%
\SetKwIF{gSi}{gSinonSi}{gSinon}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwIF{gIf}{gElsIf}{gElse}{if}{then}{else if}{else}{end if}%
\SetKwIF{gIf}{gElseIf}{gElse}{if}{then}{else if}{else}{end if}%
\SetKwIF{gWenn}{gSonstWenn}{gSonst}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwIF{gSe}{gSenaoSe}{gSenao}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwIF{gSea}{gAltSe}{gAltrimenti}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKw{Ret}{return}%
\SetKwInput{Data}{Data}%
\SetKwInput{Result}{Result}%
}{%
  \relax%
}%
%
%
%
%%
%%%
%%%% END

==> files/PF.tex <==

% ------------------------------------------------------------------------------- %
\subsection{Robot Motion Model}
Consider $N$ mobile robots that reside in a complex environment $\Omega\subset \reals^d$ with obstacles of arbitrary shape located at $O\subset\Omega$, where $d$ is the dimension of the workspace. The dynamics of the robots are described by $\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t))$,
%
%\begin{equation}\label{eq:rdynamics}
%\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t)),
%\end{equation}
for all $j\in\ccalN:=\{1,\dots,N\}$, where $\bbp_{j}(t) \in \Omega_{\text{free}}:=\Omega \backslash O$ stands for the state of robot $j$ in the obstacle-free space $\Omega_{\text{free}}$, $\bbu_{j}(t) \in\ccalU_j$ stands for a control input in a \textit{finite} space of admissible controls $\ccalU_j$. % is a \textit{finite} space of admissible controllers.
Note that the state $\bbp_{j}$ may belong to a higher dimensional space than $\Omega_{\text{free}}$\BS{Can we make this into a  remark or just remove it? It's extra clutter for something that is fairly straightforward}. For example, this is the case if $\bbp_j(t)$ includes the position and the orientation of robot $j$. Nevertheless, throughout the rest of the paper, for simplicity of notations we denote $\bbp_{j}(t) \in \Omega_{\text{free}}$. Also, note that the considered dynamics can range from simple graph-based dynamics \cite{yaziciouglu2017communication} to arbitrary nonlinear discrete dynamics \cite{fu2016optimal}. Hereafter, for simplicity of notation, we compactly denote the dynamics of all robots as $\bbp(t+1)=\bbf(\bbp(t),\bbu(t))$,
%\begin{equation}\label{eq:rdynamics}
%\bbp(t+1)=\bbf(\bbp(t),\bbu(t)),
%\end{equation}
where $\bbp(t)\in \Omega_{\text{free}}^N$, for all $t\geq 0$, and $\bbu(t)\in\ccalU:=\ccalU_1\times\dots\times\ccalU_N$.
\subsection{Estimation Task}
The task of the robots is to collaboratively estimate a \textit{hidden state} governed by the following dynamics:

\begin{equation} \label{eq:nonlinDynamics}
\bbx(t+1) =\bbg(\bbx(t),\bbw(t)),
\end{equation}
where $\bbx(t)\in\mathbb{R}^{n}$ and $\bbw(t) \in\reals^{d_w}$ denote the hidden state and the process noise at discrete time $t$, respectively. We assume that the process noise $\bbw(t)$ is normally distributed as $\bbw(t) \sim \ccalN(\bb0, \bbQ(t) )$, where $\bbQ(t)$ is the covariance matrix at time $t$. For instance, \eqref{eq:nonlinDynamics} can model static or mobile targets \cite{atanasov2014information}, spatio-temporal fields \cite{lan2016rapidly} or static fields  \cite{bennetts2013towards}.

Moreover, the robots are equipped with sensors to collect measurements associated with $\bbx(t)$ as per the \textit{observation model}: $\bby_j(t)= \bbm_j(\bbp_j(t),\bbx(t),\bbv(t))$, where $\bby_j(t)$ is the measurement signal at discrete time $t$ taken by  robot $j\in\ccalN$. Also, $\bbv_j(t) \sim \ccalN(\bb0, \bbR_j(t) )$ is sensor-state-dependent Gaussian noise with covariance $\bbR_j(t)$. 
 For instance, the observation model $\bbm_j$ can model cameras or RF-based sensors, while $\bby_j(t)$ can consist of range and/or bearing measurements. Hereafter, we compactly denote the observation models of all robots as 
 \begin{equation} \label{eq:NonLinMeasModel}
\bby(t)= \bbm(\bbp(t),\bbx(t),\bbv(t)),~\bbv(t) \sim \ccalN(\bb0, \bbR(t) ).
\end{equation}

The quality of measurements taken by all robots up to a time instant $t$, collected in a vector denoted by $\bby_{0:t}$, can be evaluated using information measures, such as the mutual information between  $\bby_{0:t}$ and $\bbx(t)$ or the conditional entropy of $\bbx(t)$ given $\bby_{0:t}$. Assuming a Gaussian distribution for $\bbx(t)$, i.e., $\bbx(t)\sim\ccalN(\boldsymbol\mu(t),\Sigma(t|\bby_{0:t}))$, alternative uncertainty measures can also be used such as the trace, determinant, or maximum eigenvalue of the covariance matrix $\Sigma(t|\bby_{0:t})$. 

\subsection{Active Information Acquisition}
Given the initial robot configuration $\bbp(0)$ and the hidden state $\bbx(t)$ that evolves as per \eqref{eq:nonlinDynamics}, our goal is to select a \textit{finite} horizon $F\geq 0$ and compute control inputs $\bbu(t)$, for all time instants $t\in\{0,\dots,F\}$, that solve the following stochastic optimal control problem
%
%$$ \abs{\bbx_t - \bar{\bbx}_{ij,t}} \to 0 \text{ as } t \to \infty , \ \forall \bbq \in \Omega, \forall r_{ij}. $$
%
\begin{subequations}
\label{eq:Prob}
\begin{align}
& \min_{\substack{ F, \bbu_{0:F}}} \left[J(F,\bbu_{0:F},\bby_{0:F}) = \sum_{t=0}^{F}   \det\Sigma(t|\bby_{0:t}) \right]  \label{obj1}\\
%&\ \ \st \ \ \ \ \ \ \ \ \ \ \ \ \bbp(F) \in \ccalP_{\text{goal}}, \label{constr1}\\
&\ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \textcolor{red}{\det\Sigma(F|\bby_{0:F})\leq \delta}, \label{constr2} \\
%&\ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \  F\leq \bar{F},\nonumber\\
& \ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \bbp(t) \in \Omega_{\text{free}}^N,  \label{constr3} \\
&\ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \bbp(t+1) = \bbf(\bbp(t),\bbu(t)), \label{constr4} \\
&\ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \bby(t) = \bbm(\bbp(t),\bbx(t),\bbv(t)), \label{constr5}
\end{align}
\end{subequations}
where the constraints hold for all time instants $t\in\{0,\dots,F\}$.
In \eqref{obj1}, with slight abuse of notation, $\bbu_{0:F}$ stands for the sequence of control inputs applied from $t=0$ until $t=F$.
%
% \{\{\bbu_j(t)\}_{j=1}^{N}
%%\Sigma_i(t)
Also, assuming a Gaussian distribution for $\bbx(t)$, $\det\Sigma(t|\bby_{0:t})$ denotes the determinant of the covariance matrix of $\bbx(t)$ given the set of measurements $\bby_{0:t}$. In words, the objective function \eqref{obj1} captures the cumulative uncertainty in the estimation of $\bbx(t)$ after fusing information collected by all robots from $t=0$ up to time $F$. 
%Moreover, the first constraint \eqref{constr1} requires that at time $F$ the configuration of the robots is within $\ccalP_{\text{goal}}\subseteq \Omega_{\text{free}}^N$; see also Remark \ref{rem1}. 
The first constraint \eqref{constr2} requires that the terminal uncertainty of $\bbx(F)$ to be below a user-specified threshold $\delta$; see also Remark \ref{rem1}.
%$h(\bbx(F)|\ccalY_{0:F})$ denotes the terminal entropy of the hidden state $\bbx(F)$ given $\ccalY_{0:F}$. In words, this constraint requires that the terminal uncertainty of $\bbx(F)$ to be below a user-specified threshold $\delta$; see also Remark \ref{rem1}. %Essentially, the thresholds $\delta_i$ allow for user-specified priorities assigned to the targets in their importance.
%Also, in \eqref{eq:Prob}, $G(\bbx_i(t)|\ccalY_{0:t})$ denotes a user-specified uncertainty metric of the hidden state $\bbx_i(t)$ given the measurements, collected in the set $\ccalY_{0:t}$, taken by all robots up to time $t$. In words, the objective function $J(F,\bbu_{0:F},\ccalY_{0:F})$ in \eqref{eq:Prob} captures the cumulative uncertainty in the estimation of all states $\bbx_i(t)$ after fusing information collected by all robots from $t=0$ up to time $F$. Moreover, the first constraint requires that all robots $j$ at time $F$ are within a region $\ccalP_j^{\text{goal}}\subseteq \Omega$ while the second constraint requires that the entropy (uncertainty) $h_i(\bbx_i(F)|\ccalY_{0:F})$ of the state $\bbx_i(F)$ at time instant $F$ should be below a user-specified threshold $\delta_i$. Essentially, the thresholds $\delta_i$ allow the user to specify which hidden states are more important than others.
%
%Note that in the second constraint any other uncertainty metric can also be used in place of the entropy, without any restrictions, such as mutual information or other scalar functions of the covariance matrix and Fisher Information Matrix (FIM). 
%In other words, the first two constraints require that the robots should sufficiently explore the workspace before reaching the goal regions $\ccalP_j^{\text{goal}}$. 
%The third constraint requires that the terminal horizon $F$ should be below a user-specified parameter $\bar{F}>0$.\footnote{In general, the purpose of the third constraint is to ensure that the terminal horizon $F$ is always finite. In practice, we select $\bar{F}$ to be arbitrarily large, but finite, so that the robots have sufficiently enough time to estimate the hidden states.}
%
The second constraint \eqref{constr3} requires that the robots should never collide with obstacles. The last two constraints capture the robot dynamics \eqref{eq:nonlinDynamics} and the observation model \eqref{eq:NonLinMeasModel}.
%\red{DELETE the third constraint. Just say that you assume that the problem is well-defined/feasible, i.e., the optimal solution has a finite path. This is also the case in a shortest path problem. Feasible solution: travel forever and reach the goal after asn inf number of steps. Pick deltai so that this is true...If obj negative then optimal solution is travel forever.}
%in rrt F is finite because you are searching an bounded domain. here you are searching an infinite domain (workspace x information)

\begin{rem}[Optimal Control Problem \eqref{eq:Prob}]\label{rem1}
In \eqref{eq:Prob}, any other optimality metric, not necessarily information-based, can be used in place of \eqref{obj1} as long as it is always positive. If non-positive metrics are selected, e.g., the entropy of $\bbx(t)$, then \eqref{eq:Prob} is not well-defined, since the  optimal terminal horizon $F$ is infinite. On the other hand, in the first constraint \eqref{constr2}, any uncertainty metric can be used without any restrictions. Moreover, note that without the terminal constraint \eqref{constr2}, the optimal solution of \eqref{eq:Prob} is  all robots to stay put, i.e., $ F=0$. 
Additional terminal constraints can be added to \eqref{eq:Prob}, such as, $\bbp(F)\in\ccalP_{\text{goal}}\subseteq\Omega_{\text{free}}^N$, to model joint task planning and estimation scenarios, where, e.g., the robots should eventually visit a user to report an estimate of the hidden state with user-specified accuracy determined by $\delta$.
\end{rem}

%Hereafter, we assume a Gaussian prior distribution for the hidden states $\bbx_i(0)$ is given, i.e., $\bbx_i(0)\sim\ccalN(\hat{\bbx}_i(0),\Sigma_i(0))$. Moreover, we require that the uncertainty metric $G(\bbx_i(t)|\ccalY_{0:t})$ is positive, i.e., $G(\bbx_i(t)|\ccalY_{0:t})\geq 0$, for all $t\geq 0$. For instance, valid selections for $G(\bbx_i(t)|\ccalY_{0:t})$ can be  the determinant, or the trace, or the minimum eigenvalue of the covariance matrix or the FIM. As it will be shown in  Section \ref{sec:convergence}, the positiveness of $G(\bbx_i(t)|\ccalY_{0:t})$ ensures that the optimal horizon $F$ in \eqref{eq:Prob} is finite. 
%where $\Sigma_i(t|\ccalY_{1:t}$ is the covariance matrix of the hidden state $\bbx_i$ at the time instant $t$ given the past measurements $\ccalY_{1:t}$. 

 %This also implies that $J(t,\bbu_{0:t})\geq 0$, for all $t\geq 0$ and, therefore, $J(t,\bbu_{0:t})$ is monotone. To see this, observe that $J(t+1,\bbu_{0:t+1},\ccalY_{0:t+1})= J(t,\bbu_{0:t}, \ccalY_{0:t})+\sum_{i=1}^{M} G(\bbx_i(t+1)|\ccalY_{0:t+1})\geq J(t,\bbu_{0:t},\ccalY_{0:t})\geq 0$, since $\sum_{i=1}^{M} G(\bbx_i(t+1)|\ccalY_{0:t+1})\geq 0$, for all $t\geq 0$. The latter result guarantees that the optimal horizon $t_f$ is finite, since increasing the horizon $t_f$ can only increase the cost  $J(t_f,\bbu_{0:t_f},\ccalY_{0:t_f})$. 
%Note that other positive  uncertainty metrics can be employed

\subsection{Problem Reformulation: A Separation Principle}\label{sec:reform}

The Active Information Acquisition problem in \eqref{eq:Prob} is a stochastic optimal control problem for which, in general, closed-loop control policies are preferred. Nevertheless, assuming linear dynamics for the hidden state in \eqref{eq:nonlinDynamics} and linear observation models in \eqref{eq:NonLinMeasModel}, i.e., 

\begin{equation} \label{eq:dynamics}
\bbx(t+1) =\bbA\bbx(t)  + \bbB\bbd(t) + \bbw(t),
\end{equation}
where $\bbd(t)$ is a control input, and 
\begin{equation} \label{eq:measModel}
\bby(t) = \bbH(\bbx(t))\bbx(t) + \bbv(\bbx(t)),%\bbh(\bbx(t), \bbq, \bbv(t)),
\end{equation}
the stochastic optimal control problem \eqref{eq:Prob} reduces to the following deterministic optimal control problem; see also \cite{atanasov2014information}.

%Deterministic optimal control problem:
\begin{subequations}
\label{eq:Prob2}
\begin{align}
& \min_{\substack{ F, \bbu_{0:F}}} \left[J(F,\bbu_{0:F}) = \sum_{t=0}^{F}  \det\Sigma(t) \right] \label{obj2}\\
%&\ \ \st \ \ \ \ \ \ \ \ \ \ \ \ \bbp(F) \in \ccalP_{\text{goal}}, \label{constr21}\\
& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \det\Sigma(F)\leq \delta,  \label{constr22} \\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \bbp(t) \in \Omega_{\text{free}}^N, \label{constr23} \\
& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \bbp(t+1) = \bbf(\bbp(t),\bbu(t)), \label{constr24}\\
& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \Sigma(t+1) =\rho(\Sigma(t)), \label{constr25}
\end{align}
\end{subequations}
where $\rho(\cdot)$ stands for the Kalman Filter Ricatti map. Note also open loop (offline) policies are optimal solutions to \eqref{eq:Prob2}. Then, the problem that we address in this paper can be summarized as follows%; \red{see also Figure ??}.
%
\begin{problem} \label{prob}(Active Information Acquisition)
Given an initial robot configuration $\bbp(0)$ and a hidden state $\bbx(t)$ that evolves as per \eqref{eq:dynamics}, select a horizon $F$ and compute control inputs $\bbu(t)$ for all time instants $t\in\{0,\dots,F\}$ as per the optimal control problem \eqref{eq:Prob2}.
%
\end{problem}

Finally, throughout the paper we make the following assumption.% and the underlying communication network between the robots.
\begin{assumption} \label{as:assumption}%[State Model]
The dynamics of the state \eqref{eq:dynamics}, the observation model \eqref{eq:measModel}, and process and measurement noise covariances $\bbQ(t)$ and $\bbR(t)$ are known. %Furthermore, the state dynamics \eqref{eq:dynamics} and sensing model \eqref{eq:measModel} are differentiable functions. 
%Finally, we assume that all robots can communicate with each other at any time $t$. 
\end{assumption}

\begin{rem}[Nonlinear \& Noisy Models]
%Note that we assume that the dynamics \eqref{eq:dynamics} and the sensing model \eqref{eq:measModel} are modeled as linear systems. Also, in \eqref{eq:rdynamics} we assume noiseless robot dynamics. As discussed before, 
Note that Assumption \ref{as:assumption} allows for offline computation of optimal policies.  Nevertheless, in Section \ref{sec:Sim}, we show that this assumption can be relaxed; in this case suboptimal controllers are synthesized. \red{[refine remark once simulations are added and problem formulation is finished]}
\end{rem}



==> files/proofs.tex <==
%\section{Proof of Completeness \& Optimality}\label{sec:prop}

In what follows, we denote by $\mathcal{G}^n=\{\mathcal{V}^{n}, \mathcal{E}^{n}, \texttt{Cost}\}$ the tree that has been built by Algorithm \ref{alg:RRT} at the $n$-th iteration. The same notation also extends to $f_{\ccalV}$, $f_{\ccalU}$, and $\bbu_{\text{new}}$. %We also denote by $f_{\ccalV}^n$ and $f_{\ccalU}^n$ the density functions used at iteration $n$ of Algorithm \ref{alg:RRT}. The same notations extends to subsets $\ccalV_{k}$ $k_{\text{rand}}$, and $\bbu_{\text{new}}$. For simplicity of notations, we denote by $\ccalV_{k_{\text{rand}}}^n\subseteq \ccalV^n$ (instead of  $\ccalV_{k_{\text{rand}}^n}^n$) the subset of nodes selected by $f_{\ccalV}^n$ at iteration $n$.
%
%
%
To prove Theorems \ref{thm:probCompl} and \ref{thm:asOpt}, we need to prove the following results. %that rely on the Borel-Cantelli lemma \cite{grimmett2001probability}.

%\begin{lem}[Borel-Cantelli \cite{grimmett2001probability}]\label{lem:bc}
%Consider a sequence of independent events $A=\{A^n\}_{n=1}^{\infty}$. If $\sum_{n=1}^{\infty}\mathbb{P}(A^n)=\infty$ then $\mathbb{P}(\limsup_{n\to\infty} A^n)=1$, i.e., the probability that infinitely many events $A^n$ occur is 1.  
%i.e., the events $A^n$ occur infinitely often meaning that $A^n$ is true for an infinite number of indices $n\in\mathbb{N}_{+}$.
%\end{lem}


\begin{lem}[Sampling $\ccalV_{k_{\text{rand}}}^n$]
Consider any subset $\ccalV_{k}^n$ and any fixed iteration index $n$ and any fixed $k\in\set{1,\dots,K_n}$. Then, there exists an infinite number of subsequent iterations $n+w$,  where $w\in\mathcal{W}$ and $\mathcal{W}\subseteq\mathbb{N}$ is a subsequence of $\mathbb{N}$, at which the subset $\ccalV_{k}^n$ is selected to be the set $\ccalV_{k_{\text{rand}}}^{n+w}$. %\footnote{The subsequences $\ccalK$ and $\ccalK'$}
\label{lem:qrand}
\end{lem}

\begin{proof}
%The proof of this results relies on Lemma \ref{lem:bc}.
Let $A^{\text{rand},n+w}(k)=\{\ccalV_{k_{\text{rand}}}^{n+w}=\ccalV_{k}^n\}$, with $w\in\mathbb{N}$, denote the event that at iteration $n+w$ of Algorithm \ref{alg:RRT} the subset $\ccalV_{k}^n\subseteq\ccalV^n$ is selected by the sampling operation to be the set $\ccalV_{k_{\text{rand}}}^{n+w}$ [line \ref{rrt:samplekrand}, Alg. \ref{alg:RRT}]. Also, let $\mathbb{P}(A^{\text{rand},n+w}(k))$ denote the probability of this event, i.e., $\mathbb{P}(A^{\text{rand},n+w}(k))=f_{\ccalV}^{n+w}(k)$. 

Next, define the infinite sequence of events $A^{\text{rand}}=\{A^{\text{rand},n+w}(k)\}_{w=0}^{\infty}$, for a given subset $\ccalV_{k}^n\subseteq\ccalV^n$. In what follows, we show that the series $\sum_{w=0}^{\infty}\mathbb{P}(A^{\text{rand},n+w}(k))$ diverges and then we complete the proof by applying the Borel-Cantelli lemma \cite{grimmett2001probability}. %Lemma \ref{lem:bc}. 
%
%Recall first that the size of $K_{n+e}$, i.e., the number of  subsets $\ccalV_{T,k}^{n+e}$ cannot grow arbitrarily large as $e\to\infinity$, since it holds that $|\ccalU|=|\ccalU_1\times\ccalU_2\times\dots\times\ccalU_n|<\infty$, by assumption. Also, 

Recall that by Assumption \ref{frand}(i), we have that  given any subset $\ccalV_{k}^n\subseteq\ccalV^n$, the probability $f_{\ccalV}^n(k|\ccalV^n)$ satisfies $f_{\ccalV}^n(k|\ccalV^n)\geq \epsilon$, for any iteration $n$. Thus we have that $\mathbb{P}(A^{\text{rand},n+w}(k))=f_{\ccalV}^{n+w}(k|\ccalV^{n+w})\geq \epsilon>0, 
$
%\begin{equation}\label{ineq1}
%\mathbb{P}(A^{\text{rand},n+w}(k))=f_{\ccalV}^{n+w}(k|\ccalV^{n+w})\geq \epsilon> 0, 
%\end{equation} 
for all $w\in\mathbb{N}$. Note that this result holds for any $k\in\set{1,\dots,K_{n+w}}$ due to Assumption \ref{frand}(i). 
%
%Since \eqref{ineq1} holds for all $w\in\mathbb{N}$, 
Therefore, we have that $\sum_{w=0}^{\infty}\mathbb{P}(A^{\text{rand},n+w}(k))\geq\sum_{w=0}^{\infty}\epsilon.$
%\begin{equation}\label{ineq2}
%\sum_{w=0}^{\infty}\mathbb{P}(A^{\text{rand},n+w}(k))\geq\sum_{w=0}^{\infty}\epsilon.
%\end{equation}
Since $\epsilon$ is a strictly positive constant, we have that $\sum_{w=0}^{\infty}\epsilon$ diverges. Then, %by the comparison test \cite{marsden1993elementary}, 
we conclude that $\sum_{w=0}^{\infty}\mathbb{P}(A^{\text{rand},n+w}(k))=\infty.$
%\begin{equation}\label{res1}
%\sum_{w=0}^{\infty}\mathbb{P}(A^{\text{rand},n+w}(k))=\infty.
%\end{equation}
%
Combining this result and the fact that the events $A^{\text{rand},n+w}(k)$ are independent by Assumption \ref{frand}(ii), we get that $\mathbb{P}(\limsup_{k\to\infty} A^{\text{rand},n+w}(k)=1,$ by the Borel-Cantelli lemma. In other words, the events $A^{\text{rand},n+w}(k)$ occur infinitely often, for all $k\in\{1,\dots,K_n\}$. This equivalently means that for every subset $\ccalV_{k}^n\subseteq\ccalV^n$, for all $n\in\mathbb{N}_{+}$, there exists an infinite subsequence $\mathcal{W}\subseteq \mathbb{N}$ so that for all $w\in\mathcal{W}$ it holds $\ccalV_{k_{\text{rand}}}^{n+w}=\ccalV^{n}$, completing the proof.
\end{proof}
    
%Using Lemma \ref{lem:qrand} we can show the following result for the control input.
\begin{lem}[Sampling $\bbu_{\text{new}}$]
Consider any  subset $\ccalV_{k_{\text{rand}}}^n$ selected by $f_{\ccalV}$ and any fixed iteration index $n$. Then, for any given control input $\bbu\in\ccalU$, there exists an infinite number of subsequent iterations $n+w$, where $w\in\mathcal{W}'$ and $\mathcal{W}'\subseteq\mathcal{W}$ is a subsequence of the sequence of $\mathcal{W}$ defined in Lemma \ref{lem:qrand}, at which the control input $\bbu\in\ccalU$ is selected to be $\bbu_{\text{new}}^{n+w}$.
\label{lem:qnew}
\end{lem}

\begin{proof}
%This proof resembles the proof of Lemma \ref{lem:qrand} and is omitted.
%
Define the infinite sequence of events $A^{\text{new}}=\{A^{\text{new},n+w}(\bbu)\}_{w=0}^{\infty}$, for $\bbu\in\ccalU$, where $A^{\text{new},n+w}(\bbu)=\{\bbu_{\text{new}}^{n+w}=\bbu\}$, for $w\in\mathbb{N}$, denotes the event that at iteration $n+w$ of Algorithm \ref{alg:RRT} the control input $\bbu\in\ccalU$ is selected by the sampling function to be the input $\bbu_{\text{new}}^{n+w}$, given the subset $\ccalV_{k_{\text{rand}}}^n\in\ccalV_{k_{\text{rand}}}^{n+w}$. Moreover, let $\mathbb{P}(A^{\text{new},n+w}(\bbu))$ denote the probability of this event, i.e., $\mathbb{P}(A^{\text{new},n+e}(\bbu))=f_{\ccalU}^{n+w}(\bbu| \ccalV_{k_{\text{rand}}}^{n+w})$. 
%
Now, consider those iterations $n+w$ with $w\in\mathcal{W}$ such that $k_{\text{rand}}^{n+w}=k_{\text{rand}}^n$ by Lemma \ref{lem:qrand}. We will show that the series $\sum_{w\in\ccalK}\mathbb{P}(A^{\text{new},n+w}(\bbu))$ diverges and then we will use Borel-Cantelli lemma  to show that any given $\bbu\in\ccalU$ will be selected infinitely often to be control input $\bbu_{\text{new}}^{n+w}$.
%
By Assumption \ref{fnew}(i)  we have that $\mathbb{P}(A^{\text{new},n+w}(\bbu))=f_{\ccalU}^{n+w}(\bbu| \ccalV_{k_{\text{rand}}}^{n+w})$ is bounded below by a strictly positive constant $\zeta>0$ for all $w\in\ccalW$. 
Therefore, we have that $\sum_{w\in\ccalW}\mathbb{P}(A^{\text{new},n+w}(\bbu))$ diverges, since it is an infinite sum of a strictly positive constant term. Using this result along with the fact that the events $A^{\text{new},n+w}(\bbu)$ are independent, by Assumption \ref{fnew}(ii), we get that $\mathbb{P}(\limsup_{w\to\infty} A^{\text{new},n+w}(\bbu))=1,$ due to the Borel-Cantelli lemma. In words, this means that the events $A^{\text{new},n+w}(\bbu)$ for $w\in\mathcal{W}$ occur infinitely often. Thus, given any subset $\ccalV_{k_{\text{rand}}}^n$, for every control input $\bbu$ and for all $n\in\mathbb{N}_{+}$, there exists an infinite subsequence $\mathcal{W}' \subseteq \mathcal{W}$ so that for all $w\in\mathcal{W}'$ it holds $\bbu_{\text{new}}^{n+w}=\bbu$, completing the proof.
\end{proof}

Before stating the next result, we first define the \textit{reachable} state-space of a state $\bbq(t)=[\bbp(t),\Sigma(t)]\in\ccalV_{k}^n$, denoted by $\ccalR(\bbq(t))$ that collects all states $\bbq(t+1)=[\bbp(t+1), \Sigma(t+1)]$ that can be reached within one time step from $\bbq(t)$.%, where recall that  $\bbp_j(t+1)=\bbf_j(\bbp_j(t),\bbu_j)\in\Omega_{\text{free}}$, $d_i(t+1)=\det\Sigma_i(t+1)=\det\rho(\Sigma_i(t))$. In math, $\ccalR(\bbq(t))$ is defined as follows. 

%\begin{align}\label{eq:reachableSet}
%\ccalR(\bbq(t))&=\{\bbq(t+1)=[\bbp(t+1), \bbd(t+1)]~|~\nonumber \\ &\bbp_j(t+1)=\bbg(\bbp_j(t),\bbu_j), \forall j,\\& d_i(t+1)=\Sigma_i(t+1)=\det\rho(\Sigma_i(t)), \forall i, \forall \bbu\in\ccalU \}\nonumber.
%\end{align}

%\subsection{Proof of Corollary \ref{cor:reach}}
\begin{cor}[Reachable set $\ccalR(\bbq(t))$]\label{cor:reach}
Given any state $\bbq(t)=[\bbp(t),\Sigma(t)]\in\ccalV_{k}^n$, for any $k\in\{1,\dots,K_n\}$, Algorithm \ref{alg:RRT} will add to $\ccalV^n$ all states that belong to the reachable set $\ccalR(\bbq(t))$ will  be added to $\ccalV^{n+w}$, with probability 1, as $w\to\infty$, i.e., $\lim_{w\rightarrow\infty} \mathbb{P}\left(\{\ccalR(\bbq(t))\subseteq\mathcal{V}^{n+w}\}\right)=1.$
%\begin{equation}\label{eq:reach2}
%\lim_{w\rightarrow\infty} %\mathbb{P}\left(\{\ccalR(\bbq(t))\subseteq\mathcal{V}^{n+w}\}%\right)=1.
%\end{equation}
Also, edges from $\bbq(t)$ to all reachable states $\bbq'(t+1)\in\ccalR(\bbq(t))$ will  be added to $\ccalE^{n+w}$, with probability 1, as $w\to\infty$, i.e., $\lim_{w\rightarrow\infty} \mathbb{P}\left(\{\cup_{\bbq'\in\ccalR(\bbq)}(\bbq,\bbq')\subseteq\mathcal{E}^{n+w}\}\right)=1.$
%\begin{equation}\label{eq:reachedge}
%\lim_{w\rightarrow\infty} %\mathbb{P}\left(\{\cup_{\bbq'\in\ccalR(\bbq)}(\bbq,\bbq')\sub%seteq\mathcal{E}^{n+w}\}\right)=1.
%\end{equation}
\end{cor}
\begin{proof}
The proof straightforwardly follows from Lemmas \ref{lem:qrand}-\ref{lem:qnew} and is omitted. 
%Specifically, recall from Lemma \ref{lem:qrand}, that for any given and fixed iteration index $n$, there exists an infinite sequence of iterations $n+e$, $w\in\ccalW$, where the subset $\ccalV_{k}^{n+w}$, for any given and fixed $k$,  will be selected to be the subset $\ccalV_{{k_{\text{rand}}}}^{n+w}$. Also, given a control input $\bbu_{\text{new}}^{n+e}$ sampled by $f_{\ccalU}^{n+w}$, we have that the state $\bbq'=[\bbp'(t+1),\bbd'(t+1)]$, where $\bbp_j(t+1)=\bbg(\bbp_j,\bbu_{j,\text{new}}^{n+w})$, for all robots $j$, will be added to the tree, if $\bbp'(t+1)\in\Omega_{\text{free}}^N$. By Lemma \ref{lem:qnew}, we get that there exist an infinite sequence number of iterations $n+w$, where $w\in\ccalE'\subseteq \ccalE$, where any given control input $\bbu\in\ccalU$ will be selected to be $\bbu_{\text{new}}^{n+w}$. Since it holds that if $\bbq\in\ccalV_{k}^{n}$, then $\bbq\in\ccalV_{k}^{n+w}$, for all $n+w\geq n$, we conclude that all states that belong to the reachable set $\ccalR(\bbq(t))$ will eventually be added to the tree structure. In mathematical terms this can be written as in \eqref{eq:reach2}, completing the first part of the proof. Moreover, observe when a state $\bbq'\in\ccalR(\bbq)$ (where $\bbq$ is selected to be the node $\bbq_{\text{rand}}^{n+w}$) is added to the set of nodes $\ccalV_T^{n+w}$, then the edge $(\bbq,\bbq')$ is also added to the set of edges $\ccalE^{n+w}$ by construction of Algorithm \ref{alg:RRT}. This means that \eqref{eq:reachedge} holds, as well, completing the proof.
\end{proof}

%Given the above results we are now ready to prove that Algorithm \ref{alg:RRT} is probabilistically complete and asymptotically optimal.
%\subsection{Probabilistic Completeness - Proof of Theorem \ref{thm:probCompl}}\label{app:compl}

%To show this result it suffices to show that $\lim_{n\rightarrow\infty} \mathbb{P}\left(A^n(\bbq_{0:F})\right)=1,$
%\begin{equation}\label{eq:show}
%\lim_{n\rightarrow\infty} %\mathbb{P}\left(A^n(\bbq_{0:F})\right)=1,
%\end{equation}
%where  $A^n(\bbq_{0:F})=\{(\bbq(f)\in\ccalV^n) \wedge ((\bbq(f-1), \bbq(f))\in\mathcal{E}^{n}), \forall f\in\{1,\dots,F\} \}$ denotes the event that at iteration $n$ of Algorithm \ref{alg:RRT} the path $\bbq_{0:F}$ in \eqref{eq:path} has been included in the tree $\ccalG^n$, i.e.,  the states $\bbq(f)$ have been added to the set of nodes $\ccalV^n$ and the edges  $(\bbq(f-1), \bbq(f))$ have been to set of edges $\mathcal{E}^{n}$ for all $f\in\{1,\dots,F\}$. %In words, \eqref{eq:show} says that the path \eqref{eq:path} will be detected with probability $1$ as $n\to\infty$. 
{\bf{Proof of Theorem \ref{thm:probCompl}}:}  
By construction of the path $\bbq_{0:F}$, it holds that $\bbq(f)\in\ccalR(\bbq(f-1))$, for all $f\in\{1,\dots,F\}$. Since $\bbq(0)\in\ccalV^1$, it holds that all states $\bbq\in\ccalR(\bbq(0))$, including the state $\bbq(1)$, will be added to $\ccalV^n$ with probability $1$, as $n\to\infty$, due to Corollary \ref{cor:reach}.%; see \eqref{eq:reach2}. 
Once this happens, the edge $(\bbq(0),\bbq(1))$ will be added to set of edges $\ccalE^n$ due to Corollary \ref{cor:reach}.%; see \eqref{eq:reachedge}.
Applying Corollary \ref{cor:reach} inductively, we get that $\lim_{n\rightarrow\infty} \mathbb{P}\left(\{\bbq_f\in\mathcal{V}^{n}\}\right)=1$ and $\lim_{n\rightarrow\infty} \mathbb{P}\left(\{(\bbq(f-1), \bbq(f))\in\mathcal{E}^{n}\}\right)=1$, for all $f\in\{1,\dots,F\}$ meaning that the path $\bbq_{0:F}$ will be added to the tree $\ccalG^n$ with probability $1$ as $n\to\infty$ completing the proof.%\red{[similar to the argument for prob completeness of rrt]}.% Therefore, \eqref{eq:show} holds completing the proof. 
%\begin{equation}\label{eq:prob3}
%\lim_{n\rightarrow\infty} \mathbb{P}\left(A^n(\texttt{path})\right)=1,
%\end{equation}
%for any finite path $\texttt{path}$ that resides in $\Omega_{\text{free}}^N\times\mathbb{R}_{+}$ generated as per the observation model \eqref{eq:measModel} and the robot dynamics \eqref{eq:rdynamics}. This means that if there exists feasible solution to Problem \ref{prob}, then Algorithm \ref{alg:RRT} will detect it with probability $1$ as $n\to\infty$. Therefore, \eqref{eq:show} holds for any feasible path $\texttt{path}$ completing the proof.

%\subsection{Asymptotic optimality - Proof of Theorem \ref{thm:asOpt}}\label{app:opt}
{\bf{Proof of Theorem \ref{thm:asOpt}}:} The proof of this result straightforwardly follows from Theorem \ref{thm:probCompl}. Specifically, recall from Theorem \ref{thm:probCompl} that Algorithm \ref{alg:RRT} can find any feasible path and, therefore, the optimal path as well, with probability $1$, as $n\to\infty$, completing the proof. %The proof for this result straightforwardly follows from Theorem \ref{thm:probCompl}. Specifically, recall from Theorem \ref{thm:probCompl} that Algorithm \ref{alg:RRT} can  find any feasible 

%\section{Convergence Proof}
%\subsection{Proof of Lemma \ref{lem:optHor}}

%This result holds by construction of the objective function in \eqref{eq:Prob2}. Specifically, recall that the cost function $G(\bbx_i(t)|\bbp(t))$ is selected to be positive, i.e., $G(\bbx_i(t)|\bbp(t))\geq 0$, for all $t\geq 0$. This also implies that $J(t,\bbu_{0:t})\geq 0$, for all $t\geq 0$. Given the positiveness of the cost function  $J(t,\bbu_{0:t})$, we show that $J(t,\bbu_{0:t})$ is monotone which then yields the desired result.
%
%Observe that $J(t+1,\bbu_{0:t+1})= J(t,\bbu_{0:t})+\sum_{i=1}^{M} G(\bbx_i(t+1)|\bbp(t+1))\geq J(t,\bbu_{0:t})\geq 0$, since $\sum_{i=1}^{M} G(\bbx_i(t+1)|\bbp(t+1))\geq 0$, for all $t\geq 0$. Thus, we conclude that $J(t,\bbu_{0:t})$ is \textit{monotone}.
%
%Next, consider the following two complementary cases: (i) there exists a finite time instant $\bar{t}\geq 0$ such that $G(\bbx_i(t)|\bbp(t))=0$, for any configuration $\bbp(t)$ and for all $t\geq \bar{t}$ and; and (ii) there does not exist a finite time instant $\bar{t}\geq 0$ such that $G(\bbx_i(t)|\bbp(t))=0$, for all $t\geq \bar{t}$. In the first case, observe that increasing the horizon $F$ can only increase the cost function $J(F,\bbu_{0:F})$ due to its monotonicity, i.e., $\lim_{F\to\infty} J(F,\bbu_{0:F})=\infty$, for any  $\bbu_{0:F}$. Therefore, if the optimum cost $J^*(F,\bbu_{0:F})$ is finite, %\footnote{Note that this a typical assumption in optimization and optimal control problems.} 
%then the optimal horizon $F$ is finite. In the second case, we conclude that  there exist more than one sequence of optimal control inputs that solve \eqref{eq:Prob2} (with cost equal to the optimum cost). Nevertheless, in this case, the optimal horizon can be selected to be  $\bar{t}\geq 0$, which is finite by assumption, completing the proof.
%This implies that the optimal horizon $F$ is finite, since increasing the horizon $F$ can only increase the cost  $J(F,\bbu_{0:F})$, i.e., $\lim_{F\to\infty} J(F,\bbu_{0:F})=\infty$, for any  $\bbu_{0:F}$. Note that if there exists a finite time instant $\bar{t}\geq 0$ such that $G(\bbx_i(t)|\bbp(t))=0$ for all $t\geq \bar{t}$ then $\lim_{F\to\infty} J(F,\bbu_{0:F})$ is finite. In this case, there exist more than one sequence of optimal control inputs that solve \eqref{eq:Prob2} (with cost equal to the optimum cost). Nevertheless, in this case, the optimal horizon can be selected to be  $\bar{t}\geq 0$, which is finite by assumption, completing the proof. \red{[not well written, explain why monotonicity is important]} 

%Lemma \ref{lem:optHor} also implies that the optimal control problem \eqref{eq:Prob2} is well-defined in the sense that the optimal cost $J(F,\bbu_{0:F})$ is finite.
%\subsection{Convergence Rate Bound - Proof of Theorem \ref{thm:conv}}

%[\red{say that the proof is inspired by [?]. briefly mention how the two proofs are different}]
{\bf{Proof of Theorem \ref{thm:conv}}:}
To prove this result, we model the sampling strategy employed by Algorithm \ref{alg:RRT} as a Poisson binomial process. Specifically, we define Bernoulli random variables $Y_n$ at every iteration $n$ of Algorithm \ref{alg:RRT} so that $Y_n=1$ only if the edge $(\bbq(f-1), \bbq(f))$ is added to the tree at iteration $n$, where $f$ is the smallest element of the set $\set{1,\dots,F}$ that satisfies $\bbq(f-1)\in\ccalV^{n-1}$ and $\bbq(f)\notin\ccalV^{n-1}$. Then, using the random variables $Y_n$, we define the random variable $Y=\sum_{n=1}^{n_{\text{max}}}Y_n$ which captures the total number of successes of the random variables $Y_n$ and we show that it follows a Poisson binomial distribution. Finally, we show that $  \mathbb{P}(A^{n_{\text{max}}}(\bbq_{0:F}^*))=\mathbb{P}(Y\geq F)$ which yields \eqref{eq:bnd1} by applying the Chernoff bounds to $Y$. The detailed proof is omitted.%-\eqref{eq:bnd2}.

Let $X_f^n$, for all $f\in\set{1,\dots,F-1}$ denote a Bernoulli random variable associated with iteration $n$ of Algorithm \ref{alg:RRT}, that is equal to $1$ if the edge $(\bbq_{f-1},\bbq_f)$ in $\bbq_{0:F}^*$ is added to the tree at iteration $n$ or has already been added to the tree at a previous iteration $m<n$, and is $0$ otherwise. Observe that $X_1^n$ is equal to  $1$ for all iterations $n\geq 1$ of Algorithm \ref{alg:RRT}, since the tree is rooted at $\bbq_1$ and, therefore, $q_P^1\in\ccalV^n$, for all $n\geq 1$. By construction of the sampling strategy the probability that $X_f^n=1$ is defined as follows


\begin{equation}\label{eq:padd}
\mathbb{P}(X_f^n)=\left\{
                \begin{array}{ll}
f_{\ccalV}^n(\bbq_{f-1})f_{\ccalU}^n(\bbu_{f-1\to f}), ~\mbox{if}~(\bbq_{f-1},\bbq_f)\notin\ccalE^n,\\
1,~~~\mbox{if}~(\bbq_{f-1},\bbq_f)\in\ccalE^n,
                \end{array}
              \right.
\end{equation}
where with slight abuse of notation $\bbu_{f-1\to f}\in\ccalU$ stands for the control input that steers the robots $\bbq_f$ to $\bbq_{f-1}$. Note that such a controller exists since $\bbq_f\in\ccalR(\bbq_{f-1})$ by construction of the path $\bbq_{0:F}^*$, where $\ccalR(\cdot)$ denotes the reachable set.
%
Observe that if $\bbq_{f-1}\notin\ccalV^n$ then $\mathbb{P}(X_f^n)=0$, since $f_{\ccalV}^n(\bbq_{f-1})=0$. Moreover, note that if an edge  $(\bbq_{f-1},\bbq_f)$ already belongs to $\ccalE^n$ from a previous iteration $m<n$ of Algorithm \ref{alg:RRT}, then it trivially holds that $\mathbb{P}(X_f^n)=1$.

Given the random variables $X_f^n$, we define the discrete random variable $Y_n$ initialized as $Y_1=X_1^1$ and for every subsequent iteration $n>1$ defined as 

\begin{equation} \label{eq:Yn}
Y_n=\left\{
                \begin{array}{ll}
                 X_f^n, ~~\mbox{if}~(Y_{n-1}=X_k^{n-1})\wedge(X_f^{n-1}=0)\\
                 X_{f+1}^n, \mbox{if}~(Y_{n-1}=X_f^{n-1})\wedge(X_f^{n-1}=1)\\
                 ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\wedge (f+1\leq F)\\
                  X_F^n, ~~\mbox{if}~(Y_{n-1}=X_f^{n-1})\wedge(X_f^{n-1}=1)\\
                 ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \wedge (f+1> F) \\
                \end{array}.
              \right.
\end{equation}


In words,  $Y_n$ is defined exactly as $Y_{n-1}$, i.e., $Y_n=Y_{n-1}=X_f^{n-1}=X_f^n$, if $Y_{n-1}=X_{f}^{n-1}=0$, i.e., if the edge $(\bbq_{f-1},\bbq_f)$ associated with the random variable $Y_{n-1}=X_f^{n-1}$ does not exist in the tree at iteration $n-1$; see the first case in \eqref{eq:Yn}. %
%
Also, $Y_n=X_{f+1}^n$, if $Y_{n-1}=X_{f}^{n-1}=1$, i.e., if the edge $(\bbq_{f-1},\bbq_f)$ was added to the tree at the previous iteration  $n-1$; see the second case in \eqref{eq:Yn}. 
%
If $f+1>F$ and $X_f^{n-1}=1$, then we define $Y_n=X_F^n$; see the last case in \eqref{eq:Yn}. Note that in this case, $Y_n$ can be defined arbitrarily, i.e., $Y_n=X_{\bar{f}}^n$, for any $\bar{f}\in\set{1,\dots,F}$, since if $f+1>K$ and $X_f^{n-1}=1$, then this means that all edges that appear in $\bbq_{0:F}^*$ have been added to $\ccalE^n$. By convention, in this case we define  $Y_n=X_F^n$.
%
%
%
Since $Y_n$ is equal to $X_n^f$ for some $f\in\{1,\dots,F\}$, as per \eqref{eq:Yn}, for all $n\geq 1$, we get that $Y_n$ also follows a Bernoulli distribution with parameter (probability of success)  $p^{\text{suc}}_n$ equal to the probability of success of $X_n^k$ defined in \eqref{eq:padd}, i.e., $$p^{\text{suc}}_n=\mathbb{P}(X_f^n),$$ where the index $f$ is determined as per \eqref{eq:Yn}.


Given the random variables $Y_n$, $n\in\{1,\dots,n_{\text{max}}\}$, we define the discrete random variable $Y$ as
\begin{equation}\label{eq:Y}
Y=\sum_{n=1}^{n_{\text{max}}}Y_n.
\end{equation}
Observe that $Y$ captures the total number of successes of the random variables $Y_n$ after $n_{\text{max}}>0$ iterations, i.e., if $Y=y$, $y\in\{1,\dots,n_{\text{max}}\}$, then $Y_n=1$ for exactly $y$ random variables $Y_n$. Therefore, if $Y\geq F$, then all edges that appear in the path $\bbq_{0:F}^*$ have been added to the tree, by definition of the random variables $Y_n$ and $Y$ in \eqref{eq:Yn} and \eqref{eq:Y}, respectively. Therefore, we conclude that 

\begin{equation}\label{eq:Psuc}
\mathbb{P}(A^{n_{\text{max}}}(\bbq_{0:F}^*))=\mathbb{P}(Y\geq K).
\end{equation}


In what follows, our goal is to compute the probability $\mathbb{P}(Y\geq K)$. Observe that $Y$ is defined as a sum of Bernoulli random variables $Y_n$ that are not identically distributed as their probabilities of success $p^{\text{suc}}_n$ are not fixed across the iterations $n$, since the definition of $Y_n$ changes at every iteration $n$ as per \eqref{eq:Yn}.
%
%
Therefore, $Y$ follows a Poisson Binomial distribution which has a rather complicated pmf which is valid for small $n$ and numerically unstable for large $n$; see e.g., \cite{choi2002approximating,hong2011computing}. Therefore, instead of computing $\mathbb{P}(Y\geq K)$, we compute a lower bound for $\mathbb{P}(Y\geq K)$ by applying the Chernoff bound to $Y$. 

Specifically, we have that
\begin{align}\label{eq:prbfailk}
&\mathbb{P}(Y<F)<\mathbb{P}(Y\leq F)=\mathbb{P}(Y\leq F\frac{\mu}{\mu})\\&
=\mathbb{P}\left(Y\leq(1-\underbrace{(1-\frac{F}{\mu})}_{=\delta})\mu\right)=\mathbb{P}(Y\leq(1-\delta)\mu)\leq e^{-\frac{\mu\delta^2}{2}},\nonumber
\end{align}
where $\mu$ is the mean value of $Y$ defined as $\mu=\sum_{n=1}^{n_{\text{max}}} p^{\text{suc}}_n$. Also, the last inequality in \eqref{eq:prbfailk} is due to the Chernoff bound in the lower tail of $Y$ and holds for  any $\delta\in(0,1)$. Observe that the Chernoff bound can be applied to $Y$, as it is defined as the sum of \textit{independent} Bernoulli random variables $Y_n$. Specifically, the random variables $Y_n$ are independent since independent samples $\bbq$ can be generated by the proposed sampling process,  specified by the density functions $f_{\ccalV}$ and $f_{\ccalU}$, due to Assumptions \ref{frand}(ii) and \ref{fnew}(ii). Substituting $\delta=1-\frac{F}{\mu}$ in \eqref{eq:prbfailk}, we get 

\begin{equation}\label{eq:bound}
\mathbb{P}(Y<F)\leq e^{-\frac{\mu}{2}+F-\frac{F^2}{\mu}}\leq e^{-\frac{\mu}{2}+F}=e^{-\frac{\sum_{n=1}^{n_{\text{max}}} p^{\text{suc}}_n}{2}+F},
\end{equation}
where the last inequality is due to $e^{-\frac{F^2}{\mu}}\leq 1$. Recall that \eqref{eq:bound} holds for any $\delta=1-\frac{F}{\mu}\in(0,1)$, i.e, for any $n_{\text{max}}$ that satisfies 
\begin{equation}\label{eq:cond1}
0<\delta<1 \implies 0<F<\mu=\sum_{n=1}^{n_{\text{max}}} p^{\text{suc}}_n\implies 0<F<n_{\text{max}},
\end{equation}
where the last inequality in \eqref{eq:cond1} is due to $ p^{\text{suc}}_n\leq 1$. Therefore, \eqref{eq:bound} holds as long as $n_{\text{max}}>F$. 

Note also that the inequality $0<F<\sum_{n=1}^{n_{\text{max}}} p^{\text{suc}}_n$ in \eqref{eq:cond1} is well defined, since $p^{\text{suc}}_n=\mathbb{P}(X_f^n)$ is strictly positive for all $n\geq 1$ by definition of $Y_n$. To show that, observe that if $Y_n=X_f^n$, for some $f\in\{1,\dots,F-1\}$, then it holds that $(\bbq_{f-2},\bbq_{f-1})\in\ccalE^n$, by definition of $Y_n$ in \eqref{eq:Yn}, i.e., $\bbq_{f-1}\in\ccalV^{n}$. Thus, we have that $f_{\ccalV}(\bbq_{f-1})>0$ by Assumption \ref{frand}(i). Also, $f_{\ccalU}(\bbu_{f-1\to f})>0$ by Assumption \ref{fnew}(i). Therefore, we have that $p^{\text{suc}}_n=\mathbb{P}(X_f^n)>0$; see also \eqref{eq:padd}.
%

Thus, we proved that there exist parameters $\alpha_n(\bbq_{0:F}^*)=p^{\text{suc}}_n\in(0,1]$ associated with every iteration $n$ of Algorithm \ref{alg:RRT} such that the probability $\mathbb{P}(A^{n_{\text{max}}}(\texttt{path}))$ of finding the finite path $\bbq_{0:F}^*$  within $n_{\text{max}}>F$ iterations satisfies
%
\begin{equation}
1\geq\mathbb{P}(A^{n_{\text{max}}}(\bbq_{0:F}^*))=1-\mathbb{P}(Y<F)\geq 1-e^{-\frac{\sum_{n=1}^{n_{\text{max}}} \alpha_n(\bbq_{0:F}^*)}{2}+F},\nonumber 
\end{equation}
completing the proof.

==> files/targetTracking.tex <==
In this section, we consider an application to target localization and tracking for Algorithm \ref{alg:RRT}. In this scenario, the hidden state $\bbx(t)$ is created by stacking the positions of all targets at time $t$, i.e., $\bbx(t)=[\bbx_1^T(t),\bbx_2^T(t),\dots,\bbx^T_M(t)]^T$, where $\bbx_i(t)$ is the position of target $i\in\ccalM:=\{1,\dots,M\}$ at time $t$ and $M>0$ is the number of targets. We require the constraint \eqref{constr22} to hold for all states $\bbx_i(F)$, for some $\delta_i$.
%
As discussed in Section \ref{sec:samplingAlg}, any density functions $f_{\ccalV}$ and $f_{\ccalU}$ that satisfy Assumptions \ref{frand} and \ref{fnew} can be employed to generate states $\bbq_{\text{new}}(t)$ in Algorithm \ref{alg:RRT}. In what follows, we design density functions that allow us to address large-scale estimation tasks that involve large teams of robots and targets. The main idea is to build $f_{\ccalV}$ and $f_{\ccalU}$ so that the tree is biased to explore regions of $\Omega_{\text{free}}$ where targets are predicted to be. 

\subsection{Density Function $f_{\ccalV}$} \label{sec:frand}
Let $L(\bbq)$ denote the length (number of hops) of the path that connects the node $\bbq\in\ccalV$ to the root $\bbq(0)$ of the tree. Let also $L_{\text{max}}$ denote the maximum $L(\bbq)$ among all nodes $\bbq\in\ccalV$, i.e.,
$L_{\text{max}}=\max_{\bbq\in\ccalV} L(\bbq)$. Hereafter, we denote by $\ccalL_{\text{max}}$ the set that collects all nodes $\bbq\in\ccalV$ that satisfy $L(\bbq)=L_{\text{max}}$, i.e., $\ccalL_{\text{max}}=\set{\bbq\in\ccalV~|~L(\bbq)=L_{\text{max}}}$.
%
Given the set $\ccalL_{\text{max}}$, we construct the density function $f_{\ccalV}$ so that it is biased to select subsets $\ccalV_k\subseteq\ccalV$ that contain at least one node $\bbq\in\ccalV$ that  belongs to $\ccalL_{\text{max}}$. Specifically, $f_{\ccalV}(k|\ccalV)$ is defined as follows

\begin{equation}\label{eq:frand}
f_{\ccalV}(k|\ccalV)=\left\{
                \begin{array}{ll}
                  p_{\ccalV}\frac{1}{|\ccalK_{\text{max}}|}, ~~~~~~~~~~~~\mbox{if}~k\in\ccalK_{\text{max}}\\
                  (1-p_{\ccalV})\frac{1}{|\ccalV\setminus\ccalK_{\text{max}}|},~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
where % (i) $\ccalL_{\text{max}}\subseteq\ccalV$ is a set that collects the leaf nodes that have the longest path to the root among all other leaf nodes, 
(i) $\ccalK_{\text{max}}$ is a set that collects the indices $k$ of the subsets $\ccalV_k$ that satisfy $\ccalV_k\cap\ccalL_{\text{max}}\neq\emptyset$, and (ii) $p_{\ccalV}\in(0.5,1)$ stands for the probability of selecting \textit{any} subset $\ccalV_k$ that satisfies $\ccalV_k\cap\ccalL_{\text{max}}\neq\emptyset$. Note that $p_{\ccalV}$ can change with iterations $n$ but it should always satisfy $p_{\ccalV}\in(0.5,1)$ to ensure that subsets $\ccalV_k$ with $\ccalV_k\cap\ccalL_{\text{max}}\neq\emptyset$ are selected more often. 

\subsection{Density Function $f_{\ccalU}$}\label{sec:fnew_target}

The density function $f_{\ccalU}$ is designed so that control inputs $\bbu_j$ that drive robot $j$ towards regions that are predicted to be informative are selected more often. Specifically, given a state $\bbq_{\text{rand}}(t)\in\ccalV_{k_{\text{rand}}}$, where $k_{\text{rand}}$ is sampled from $f_{\ccalV}(k|\ccalV)$, we design $f_{\ccalU}(\bbu|\bbq_{\text{rand}}(t))$ as follows.
The construction of $f_{\ccalU}(\bbu|\bbq_{\text{rand}}(t))$ presumes that targets are assigned to each robot, when the robots are in state $\bbq_{\text{rand}}(t)$; the target assignment process is described in Section \ref{sec:targetAs}. Given the assigned targets, $f_{\ccalU}$ is designed so that control inputs $\bbu_j$ that minimize the \textit{geodesic distance} (see e.g., \cite{kantaros2016global}) between the next robot position $\bbp_{j}(t+1)=\bbf_j(\bbp_{j,\text{rand}}(t),\bbu_j)$ and the predicted position of target $j$, denoted by $\hat{\bbx}_i(t+1)$, are selected more often. Note that the predicted position $\hat{\bbx}_i(t+1)$ can be computed using, e.g., the Kalman filter prediction  step. Specifically, $f_{\ccalU}$ is defined as $f_{\ccalU}(\bbu|\bbq_{\text{rand}}(t))= \prod_{j\in\ccalN} f_{\ccalU}^j(\bbu_j)$, where $f_{\ccalU}^j(\bbu_j)$ is constructed as follows.
\begin{equation}\label{eq:fnew}
f_{\ccalU}^j(\bbu_j)=\left\{
                \begin{array}{ll}
                  p_{\ccalU}, ~~~~~~~~~~~~\mbox{if}~(\bbu_j=\bbu_j^*)\wedge(d_{ij} >R_j)\\
                  (1-p_{\ccalU})\frac{1}{|\ccalU_j|},~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
%\hat{\bbx}_i(t+1) - \bbp_j(t+1) \right\rVert_2
%rrt condiotion for steering function here...
where (i) $d_{ij}=\left\lVert\hat{\bbx}_i(t+1) - \bbp_j(t+1) \right\rVert_2$ and $i$ is the index of the target assigned to robot $j$, (ii) $R_j$ denotes the sensing range of robot $j$, and (iii) $\bbu_j^{*}\in\ccalU_j$ is the control input that minimizes the geodesic distance between $\bbp_j(t+1)$ and $\hat{\bbx}_i(t+1)$, i.e., $\bbu_j^*=\argmin_{\bbu_j\in\ccalU_j} \left\lVert \hat{\bbx}_i(t+1) - \bbp_j(t+1) \right\rVert_g,$
%\begin{equation}\label{eq:ujstar}
%\bbu_j^*=\argmin_{\bbu_j\in\ccalU_j} \left\lVert \hat{\bbx}_i(t+1) - \bbp_j(t+1) \right\rVert_g,
%\end{equation}
 where $\left\lVert \cdot \right\rVert_g$ denotes the geodesic norm/distance. Observe that the density functions \eqref{eq:frand} and \eqref{eq:fnew} satisfy Assumptions \ref{frand} and \ref{fnew}, respectively, by construction. 
 %
In words, \eqref{eq:fnew} selects more often control inputs that drive the robots close to the predicted positions $\hat{\bbx}_i(t+1)$ of their corresponding assigned targets $i$, until these predicted positions are within the robots' sensing range. Once this happens, controllers are selected randomly. %In fact, the control input \eqref{eq:ujstar} "convexifies"\BS{What is meant by this statement? Do you just mean that the field of view constraint is now satisfied? } planning in the vicinity of every robot and decreases the rate at which samples $\bbp_{\text{new}}$ are rejected due to collisions with obstacles.

Finally, observe that \eqref{eq:fnew} is designed independently of the sensor models. Alternative density functions $f_{\ccalU}$ can also be proposed in place of \eqref{eq:fnew} that exploit the sensor model. For instance, in case of a bearing sensor or monocular camera, it may be desirable to select control inputs that drive the robots around their assigned targets, once the latter are inside the field-of-view of the corresponding robots (instead of selecting random control inputs); however, such a design process will be explored in the future.
 
 
%In case of the nonlinear dynamics in \eqref{eq:nonlinDynamics}, there may not exist such a control input $\bbu_j^{*}\in\ccalU_j$. In this case, we pick the control action that adjusts the heading $\theta_j(t+1)$, so that it is aligned along the geodesic path that connects $\bbp_j(t+1)$ to $\hat{\bbx}_i(t+1)$ \cite{kantaros2016global}....

\begin{rem}[On-the-fly update of sampling strategy]
Note that once a feasible solution to \eqref{eq:Prob2} is found, or after a user-specified number of iterations, we can switch to uniform density functions by selecting $p_{\ccalU}=p_{\ccalV}=0$ that promote random exploration, or to any other density function. Recall that the theoretical guarantees provided in Section \ref{sec:complOpt} hold even if the density functions $f_{\ccalV}$ and $f_{\ccalU}$ change with iterations $n$ of Algorithm \ref{alg:RRT}, as long as Assumptions \ref{frand} and \ref{fnew} are always satisfied.
\end{rem} 
 
 
%\begin{rem}[Deterministic strategies]
%Deterministic strategies can also be developed to build trees $\ccalG$ so that the nodes that are closer to their assigned targets are extended more often towards them than other nodes. Such approaches would require to store a set $\ccalU_{\bbq}\subseteq\ccalU$ that collects the control inputs that have not been applied to $q\in\ccalV$ yet, for each node $q\in\ccalV$. This way, a control input $\bbu$ is selected from $\ccalU_{\bbq}$ (instead of $\ccalU$ as in Alg. \ref{alg:RRT}), when $q\in\ccalV$ is selected to be extended. This would guarantee that the optimal solution can be found within a finite number of iterations. However, such an approach would require excessive memory requirements as the number of robots increases and the tree grows. 
%\end{rem}

 
 
\subsection{On-the-fly Target Assignment}\label{sec:targetAs}
In what follows, we describe the target assignment process that is executed every time a state $\bbq_{\text{new}}(t+1)=[\bbp_{\text{new}}(t+1),\Sigma_{\text{new}}(t+1)]$ is added to the tree; see also Algorithm \ref{alg:assignment}. The goal of Algorithm \ref{alg:assignment} is to assign targets to each robot when they are in the state $\bbq_{\text{new}}(t+1)$. Specifically, for each state $\bbq(t)\in\ccalV$, we construct a function $s_{\bbq}:\ccalN\to\ccalM$ that assigns to each robot $j\in\ccalN$ a single target $i\in\ccalM$. Hereafter, we denote by $s_{\bbq}(j)$ the target that is assigned to robot $j$ in state $\bbq(t)$. Recall from Section \ref{sec:fnew_target}, that the assigned targets associated with the state $\bbq_{\text{rand}}(t)$ are used to construct $f_{\ccalU}(\bbu|\bbq_{\text{rand}}(t))$. %Hereafter, we drop the dependence of $t$ for simplicity of notations. %In Algorithm \ref{alg:assignment}, the targets that are assigned to the robots when they are in a state $\bbq(t)$ are captured by the vector $\bbs_{\bbq(t)}\in\mathbb(R)^N$. 

\begin{algorithm}[t]
\footnotesize
\caption{On-the-fly Target Assignment}
\LinesNumbered
\label{alg:assignment}
\KwIn { (i) $s_{\bbq_{\text{rand}}}$, (ii) $\det\Sigma(F)$ \& $\delta_i, \forall i\in\ccalM$}
\KwOut {$s_{\bbq_{\text{new}}}:\ccalN\to\ccalM$}
  $s_{\bbq_{\text{new}}}=s_{\bbq_{\text{rand}}}$\;\label{as:init}
 Compute set $\ccalD$ of robots that are candidate to update their assigned targets\;\label{as:D}
 Initialize set of targets to be assigned to robots as $\ccalT_{\text{to-assign}}=\ccalM\setminus\set{\ccalT_{\text{as}}\cup\ccalT_{\text{sat}}}$\; \label{as:Tassign}
\If {$\ccalT_{\text{to-assign}}=\emptyset$}{\label{as:Tassign2}
 $\ccalT_{\text{to-assign}}=T_{\text{unsat}}$\;\label{as:Tassign3}}
%if empty go to goal regions
\For {$j\in\ccalD$}{\label{as:as1}
 $s_{\bbq_{\text{new}}}(j)=i_{\text{closest}}$, where $i_{\text{closest}}\in\ccalT_{\text{to-assign}}$\;\label{as:as2}
 Update $\ccalT_{\text{to-assign}} = \ccalT_{\text{to-assign}}\setminus\set{i_{\text{closest}}}$\;\label{as:upd1s}
\If {$\ccalT_{\text{to-assign}} =\emptyset$}{\label{as:sempty}
 $\ccalT_{\text{to-assign}}=\ccalT_{\text{unsat}}$\;\label{as:upds2}
}
}\label{as:asend}
\end{algorithm} 


%Given the targets assigned to the robots when they are in state  $\bbq_{\text{rand}}(t)$, the density function $f_{\ccalU}$ selects more often control inputs $\bbu_{\text{new}}$ that drive the robots toward the respective assigned targets.

First, the function $s_{\bbq_{\text{new}}}$ is initially defined as $s_{\bbq_{\text{new}}}=s_{\bbq_{\text{rand}}}$, where recall that $\bbq_{\text{rand}}$ is the parent node of $\bbq_{\text{new}}$ in the tree $\ccalG$ [line \ref{as:init}, Alg. \ref{alg:assignment}]. Then, we compute (i) the set $\ccalD\subseteq\ccalN$ that collects the indices of the robots that need to update their assigned targets [line \ref{as:D}, Alg. \ref{alg:assignment}], and (ii) the set $\ccalT_{\text{to-assign}}\subseteq\ccalM$ that collects the indices of the targets that are available to be assigned to the robots in $\ccalD$ [lines \ref{as:Tassign}-\ref{as:Tassign3}, Alg. \ref{alg:assignment}]. Then, targets from $\ccalT_{\text{to-assign}}$ are assigned to the robots in $\ccalD$ [lines \ref{as:as1}-\ref{as:asend}].

In particular, the set $\ccalD$ collects the indices $j\in\ccalN$ of robots that in state $\bbq_{\text{new}}$ either (i) satisfy $\det\Sigma_i(F)\leq \delta_i$, where $i$ is the target assigned to robot $j$, i.e., $i=s_{\bbq_{\text{new}}}(j)$, and $\Sigma_{i,\text{new}}$ is its respective covariance, or (ii) the set $\ccalN_i=\set{j~|~i=\bbs_{j,\bbq_{\text{new}}} }$ that collects the robots that are responsible for target $i$, contains more than one robot, i.e., $|\ccalN_i|>1$, or both (i) and (ii). 
%\footnote{Note that $\det\Sigma_i(F)\leq \delta_i$ may hold due to measurements taken by any robot $r\neq j$, even though $i$ has been assigned to robot $j$.}
%Third, we construct the set $\ccalT_{\text{to-assign}}$ that collects the indices of the targets that should be assigned to the robots $j\in\ccalD$ [lines \ref{as:Tassign}-\ref{as:Tassign4}, Alg. \ref{alg:assignment}]. %
Next, the set $\ccalT_{\text{to-assign}}$ is constructed. First, it is initialized as  $\ccalT_{\text{to-assign}}=\ccalM\setminus\set{\ccalT_{\text{as}}\cup\ccalT_{\text{sat}}}$, where  $\ccalT_{\text{as}}\subseteq\ccalM$ collects the indices of the targets that have already been assigned to robots (recall that, in general, it may hold $M>N$) and $\ccalT_{\text{sat}}\subseteq\ccalM$ collects the indices $i\in\ccalM$ of the targets that already satisfy $\det\Sigma_i(F)\leq \delta_i$ [line \ref{as:Tassign}, Alg. \ref{alg:assignment}]. If $\ccalT_{\text{to-assign}}=\emptyset$, then it is redefined as $\ccalT_{\text{to-assign}}=\ccalT_{\text{unsat}}$, where $\ccalT_{\text{unsat}}$ collects the indices $i\in\ccalM$ of the targets that do not satisfy $\det\Sigma_i(F)\leq \delta_i$ [lines \ref{as:Tassign2}-\ref{as:Tassign3}, Alg. \ref{alg:assignment}].%\footnote{Observe that $\ccalT_{\text{sat}}\cup \ccalT_{\text{unsat}}=\ccalM$. } %Notice that $i\in \ccalT_{\text{unsat}}$ does not necessarily imply that $i\notin\ccalT_{\text{as}}$. 


Given $\ccalD$ and $\ccalT_{\text{to-assign}}$, our goal is to assign the targets  $i\in\ccalT_{\text{to-assign}}$ to the robots $j\in\ccalD$ [lines \ref{as:as1}-\ref{as:asend}, Alg. \ref{alg:assignment}]. To do this, the robots $j\in\ccalD$ sequentially select the closest target $i\in\ccalT_{\text{to-assign}}$ to them, denoted by $i_{\text{closest}}$. Every time a robot $j$ picks a target from $\ccalT_{\text{to-assign}}$, the mapping $s_{\bbq_{\text{new}}}$ and set $\ccalT_{\text{to-assign}}$ are updated as $s_{\bbq_{\text{new}}}(j)=i_{\text{closest}}$ and $\ccalT_{\text{to-assign}} = \ccalT_{\text{to-assign}}\setminus\set{i_{\text{closest}}}$ [lines \ref{as:as2}-\ref{as:upd1s}, Alg. \ref{alg:assignment}]. If during this assignment process, it holds that $\ccalT_{\text{to-assign}}=\emptyset$, then $\ccalT_{\text{to-assign}}$ is reinitialized as $\ccalT_{\text{to-assign}}=\ccalT_{\text{unsat}}$ [lines \ref{as:sempty}-\ref{as:upds2}, Alg. \ref{alg:assignment}]. The latter happens if there more robots in $\ccalD$ than targets to be assigned. %Finally, note that in case there are terminal constraints, Algorithm \ref{alg:assignment} can straightforwardly be extended so that it assigns as pseudo-targets to robots locations in $\ccalP_j^{\text{goal}}$ when there more robots in $\ccalD$ than targets to be assigned.
Finally, note that any other task assignment algorithm can be employed in place of lines \ref{as:as1}-\ref{as:asend} that may improve the performance of Algorithm \ref{alg:RRT}; see e.g., \cite{turpin2014capt,michael2008distributed}.




==> files/tree.tex <==
\subsection{Incremental Construction of Trees}\label{sec:constructTree}
At every iteration $n$ of Algorithm \ref{alg:RRT}, a new state $\bbq_\text{new}(t+1) =[\bbp_{\text{new}}(t+1),\Sigma_{\text{new}}(t+1)]$ is sampled. The construction of the state  $\bbq_\text{new}(t+1)$ relies on two steps. Specifically, first we sample a state $\bbp_{\text{new}}(t+1)$ [lines \ref{rrt:samplekrand}-\ref{rrt:sampleu}, Alg. \ref{alg:RRT}]; see Section \ref{sec:sample}. Second, given $\bbp_{\text{new}}(t+1)$ we compute the covariance matrix $\Sigma_{\text{new}}(t+1)$, giving rise to $\bbq_{\text{new}}(t+1)$ which is added to the tree structure [line \ref{rrt:dnew}, Alg. \ref{alg:RRT}]; see Section \ref{sec:extend}.



%To do this, we first sample a state $\bbp_{\text{new}}$; see Section \ref{sec:sample} [lines \ref{rrt:samplekrand}-\ref{rrt:sampleu}, Alg. \ref{alg:RRT}]. Then, we select a state $\bbq_{\text{rand}}(t)=[\bbp_{\text{rand}}(t),\bbd_{\text{rand}}(t)]\in\ccalV$ that will be the parent node of $\bbq_{\text{new}}(t+1)$[line \eqref{rrt:for2}, Alg. \ref{alg:RRT}]. Note that the time instant $t+1$ which $\bbq_{\text{new}}$ is associated with, is determined by the parent node $\bbq(t)$. Given $\bbp_{\text{new}}$ and the parent node $\bbq_{\text{rand}}(t)$, we compute $\bbd_{\text{new}}(t+1)$ which then gives rise to the new state $\bbq_\text{new}(t+1) =[\bbp_{\text{new}}(t+1),\bbd_{\text{new}}(t+1)]$ that will be added to the tree at iteration $n$ [lines \ref{rrt:dnew}-\ref{rrt:updCost}, Alg. \ref{alg:RRT}]; see Section \ref{sec:extend}.

\subsubsection{Sampling Strategy}\label{sec:sample} 
To construct the state $\bbp_{\text{new}}$, we first divide the set of nodes $\ccalV$ into a \textit{finite} number of sets, denoted by $\ccalV_{k}\subseteq\ccalV$, based on the robot-configuration component of the stats $\bbq\in\ccalV$. Specifically, a $\ccalV_{k}$ collects all states $\bbq\in\ccalV$ that share the same robot configuration $\bbp$; see Figure \ref{fig:tree}.%\footnote{Decomposition of $\ccalV$ into subsets $\ccalV_k$ is required to ensure completeness and optimality of Algorithm \ref{alg:RRT}; see Appendix \ref{sec:prop}.}
%$\bbq(t)=[\bbp(t),\Sigma(t)]\in\ccalV$ that have the same robot configuration $\bbp$ but possibly different covariance matrices $\Sigma(t)$ and different time stamps $t$; see Figure \ref{fig:tree}. %Also, note that the states $\bbq\in\ccalV_k$ do not necessarily have the same time stamp $t$, since, in general, there are multiple paths that connect the root $\bbq(0)$ to $\bbq$.
%
By construction of $\ccalV_{k}$, we get that  $\ccalV = \cup_{k=1}^{K_n}\ccalV_{k}$, where $K_n$ is the number of subsets $\ccalV_{k}$ at iteration $n$.
Also, notice that $K_n$ is finite for all iterations $n$, since the set of admissible control inputs $\ccalU$ is finite, by assumption. %for all robots $j$, i.e., the number of all possible different robot configurations contained in $\ccalV$ is finite for all iterations $n$. 
At iteration $n=1$ of Algorithm \ref{alg:RRT}, it holds that $K_1=1$, $\ccalV_1=\ccalV$ [line \ref{rrt:init}, Alg. \ref{alg:RRT}]. %\red{[maybe a figure would make this definition much cleaner]}%%the (global) set V can be 'infinite'!
% 

Second, given the sets $\ccalV_k$, we first sample from a given discrete distribution $f_{\ccalV}(k|\ccalV):\set{1,\dots,K_n}\rightarrow[0,1]$ an index $k\in\set{1,\dots,K_n}$ that points to the set $\ccalV_{k}$ [line \ref{rrt:samplekrand}, Alg. \ref{alg:RRT}]. The density function $f_{\ccalV}(k|\ccalV)$ defines the probability of selecting the set $\ccalV_{k}$ at iteration $n$ of Algorithm \ref{alg:RRT} given the set $\ccalV$. Any density function $f_{\ccalV}$ can be used to draw samples $k_{\text{rand}}$ as long as it satisfies the following assumption.%\NA{It is not allowed to sample control at the same node twice, correct? To me the discrete distributions are more of a prioritization of the search of the tree -- does it have to be random?} %\BS{How do you choose amongst the different possible nodes in the set $\ccalV_k$, once $k$ is chosen?}

Next, given the set $\ccalV_{k_{\text{rand}}}$ sampled from $f_{\ccalV}$ and the corresponding robot state $\bbp_{\text{rand}}$, we sample a control input $\bbu_{\text{new}}\in\ccalU$ from a discrete distribution $f_{\ccalU}(\bbu):\ccalU\rightarrow [0,1]$ [line \ref{rrt:sampleu}, Alg. \ref{alg:RRT}]. 
%
Given a control input $\bbu_{\text{new}}$ sampled from $f_{\ccalU}$, we construct the state $\bbp_{\text{new}}$ as $\bbp_{\text{new}}=\bbf(\bbp_{\text{rand}},\bbu_{\text{new}})$ [line \ref{rrt:sampleu}, Alg. \ref{alg:RRT}]. Any density function $f_{\ccalU}$ can be used to draw samples $\bbu_{\text{new}}$ as long as it satisfies the following assumption.
%The density function $f_{\ccalU}$ should be designed so that it satisfies the following assumption.

\subsubsection{Extending the tree}\label{sec:extend}

If the configuration $\bbp_\text{new}$, constructed as in Section \ref{sec:sample}, does not belong to the obstacle-free space, then the current sample $\bbp_\text{new}$ is rejected and the sampling process is repeated [line \ref{rrt:obsFree}, Alg. \ref{alg:RRT}]. Otherwise, the tree is extended towards states $ \bbq_\text{new}$ that are constructed as follows; see also Figure \ref{fig:tree2}. %\footnote{The condition $(\bbq_\text{rand}(t),\bbq_\text{new}(t))\notin \ccalE$ in line \ref{rrt:newedge} prevents from adding the same edgeadding }%if $\bbp_\text{new}\in \Omega_{\text{free}}^N$ and $(\bbq_\text{rand}(t),\bbq_\text{new}(t))\notin \ccalE$,
%
Given a state $\bbq_{\text{rand}}(t)=[\bbp_{\text{rand}}(t),\Sigma_{\text{rand}}(t)]\in\ccalV_{k_{\text{rand}}}$, we construct a state $ \bbq_\text{new}$ by appending to $\bbp_{\text{new}}(t+1)$, the covariance matrix $\Sigma_{\text{new}}(t+1)$ computed as $\Sigma_{\text{new}}(t+1)=\rho(\bbp_{\text{rand}}(t),\Sigma_{\text{rand}}(t))$, where recall that $\rho(\cdot)$ is the Kalman filter Ricatti map [lines \ref{rrt:dnew}-\ref{rrt:qnew}, Alg. \ref{alg:RRT}]. %
Next, we update the set of nodes and edges of the tree as $\ccalV = \ccalV\cup\{\bbq_{\text{new}}(t+1)\}$ and $\ccalE = \ccalE\cup\{(\bbq_{\text{rand}}(t),\bbq_{\text{new}}(t+1))\}$, respectively [lines \ref{rrt:updV}-\ref{rrt:updE}, Alg. \ref{alg:RRT}]. The cost of the new node $\bbq_{\text{new}}(t+1)$ is computed as in \eqref{eq:costUpd}, i.e., $J_{\ccalG}(\bbq_{\text{new}}(t+1))=J_{\ccalG}(\bbq_{\text{rand}}(t))+\det \Sigma_{\text{new}}(t+1)$ [line \ref{rrt:updCost}, Alg. \ref{alg:RRT}]. Finally, the sets $\ccalV_{k}$ are updated, so that if there already exists a subset $\ccalV_k$ associated with the configuration  $\bbp_{\text{new}}$, then $\ccalV_{k}=\ccalV_{k}\cup\set{\bbq_{\text{new}}(t+1)}$. Otherwise, a new set $\ccalV_{k}$ is created, i.e., $K_n = K_n +1$ and $\ccalV_{K_n}=\set{\bbq_{\text{new}}}$ [lines \ref{rrt:if2}-\ref{rrt:updKn}, Alg. \ref{alg:RRT}]. This process is repeated for all states  $\bbq_{\text{rand}}(t)\in\ccalV_{k_{\text{rand}}}$ [line \ref{rrt:for2}, Alg. \ref{alg:RRT}]. Recall that the states in $\ccalV_{k_{\text{rand}}}$ share the same robot configuration $\bbp_{\text{rand}}$ but they are possibly paired with different time stamps $t$ and covariance matrices $\Sigma(t)$; see Figure \ref{fig:tree}.

%
%Finally, if the state $\bbq_{\text{new}}$ satisfies the constraints captured by the goal set \eqref{eq:goalRegion}, i.e.,  $\bbq_{\text{new}}\in\ccalQ_{\text{goal}}$, then the set $\ccalX_{{g}}$  is updated as $\ccalX_{g} = \ccalX_{g}\cup\set{\bbq_{\text{new}}}$ [lines \ref{rrt:updGoal1}-\ref{rrt:updGoal2}, Alg. \ref{alg:RRT}]. This process is repeated for all states in the set $\ccalV_{k_{\text{rand}}}$ [line \ref{rrt:for2}, Alg. \ref{alg:RRT}]. Algorithm \ref{alg:RRT} terminates after $n_{\text{max}}$ iterations, where $n_{\text{max}}>0$ is user-specified [line \ref{rrt:forn}, Alg. \ref{alg:RRT}]. 

%\begin{rem}[Alternative Approaches]
%Note that an alternative solution to Problem \ref{prob} is to exhaustively search the infinite state-space$\Omega_{\text{free}}^N\times\mathbb{R}_{+}$ in a similar way as e.g., in [LeNy] that relies on feedforward value iteration or as in [Atanasov] that relies on a Reduced Value Iteration. Nevertheless, such approaches do not scale well as the required horizon $F$ or the number of robots increases, since they require at to compute the reachable set of any node $\bbq(t)$ and extend the search tree towards all reachable states. To the contrary, here we extend the nodes $\bbq(t)\in\ccalV$ to a single reachable state in a probabilistic way as described in Section \ref{sec:sample}. As it will be shown in Section \ref{sec:Sim}, this allows us to address large-scale estimation tasks.
%\end{rem}
%

